Regret-Optimal Federated Transfer Learning for Kernel Regression with Applications in American Option Pricing

We propose an optimal iterative scheme for federated transfer learning, where a central planner has access to datasets ${\cal D}_1,\dots,{\cal D}_N$ for the same learning model $f_{\theta}$. Our objective is to minimize the cumulative deviation of the generated parameters $\{\theta_i(t)\}_{t=0}^T$ across all $T$ iterations from the specialized parameters $\theta^\star_{1},\ldots,\theta^\star_N$ obtained for each dataset, while respecting the loss function for the model $f_{\theta(T)}$ produced by the algorithm upon halting. We only allow for continual communication between each of the specialized models (nodes/agents) and the central planner (server), at each iteration (round). For the case where the model $f_{\theta}$ is a finite-rank kernel regression, we derive explicit updates for the regret-optimal algorithm. By leveraging symmetries within the regret-optimal algorithm, we further develop a nearly regret-optimal heuristic that runs with $\mathcal{O}(Np^2)$ fewer elementary operations, where $p$ is the dimension of the parameter space. Additionally, we investigate the adversarial robustness of the regret-optimal algorithm showing that an adversary which perturbs $q$ training pairs by at-most $\varepsilon>0$, across all training sets, cannot reduce the regret-optimal algorithm's regret by more than $\mathcal{O}(\varepsilon q \bar{N}^{1/2})$, where $\bar{N}$ is the aggregate number of training pairs. To validate our theoretical findings, we conduct numerical experiments in the context of American option pricing, utilizing a randomly generated finite-rank kernel.

==> Formatting/Checklist/neurips_checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newpage
\section*{NeurIPS Paper Checklist}
\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The claims asserted in Abstract and \S\ref{s:Intro} are directly connected and substantiated by our theory in Section~\ref{s:Main} and later experiments and results sections \S\ref{s:Experiments_n_Validation}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer:  \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    At the beginning of Section\S~\ref{s:Experiments_n_Validation}, we acknowledge the limitation of our experimental study as there are no available benchmarks to the considered regret-optimal meta-optimization problem.  Thus, we could only compare our results experimentally against ablated versions of our algorithms and natural naive benchmarks. 
    % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    All assumptions are clearly stated in Section~\ref{s:Main} and at the beginning of each of our results.
    % This paper does not include theoretical results. % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    Our paper clearly outlines all hyperparameters used to train the kernel models and all data in the Experiments section~\ref{s:Experiments_n_Validation} as well as all additional information in Appendix~\ref{a:ExperimentDetails}, including hardware specifications.  Further, all code is provided in our supplementary material.
    % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All code used to generate data and train our models is provided in the supplementary material.   All hyperparameters are specified in sections~\ref{s:Experiments_n_Validation} and in Appendix~\ref{a:ExperimentDetails}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: These details are specified in sections~\ref{s:Experiments_n_Validation} and, further in Appendix~\ref{a:ExperimentDetails}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, all plots and tables contain error bars and confidence intervals.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} %\answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: These are provided in Appendix~\ref{a:ExperimentDetails__ss:hardware}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: 
    Our paper is largely theoretical and the experiments are synthetic.  Therefore, it complies with the NeurIPS Code of Ethics.
    % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We justify the broader impact of our results, as well as both the positive and negative societal implications due to applicability in quantitative finance, at the end of our paper's main body.
    % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  As our contributions are theoretical and our experiments are synthetic, the paper poses no such risks.
    % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper does not use existing assets.
    % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper does not use new assets.
    % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> OLD/OLD_Introduction.tex <==
% players are \textit{indifferent}, leaving them to have equal influence on the model selection problem, and 

\begin{comment}
    \subsection{Regression from Multi-Sourced Data}
    % The situation complicates when trying to identify an fKRR on a main dataset $\mathcal{D}^{(1)}$ while extracting a useful inductive bias from $N-1$ related (finite) datasets $\mathcal{D}^{(2)}$,$\dots$, $\mathcal{D}^{(N)}$; each of which is drawn from possibly \textit{different} data-generating distributions $\mathbb{P}^{(1)}$,$\dots$, $\mathbb{P}^{(N)}$ on $\mathbb{R}^d\times \mathbb{R}$.  Thus each distribution $\mathbb{P}^{(n)}$ formalizes a (possibly) distinct \textit{data-source}.
    The dilemma is illustrated by considering two extremal interpretations of training a \textit{single} fRKR using \textit{all} these datasets.  
    
    The first extreme is the \textit{pooled regime}, in which all datasets are equally aggregated and we simply solve~\eqref{eq:FRKR} while summing over all points in $\mathcal{D}\eqdef \cup_{i=1}^N\,\mathcal{D}^{(i)}$.   The optimal fRKR parameter in this regime is defined analogously to~\eqref{eq:loss_one_dataset}.  
      %where $x$ run through the aggregated dataset $\mathcal{D}$ and $y$ are the targets from this aggregated dataset.  
    The main trouble with this regime/interpretation of the problem is that each dataset's importance is drowned out, and the fact that each dataset $\mathcal{D}^{(i)}$ is drawn from a \textit{different} data-generating distribution is forgotten.  In particular, the main dataset $\mathcal{D}^{(1)}$ is no more important than any other one.  
    This regime is called ``hard parameter sharing'' in multi-task learning (MLT).  Additionally, there is a computational challenge when $N$ is large, since the cost of computing this optimal parameter choice is at-least $\mathcal{O}(Np^2 + p^{2.37})$ due to the cost of computing $\Phi(x^1)^{\top}\Phi(x^1)$ and the cost of inverting a $p\times p$ matrix, using \cite{LeGall_Complexity_CWLikeMatrixInversion_2014}.  
    % Nevertheless, this computational issue can be alleviated by turning to iterative optimization schemes, such as gradient descent, implicitly approximate the matrix inverse in~\eqref{eq:loss_one_dataset} using $\mathcal{O}(Np)$ complexity \cite{YaoRosascoCoponnetto_2007_CA,}.
    
    % \Aurelien{This is assuming that one finds the solution by computing the inverse, but gradient descent is known to approximate it, see e.g.\url{https://yao-lab.github.io/publications/earlystop.pdf} and it only has cost $O(N)$. One can even find the solution independently of $N$ using SGD.}
    % \Anastasis{AL you're referring to 3.1 which you showed me in our meeting right?  Also, shouldn't this be $O(TN)$ where $T$ are the number of GD iterations, but I guess we don't need many since it converges exponentially fast to this strongly convex objective with Lipschitz grads.
    % }
    % \Aurelien{1) Yes, section 3.1. The proof is essentially based on the Neumann series of an inverse matrix and the fact that GD constructs an approximation of the inverse matrix by building the Neumann series. \\
    % 2) Yes, you can say $O(TN)$, although we have a very fast rate of convergence for gradient descent of the form $O((1-\alpha)^T)$. \\
    % }

    The other extreme, which we call the \textit{selfish regime}, is to interpret the problem as a competition between $N$ self-interest players, each of which is only interested in optimizing the fRKR on their dataset according to~\eqref{eq:loss_one_dataset} resulting in $N$ (possibly) different parameter specifications $\theta^\star_1$,\dots, $\theta^\star_N$.  We, acting as a ``central planner'', need to aggregate each player's parameters into a \textit{single} parameter defining our \textit{single} fRKR model.  
    This aggregation can naively be approached by bagging $\frac1{N}\sum_{i=1}^N\, \theta^\star_i$, by data-driven weighting procedures \cite{Baxter_2000_JAIR__AmodelIndutvieBiasLearning}, via a Bayesian aggregation \cite{MR2280214,PACOH_rothfuss_2021,pavasovic2022mars}, or using dictionaries \cite{argyriou2006multi}.  
    The quality/goodness of the selected learned  parameters is ultimately valued by the aggregate (terminal-time) loss
    \allowdisplaybreaks\begin{align} 
    \label{eq:terminal_time_objective}
    \begin{aligned}
            l(\theta_1,\dots,\theta_N, w;\,\mathcal{D} )  
        \eqdef & 
            \sum_{i=1}^N 
            w_i
            % \biggl(
                \sum_{j=1}^{S_i} 
                    (
                    f_{\theta^w}(x_j^i)
                    % (u^i_j)^{\top} 
                    % \langle 
                    %     u^i_j
                    %     ,
                    %     \theta^{w}
                    % \rangle 
                    - y^i_j  
                    )^2 
            % \biggr)
        \\
        % \,\,
        \mbox{ s.t. }
        \,%\,
        \theta^w\eqdef & \sum_{i=1}^N \theta_i
            w_i
     ,
    \end{aligned}
    \end{align} 
    % \allowdisplaybreaks\begin{align} 
    % \label{eq:terminal_time_objective__fKRR}
    % \begin{aligned}
    %         l(\theta_1,\dots,\theta_N, w;\,\mathcal{D} )  
    %     \eqdef & 
    %         \sum_{i=1}^N 
    %         w_i
    %         \biggl(
    %             \sum_{j=1}^{S_i} 
    %                 \big| 
    %                 % (u^i_j)^{\top} 
    %                 \langle 
    %                     u^i_j
    %                     ,
    %                     \theta^{w}
    %                 \rangle - y^i_j  \big|^2 
    %         \biggr)
    %     \\
    %     % \,\,
    %     \mbox{ s.t. }
    %     \,%\,
    %     \theta^w\eqdef & \sum_{i=1}^N \theta_i
    %         w_i
    %  ,
    % \end{aligned}
    % \end{align} 
    where $w = (w_1, \cdots, w_N) \in [0,1]^N$ with $\sum_{i=1}^N\,w_i=1$, 
    % $\langle\cdot,\cdot\rangle$ denotes the Euclidean inner-product, $u^i_j\eqdef \phi(x^i_j)$
    %\Aurelien{Is it supposed to be $\sum_{i=1}^N\,w_i^\star$? same comment above, $\mathbf{w}$ is the same as $w^\star$?} 
    %\Xuwei{The aggregation parameter $w$ here is generic and satisfy $\sum_{i=1}^N w_i=1$.}
\end{comment}
% \Anastasis{Update: Since we are not doing multi-task learning but rather a more "transfer-learning problem" then we should only sum over the main/first dataset
% \allowdisplaybreaks\begin{align} 
% \tag{T-Obj}
% \label{eq:terminal_time_objective}
%         l(\theta_1,\dots,\theta_N, w;\,\mathcal{D} )  
%     \eqdef  
%         \sum_{i=1}^N 
%         {\color{red}{w_i}}\,
%         \sum_{j=1}^{S_i} 
%             \big| u^i_j \theta^{w}  - y^i_j  \big|^2 
%     % \\
%     \,\,
%     \mbox{ where }
%     \,\,
%     \theta^w\eqdef \sum_{i=1}^N \theta_i
%         w_i
% \end{align} 
% The addition of $w_i$ automatically removes the effect of the dataset from the objective function, while the $w_i$ in the summoned removes the impact of the $i^{th}$ learner from the "averaged" learner.
% } 
% \Aurelien{I'm a bit confused by the notation above. Isn't $u^i_j$ a vector? If so, it seems to me we should write $\langle u^i_j, \theta^w \rangle$.}\Anastasis{Sure :) }

==> OLD/Pre_TMLR_Review__1.tex <==
% %%%%%%%% NeurIPS 2020 EXAMPLE LATEX SUBMISSION FILE %%%%%%%%%%%%%%%%%
% % \documentclass{article}
% % to avoid loading the natbib package, add option nonatbib:
% % \usepackage{Formatting/neurips_2020}

% %%%%%%%% ICML 2021 EXAMPLE LATEX SUBMISSION FILE %%%%%%%%%%%%%%%%%
% % \documentclass[preprint]{article}


% % \usepackage{xcolor} 
% % \usepackage{amsthm}
% % \usepackage{neurips_2020}

% % \documentclass[jair,twoside,11pt,theapa]{article}
% \documentclass[10pt]{article} % For LaTeX2e
% \usepackage{tmlr}

% % \usepackage{jair, theapa, rawfonts}
% \usepackage{svg}
% \usepackage{csvsimple}

% % \jairheading{1}{1993}{1-15}{6/91}{9/91}
% % \ShortHeadings{Regret-Optimal Federated Transfer Learning - KRR}{Yang, Kratsios, Krach, Grasselli, \& Lucchi}

% \title{Regret-Optimal Federated Transfer Learning for Kernel Regression -- with Applications in American Option Pricing}

% % Authors must not appear in the submitted version. They should be hidden
% % as long as the tmlr package is used without the [accepted] or [preprint] options.
% % Non-anonymous submissions will be rejected without review.

% \author{\name Xuwei Yang \email yangx212@mcmaster.ca \\
%       \addr Department of Mathematics\\
%       McMaster University
%       \AND
%       \name Anastasis Kratsios \email kratsioa@mcmaster.ca \\
%       \addr Department of Mathematics\\
%       McMaster University and Vector Institute
%       \AND
%       \name Florian Krach \email florian.krach@math.ethz.ch\\
%       \addr Department of Mathematics\\
%       ETH Z\"{u}rich
%       \AND Matheus Grasselli \email grassel@mcmaster.ca\\
%       \addr Department of Mathematics\\
%       McMaster University
%        \AND Aurelien Lucchi \email aurelien.lucchi@unibas.ch\\
%     \addr Department of Mathematics and Informatics\\
%       University of Basel}


% % \def\month{MM}  % Insert correct month for camera-ready version
% % \def\year{YYYY} % Insert correct year for camera-ready version
% % \def\openreview{\url{https://openreview.net/forum?id=XXXX}} % Insert correct link to OpenReview for camera-ready version

% \usepackage{amsthm}
% \newtheorem{proposition}{Proposition}%[section]
% \newtheorem{lemma}{Lemma}%[section]
% \newtheorem{definition}{Definition}%[section]
% \newtheorem{theorem}{Theorem}%[section]
% \newtheorem{remark}{Remark}%[section] 
% \newtheorem{assumption}{Assumption} 
% \newtheorem{corollary}{Corollary}
% \newtheorem{experiment}{Experiment}


% \newcommand{\com}[1]{{\color{orange}{#1}}}


% %To display labels in the PDF. Comment at the end!
% % Code
% \usepackage{algpseudocode}
% \usepackage[linesnumbered,lined,boxed,commentsnumbered,ruled,longend]{algorithm2e}
%     \RestyleAlgo{ruled}
% \newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
% \SetCommentSty{mycommfont}

% % TABLE Formatting
% \raggedbottom
% \newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
% % \setlength\heavyrulewidth{0.3ex}
% \usepackage{lscape}



% % Packages and Macros
% \input{Formatting/macros}
% % For Annotating + Commenting
% \input{Formatting/comment}

% % Code link:
% \newcommand{\code}{%
%     %\url{https://github.com/FlorianKrach/RegretOptimalFederatedTransferLearning} %
%     \url{https://github.com/???}%
% }


% \begin{document}

% % \title{Regret-Optimal Federated Transfer Learning for Kernel Regression -- with Applications in American Option Pricing}

% % \author{\name Xuwei Yang \email yangx212@mcmaster.ca \\
% %        \name Anastasis Kratsios \email kratsioa@mcmaster.ca \\
% %         \name Florian Krach \email florian.krach@math.ethz.ch\\
% %         \name Matheus Grasselli \email grassel@mcmaster.ca\\
% %        \name Aurelien Lucchi \email aurelien.lucchi@unibas.ch}



% \maketitle

% \begin{abstract}
% We propose an optimal iterative scheme for federated transfer learning, where a central planner has access to datasets ${\cal D}_1,\dots,{\cal D}_N$ for the same learning model $f_{\theta}$.  Our objective is to minimize the cumulative deviation of the generated parameters $\{\theta_i(t)\}_{t=0}^T$ across all $T$ iterations from the specialized parameters $\theta^\star_{1},\ldots,\theta^\star_N$ obtained for each dataset while respecting the loss function for the model $f_{\theta(T)}$ produced by the algorithm upon halting.  We only allow for continual communication between each of the specialized models (nodes/agents) and the central planner (server) at each iteration (round).  For the case where the model $f_{\theta}$ is a finite-rank kernel regression, we derive explicit updates for the regret-optimal algorithm.  By leveraging symmetries within the regret-optimal algorithm, we further develop a nearly regret-optimal heuristic that runs with $\mathcal{O}(Np^2)$ fewer elementary operations, where $p$ is the dimension of the parameter space.  Additionally, we investigate the adversarial robustness of the regret-optimal algorithm, showing that an adversary which perturbs $q$ training pairs by at most $\varepsilon>0$, across all training sets, cannot reduce the regret-optimal algorithm's regret by more than $\mathcal{O}(\varepsilon q \bar{N}^{1/2})$, where $\bar{N}$ is the aggregate number of training pairs. To validate our theoretical findings, we conduct numerical experiments in the context of American option pricing, utilizing a randomly generated finite-rank kernel. 
% \end{abstract}

% % \tableofcontents

% \section{Introduction}
% \label{s:Intro}

% In classical regression analysis, one typically selects a regression model $f:\Theta \times \mathbb{R}^d\rightarrow \mathbb{R}$ by optimizing a performance criterion on a (finite) training dataset $\mathcal{D}_1\subset \mathbb{R}^d\times \mathbb{R}$. The model $f$ is parameterized by $\Theta\subseteq \mathbb{R}^p$, with $p,d\in \mathbb{N}_+$, and for fixed $\theta \in \Theta$ we write $f_\theta \eqdef f(\theta, \cdot)$ for the function that maps the input $x\in \mathbb{R}^d$ to the model's output $y\in \mathbb{R}$.
% Selecting a regression model then amounts to identifying a \textit{parameter vector} $\theta_1 \in \Theta$ which is typically chosen to minimize the penalized sum-of-squares errors (SSE) on the given dataset
% \begin{equation}
% \label{eq:Regression_Klassische0}
%     \inf_{\theta \in \Theta}\, 
%             \sum_{(x,y)\in \mathcal{D}_1}\,
%                 (f_\theta(x)-y)^2
%         +
%             \kappa \,
%                 \|\theta\|_2.
% \end{equation}
% Here, $\kappa \geq 0$ is a hyperparameter controlling the regularity of the model, which is often implicitly reflected by the Euclidean norm of its parameter vector $\|\theta\|_2$, though other regularizers are available, for example in \cite{VDG_Sara_HighDimenisonalGLMsandLassi_AnnStat,simon2013sparse,AdcockAnyiBrugiapaglia_2019_NumerischeMath}.  Even if $y$ is obscured by ``noise'', there is an underlying homogeneity assumption underpinning~\eqref{eq:Regression_Klassische0}, namely that the training data all belongs to the same dataset and the elements of that dataset represent the same task.  Typically (see e.g.~\cite{bartlett2002rademacher,ZouAdaptiveLassoOracle_AnnStat_2006}), one assumes that there is a suitable, yet unknown, ``target'' function $f^\star:\mathbb{R}^d\rightarrow \mathbb{R}$ and a ``noise'' generating probability distribution $\mu$ on $\mathbb{R}$ such that for every $(x,y)$ in the training dataset $\mathcal{D}_1$ one has $y=f^{\star}(x)+\varepsilon_y$ where $\{\varepsilon_y\}_{(x,y)\in \mathcal{D}_1}$ are i.i.d.\ random variables with law $\mu$.
 
% A parameter vector optimizing~\eqref{eq:Regression_Klassische0} need not be available in closed-form.  Instead, provided it exists, it is typically identified approximately via an iterative gradient descent-type procedure.  Even if a closed-form expression exists, it is often more computationally efficient to resort to iterative algorithms \citep{YaoRosascoCoponnetto_2007_CA}.  A \textit{deterministic} iterative algorithm initialized at $\theta_0\in\mathbb{R}^p$ and running for $T\in\mathbb{N}_+$ iterations is characterized by its iterates.  Thus, any such iterative deterministic algorithm is identifiable with a sequence in $\mathbb{R}^p$ of length $1+T$; i.e.
% \begin{equation}
% \label{eq:algorithms}
%     \theta^{0\cdots T}\eqdef \left\{\theta(t)\right\}_{t=0}^T, 
%     \qquad 
%     \theta(0)=\theta_0.
% \end{equation}
% % \begin{equation}
% % \label{eq:algorithms}
% %     \theta_{\cdot}\eqdef (\theta(0),\dots,\theta(T)) 
% %     \qquad 
% %     \theta(0)=\theta_0.
% % \end{equation}
% With this identification and a measure of algorithmic efficiency, e.g.\ \textit{regret}, one can characterize the most efficient algorithm as in \cite{casgrain2019latent,casgrain2021optimizing}.

% The situation becomes more complicated in modern machine learning, where one often has access to large amounts of data, typically drawn from several \textit{similar}, yet \textit{distinct} sources.  
% These types of comparable datasets arise in meta-learning \citep{finn2017model,pavasovic2022mars}), in multi-task learning \citep{kumar2012learning,NEURIPS2020_3fe78a8a}, in quantitative finance due to natural market cycles \citep{lowry2002ipo}, or in robust finance approaches to model uncertainty resulting in several plausible stochastic time-series models wherewith data can be simulated \citep{hou2018robust,aksamit2019robust,prashanth2022wasserstein}.

% This paper focuses on the optimization aspect of the regression problem under multi-sourced data, with a focus on applications in mathematical finance, instead of the more often explored questions of learning-theoretic nature such as the risk of a federated learning procedure as in \cite{hu2023generalization,sun2023fedspeed}.  Specifically, we construct a \textit{regret-optimal federated optimization algorithm}, as defined shortly, under no communication restrictions between the server (central planner) and the local nodes (agents) at each round. 


% \paragraph{Optimizing with Multi-Sourced Data:}
% In situations where we have access to several distinct \emph{additional} datasets $\mathcal{D}_2,\dots,\mathcal{D}_N$ whose information we wish to leverage, we can improve the predictive performance of our regression model past what can be achieved using the focal or \textit{primary} dataset $\mathcal{D}_1$ in the classical approach~\eqref{eq:Regression_Klassische0}.
% Here, the underpinning assumption is that the datasets $\mathcal{D}_i$, for $i\neq 1$, are generated by a different, but comparable, mechanism from which $\mathcal{D}_1$ was generated.  

% The introduction of \textit{multi-sourced data} yields a spectrum of interpretations of optimality extending~\eqref{eq:Regression_Klassische0}, which can be naturally organized from a game-theoretic point of view.  In this perspective, we can consider several \textit{agents} (or nodes), each representing the influence of a dataset $\mathcal{D}_i$ on the model selection problem, who propose parameter vectors $\theta_1,\dots,\theta_N$ optimized for their own datasets. The agents are then  assumed to be organized by a \textit{central planner} (or server), representing the user. The objective of this central planner is to maximize the predictive power of the selected model on new data sampled from the same process which generated the focal dataset $\mathcal{D}_1$.  




% \paragraph{The Central Planner:}
% The purpose of the central planner is to avoid the situation whereby the structure of the different datasets is ignored in the model selection problem, by merging them into a single dataset $\mathcal{D}\eqdef \cup_{i=1}^N\,\mathcal{D}_i$ and thereby reducing the problem to~\eqref{eq:Regression_Klassische0}. Though intuitively simple, such merging  approach can be particularly disadvantageous in the presence of heterogeneity among the datasets, since a dataset that is potentially very different from the focal dataset $\mathcal{D}_1$ would be equally influential in the regression problem~\eqref{eq:Regression_Klassische0}.  
% Instead, the user, acting as a central planner, organizes the model selection problem through a cooperative objective
% \allowdisplaybreaks\begin{align} 
% \label{eq:terminal_time_objective}
% \begin{aligned}
%         l(\Theta, w;\,\mathcal{D} )  
%     \eqdef & 
%         \sum_{i=1}^N 
%         w_i
%             \sum_{j=1}^{|\mathcal{D}_i|} 
%                 (
%                 f_{\theta^w}(x_j^i)
%                 - y^i_j  
%                 )^2,
%     \\
%     \mbox{ with }
%     \,
%     \theta^w\eqdef & \sum_{i=1}^N 
%         w_i\,\theta_i
%  ,
% \end{aligned}
% \end{align} 
% where $\Theta\eqdef (\theta_1^{\top}, \cdots, \theta_N^{\top})^\top\in \mathbb{R}^{Np \times 1}$. Here, the central planner \textit{ascribes} the influence of each agent on the model selection problem through the weight vector $w=(w_1, \cdots, w_N)\in [0,1]^N$ with $\sum_{i=1}^N\,w_i=1$.  
% As can be seen in \eqref{eq:terminal_time_objective}, this influence is two-fold: on the one hand, it impacts the cooperative objective $l$ in the aggregation of the SSE of each player; on the other hand, it affects the proportion of each player's preferred parameter choice entering into the collectively selected parameter $\theta^{w}$.
% %
% The choice of $w$ is approached in different ways in the literature, e.g.\ by bagging 
% % $\frac1{N}\sum_{i=1}^N\, \theta^\star_i$ 
% reminiscent of mean-field games \citep{carmona2018probabilistic}, by data-driven weighting procedures \citep{Baxter_2000_JAIR__AmodelIndutvieBiasLearning}, Bayesian aggregation \citep{MR2280214,PACOH_rothfuss_2021,pavasovic2022mars}, or with dictionaries \citep{argyriou2006multi}.  

% \paragraph{The Agents:}
% When acting in isolation, each agent's preferred model is determined by optimizing a version of ~\eqref{eq:Regression_Klassische0} using only their dataset.  Under mild conditions\footnote{E.g.\ coercivity and lower semi-continuity in $\theta$.} on $f$, this corresponds to an {\em individual} parameter selection
% \begin{align}
%     \theta^{\star}_i \in 
%     \operatorname{argmin}_{\theta \in \Theta}
%         \, 
%             \sum_{(x,y)\in \mathcal{D}_i}\,
%                 (f_\theta(x)-y)^2
%         +
%             \kappa \,
%                 \|\theta\|_2, 
% \label{eq:Regression_Klassische1}
% \end{align}
% for $i=1,\dots,N$, which we assume to be fixed and known to all agents prior to their {\em collective} parameter selection. Taking into account the other agents, each agent \textit{acts} by specifying an iterative deterministic algorithm of the form~\eqref{eq:algorithms}, with the intent of maximizing their influence on the joint model selection problem~\eqref{eq:terminal_time_objective}.  Thus, the $i^{th}$ player wants the jointly selected model, specified by $\theta^{w}(T)=\sum_{n=1}^N\, w_i\,\theta_i(T)$, to be as close to $\theta_i^{\star}$ as possible, thereby maximally encoding the characteristics of the $i^{th}$ dataset into the selected model $f_{\theta^w(T)}$. The accumulated \textit{regret} which the $i^{th}$ player incurs by deploying an algorithm $\theta^{0\cdots T}_{i}$ that deviates from their preferred selection $\theta^*_i$ is measured by
% \begin{equation}
% \label{eq:penalized_regret_functional__REGRETFORM___Individual}
% \begin{aligned}
%     %     \mathcal{R}_i(\theta^{0\cdots T}_{i})
%     % \eqdef &
%             \sum_{t=0}^{T-1}  
%             \,
%                 \underbrace{
%                     \lambda \,
%                     \left\| \theta_i(t+1) - \theta^\star_{i} \right\|_2^2
%                 }_{\text{Preference Strength}}
%             + 
%                 \underbrace{
%                       \beta \, \left\| \Delta \theta_i(t) \right\|_2^2 
%                 }_{\text{Algorithm Stability}}
% ,
% \end{aligned}
% \end{equation}
% % \begin{equation}
% % \label{eq:penalized_regret_functional__REGRETFORM___Individual}
% % \begin{aligned}
% %         \mathcal{R}_i(\theta_{\cdot})
% %     \eqdef &
% %             \sum_{t=0}^{T-1}  
% %             \,
% %                 \underbrace{
% %                     \lambda \,
% %                     \left\| \theta(t+1) - \theta^\star_{i} \right\|_2^2
% %                 }_{\text{Preference Strength}}
% %             + 
% %                 \underbrace{
% %                       \beta \, \left\| \Delta \theta(t) \right\|_2^2 
% %                 }_{\text{Algorithm Stability}}
% % ,
% % \end{aligned}
% % \end{equation} 
% % \begin{align} 
% %  \frac{1}{|\mathcal{D}_i|} \sum_{(x,y)\in \mathcal{D}_i}\,
% %                 (f(\theta,x)-y)^2
% %         +
% %             \kappa \,
% %                 \|\theta\|_2 + \sum_{t=0}^T 
% %  \lambda \|\theta_i(t+1) - \theta_i^\star \|_2^2 
% %  + \beta\|\Delta \theta_i(t) \|_2^2
% % \end{align}
% where $\lambda>0$ is a hyperparameter quantifying the player's \textit{attachment} towards their preferred model choice $\theta^{\star}_i$ and the hyperparameter $\beta > 0$ quantifies the the stability of the algorithm during the iterations, where  $\Delta \theta_i(t)\eqdef \theta_i(t+1)-\theta_i(t)$.  
% % The regularization term $\sum_{t=0}^{T-1}\, \left\| \Delta \theta_i(t) \right\|_2^2$, in~\eqref{eq:penalized_regret_functional__REGRETFORM___Individual}, prohibits unstable algorithms from being deployed which ``teleport/jump'' to $\theta_i^{\star}$ and to their terminal position $\theta_i(T)$.  
% % \Anastasis{@Aurelien can you add a reference here, in the context of optimization for the quadratic term.}
% % \Aurelien{Can probably cite Convex Optimization Algorithms Dimitri P. Bertsekas} 


% The central planner then organizes the action $\Theta^{0\cdots T}\eqdef 
% \left\{\Theta(t)\right\}_{t=0}^{T}$ of the system of $N$ players to reach the objective~\eqref{eq:terminal_time_objective} while encoding their individual regrets~\eqref{eq:penalized_regret_functional__REGRETFORM___Individual}, where
% \begin{equation}
% \Theta (t) = (\theta_1(t)^\top,\ldots,\theta_N(t)^\top)^\top \in \mathbb{R}^{Np \times 1}. \notag 
% \end{equation}
% This is achieved by coupling the individual agent's regret functionals~\eqref{eq:penalized_regret_functional__REGRETFORM___Individual} through the \textit{systemic regret functional}
% \begin{equation}
% \label{eq:penalized_regret_functional__REGRETFORM}
% \begin{aligned}
%     \mathcal{R}(\Theta^{0\cdots T})
% \eqdef &
%         \underbrace{
%         l (\Theta(T), w;\,\mathcal{D} ) 
%         }_{\text{Cooperative Objective}}
%     -
%                   \,\,  l^{\star}
%     +
%         \sum_{t=0}^{T-1}  
%         \,
%              \big(
%                     \underbrace{
%                         \lambda \left\| \Theta(t+1) - \Theta^\star \right\|_2^2    
%                     }_{\text{Preference Strength}}
%                 + 
%                     \underbrace{
%                         \beta  \left\| \Delta \Theta(t) \right\|_2^2 
%                     }_{\text{Algo. Stability}}
%                 \big) 
%     ,
% \end{aligned}
% \end{equation} 
% where
% \begin{equation}
%     \label{Theta_star}
%     \Theta^\star\eqdef (\theta_1^{\star \top}, \cdots, \theta_N^{\star\top})^\top
%     \in \mathbb{R}^{Np \times 1}
% \end{equation}
% encodes the individual preferences of the players,
% % is a \textit{fixed initial condition} and the $N$-player system evolves according to 
% % \allowdisplaybreaks
% % \begin{align}
% % & \Theta(0)=\Theta^\star, 
% % \quad 
% % \Theta(t+1) = \Theta(t) + \Delta \Theta(t), 
% % \label{Theta-simple__nocontrol}
% % \end{align} 
% % for $\quad 0\leq t \leq T-1$, where 
% % $\Theta(0)=(\theta_1(0)^\top, \cdots, \theta_N(0)^\top)^\top \in \mathbb{R}^{Np\times 1}$, $\Theta(t)=(\theta_1^\top(t),\dots,\theta_N^\top(t))^\top$ is matrix notation, and 
% \begin{equation}
%     \Delta \Theta(t)\eqdef \Theta(t+1)-\Theta(t) 
%     \label{Theta-simple__nocontrol}
% \end{equation}
% quantifies the integrative updates of any candidate optimizing sequence $\Theta^{0\cdots T}$, and the \textit{ideal terminal loss} is 
% \[
%         l^{\star}
%     \eqdef 
%         \underbrace{
%             \min_{\Xi \in \mathbb{R}^{Np\times 1}}\, 
%                 l(\Xi,w; \mathcal{D}) 
%                 % + \lambda \|\Xi - \Theta^{\star} \|_2
%         }_{\text{Cooperative Sub-optimality}}
%     .
% \]
% The term $(l(\cdot,\cdot;\cdot)-l^{\star})$ measures the central planner's regret in failing to optimize~\eqref{eq:terminal_time_objective}.  The algorithm stability term in~\eqref{eq:penalized_regret_functional__REGRETFORM} appears in forward-backward proximal splitting algorithms with quadratic objectives (e.g. \cite{MR3619041,MR4490614}) and several standard proximal algorithms (see \cite[Section 5.1]{bertsekas2015convex}).

% The systemic regret functional~\eqref{eq:penalized_regret_functional__REGRETFORM} acts as a performance criterion for any optimization algorithm, played by $N$ players, initialized at an arbitrary $\Theta(0)$, and running for $T$ iterations.  
% In what follows, we take the initial condition of the algorithm as $\Theta(0)=\Theta^\star$ for simplicity, but other choices are possible. In other words, the regret of each player is initialized at zero, as they all start from their individually preferred parameter $\theta^\star_i$, and starts to accumulate as the system moves away from $\Theta^\star$ towards the optimizer of  \eqref{eq:penalized_regret_functional__REGRETFORM}.       


% \subsection{Contributions}
% \label{s:Introduction_Contrib}
% We exhibit a \textit{regret optimal} algorithm, by which we mean an optimizer of~\eqref{eq:penalized_regret_functional__REGRETFORM} when $f_{\theta}:\mathbb{R}^d\rightarrow \mathbb{R}$ is linear in its trainable parameter%%
% \footnote{We emphasize that all vectors are represented as column-vectors and not row vectors.} %%
% $\theta\in \mathbb{R}^p$ but non-linear in its inputs $x\in \mathbb{R}^d$ through
% a feature map $\phi:\mathbb{R}^d\rightarrow \mathbb{R}^p$, typically with $p\gg d$, namely 
% \begin{equation}
% \label{eq:FRKR}
% f_{\theta}(x)=\phi(x)^\top\theta.
% \end{equation}
% In this case, $f_\theta$ is called a \emph{finite-rank kernel ridge regressor} (fKRR) and a closed-form solution to the ridge-regression problem \eqref{eq:Regression_Klassische1} exists and is given by \eqref{eq:loss_one_dataset} in Appendix~\ref{s:Background}.

% A key insights is that~\eqref{eq:penalized_regret_functional__REGRETFORM} has the same minimizers as the energy functional 
% \allowdisplaybreaks\begin{align} 
% \label{eq:penalized_regret_functional}
%     {\cal L}(\Theta^{0\cdots T})
% \eqdef &
%     \underbrace{
%         \sum_{t=0}^{T-1}  
%         \,
%              \left[  
%                     \lambda \left\| \Theta(t+1) - \Theta^\star \right\|_2^2    
%                 + 
%                     \beta \left\| \Delta \Theta(t) \right\|_2^2 
%             \right] 
%     }_{\text{
%         Running-Cost
%     }}
%     + 
%     \underbrace{
%         l (\Theta(T), w;\,\mathcal{D} ) 
%     }_{\text{
%     Terminal Cost
%     }}
% .
% \end{align} 
% Every algorithm~\eqref{eq:algorithms} can be regarded as driven by a ``control'', and the functional ${\cal L}$ has the form of a ``cost function'' of an optimal control problem,  decomposable into the sum of a ``running/operational cost'' and a ``terminal/objective cost''.  This allows us to leverage tools from optimal control \citep{touzi2013optimal} to derive a  closed-form expression of the unique regret-optimal algorithm driven by the unique ``optimal control'' as defined in Algorithm~\ref{alg:RegretOptimization}.  

% We prove that this procedure is adversarially robust, meaning that the value of~\eqref{eq:penalized_regret_functional} varies by $\mathcal{O}(\varepsilon \sqrt{\bar{N}}q)$ if a malicious adversary can perturb at most $1/q$ percent of all the data in each of the dataset $\mathcal{D}_i$ by at-most $\varepsilon\ge 0$, where $\bar{N}=\sum_{i=1}^N |\mathcal{D}_i|$.  
% Furthermore, we show that our regret-optimal algorithm has a computational complexity of $\mathcal{O}(N^2p^3 + T\,(Np)^{2.373})$.  
% Moreover, we characterize the optimal choice of the weights $w$ 
% % defining~\eqref{eq:terminal_time_objective} 
% which the central planner must use to maximize the selected model's performance on the primary/focal dataset $\mathcal{D}_1$.  

% Finally, we show that if all the datasets $\mathcal{D}_1$, $\dots$, $\mathcal{D}_N$ are equally dissimilar (but not necessarily similar) then the regret-optimal algorithm can be accelerated.  This acceleration requires $\mathcal{O}(N\,p^2)$ fewer elementary operations.  We also show that if this ``accelerated'' algorithm is used in situations when the datasets differ by a little, then it does not deviate far from the regret-optimal algorithm.  Thus it can be used as an accelerated heuristic.  


% \subsection*{Outline}   
% The paper is organized as follows. In Section~\ref{s:Main}, we introduce the regret-optimal algorithm and demonstrate the optimality, computational complexity, and adversarial robustness of the algorithm. We  further introduce an accelerated algorithm of lower computational complexity that can achieve near-regret optimality. 
% In Section~\ref{s:Experiments_n_Validation}, we conduct a convergence analysis of the regret-optimal algorithm and compare it to the standard gradient descent approach. Then we show the transfer learning capabilities of the algorithm for American option pricing.  
% Appendix~\ref{s:Proofs_TechnicalLemmata} is denoted to proving the optimality, adversarial robustness, and computational complexity of the regret-optimal algorithm. The near-regret optimality and computational complexity of the accelerated algorithm are also proven. Appendix~\ref{s:Background} briefly introduces the background of finite-rank kernel ridge regressors.   

% \subsection*{Notation}
% We briefly introduce some additional notation.
% Each dataset has a finite number of samples which we write as $\mathcal{D}_i = \{ (x_j^i, y_j^i) \, | \, 1 \leq j \leq |\mathcal{D}_i| \}$. We assume that some feature map $\phi$ is fixed and denote the features of each sample of $\mathcal{D}_i$ as 
% $$u_j^i \eqdef \phi(x_j^i).$$ 
% Moreover, we denote the joint inputs and outputs for each dataset as 
% \begin{align}
%     X^i \eqdef \left( x^i_1, \cdots , x^i_{|\mathcal{D}_i|} \right)^\top \in \mathbb{R}^{|\mathcal{D}_i| \times d} \quad \text{ and } \quad
%     Y^i \eqdef (y^i_1, \cdots, y^i_{|\mathcal{D}_i|})^\top \in \R^{|\mathcal{D}_i|}, \notag 
% \end{align}
% and the joint features as
% \begin{align} 
% U^i \eqdef \Phi(X^i) \eqdef 
% \left( \phi(x^i_1), \cdots , \ 
%  \phi(x^i_{|\mathcal{D}_i|}) \right)^\top \in \mathbb{R}^{|\mathcal{D}_i| \times p}. \notag  
% \end{align} 
% Finally, we use $I_p$ to denote a $p\times p$ identity matrix. 

% \subsection{Related Work}
% \label{s:Introduction__sss:RelatedWork}

% Examples of $f_\theta$ of the form \eqref{eq:FRKR} include extreme learning machine \citep{gonon2020risk,gonon2022approximation,ghorbani2022linearized,MeiMontanari_CommPaAMath_2022__DoubleDescent} or any finite-rank kernel ridge regressor (fKRR) \citep{Amini_2021_EJS_SpectrallyTruncatedKernel,amini2022target}.  Random feature models, and finite-rank ridge regressors, are typical in contemporary quantitative finance \citep{gonon2021random,herrera2023optimal} or reservoir computing \citep{cuchiero2021discrete}, where it is favourable to rapidly deploy a deep learning model due to time or computing-power limitations/constraints.  Finite-rank kernel ridge regressors are also typical in the setting of standard transfer \citep{howard2018universal} and multi-task learning \citep{ren2018cross,jia2019leveraging} pipelines where one often has a pre-trained deep neural network model and, for any novel task, the user freezes the hidden layers in the deep neural network model and only fine-tunes/trains the deep neural network's final linear layer.  
% This is useful, since the hidden layers of most deep neural network architectures are known to process general, cruder features and the final layer of any such model captures finer, task-specific features \citep{zeiler2014visualizing,yosinski2014transferable}.


% The optimization of a model trained from multiple data sources lies at the heart of multi-task learning.  In  \cite{SenerKoltun_MultiTaskLEarningMultiObjectiveOptimization__NeurIPS2018}, the authors cast the task of optimizing~\eqref{eq:terminal_time_objective} as a multi-objective optimization problem.  They propose to solve it via a multi-gradient descent algorithm which, under mild conditions, converges to a Pareto stationary point; i.e.\ which is essentially a critical point of each of the $i$-th player's penalized SSE.  
% Though iterative schemes for multi-objective optimization can efficiently reach critical points \citep{fliege2019complexity}, this problem's critical point is not necessarily a minimum since the problem~\eqref{eq:terminal_time_objective} is not convex when $w$ is shared amongst all $N$ players.  

% This proposed algorithm reflects the ideas of the federated stochastic gradient descent (FedSGD) algorithm of \cite{SINGHZHU_FedSGD_2018} and of its online counterpart FedOGD which is an online federated version of online gradient descent\footnote{See \cite[Chapter 3]{hazan2016introduction} for details on online gradient descent} and more efficient online versions thereof such as \cite{kwon2022tighter}.  From the federated learning perspective, the problem of training individual fKRR on each dataset, and then centralizing them by optimizing the mixing parameter $w$ in~\eqref{eq:terminal_time_objective} and its origins date back to local gradient descent introduced in the optimization and control literature in \cite{Mangasarian_1995_localGD}.  Though several authors (e.g. \cite{TighterTheoryLocalSGD}) have proposed various progressive improvements of federated gradient-descent-type algorithms for training a learner from several data sources, the problem of studying \textit{the} most efficient iterative federated learning algorithm for regret minimization has not yet been tackled.  

% We note that (stochastic) optimal control tools have revealed new insights into machine learning.  Examples include an optimal step-size control \citep{li2017stochastic} and batch-size control \citep{zhao2022batch}, developing online subgradient methods that adapt to the data's observed geometry \citep{DuchiHazanSinger_2011_JMLR_adaptiveSGOnlineOptim}, developing new maximum principle-based training algorithms for deep neural networks \citep{JMLR:v18:17-653}, or unifying (stochastic) optimization frameworks \citep{Casgrain_LatentVarStochOptim_2019}.

% \section{Main Results}
% \label{s:Main}

% This section contains the description of the \textit{unique} regret-optimal algorithm and an analysis of its theoretical properties. Throughout our manuscript, we maintain the following two assumptions.  
% \begin{assumption}[$\mathcal{D}$-Boundedness]
% \label{assm:bddxy} 
% There are constants $K_x,K_y>0$ such that all 
% $(x^i_j, y^i_j) \in \mathcal{D}$ satisfy $\|u^i_j\|_2 \leq K_x$ and $|y^i_j|^2 \leq K_y$, where $u^i_j = \phi (x^i_j)$. 
% \end{assumption}
% % \begin{assumption}[$\mathcal{D}$-Boundedness]
% % \label{assm:bddxy} 
% % There are constants $K_x,K_y>0$ such that all 
% % $(u^i_j, y^i_j) \in \cup_{i=1}^N \mathcal{D}_i$ are norm-bounded
% % $\|u^i_j\|_2 \leq K_x$ and $\|y^i_j\|_2 \leq K_y$. 
% % \end{assumption}
% \begin{assumption}[$(w^{\star},\mathcal{D})$-Compatibility]
% \label{assm:PD}
% The data ${\cal D} = \cup_{i=1}^N\,\mathcal{D}_i$ and the weights $w^{\star}$ satisfy 
% \allowdisplaybreaks
% \begin{align} 
%  & \sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|} u^i_j u^{i\top}_j \geq 0 , 
%  \label{Sum(uij)Tuij>=0}\\  
% & [w^\star_1 I_p ,\cdots, w^\star_N I_p]^{\top} 
%  \left( \sum_{i=1}^N
%  w^\star_i \,
%  \sum_{j=1}^{|\mathcal{D}_i|}  u^i_j u^{i\top}_j \right)  
%  [ w^\star_1 I_p, \cdots, w^\star_N I_p ] \geq 0 . 
%  \label{WeightedSum(uij)Tuij>=0}
%  \end{align} 
% \end{assumption}
% With the notation introduced before, the 
% object $[w_1^\star I_p, \cdots, w_N^\star I_p ]$ above is a $p \times Np$ matrix.



% \subsection{The Algorithms}
% \label{s:Main_ss:Algorithm}

% \begin{figure}[H]%[ht!]%
%     \centering
%      \begin{subfigure}[b]{0.45\textwidth}
%      \centering
%         \includegraphics[width=0.75\textwidth]{Graphics/Information_Sharing.pdf}
%     \caption{Step 1: Adaptive ``Prior'' Sharing: The $i^{th}$ dataset $\mathcal{D}_i$ is shared with the main dataset $\mathcal{D}_1$ if the best model $f_{\theta^\star_i}$, optimizing~\eqref{eq:Regression_Klassische1} on dataset $\mathcal{D}_i$, can outperform the optimal model trained on the main dataset, up to a slack factor $\eta>0$.  The relative importance of each dataset is proportional to $f_{\theta^\star_i}$'s performance relative to the training performance of the best model trained on the main dataset.
%     When $\eta$ is small, sharing is unlikely; when $\eta$ is large, nearly all datasets are pooled together with approximately the same relative importance.}
%         \label{fig:information_sharing_prior}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.45\textwidth}
%          \includegraphics[width=0.6\textwidth]{Graphics/Information_Sharing_inhomogeneous.pdf}
%     \caption{Step 2: Optimized ``Posterior'' Sharing: We then optimize the relative importance/weights given to the shared datasets from the naive adaptive sharing.  The optimization is a closed-form update of the adaptive ``prior'' weights which optimize a certain maximum expected performance criterion subject to a relative entropy penalization against the weights obtained from adaptive prior sharing.}
%     \label{fig:information_sharing_posterior}
%      \end{subfigure}
%     \caption{Visual Summary of Optimal Information Sharing (Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart}).}
%     \label{fig:information_sharing}
% \end{figure}

% We begin by describing our procedure for determining the optimal mixture weights defining the cooperative objective function \eqref{eq:terminal_time_objective} used in ~\eqref{eq:penalized_regret_functional__REGRETFORM}.  This procedure is illustrated graphically in Figure~\ref{fig:information_sharing} and detailed in Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart}.   


% \begin{algorithm}[ht!]%[H]%
% \caption{{Optimal Information Sharing - Initialization to Algorithm~\ref{alg:RegretOptimization}}}
% %\label{alg:RegretOptimization}
% \label{alg:RegretOptimizationHeuristic__WarmStart}
% \begin{algorithmic}
% \SetAlgoLined
% \Require Datasets $\mathcal{D}_1,\dots,\mathcal{D}_N$, finite-rank kernel $\phi$, hyperparameters\footnote{Different ridge hyperparameters $\kappa$ can be used to define each regressor in Algorithm ~\ref{alg:RegretOptimizationHeuristic__WarmStart}} $\kappa,\eta>0$.
% \DontPrintSemicolon
%     \State \tcp{Initialize Locally-Optimal Learners and Record Scores on Main Dataset}  
%     %\tcc{Initialize Locally-Optimal Learners and Record Scores on Main Dataset} 
%     \State \SetKwBlock{ForParallel}{For $i:1,\dots,N$ in parallel}{end}
%         \ForParallel{\State 
%         $\theta^\star_i \leftarrow  
%  ( \Phi^\top(X^i) \Phi(X^i)  
%   + \kappa I_p )^{-1} 
%   \Phi^\top(X^i) Y^i$ 
%             \tcp*{Optimize each fKRR}
%         \State $s^i
%             \leftarrow  
%         \frac1{|\mathcal{D}_1|}\sum_{j=1}^{|\mathcal{D}_1|}\,
%                 \big\|
%                         f_{\theta^\star_i}(u_j^1)
%                     -  y_j^1
%                 \big\|_2^2
%         $
%         % \State 
%         \tcp*{Score predictive power of fKRR on main dataset}
%         } 
%         \State \tcp{Get Adaptive Prior} 
%         \State \SetKwBlock{ForParallel}{For $i:1,\dots,N$ in parallel}{end} 
%         \ForParallel{\State $
%             w_i
%                 \leftarrow 
%             \frac{   
%                 [s^1+\eta-s^i]_+
%             }{ \sum_{j=1}^N\, [s^1+\eta-s^j]_+ }
%         $}
%         \State \tcp{Get Optimized Posterior} 
% \State \SetKwBlock{ForParallel}{For $i:1,\dots,N$ in parallel}{end} 
%         \ForParallel{\State $
%             w^\star_i
%                 \leftarrow 
%             \frac{
%                     e^{
%                     s_i/\eta
%                 }   
%                 \,
%                 [s^1+\eta-s^i]_+
%             }{
%                 \sum_{j=1}^N\,
%                     e^{s_j/\eta}[s^1+\eta-s^j]_+
%             }
%         $}
%     \State \Return Optimal Weights $w^\star$ and Locally-Optimal fKRR Parameters $\theta^\star_1,\dots,\theta^\star_N$.
% \end{algorithmic}
% \end{algorithm}

% \vspace{0.2in}

% Suppose now that we have used Algorithm \ref{alg:RegretOptimizationHeuristic__WarmStart} to compute weights $w^\star=(w^\star_1, \cdots, w^\star_N)$ and the locally optimal fKRR parameters $\theta^\star_1$, ..., $\theta^\star_N$, and $w^{\star}$. The key novelty in the next algorithm follows a similar spirit to \cite{JMLR_MaximumBasedDL_LiChenTaiCheng} and \cite{casgrain2021optimizing}, by casting the problem of constructing a regret-optimal algorithm as an optimal control problem. 

% As before, denote 
% \allowdisplaybreaks\begin{align} 
%  & \Theta(t)\eqdef [ \theta_1^{\top}(t), \cdots, \theta_N^{\top}(t) ]^{\top}, \quad 
%  \Theta^\star \eqdef [ \theta^{\star \top}_1, \cdots, \theta^{\star \top}_N ]^{\top} , 
%  \notag \\ 
%  & \boldsymbol\alpha(t) \eqdef [\alpha_1^{\top}(t), \cdots, \alpha_N^{\top}(t)]^{\top}, \notag   
% \end{align} 
% which are all elements of $\R^{Np}$, and introduce the dynamics that $\Theta$ follows    \allowdisplaybreaks\begin{align} 
% & \Theta(0)=\Theta^\star, 
% \quad 
% \Theta(t+1) = \Theta(t) + \boldsymbol\alpha(t) , 
% \quad 0\leq t \leq T-1 ,   
% \label{Theta-simple}  
% \end{align} 
% which is equivalently written as   \allowdisplaybreaks\begin{align} 
%  \Theta(t+1) = \Theta^\star + \sum_{u=0}^{t} \boldsymbol\alpha(u) , \quad 0\leq t \leq 
%   T-1 . 
% \label{Theta(t)Theta(0)} 
% \end{align}

% Then, since the optimizers of the energy~\eqref{eq:penalized_regret_functional} coincide with the optimizers of the systemic regret functional~\eqref{eq:penalized_regret_functional__REGRETFORM}, searching for a regret-optimal algorithm reduces to solving for an optimal control $\mathbf{\alpha}$ to minimize the cost 
% \eqref{eq:penalized_regret_functional} subject to \eqref{Theta-simple}.  
% The optimal control problem 
% \eqref{eq:penalized_regret_functional} and \eqref{Theta-simple} is a discrete-time linear quadratic optimal control problem, and can be solved by dynamic programming methods that are standard in the literature. For instance, by \cite[Proposition 5.1]{BO1998}, we obtain the solution for the regret-optimal algorithm in closed-form as solutions of a system of Riccati equations \eqref{eqnP(t) 0} and \eqref{eqnS(t) 0}, given in
% Theorem~\ref{thm:RegretOptimal_Dynamics__MainTextFormulation}. 

% Algorithm~\ref{alg:RegretOptimization} below implements the optimal control approach in two steps. In Step 1, we solve the equation system \eqref{eqnP(t) 0} and \eqref{eqnS(t) 0} backwards for $t=T$, $T-1$, ..., $1$. Then in Step 2, we obtain the optimal control $\boldsymbol\alpha(t)$ and update the parameter $\Theta(t)$ for $t=0$, $1$, ... $T$. 

% %by Algorithm~\ref{alg:RegretOptimization}.
% \begin{algorithm}[ht]%[H]
% \caption{Regret-Optimal Optimization Algorithm}
% \label{alg:RegretOptimization}
% \begin{algorithmic}
% \SetAlgoLined
% \Require Datasets $\mathcal{D}_1,\dots,\mathcal{D}_N$, $N$.\ Iterations $T\in \mathbb{N}_+$, finite-rank kernel $\phi$ and hyperparameters $\lambda, \beta, \kappa, \eta >0$.
% \DontPrintSemicolon
%     \State 
%     \tcp{Get Initialize Weights and Locally-Optimal fKRR Parameters}
%     %%%% Externalized
%         \State $\theta^\star_1,\dots,\theta^\star_N,w^{\star}$ $\leftarrow$ Run: Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart} with $\mathcal{D}_1,\dots,\mathcal{D}_N$, $\phi$, and $\kappa,\eta$.
   
%     \State 
%     \tcp{Initialize Updates}
%     \State $P(T) 
%     = [w_1^\star I_p , \cdots, w_N^\star I_p ]^\top \left(\sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|}  u^i_j u_j^{i\top}\right) [w_1^\star I_p, \cdots, w_N^\star I_p ] $ 

% \State $S(T) = -[w_1^\star I_p , \cdots, w_N^\star I_p ]^\top \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|}  u^i_j y^i_j$ 

% \State $\Theta(0) = \Theta^\star \eqdef (\theta_1^{\star \top}, \cdots, \theta_N^{\star \top} )^\top$ 

%     \State \tcp{Generate Iterates}
%     \State \For{$t=T-1,\dots,1$}{
%         \State \tcp{Update Driving Parameters} 

% \State $P(t)= \beta I_{Np} - \beta^2 [(\lambda+\beta)I_{Np} + P(t+1)]^{-1}$

% \State $S(t) = \beta [(\lambda + \beta )I_{Np} + P(t+1)]^{-1} (S(t+1) - \lambda \Theta^\star)$
% }


% \State\For{$t=0, ..., T-1$}{
%   \State\tcp{Update Control} 

% \State 
% $\boldsymbol{\alpha}(t) = -[(\lambda+\beta )I_{Np} + P(t+1)]^{-1} 
% [(\lambda I_{Np} + P(t+1))\Theta(t) - \lambda \Theta^\star + S(t+1) ]$

% \State 
% $\Theta(t+1)=\Theta(t)+\boldsymbol{\alpha}(t)$
% }

% \State \Return Return the Optimized fKRR $f_{\theta^{w^\star}}$
% \end{algorithmic}
% \end{algorithm} 

% In the next subsections, we state our primary results, whose proofs are presented in Appendix \ref{s:Proofs_TechnicalLemmata}. We first quantify the optimality of Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart}. Next, we establish the optimality, complexity, and adversarial robustness of Algorithm~\ref{alg:RegretOptimization}.  

% \subsection{{Properties of Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart}}}
% \label{s:Main_Algorithm_2}

% By decoupling the optimization of the ``dataset-relevant weights'' $w$ in Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart} from the optimization of the parameter $\theta$ in Algorithm ~\ref{alg:RegretOptimization}, we avoid open-loop forward-backward iterations, which iterate between optimizing $w$ and $\theta$.  We now study the optimality of the weight $w^{\star}$ generated by Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart}.  The weights $w^{\star}$ represent the optimal probability distributions of randomly selecting amongst the $N$ optimized regressors $\{ f_{\theta^\star_i} \}_{i=1}^N$, each optimized locally on their dataset $\mathcal{D}_i$ by solving~\eqref{eq:Regression_Klassische1}.  Here, optimality is quantified in terms of the best-expected prediction on the focal dataset $\mathcal{D}_1$ subject to a penalty for deviating too far from a reference distribution.  This reference distribution serves to automatically delete models whose datasets are too dissimilar to $\mathcal{D}_1$.  Inspired by most meta-learning problems, e.g. \cite{pavasovic2022mars}, similarity is quantified by extracting a ``similarity score'' from each learner.  


% Let $\mathcal{P}(\{\theta^\star_i\}_{i=1}^N)$ consist of all probability measures on the set $\{\theta^\star_i \}_{i=1}^N$.  Any probability measure $\mathbb{P}_w$ in $\mathcal{P}(\{\theta^\star_ i\}_{i=1}^N)$ is uniquely determined by a weight $w$ in the $N$-simplex; consisting of all $w\in [0,1]^N$ whose entries sum to $1$.  Let $\theta$ be a random variable with law $\mathbb{P}_{w}$, for some $\mathbb{P}_w\in \mathcal{P}(\{\theta^\star_i \}_{i=1}^N)$.  The average performance of the random learner $f_{\theta}$ on the dataset $\mathcal{D}_1$ is
% \begin{equation}
% \label{eq:optimizingQ}
%     \mathbb{E}_{\theta \sim \mathbb{P}_w}\,
%         \left[
%             \frac1{|\mathcal{D}_1|}\sum_{j=1}^{|\mathcal{D}_1|}\,
%             \big\|
%                     f_{\theta}(u_j^1)
%                 -
%                     y_j^1
%             \big\|_2^2
%         \right]
%     =
%         \sum_{i=1}^N\,
%             w_i
%             %%% Score
%             \underbrace{
%             \biggl[
%                 \frac1{|\mathcal{D}_1|}\sum_{j=1}^{|\mathcal{D}_1|}\,
%                 \big\|
%                         f_{\theta^\star_i}(u_j^1)
%                     -
%                         y_j^1
%                 \big\|_2^2
%             \biggl]
%             }_{i^{th} \mbox{ learner's score }(s_i)} .
% \end{equation}


% Fix an \textit{information sharing level} $ \eta > 0$.  The information sharing level $\eta$ adaptively determines which of the datasets in $\mathcal{D}$ are implicitly shared with the principle dataset $\mathcal{D}_1$.  The information sharing is formalized through the probability measure 
% \[
% \bar{\mathbb{P}}^{\eta}(\theta^\star_i) \eqdef 
% \frac{
% [s^1+\eta -s^i]_+
% }{
% \sum_{i=1}^N\, [s^1 + \eta - s^i]_+
% }
% .
% \]
% on the set of $N$ learners, or equivalently on the parameters $\theta^\star_1,\dots,\theta^\star_N$.  
% The measure $\bar{\mathbb{P}}^{\eta}$ thus allows us to minimize the regularized version of the loss in~\eqref{eq:optimizingQ},
% \begin{equation}
% \label{eq:optimizingQ__regularized}
%     \min_{
%         \mathbb{P}_w
%     }
%     \,
%     \,
%     \underbrace{
%     \mathbb{E}_{\theta \sim \mathbb{P}_w}\biggl[
%         % \Big[
%             \frac1{|\mathcal{D}_1|}\sum_{j=1}^{|\mathcal{D}_1|}\,
%             % w_i\,
%             \big\|
%                     f_{\theta}(u_j^1)
%                 -
%                     y_j^1
%             \big\|_2^2
%     \biggr]
%     }_{i^{th} \mbox{ learner's score }(s_i)}
%     +
%     \underbrace{
%         % (1-\eta)
%         \eta\,
%         \operatorname{D}_{\operatorname{KL}}\big(
%             \mathbb{P}_w
%         \|
%             \bar{\mathbb{P}}^{\eta}
%         \big)
%     }_{
%     \underset{\mbox{information sharing}}{\mbox{Inhomogeneity of}}
%     }
% ,
% \end{equation}
% where the infimum is taken over all $\mathbb{P}_w$ in $\mathcal{P}(\{\theta^\star_i\}_{i=1}^N)$ and  $\operatorname{D}_{\operatorname{KL}}$ denotes the \textit{Kulbeck-Leibler divergence with respect to $\bar{P}^{\eta}$} given for any probability measure $\mathbb{P}_w$ on $\{\theta^\star_i\}_{i=1}^N$, namely 
% \[
%         \operatorname{D}_{\operatorname{KL}}\big(\mathbb{P}_w\| \bar{\mathbb{P}}^{\eta})
%     \eqdef 
%         % \begin{cases}
%             \sum_{i=1}^N\,
%                 w_i\,
%                 % \Biggl(
%                     \log\biggl(
%                         % \sum_{j=1}^N\,[s^1+\eta-s^j]_+
%                         \frac{w_i}{
%                         [s^1+\eta-s^i]_+
%                         }
%                         % \Big)
%                     % +
%                     % \log\big(
%                         % \sum_{j=1}^N\,[s^1+\eta-s^j]_+
%                         C_{\eta}
%                     % \big)
%                     \biggr)
%                 % \Biggr)
%         %         & \mbox{ if } \mathbb{P}\ll \mathbb{Q} \\
%         %     \infty & \mbox{ otherwise } 
%         % \end{cases}
% ,
% \]
% where $C_{\eta}\eqdef  \sum_{j=1}^N\,[s^1+\eta-s^j]_+$, if $\mathbb{P}_w$ is absolutely continuous with respect to $\bar{\mathbb{P}}^{\eta}$ and otherwise $\operatorname{D}_{\operatorname{KL}}\big(\mathbb{P}_w\| \bar{\mathbb{P}}^{\eta})=\infty$.  
% There is a unique probability measure optimizing the penalized functional~\eqref{eq:optimizingQ__regularized} determined by the weight $w^{\star}$ in Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart}.
% %%
% %%
% %%
% \begin{theorem}[Optimality of Weights $w^{\star}$ in Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart}]
% \label{prop:Optimal_Bayes_Weighting}
% Fix $\eta>0$.  The unique weights $w^{\star}_i$ on the $N$-simplex minimizing~\eqref{eq:optimizingQ__regularized} are given by 
% \begin{equation}
% \label{eq:prop:Optimal_Bayes_Weighting__OptimalWeights}
% \begin{aligned}
%     w^{\star}_i
% = 
%         \frac{
%                 e^{
%                 s^i/\eta
%             }   
%             \,
%             [s^1+\eta-s^i]_+
%         }{
%             \sum_{j=1}^N\,
%                 e^{s^j/\eta}[s^1+\eta-s^j]_+
%         }
% , \qquad  i=1,\dots,N.
% \end{aligned}
% \end{equation}

% \end{theorem}


% \subsection{Guarantees for Algorithm~\ref{alg:RegretOptimization}}
% \label{s:GuaranteesTheoretical__ss:Algo_1}



% %Our first result shows that Algorithm~\ref{alg:RegretOptimizationHeuristic}, and its iterates, are near-regret optimal.  Moreover, the degree of near-optimality depends only on the data, through the mixing parameter $w^{\star}$.  

% Our next result shows that Algorithm~\ref{alg:RegretOptimization}, and its iterates, are regret-optimal. 

% \begin{theorem}[Algorithm~\ref{alg:RegretOptimization} Computes the Unique Regret-Optimal Algorithm]
% \label{thm:RegretOptimal_Dynamics__MainTextFormulation}
% Suppose that Assumptions~\ref{assm:bddxy} and~\ref{assm:PD} hold and fix $\Theta^{\star}\in \mathbb{R}^{N\,p}$ as in \eqref{Theta_star}.  Then, the systemic regret functional $\mathcal{R}$ defined in~\eqref{eq:penalized_regret_functional__REGRETFORM} admits a unique minimizer $\hat\Theta_{\cdot}\eqdef (\hat\Theta(t))_{t=0}^T$ of the form~\eqref{Theta-simple__nocontrol} with $\hat\Theta(0) = \Theta^{\star}$ aand increments
% \allowdisplaybreaks\begin{align} 
%  \Delta \hat\Theta(t)  
%  = & -[(\lambda + \beta )I_{Np} + P(t+1)]^{-1} 
%  \big[ (\lambda I_{Np} + P(t+1)) \hat\Theta(t) 
%  - \lambda  \Theta^\star + S(t+1)  \big] ,   \label{optimala 0} 
% \end{align} 
% where, for $t=1,\dots,T$,  the matrices $P(t)$ and $S(t)$ in \eqref{optimala 0} are determined by
% \allowdisplaybreaks\begin{align} 
% & \begin{cases}
%  P(T) =  [w^\star_1 I_p ,\cdots, w^\star_N I_p]^{\top} 
%  \left( \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|}   u^i_j u^{i\top}_j \right)  
%  [ w^\star_1 I_p, \cdots, w^\star_N I_p] \\
%    P(t)  =  \beta I_{Np} - \beta^2 [(\lambda+\beta) I_{Np} + P(t+1) ]^{-1}  \label{eqnP(t) 0} 
% \end{cases},   \\
% %%%  
% & \begin{cases}
%  S(T) =  - [ w^\star_1 I_p, \cdots, w^\star_N I_p]^{\top} \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|}  {u^i_j} y^i_j \\
%   S(t) =  \beta \big[ (\lambda+\beta)I_{Np} + P(t+1) \big]^{-1} (S(t+1) - \lambda \Theta^\star )
%   \label{eqnS(t) 0}    
% \end{cases} .
% %\begin{align} 
% \end{align} 
% In particular, for each $t=0,\dots,T-1$ 
% \[
%         \Delta \hat\Theta(t) 
%     = 
%         \boldsymbol{\alpha}(t)
% ,
% \]
% where $\boldsymbol{\alpha}$ is as in Algorithm~\ref{alg:RegretOptimization}. 
% \end{theorem}
% \begin{remark}
%     Instead of the sums we can equivalently use our matrix notation to write $\sum_{j=1}^{|\mathcal{D}_i|} u^i_j u^{i\top}_j = {U^i}^\top U^i$ and $\sum_{j=1}^{|\mathcal{D}_i|}  {u^i_j} y^i_j = U^{i\top} Y^i$. 
% \end{remark}

% The explicit update rules for the regret-optimal optimization algorithm presented above permit us to compute its complexity.  Since we will be assuming that we work with \textit{floating-point arithmetic}, all elementary arithmetic operations (e.g.\ addition, subtraction, multiplication) are of constant (i.e.\ $\mathcal{O}(1)$) complexity.  We are most interested in the regime where the number of datasets is much larger than the typical number of instances/data per dataset; i.e.\ when
% \begin{equation}
% \label{eq:moredatasets_than_dataperdataset}
%         \frac1{N}\sum_{i=1}^N\,|\mathcal{D}_i| 
%     \le 
%         N
% .
% \end{equation}
% %%
% %%%
% %% 
% \begin{theorem}[Complexity of Regret-Optimal Algorithm]
% %\label{cor:ComplexityAlgorithm}
% \label{thm:ComplexityAlgorithm}
% In the setting of Theorem~\ref{thm:RegretOptimal_Dynamics__MainTextFormulation}, the computational complexity\footnote{We emphasize that we have assumed that computational complexity of all elementary arithmetic operations (e.g.\ addition, subtraction, multiplication) is $\mathcal{O}(1)$.} of computing the sequence $(\hat \Theta(t))_{t=0}^T$ defining the regret-optimal algorithm is $
%     \mathcal{O}\big( N^2 p^3 +
%         T
%         \, 
%         (Np)^{2.373}
%         %N^{2.373}\, p^2
%     \big)
% .
% $
% \end{theorem}




% Next, we quantify the sensitivity of Algorithm~\ref{alg:RegretOptimization} to adversarial attacks.  We study the robustness of Algorithm~\ref{alg:RegretOptimization} with respect to a family of perturbations that switch a given percentage $0\le q\le 1$ of all training data by selecting fake data points at a distance of at-most $\varepsilon\ge 0$ for any perturbed datapoint.  Thus, for a fixed set of datasets 
% $\{ \mathcal{D}_i \}_{i=1}^N$, and $q,\varepsilon$ as above, 
% we define the class $\mathbb{D}^{q,\varepsilon}$ of \textit{adversarially generated datasets} of ``magnitude'' $(q,\varepsilon)$ as all sets of datasets 
% $\{ \widetilde{\mathcal{D}}_i \}_{i=1}^N$, $\widetilde{\mathcal{D}}_i=\{ \{(\tilde{x}^i_j,\tilde{y}^i_j) \, | \, 1 \leq j \leq |\mathcal{D}_i| \}\subseteq \mathbb{R}^{d}\times \mathbb{R}$ satisfying Assumptions~\ref{assm:bddxy} and~\ref{assm:PD}, as well as
% % we define the class $\mathbb{D}^{q,\varepsilon}\subseteq \mathbb{R}^{d}\times \mathbb{R}^d$ of \textit{adversarially generated datasets} of ``magnitude'' $(q,\varepsilon)$ as all sets of datasets $\widetilde{\mathcal{D}}=\{ \{(\tilde{x}^i_j,\tilde{y}^i_j) \, | \, 1 \leq j \leq |\mathcal{D}_i| \} \, | \, 1 \leq i \leq N\}$ satisfying Assumptions~\ref{assm:bddxy} and~\ref{assm:PD}, as well as
% \[
%         %%%% Number of Perturbed Instances
%         \underbrace{
%                     \frac{
%                         \#\{
%                             (i,j):\, u^i_j\neq \tilde{u}^i_j \mbox{ or } y^i_j\neq \tilde{y}^i_j
%                         \}
%                     }{
%                         \sum_{i=1}^N\,|\mathcal{D}_i|
%                     }
%                 \le 
%                     q
%         }_{\mbox{Attack Persistence}}
%     \mbox{ and }
%             %%%% Maximum Magnitude of Adversarial Perturbations
%         \underbrace{
%                     \max_{i,j} \left\{ \,
%                         \max\left(
%                             \|u^i_j-\tilde{u}^i_j\|_2 
%                         ,
%                             |y^i_j-\tilde{y}^i_j|^2
%                         \right) \right\}
%                 \le 
%                     \varepsilon
%         }_{\mbox{Attack Severity}}
% ,
% \]
% where the indices $(i,j)$ run over $\{(i,j) \, | \, 1 \leq i \leq N,\,1 \leq j \leq |\mathcal{D}_i|\}$ and $\tilde{u}^i_j\eqdef \phi(\tilde{x}^i_j)$.

% In view of Theorem~\ref{thm:RegretOptimal_Dynamics__MainTextFormulation}, the updates of the unique regret-optimal algorithm $\hat \Theta^{0\cdots T}$ are determined by the sequence $\boldsymbol{\alpha}_{\cdot}\eqdef (\boldsymbol{\alpha}(t))_{t=0}^T$ computed by Algorithm~\ref{alg:RegretOptimization}.  It is convenient to emphasize this connection on $\boldsymbol{\alpha}_{\cdot}$ and the connection with the dataset $\mathcal{D}$ when expressing the following theorem, with the energy~\eqref{eq:penalized_regret_functional} determining the value of the systematic regret functional $\mathcal{R}$.  We therefore write $
%     {\cal L}(\boldsymbol{\alpha};\mathcal{D})
%         \eqdef 
%     {\cal L}(\hat\Theta^{0\cdots T})
% .$
% \begin{theorem}[Adversarial Robustness]
% \label{thrm:adv_robust}
% Fix a $\mathcal{D}$ satisfying Assumptions~\ref{assm:bddxy} and~\ref{assm:PD}.  For any level of ``attack persistence'' $0\le q\le 1$ and any degree of ``attack severity'' $\varepsilon\ge 0$ we have that
% \[
%         \big| {\cal L} (  \boldsymbol\alpha ; \mathcal{D} ) 
%         -  
%         {\cal L}(  \widetilde{\boldsymbol\alpha} ;  \widetilde{\mathcal{D}} )  \big|
%     \le 
%         \mathcal{O}\Big(
%             \varepsilon
%             \sqrt{\bar{N}\,q}
%         \Big)
% ,
% \]
% where 
% $\widetilde{\boldsymbol\alpha}$ is the output of Algorithm~\ref{alg:RegretOptimization} for any given adversarially-generated set of datasets 
% $\{ \widetilde{\mathcal{D}}_i \}_{i=1}^N\in \mathbb{D}^{q,\varepsilon}$ and $\bar{N}=\sum_{i=1}^N |\mathcal{D}_i|$.  Here $\mathcal{O}$ hides a constant depending only on Assumption~\ref{assm:bddxy}.  
% \end{theorem}



% \subsection{An Accelerated Heuristic}
% \label{s:Main__ss:AcceleratedHeuristic}
% We now discuss a situation in which the computational complexity of the regret-optimal algorithm can be reduced.  This is achieved by exploiting symmetries in the optimal policy computed by Algorithm~\ref{alg:RegretOptimization}.

% Examining the explicit update rules, we notice that \textit{if} the weights $w$ defining the energy~\eqref{eq:penalized_regret_functional} were to be $\overline{1/N}\eqdef (1/N,\dots,1/N)$ then the matrices defining the optimal policy/control's updates would become highly symmetric Toeplitz matrices, depending on exactly three $p$-dimensional block sub-matrices.  This allows us to parameterize the entire regret-optimal algorithm, for the sub-optimal weights $\overline{1/N}$, using only three low-dimensional systems whose dimension is \textit{independent} of the number of datasets $N$.  In line with this, Algorithm~\ref{alg:RegretOptimizationHeuristic} implements the regret-optimal algorithm for the weight specification $\overline{1/N}$ by only keeping track of these three optimal low-dimensional systems, and then efficiently recombining them by leveraging the Toeplitz structure defining the optimal policy/control.  These low-dimensional systems are defined using \textit{helper functions}, listed in equations \eqref{gamma1}-\eqref{eq:RegretOptimizationHeuristic_Helper__1}.

% The approximate near-optimality of Algorithm~\ref{alg:RegretOptimizationHeuristic} only depends on the stability of the optimal policy/control, defining the algorithm's updates as a function of the weights $w$.  If the optimal weights defining the systemic regret functional~\eqref{eq:penalized_regret_functional__REGRETFORM} are close to $\overline{1/N}$, then Algorithm~\ref{alg:RegretOptimizationHeuristic} is nearly regret-optimal.  Otherwise, the sub-optimality it incurs in favor of computational efficiency is explicitly quantifiable and depends only on the difference between the optimal weights computed in Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart} and the symmetric weights $\overline{1/N}$.


% Note now record, the matrix-valued functions $\gamma_1(\cdot)$ and $\gamma_2(\cdot)$ used to define the updates in Algorithm~\ref{alg:RegretOptimizationHeuristic}.  

% \begin{algorithm}[htp!]%
% \caption{Accelerated (Nearly) Regret-Optimal Algorithm}
% \label{alg:RegretOptimizationHeuristic}
% \begin{algorithmic}
% \SetAlgoLined
% \Require Datasets  $\mathcal{D}_1,\dots,\mathcal{D}_N$, $N$.\ Iterations $T\in \mathbb{N}_+$, finite-rank kernel $\phi$, hyperparameters $\lambda, \beta, \kappa, \eta >0$.
% \DontPrintSemicolon
%     \State  
% \tcp{Get Initialize Weights and Locally-Optimal fRKR Parameters}
%     %%%% Externalized
%        \State $\theta^\star_1,\dots,\theta^\star_N,w^{\star}$ $\leftarrow$ Run: Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart} with $\mathcal{D}_1,\dots,\mathcal{D}_N$, $\phi$, and $\kappa,\eta$.
%     \State 
%   \tcp{Initialize Updates}
%     \State $\pi_1(T) 
%     = \pi_2(T) 
%     = (1/N^3) \sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|}  u^i_j u^{i\top}_j$
%     \State $\pi_3(T) 
%     =  - (1/N^2) \sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|}  {u^i_j} y^i_j $
%  \State $\theta_1(0) = \theta^\star_1$, $\theta_2(0) = \theta^\star_2$, $\dots$, $\theta_N(0) =\theta^\star_N$
% \State $\theta^\star_{(N)} = \frac{1}{N} \sum_{i=1}^N \theta^\star_i .$
%     \State \tcp{Generate Iterates}
%     \State \For{$t=T-1,\dots,0$}{
%         \State \tcp{Update Low-Dimensional Driving Parameters} 

% \State$\pi_1(t)= \beta I_p- \beta^2 \gamma_1(t+1)$ 
% \tcp{$\gamma_1(\cdot)$ is defined by \eqref{gamma1}}

% \State $\pi_2(t) = - \beta^2 \gamma_2(t+1)$ 
% \tcp{$\gamma_2(\cdot)$ is defined by \eqref{gamma2}}

% \State $\pi_3(t)
% = \beta \big[ \gamma_1(t+1)
% + (N-1) \gamma_2(t+1)
% \big] ( \pi_3(t+1) -\lambda \theta^\star_{(N)})$ }

% \State\For{$t=0, ..., T-1$}{ 
%   \State \tcp{Update Low-Dimensional Control} 
%  \State \For{$i=1, ..., N$}{
%   \State $\widehat{\alpha}_i(t)
%   =  \widehat{\alpha}\big(\theta_i(t) ,\ 
%  (\theta_j(t))_{j = 1,j\neq i}^N ,\ (\gamma_i(t+1))_{i=1}^2, 
%    \ (\pi_i(t+1))_{i=1}^3 \big)$ 
   
%  \State $\theta_i(t+1) =\theta_i(t) + \widehat{\alpha}_i(t)$ } } 
 
%  \State \Return Synchronized fKRR 
% $f_{\theta^{w^\star}}$
% \end{algorithmic}
% \end{algorithm} 

% The matrix-valued functions $\gamma_1(\cdot)$ and $\gamma_2(\cdot)$ in Algorithm~\ref{alg:RegretOptimizationHeuristic} are defined as 
% \allowdisplaybreaks 
% \begin{align} 
% & \gamma_1(\cdot) \eqdef 
% \big\{ (\lambda+\beta )I_p
% +\pi_1(\cdot) \notag \\
% & \hspace{2cm} - (N-1) \pi_2(\cdot)\big[ (\lambda+ \beta )
% I_p + \pi_1(\cdot) 
% + (N-2)\pi_2(\cdot)]^{-1} \pi_2(\cdot) \big\}^{-1} , 
% \label{gamma1} \\ 
%  & \gamma_2(\cdot)  \eqdef 
%  - \gamma_1(\cdot) \pi_2(\cdot) 
%  \big[ (\lambda+\beta )I_p + \pi_1(\cdot) 
%  + (N-2)\pi_2(\cdot) \big]^{-1},  \label{gamma2}
% \end{align} 
% where 
% \begin{align*}
%     \pi_1(T) = \pi_2(T) = \frac{1}{N^3} \sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|}  u^i_j u^{i\top}_j 
%     \qquad 
%     \mbox{ and }
%     \qquad
%     \pi_3(T) =  - \frac{1}{N^2} \sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|}  {u^i_j} y^i_j 
% \end{align*}
% and, for $t=T-1,\dots,0$,
% \begin{align*}
%   \pi_1(t) &= \beta I_p- \beta^2 \gamma_1(t+1) \\ 
%   \pi_2(t) &= - \beta^2 \gamma_2(t+1) \\
%   \pi_3(t) &= \beta \big[ \gamma_1(t+1)
% + (N-1) \gamma_2(t+1)
% \big] \left( \pi_3(t+1) -\lambda \theta^\star_{(N)}\right)
% \end{align*}
% where $\theta^\star_{(N)} = \frac{1}{N} \sum_{i=1}^N \theta^\star_i$.

% The updates of the low-dimensional systems which Algorithm~\ref{alg:RegretOptimizationHeuristic} exploits are implemented via the helper function $\hat \alpha$, defined as 
% \allowdisplaybreaks 
% \begin{align} 
% \label{eq:RegretOptimizationHeuristic_Helper__1}
%   \widehat{\alpha}\big( \theta_i, ((\theta_j)_{j=1,j\neq i}^N) , (\gamma_i)_{i=1}^2,(\pi_i)_{i=1}^3 \big)  \eqdef &  
%  - (\gamma_1-\gamma_2)(\lambda I_p + \pi_1 - \pi_2 )\theta_i \notag \\ & 
%  - \big\{ \gamma_1 \pi_2 + \gamma_2 [ \lambda I_p + \pi_1 + (N-2)\pi_2 ] \big\} \sum_{j=1}^N \theta_j \notag \\ 
%  & - \big[ \gamma_1 + (N-1) \gamma_2 \big] 
%  (\pi_3 - \lambda \theta^\star_{(N)}) . 
%  \end{align}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% \vspace{0.2in} 
% The degree to which Algorithm~\ref{alg:RegretOptimizationHeuristic} is nearly regret-optimal depends on how far the weights $w$ determined by Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart} are from the equal weighting $\overline{1/N}$.  This is precisely quantified by the following results.

% \begin{theorem}[Near-Regret Optimality]\label{thrm:Epsilon_Efficiency}
% Suppose that $\mathcal{D}$ satisfies Assumptions~\ref{assm:bddxy} and~\ref{assm:PD}.  and let $\hat\Theta^{0\cdots T}$ denote the unique regret-optimal algorithm\footnote{That is, the unique optimizer of~\eqref{eq:penalized_regret_functional}} computed according to Algorithm \ref{alg:RegretOptimization}. Then, the output $\vartheta^{0\cdots T}$ of Algorithm~\ref{alg:RegretOptimizationHeuristic} satisfies
% \vspace{0.2in}
% \begin{enumerate}
%     \item[(i)] \textbf{Near-Optimality:} The difference $\big|
%             {\cal L}(\Theta^{0\cdots T})
%             -
%             {\cal L}(\vartheta^{0\cdots T})
%         \big|$ is of the order
%     \begin{align}
%     %    & \big|
%     %         {\cal L}(\Theta^{0\cdots T})
%     %         -
%     %         {\cal L}(\vartheta^{0\cdots T})
%     %     \big|
%     % \in 
%     &
%         \mathcal{O}\Big(
%                    \bar{N} N^3 \max_{1\leq i, k, l \leq N} \Big| \frac{1}{N^3} -  w^\star_k w^\star_l w^\star_i\Big| 
%                   + \bar{N} N^{3/2} \max_{1\leq k, l\leq N} \Big| \frac{1}{N^2} - w^\star_k w^\star_l \Big| 
%                   \notag \\ 
% & \hspace{5cm} + \bar{N}  \max_{1\leq i \leq N} \Big|\frac{1}{N} - w_i^\star \Big| 
%  + N \big\|\Theta^\star - \Theta^\star_{(N)} \big\|_2 
%         \Big)
%         \notag
%     ,
%     \end{align}
%     \item[(ii)] \textbf{Near-Optimal Increments:} The difference $\|\Delta \Theta^{0\cdots T-1}-\Delta \vartheta^{0\cdots T-1} \|_{\ell^1}$ is of the order
%     \begin{align} 
%        & 
%     %    \|\Delta \Theta^{0\cdots T-1}-\Delta \vartheta^{0\cdots T-1} \|_{\ell^1}
%     % \in 
%         \mathcal{O}\Big(
%                 \bar{N} N^{3/2} \max_{1\leq i, k, l \leq N} \Big| \frac{1}{N^3} -  w^\star_k w^\star_l w^\star_i \Big| \notag \\  
%  & %\hspace{5cm} 
%  + \bar{N} N^{1/2} \max_{1\leq k, l\leq N} \Big| \frac{1}{N^2} - w^\star_k w^\star_l \Big| 
%   +  \big\|\Theta^\star - \Theta^\star_{(N)}\big\|_2
%         \Big),
%         \notag
%     \end{align}
% \end{enumerate}
% where $\mathcal{O}$ hides a constant depending only on $\lambda$, $\beta$, 
% $\Theta^{\star}$, $(w_1^\star, ..., w_N^\star)$, $T$, $K_x$, and in $K_y$.  
% \end{theorem}

% The next result shows that Algorithm~\ref{alg:RegretOptimizationHeuristic} accelerates the regret-optimal algorithm by a linear factor in $N$ and by a quadratic factor in $p$, when $N$ is large.  
% %%%
% \begin{theorem}[$\mathcal{O}\big(N\,p^2\big)$-Acceleration over Regret-Optimal Algorithm]
% \label{thrm:accelertion_heuristic_regret_optimal_algorithm}
% With the convention that floating-point arithmetic operations are $\mathcal{O}(1)$, we have that:
% \begin{enumerate}
%     \item[(i)] \textbf{Complexity:} Algorithm~\ref{alg:RegretOptimizationHeuristic} has a complexity of $\mathcal{O}(TNp\max\{N,p\}))$
%     \item[(ii)] \textbf{Acceleration over Regret-Optimal Algorithm:} The regret-optimal algorithm has a complexity of $\mathcal{O}\big(TN^3 p^3\big)$.
% \end{enumerate}
% When $N\ge p$, Algorithm~\ref{alg:RegretOptimizationHeuristic} requires $\mathcal{O}(N\,p^2)$ fewer operations than the regret-optimal algorithm.  
% \end{theorem}

% % \Anastasis{I added this to held the reader understand Algo 1's solution:}\hfill\\
% % {\color{violet}{
% Finally, we establish that Algorithm~\ref{alg:RegretOptimizationHeuristic} is the regret-optimal algorithm, optimizing the systemic regret functional~\eqref{eq:penalized_regret_functional}, in the ``symmetric'' case where the optimal weights $w^{\star}$ are all $(1/N,\dots,1/N)$.  
% \begin{theorem}[Regret-Optimality in the Symmetric Case]
% \label{thrm:regretoptimality_SymmetricCase}
% Suppose that $w^{\star}_i=1/N$ for $i=1,\dots,N.$  Then, $\hat\Theta^{0\cdots T}=\vartheta^{0\cdots T}$.  
% \end{theorem}
% % }}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % We now examine the empirical performance of our algorithm.

% \section{Experiments}
% \label{s:Experiments_n_Validation}
% We now experimentally verify our theoretical results, with a focus on quantitative finance.
% In particular, we implemented the regret-optimal algorithm as well as its accelerated version and provide them together with the code for all experiments described in this section at \code.

% First, we conduct a convergence analysis of our regret-optimal algorithm, comparing it to standard gradient descent. We then demonstrate the transfer learning capabilities of our algorithm in the context of American option pricing.  
% We use the randomized neural networks approach of \cite{herrera2023optimal} as our fKRR model, since it best balances computational efficiency and expressiveness amongst the available non-linear versions of the \cite{longstaff2001valuing} algorithm for American option pricing.


% \subsection{Convergence of the Regret-Optimal Algorithm}
% \label{sec:Convergence of the Regret Optimal Algorithm}
% We first study the evolution of the energy functional  \eqref{eq:penalized_regret_functional} and loss \eqref{eq:terminal_time_objective} achieved in each iteration by our regret-optimal Algorithm~\ref{alg:RegretOptimization} with weights initialized by Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart}. That is to say, we compute ${\cal L}(\Theta^{0\cdots t})$ as defined in \eqref{eq:penalized_regret_functional} but for intermediate iterations $t$, as well as the loss $l(\Theta(t), w;\,\mathcal{D})$. 
% % the sum over the weights stops at $t-1$ and for the loss $l(\Theta(t), w;\,\mathcal{D})$ of the current weights is used. 
% We compare the regret-optimal algorithm with its accelerated version, given by Algorithm~\ref{alg:RegretOptimizationHeuristic} with weights given by Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart}, where we use $\Theta(0) = \Theta^\star_{(N)}$ and replace $\Theta^\star$ by $\Theta^\star_{(N)}$ in \eqref{eq:penalized_regret_functional}.
% Moreover, we compare to the results when using gradient descent to optimize the loss \eqref{eq:terminal_time_objective} directly.
% For all algorithms we use a ridge coefficient $\kappa=0$, regret coefficients $\lambda = 0$, $\beta=1$  and Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart} with information sharing level $\eta=10$ to get the corresponding optimal weights $w^\star$ and to initialize $\Theta(0)$ with the locally optimal parameters.
% We note that the comparison of our algorithms to gradient descent optimizing the loss \eqref{eq:terminal_time_objective} only makes sense in the $\lambda=0$ regime, since otherwise the objectives and therefore the behaviour are different. On the other hand, using $\beta > 0$ doesn't change the objective, but only forces our algorithm to make equally sized steps $\Delta \Theta (t)$, where the step size depends on $\beta$ and $T$.

% For our convergence analysis we use $N=5$ randomly generated datasets. In particular, each dataset $\mathcal{D}_i$ corresponds to a neural network $g_{\omega_i}$ with fixed randomly-generated hidden weights and biases.  Here $\omega_i$ denotes the vector of all these hidden weights and bias parameters. The networks have $d=5$ dimensional input, one hidden layer with $10$ hidden nodes, $\operatorname{ReLU}$ activation function and map to a $1$-dimensional output. The dataset is generated by sampling $S_i = 100$ inputs $x^i_j$ from a $d$-dimensional standard normal distribution and the corresponding target values are given by $g_{\omega_i}(x^i_j)$, i.e.,
% \begin{equation*}
%     \mathcal{D}_i = \{ (x^i_j, g_{\omega_i}(x^i_j)) \, | \, 1 \leq i \leq S_i, x^i_j \sim N(0,I_d) \}.
% \end{equation*}

% Our feature map $\phi$ in~\eqref{eq:FRKR} is a randomized neural network%
% \footnote{Also called a random feature model or an extreme learning machine} %
% with one hidden layer, $500$ hidden nodes and $\operatorname{ReLU}$ activation as studied by \cite{mei2021generalization,gonon2020risk,gonon2021random}. In particular, the weights of the hidden layers are randomly initialized and fixed and only the weights of the last layer, corresponding to $\theta$ in \eqref{eq:FRKR}, are optimized. We note that by our choice for the number of hidden nodes to equal the total number of samples, the algorithms can in principle learn to have perfect replication on the training set, i.e., loss $l(\Theta(t), w;\,\mathcal{D}) = 0$.
% For a fair comparison between the algorithms, we use the same randomly generated datasets and the same randomized neural networks for each of the methods.

% Figure~\ref{fig:convergence analysis} shows the averaged results for 10 runs each with a different set of randomly generated datasets and a different randomized neural network as fKRR. For the regret-optimal algorithm and for its accelerated version we use $T=10^3$ iterations, while we use $10^5$ steps for gradient descent with learning rate $7 \cdot 10^{-5}$. We note that for learning rates $\geq 8 \cdot 10^{-5}$ the training becomes unstable such that the loss explodes. 
% The gradient descent method gradually but slowly reduces the loss.
% Since the gradient descent method makes so small parameter updates (and since $\lambda=0)$, the regret is nearly $0$ and the energy ${\cal L}$ nearly equal to the loss. Even though it runs $100$ times the number of iterations of our algorithms, it would still need much more training to achieve the same loss.
% On the other hand, the regret-optimal algorithm and its accelerated version behave nearly indistinguishably, reducing the loss nearly to $0$ and piling up a little bit of regret. We note that by increasing the number of iterations, our algorithms could reduce the loss further by making smaller parameter updates and therefore piling up less regret, allowing them to focus even more on reducing the loss.

% \begin{figure}[!ht]%[H]
%         \centering            
%         \includegraphics[width=0.32\textwidth]{Graphics/conv_analysis-1}
%         \includegraphics[width=0.32\textwidth]{Graphics/conv_analysis-2}
%         \includegraphics[width=0.32\textwidth]{Graphics/conv_analysis-3}
%         \caption{Loss and energy ${\cal L}$ for gradient descent (GD), the regret-optimal algorithm (RO) and the accelerated regret-optimal algorithm (ARO). Means and standard deviations over 10 runs are shown. Left: all iterations; middle: first 1000 iterations; right: iterations 500 to 1000 for our algorithms.}
%         \label{fig:convergence analysis}
% \end{figure}

% In the regime where $\lambda > 0$ the behaviour of the algorithm changes drastically. In particular, since deviating from $\Theta(0) = \Theta^\star$ is penalised, the algorithm remains at the starting point in the initial steps and only starts to converge when approaching $T$. The exact behaviour depends on the choice of $\lambda$ (and is additionally influenced by the choice of $\beta$). In Figure~\ref{fig:convergence analysis 2} we compare the behaviour for $\lambda=10^{-4}$ and $\lambda = 2$ while otherwise using the same setup as before.  For the smaller value of $\lambda$, the algorithm starts the decent earlier and decreases the loss by more compared to the larger value for $\lambda$, where the algorithm deviates from $\Theta^\star$ only in the very last steps. 
% \begin{figure}[!ht]%[H]
%         \centering            
%         \includegraphics[width=0.48\textwidth]{Graphics/conv_analysis-4}
%         \includegraphics[width=0.48\textwidth]{Graphics/conv_analysis-5}
%         \caption{Loss and energy ${\cal L}$ for the regret-optimal algorithm (RO) and the accelerated regret-optimal algorithm (ARO). Means and standard deviations over 10 runs are shown. Left: $\lambda = 10^{-4}$; right: $\lambda=2$.}
%         \label{fig:convergence analysis 2}
% \end{figure}







% \subsection{American Option Pricing}
% \label{sec:American Option Pricing}
% We test our algorithm in the context of the optimal stopping problem for American option pricing, a computationally highly challenging problem which has recently become tractable also in higher dimensional settings through deep learning \citep{PatrickDOSJMLR_2019,Ruimeng_QF_OptimStopping,Timo_DOS_2021,herrera2023optimal}. This is a good example for our purpose for two reasons. 
% On the one hand, \cite{herrera2023optimal} did show that randomized neural networks, which are one class of fKRR, are well suited to (approximately) solve these optimal stopping problems. Moreover, it was shown that using randomized neural networks can heavily improve the computation time, which is also of importance to us since we need to solve several optimizations problems for a potentially large number of datasets.
% On the other hand, to solve the optimal stopping problem one needs to generate synthetic datasets. Hence, this problem allows us to generate multiple synthetic datasets of different sizes and varying similarity on which we can test the transfer-learning capabilities of our algorithm. The performance can be measured by comparing the achieved prices with those of several baseline methods.

% We first provide a short recap of the optimal stopping problem in American option pricing and then present our transfer-learning experiments.

% \subsubsection{Background: American Option Pricing and Optimal Stopping}\label{sec:Recap: American Option Pricing and Optimal Stopping}
% An American option is a financial derivative that gives its owner the right to execute a certain predetermined trade at any time between the start date and the maturity of the option. For example, a call (put) option gives its owner the right to buy (sell) a certain stock from the writer of the option for a fixed price $K$, called the strike. If the current stock price $X_t$ is higher (lower) than $K$ then the option owner can make a profit of $(X_t - K)_+$ (or $(K - X_t)_+$ respectively) by directly selling (buying) the stock again in the open market after having exercised their right to buy (sell) from the option writer. 
% While American options allow for continuous-in-time execution, it is common practice to approximate them via Bermudan options, which can be executed on a predetermined time grid $t_0 < \dotsb t_M$. We briefly overview the American option pricing problem, details of which can be found in \citep[Chapter 25]{PeshirShiryaev_FreeBoundaryProblems_2006Book}.


% In order to capture the computational challenges posed by the American option pricing problem in higher dimensions, we consider a stochastic process $(X_t)_{t=0}^M \in (\R^d)^{(M+1)}$ describing the price of $d$ stocks on the time grid 
% % Let $(X_t)_{t=0}^M \in \R^{(M+1)}$ be a stochastic process describing the price of a stock on the time grid
% and let $(Z_t)_{t=0}^M \in \R^{(M+1)}$ be the corresponding discounted payoff process of an American option written on a one-dimensional process obtained from $X_t$ (e.g. the largest price among the $d$ stocks). We define the filtration $\mathbb{F} = (\mathcal{F}_t)_{t=0}^M$ generated by $X$ via $\mathcal{F}_t = \sigma(X_s | s\leq t)$. Then the price of the American option is given by the starting value $U_0$ of the \emph{Snell envelope} \citep{SnellOGPaper_1952_SemiMartingaleOptimalStopping}, given by
% \begin{equation}\label{equ:snell envelope 2}
% U_m = \operatorname{sup}_{\tau \in \mathcal{T}_m} \E[ Z_{\tau} \, | \, \mathcal{F}_m ],
% \end{equation}
% where $\mathcal{T}_m$ is the set of all stopping times $\tau \geq m$. 
% The smallest optimal stopping time is
% \begin{align}\label{equ: optimal stopping time}
% \tau_M &:= M, \\
% \tau_m &:= \begin{cases}
% m, & \text{if } Z_m \geq \E[U_{m+1}  \, | \, \mathcal{F}_m],\\
% \tau_{m+1}, & \text{otherwise},
% \end{cases} \nonumber
% \end{align}
% hence, to compute the price of the American option it suffices to compute the \emph{continuation values} $\E[U_{m+1}  \, | \, \mathcal{F}_m]$ for all $m$. 
% In the following, we will use the \textit{randomized least squares Monte Carlo} (RLSM) algorithm of \cite{herrera2023optimal}, which utilises randomized neural networks to approximate the continuation values via backward induction (note the backward recursive scheme that \eqref{equ:snell envelope 2} and \eqref{equ: optimal stopping time} imply).
% In particular, this leads to $M$ backward-recursively defined regression problems that need to be solved sequentially. Since \eqref{equ:snell envelope 2} is a maximisation problem and since we only approximate the optimal stopping time, we compute lower bounds of the price $U_0$.
% The standard procedure is to fix some law for the process $X$ and to sample a dataset of $\nu = \nu_1+\nu_2$ i.i.d.\ paths of $X$, where $\nu_1$ of them are used for training the randomized neural networks (approximating the continuation value functions) and $\nu_2$ of them are used to evaluate the resulting price $U_0$ (using these trained networks). 
% Through the independence of the two parts of the dataset it is clear that any over-fitting bias the networks might learn will \emph{not} lead to prices that are too large. This is important, since the quality of a method can therefore be evaluated by the resulting price, using a higher price indicating a a better result. 
% % For more details we refer the interested reader to \cite{herrera2023optimal}.


% \subsubsection{Transfer Learning in American Option Pricing}\label{sec:Transfer Learning in American Option Pricing}
% In order to test the transfer learning capabilities of our algorithm, we do not generate a very large dataset of the most plausible distribtution of $X$ as is standard practice. Instead we generate many smaller, more or less similar datasets $\mathcal{D}_1, \dotsc, \mathcal{D}_N$ out of which  $\mathcal{D}_1$ is considered our main dataset on which we evaluate the performance.

% We always use the RLSM algorithm to price the American options and only vary the optimization method used internally by RLSM to solve the $M$ recursive regression problems arising at the exercise dates. Depending on the chosen optimisation method only one, multiple or all datasets are taken into account to compute the parameters of the randomized neural network at the given exercise date. 
% We compare our regret-optimal (RO) optimisation method of Theorem~\ref{thm:RegretOptimal_Dynamics__MainTextFormulation} to the following baselines.
% \begin{itemize}
%     \item \textbf{Local optimizer (LO-$i$).} The local optimizers $\theta^\star_i$ solves the individual optimisation problem on the datasets $\mathcal{D}_i$ without considering the other datasets.
%     \item \textbf{Mean Local optimizer (MLO).} The mean of the local optimizers $ \bar{\theta}^\star = \frac{1}{N} \sum_{i=1}^N \theta^\star_i$ is the bagging aggregation.
%     \item \textbf{Joint optimizer (JO).} The joint optimizer ${\theta}^\star_{\mathcal{N}}$ with $\mathcal{N}=\{ 1, \dotsc, N\}$ solves the optimisation problem of the pooled regime $\mathcal{D} = \cup_{i=1}^N \mathcal{D}_i$.
%     \item \textbf{Joint Subset optimizer.} This is the joint optimizer for any subset $\mathcal{I} \subset \mathcal{N}$ of the datasets $\mathcal{D}_{\mathcal{I}} = \cup_{i \in \mathcal{I}} \mathcal{D}_i$.
% \end{itemize}
% In this application we are only interested in the terminal parameters $\Theta(T)$. We know that our algorithm yields the parameters optimising \eqref{eq:penalized_regret_functional} for any $T\geq 1$ since there exists a closed-form solution. Hence, we choose $T=1$ which is most specialized on minimizing \eqref{eq:terminal_time_objective}, while the influence of the running costs \eqref{eq:penalized_regret_functional__REGRETFORM___Individual} can be controlled via the choice of $\lambda$ and $\beta$. Additionally, this minimizes the computation time for our algorithm.

% As fKRR we use the same randomized neural networks as in Section~\ref{sec:Convergence of the Regret Optimal Algorithm}.
% The random weights of the randomized neural networks, as well as the randomly sampled paths both introduce some randomness into the pricing problem. Therefore we follow \cite{herrera2023optimal} by always running the experiments $n_{runs} = 100$ times with different seeds and taking means over the prices. For easier comparison, we then consider the relative performance ($RP$) on our main dataset, computed as the mean price of any given method divided by the mean price of the local optimizer on the main dataset.
% Additionally, we compute asymptotically valid (by the central limit theorem) $95\%$-confidence-intervals as $RP \pm z_{0.975}\hat\sigma/\sqrt{n_{runs}}$, where $z_{0.975}$ is the $0.975$-quantile of the standard normal distribution and $\hat\sigma$ is the standard deviation  of $RP$ (computed as the sample standard deviation of the prices over the runs divided by the mean price of the local optimizer on the main dataset).
% To make the results comparable between the optimization methods, we use the same seeds for all of them, such that run $i$ always uses the exact same paths and the exact same random weights in the randomized neural network, independently of the chosen method.
% Moreover, we always use $\nu_2 \geq 50,000$ evaluation paths, such that the noise of the Monte Carlo approximation of the expectations is relatively small when evaluating the prices, even if we use much smaller training set sizes $\nu_1$.

% In the first experiment we study the ability of our method to transfer knowledge of those datasets, out a large number of small equally-sized datasets, benefiting the main task.

% \begin{experiment}\label{exp:1}{\rm 
%     In this experiment we generate $13$ different datasets, all of a Heston model with $\nu_1 = 100$ training samples but with different parameters.
%     The Heston model is defined as
%     \begin{equation}\label{equ:heston model}
%     \begin{split}
%     d X_t &= (r - \delta) X_t dt + \sqrt{v_t} X_t d W_t, \\
%     d v_t &= -k (v_t - v_{\infty}) dt + \sigma \sqrt{v_t}d B_t,
%     \end{split}
%     \end{equation}
%     where $W$ and $B$ are two Brownian motions with correlation $\rho \in [-1,1]$.
%     The main dataset $\mathcal{D}_1$ has the parameters $r=0.05$, $\delta=0.1$, $k=2$, $v_{\infty}=0.01$, $\sigma=0.2$, $\rho=-0.3$ and starting values $X_0=100$ and $v_0=v_\infty$.
%     The other datasets are define as all combinations of $r \in \{0.05, 0.5\}$, $\sigma \in \{ 0.15, 0.2, 0.25 \}$, $v_{\infty} \in \{ 0.005, 0.015 \}$ and otherwise the same parameters as the main dataset.
%     For all datasets we use a max call option with strike $K=100$ on $d=2$ i.i.d.\ stocks of the given model with $M=9$ equidistant exercise dates until the maturity $T_{mat} = 3$. The discounting factor is $e^{-r\,T_{mat}\,t/M}$ for $0\leq t \leq M$.
%     Moreover, we use a randomized neural network with one hidden layer with $300$ nodes and all methods use the ridge coefficient $\kappa=2$ and, where applicable, regret coefficients $\lambda=2, \beta=1$.
    
%     We report the results in Table~\ref{table:results exp 1}.
%     For our regret-optimal method (RO) we use information sharing levels $\eta \in \{  10, 100, 500\}$ and see that $\eta=100$ leads to the best result outperforming the local optimizer of the main dataset (LO-1) by $9\%$. It also outperforms all other local optimizers (LO-$i$), the mean local optimizer (MLO) and the joint optimizer (JO).
%     For $\eta=10$ we have similar performance as LO-1 and for $\eta=500$ we also have significant outperformance, though smaller than for $\eta=100$. 
    
%     The 6 datasets with $r=0.05$ (LO-2, $\dotsc$, LO-7) are relatively similar to the main dataset (with $RP \geq 0.96$), while the other 6 (LO-8, $\dotsc$, LO-13) are quite different (with $RP < 0.73$).
%     Therefore, we claim that our algorithm should mainly transfer knowledge from those 6 datasets with $r=0.05$ while avoiding to learn something wrong from the others.
%     In line with this we provide results of the joint optimizer on the 7 datasets with $r=0.05$, which performs better than the other baselines and outperforms LO-1 by $6.2\%$. In particular, this confirms that the datasets with $r=0.05$ are those to transfer knowledge from, since the joint optimizer for all datasets performs worse than LO-1. The joint subset optimizer is significantly outperformed by our regret-optimal algorithm RO ($\eta=100$) by about $3\%$, which shows that our method constitutes a better way for transfer learning than simply selecting the datasets most similar to $\mathcal{D}_1$.
    
%     We additionally compare our method to the local optimizer for the main dataset which uses either $700$ (the number of training samples in the 7 similar datasets with $r=0.05$) or $50,000$ training samples. Importantly, both are just references that would not be available in a real world setting where the datasets are limited.
%     The first one only leads to a slight increase in $RP$ of about $1\%$, which shows that our method extracts nearly as much knowledge out of the (same amount of) samples of the similar datasets with $r=0.05$. 
%     The second one (which is considered a good proxy for the true American option price on the main dataset) has about $10\%$ better performance. This also shows the limitations of our method, in particular, it can only transfer as much knowledge as available in the other datasets.}
% \end{experiment}

% \begin{table}[hbt]
%     \centering
%     \caption{Relative performance (RP) and $95\%$-confidence-intervals for different optimization methods in Experiment~\ref{exp:1}. We compare the local optimizers on the different datasets (LO-$n$), with the mean local optimizer (MLO), the joint optimizer (JO) and our regret-optimal method (RO). The ``oracle'' local optimizer on the main dataset with additional training samples (standard: $100$ samples per dataset) is included.  
%     \hfill\\
%     When the information sharing parameter $\eta$ is set to $100$, the regret-optimal (RO) algorithm outperforms all ``non-oracle'' baselines. }
%     % \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{@{}ccc@{}}
%     \cmidrule[0.3ex](){1-3}
%     method &  $RP$ &  $95\%$-CI \\
%     \midrule
%     \csvreader[head to column names, late after line=\\]
%     {Tables/training_overview-1-1.csv}{}%
%     {  \name & \RP & \CI }%
%     \midrule
%     \csvreader[head to column names, late after line=\\]
%     {Tables/training_overview-1-2.csv}{}%
%     {  \name & \RP & \CI }%
%     \bottomrule
%     \end{tabular}
%     % }% END Resize box
%     \label{table:results exp 1}
%     \end{table}
    


% In the second experiment we test the ability of our method to transfer knowledge from a small dataset which is similar to the small main dataset, even if it is confronted with a very different and much larger (dominating in terms of samples) dataset.

% \begin{experiment}\label{exp:2}{\rm 
%     In this experiment we generate 3 different datasets. The main dataset is generated from a rough Heston model
%     \begin{align*}
%     dX_t &=  (r - \delta) X_t dt +  \sqrt{v_t} X_t dW_t, \\
%     v_t &= v_0 + \int_0^t \frac{(t-s)^{H-1/2} }{\Gamma(H + 1/2)} \kappa (v_\infty - v_s)ds + \int_0^t \frac{(t-s)^{H-1/2} }{\Gamma(H + 1/2)} \sigma \sqrt{v_s}dB_s,
%     \end{align*}
%     which is similar to the Heston model except that the volatility is  a rough process with Hurst parameter $H\in(0,1/2]$, where the case $H=1/2$ coincides with the standard Heston model. 
%     We use $H=0.1$ and otherwise the same parameters as for the main dataset in Experiment~\ref{exp:1}. The second and third dataset generated from standard Heston model (i.e.\  $H=1/2$), with the same parameters, except for the drift $r=0.5$ for the second dataset.
%     In particular, dataset 3 is the closest non-rough dataset to the main dataset, while dataset 2 is quite different.
%     For datasets 1 and 3 we use $\nu_1=100$ training samples, while we use $\nu_1=50,000$ for dataset 2, such that it dominates the others in its size.
%     All the other choices are the same as in Experiment~\ref{exp:1}.

%     The results are reported in Table~\ref{table:results exp 2}. The baselines MLO and  JO perform significantly worse than the LO on the main dataset. As expected, the JO suffers much more from the dominating dataset 2 than the MLO. Indeed, the MLO would suffer more from a large number of datasets that are quite different from the main dataset, no matter their sample size.
%     In contrast to this, our regret optimal method with $\eta \in\{50,100\}$ outperforms the LO-1 by $4\%$, showing that also a quite different dataset dominating in sample size is not a problem.}
% \end{experiment}

%     \begin{table*}[!htb]
%     \centering
%     \caption{Relative performance (RP) and $95\%$-confidence-intervals for different optimization methods in Experiment~\ref{exp:2}. We compare the local optimizers on the different datasets (LO-$n$), the mean local optimizer (MLO), the joint optimizer (JO) and our regret-optimal method (RO). With $\eta=100$ RO outperforms all baselines. }
%     \begin{tabular}{@{}ccc@{}}
%     \cmidrule[0.3ex](){1-3}
%     method &  $RP$ &  $95\%$-CI \\
%     \midrule
%     \csvreader[head to column names, late after line=\\]
%     {Tables/training_overview-2.csv}{}%
%     {  \name & \RP & \CI }%
%     \bottomrule
%     \end{tabular}
%     % }% END Resize box
%     \label{table:results exp 2}
%     \end{table*} 
    


% Both of these experiments show that our regret optimal method is well suited for automatic (up to the hyper-parameter $\eta$) dataset selection in transfer learning tasks that have potentially large numbers of datasets and do not allow a (manual) pre-selection. 
% In particular, neither a large number of ``bad'' datasets (of which the MLO suffers) nor some ``bad'' datasets that dominate in sample size (of which the JO suffers) constitute a problem for our regret-optimal method.
% Moreover, the sample efficiency when transferring knowledge from similar datasets to the main task is very high (outperforming the JO on the respective subset of similar datasets and nearly being on par with the LO on the main dataset using a larger training sample), as we saw in Experiment~\ref{exp:1}.





































% \section{Conclusion}
% In this work we presented a regret-optimal algorithm for federated transfer learning based on finite-rank kernel ridge-regressors (fKRR). 
% Besides the theoretical properties of this algorithm, we also provided experiments demonstrating the transfer learning capabilities of our method in the context of American option pricing.

% One possible future research direction is to apply our transfer learning method to real world datasets, where the similarity between the datasets is a priori not easy to quantify.
% From the theoretical side we would like to extend our method to regression models that do not necessarily permit a closed-form solution.



% % \acks{}
% % \section*{Acknowledgments}
% % AK acknowledges financial support from an NSERC Discovery Grant No.\ RGPIN-2023-04482 and their McMaster Startup Funds. 
% % MG acknowledges support from an NSERC Discovery Grant No.\ RGPIN-2013-276671.



% \bibliography{Formatting/References}
% \bibliographystyle{icml2021}


% \appendix


% \section{Proofs and Technical Results}
% \label{s:Proofs_TechnicalLemmata}



% \begin{remark}
% \label{rem:Notation_InnerProduct}
% We keep our notation light and use $u^{\top}v$ to implement the Euclidean inner-product between any two vectors $u,v\in \mathbb{R}^k$ for any $k\in \mathbb{N}_+$. 
% We use $| \cdot |$ to denote the Euclidean norm of a vector or Fr\"{o}benius norm of a matrix, whichever is applicable. 
% For two square matrices $A$ and $B$, $A\leq B$ ($A<B$, resp.) means that $B-A$ is positive semi-definite (positive definite, resp.); see \citep[page 146 - Equation (7)]{LaxBookLinearAlgebra_2007} for details.
% \end{remark} 

% Lemmas~\ref{lm:|AB|<=|A||B|} and \ref{lm:|A1+An|2<=(|A1|2+|An|2)n} give some elementary properties of matrix algebra, which will be used repeatedly in the subsequent proofs. 
% \begin{lemma} 
% \label{lm:|AB|<=|A||B|}
% The Euclidean norm $|\cdot|$ of matrices has the following properties: 

% \noindent\emph{i)}. For any matrices $A\in \mathbb{R}^{n_1 \times n_2}$ and $B\in\mathbb{R}^{n_2\times n_3}$, we have that
% $|AB| \leq |A|\cdot |B|$;   

% \noindent\emph{ii)}. For any matrices $A$, $B\in \mathbb{R}^{n_1 \times n_2}$, we have $|A+B| \leq |A|+|B|$.  
% \end{lemma} 
% \begin{proof}  
% Denote $A=(A_{ij})_{1\leq i\leq n_1 , 1\leq j \leq n_2}$ and $B=(B_{jk})_{1\leq j \leq n_2, 1\leq k \leq n_3}$. 
% %Further denote the $k$-th column vector of $B$ by $b_{\cdot k}$. 
% By the Cauchy-Schwarz inequality, we have for each column vector $B_{\cdot k}$ of $B$ that 
% \begin{align} 
%  |A B_{\cdot k}|^2 = \sum_{i=1}^{n_1} \big( \sum_{j=1}^{n_2} A_{ij} B_{jk} \big)^2 
%   \leq \sum_{i=1}^{n_1} \big( \sum_{j=1}^{n_2} A_{ij}^2 \sum_{j=1}^{n_2} B_{jk}^2 \big) 
%   = \big( \sum_{i=1}^{n_1} \sum_{j=1}^{n_2} A_{ij}^2 \big) \sum_{j=1}^{n_2} B_{jk}^2 
%   = |A|^2 \sum_{j=1}^{n_2} B_{jk}^2 . 
%   \notag 
% \end{align} 
% It then follows that 
% \begin{align} 
%  |AB|^2 = & |(A B_{\cdot 1}, A B_{\cdot 2}, ..., A B_{\cdot n_3} ) |^2 
%  = |A B_{\cdot 1}|^2 + |A B_{\cdot 2}|^2 + \cdots + |A B_{\cdot n_3}|^2 \notag \\ 
%  \leq & |A|^2 \sum_{j=1}^{n_2} \sum_{k=1}^{n_3} B_{jk}^2 = |A|^2 |B|^2 , \notag 
% \end{align} 
% and assertion i) is proved. 

% For $A$, $B\in \mathbb{R}^{n_1\times n_1}$, we have 
% \begin{align} 
% |A+B|^2 = & \sum_{i=1}^{n_1} \sum_{j=1}^{n_2} (A_{ij} + B_{ij})^2  
%  =   \sum_{i=1}^{n_1} \sum_{j=1}^{n_2} A_{ij}^2 + \sum_{i=1}^{n_1} \sum_{j=1}^{n_2} B_{ij}^2 
%  + 2 \sum_{i=1}^{n_1} \sum_{j=1}^{n_2} A_{ij} B_{ij} \notag \\ 
%  \leq & |A|^2 + |B|^2 + 2 |A|^2 |B|^2 
%   = (|A|+|B|)^2 , \notag 
% \end{align} 
% which proves assertion ii). 
% \end{proof} 








% \begin{lemma} 
% \label{lm:|A1+An|2<=(|A1|2+|An|2)n} 
% Let $w_1$, $w_2$, ..., $w_n$ be positive numbers such that $\sum_{k=1}^n w_k = 1$. 
% For any $n$ matrices $A_1$, ..., $A_n\in \mathbb{R}^{n_1 \times n_2}$, it satisfies that 
% $\big| \sum_{k=1}^n w_k A_k \big|^2 \leq \sum_{k=1}^n w_k |A_k|^2$; 
% particularly, when $w_1=w_2=\cdots = w_n=1/n$, we have 
% $\big|\sum_{k=1}^n  A_k \big|^2 \leq n \sum_{k=1}^n |A_k|^2$ . 
% \end{lemma} 
% \begin{proof} 
% Denote $A_k = ( A_{k, ij})_{1\leq i\leq n_1,  1\leq j \leq n_2}$, $k=1$, ..., $n$. 
% By the Jensen's inequality, we have 
% \begin{align} 
%  ( w_1 A_{1, ij} + \cdots + w_n A_{n, ij})^2 \leq  w_1 A_{1, ij}^2 + \cdots + w_n A_{n, ij}^2  . \notag 
% \end{align}  
% It then follows that 
% \begin{align} 
%  |w_1 A_1 + \cdots + w_n A_n|^2 = & \sum_{i=1}^{n_1} \sum_{j=1}^{n_2} (w_1 A_{1, ij} + \cdots + w_n A_{n, ij})^2 
%  \leq  \sum_{i=1}^{n_1} \sum_{j=1}^{n_2} w_1 A_{1, ij}^2 + \cdots + w_n A_{n, ij}^2   \notag \\ 
%   = &   w_1 \sum_{i=1}^{n_1} \sum_{j=1}^{n_2} A_{1, ij}^2 + \cdots + w_n \sum_{i=1}^{n_1} \sum_{j=1}^{n_2} A_{n, ij}^2  \notag \\ 
%   = &   w_1 |A_1|^2 + \cdots + w_n |A_n|^2  .   
%   \notag 
% \end{align} 


% \end{proof} 

% We begin with the relatively short proof of Theorem \ref{prop:Optimal_Bayes_Weighting} establishing the optimality of the weights obtained in Algorithm \ref{alg:RegretOptimizationHeuristic__WarmStart}. 

% \begin{proof}[{Proof of Theorem~\ref{prop:Optimal_Bayes_Weighting}}]
% For $i=1,\dots,N$, consider the probability measure 
% \[
% \bar{\mathbb{P}}^{\eta}
% \eqdef 
% \sum_{i=1}^N\,
% \frac{
% [s^1+\eta -s^i]_+
% }{
% \sum_{k=1}^N\, [s^1 + \eta - s^k]_+
% }
% \,
% \delta_{\theta^\star_i}
% \] 
% on the discrete space $\{\theta^\star_i\}_{i=1}^N$ topologized by the discrete metric.
% % Since arg-minima are invariant under multiplication by positive constants, then i
% Any minimizer of~\eqref{eq:optimizingQ__regularized} is a minimizer of the following problem, and vice-versa
% \begin{align}
% \nonumber
% &
%     \min_{
%         \mathbb{P}_w \in \mathcal{P}(\{\theta^\star_i\}_{i=1}^N)
%     }\,
%             \frac1{|\mathcal{D}_1|}\sum_{j=1}^{|\mathcal{D}_1|}\,
%             \big\|
%                     f_{\theta}(u_j^1)
%                 -
%                     y_j^1
%             \big\|_2^2
%     +
%         \eta\,
%         % \frac{(1-\eta)}{\eta}
%         \operatorname{D}_{\operatorname{KL}}\big(
%             \mathbb{P}_w
%         \|
%             \bar{\mathbb{P}}^{\eta}
%         \big)
%     % +\iota(\mathbb{P}_w \ll \bar{P}^{\eta})
% \\
% \nonumber
% & =
%     \min_{
%         \mathbb{P}_w \in \mathcal{P}(\{\theta^\star_i\}_{i=1}^N)
%     }\,
%         \mathbb{E}_{\theta \sim \mathbb{P}_w}\,
%         \Biggl[
%             \frac1{|\mathcal{D}_1|}\sum_{j=1}^{|\mathcal{D}_1|}\,
%             \big\|
%                     f_{\theta}(u_j^1)
%                 -
%                     y_j^1
%             \big\|_2^2
%         \Biggr]
%     +
%         % \frac{(1-\eta)}{\eta}
%         \eta\,
%         \operatorname{D}_{\operatorname{KL}}\big(
%             \mathbb{P}_w
%         \|
%             \bar{\mathbb{P}}^{\eta}
%         \big)
%     +
%     \iota(\mathbb{P}_w \ll \bar{P}^{\eta})
% \\
% \label{eq:optimizingQ__regularized__Renormalized}
% & =
%     \min_{
%         \mathbb{P}_w \in \mathcal{P}(\{\theta^\star_i\}_{i=1}^N)
%     }\,
%         \mathbb{E}_{\theta \sim \mathbb{P}_w}\,
%         \biggl[
%         \sum_{i=1}^N\,
%         I_{\theta = \theta^\star_i}
%             s_i
%         \biggl]
%     +
%         % \frac{(1-\eta)}{\eta}
%         \eta\,
%         \operatorname{D}_{\operatorname{KL}}\big(
%             \mathbb{P}_w
%         \|
%             \bar{\mathbb{P}}^{\eta}
%         \big)
%     +
%     \iota(\mathbb{P}_w \ll \bar{P}^{\eta})
% ,
% \end{align}
% where the map $\iota(\mathbb{P}_w \ll \bar{P}^{\eta})$ is an ``indicator function in the sense of convex analysis''; that is, $\iota(\mathbb{P}_w \ll \bar{P}^{\eta})=0$ if $\mathbb{P}_w$ is absolutely continuous with respect to $\bar{P}^{\eta}$ and $\infty$ otherwise.  
% We may now apply \citep[Proposition 1]{WangHyndmanKratsios_EMT_2020}\footnote{This result is an extension of \citep[Proposition 2.3]{DaiPraMenghiniRunggaldier_ConnectionStochControlDynGames__1996__MathControlSigSys} which allows us to vary the influence of the regulative-entropy term in~\eqref{eq:optimizingQ__regularized__Renormalized}.} to~\eqref{eq:optimizingQ__regularized__Renormalized} deducing that it admits a minimizer $\mathbb{P}_{w^{\star}}=\sum_{i=1}^N\,w_i^{\star}\,\delta_{\theta^\star_i}$ and its Radon-Nikodym derivative with respect to the measure $\bar{\mathbb{P}}^{\eta}$ is 
% \allowdisplaybreaks
% \begin{align}
% \label{eq:optimizingQ__regularized__Renormalized____density_____BEGIN}
%     \frac{
%         d\mathbb{P}_{w^{\star}}
%     }{
%         \bar{\mathbb{P}}^{\eta}
%     }
%     (\theta^\star_i)
% = &
%         \frac{
%                 e^{
%                 \sum_{l=1}^N \, I_{\theta^\star_l=\theta^\star_i}
%                 s_i/\eta
%             }        
%         }{
%             \mathbb{E}_{\bar{\mathbb{P}^{\eta}}}\biggl[
%              \exp\big(
%                 \sum_{i=1}^N\,
%                 I_{\theta = \theta^\star_i}
%                     s_i
%                 \big)    
%             \biggr]
%         }
% \\
% \nonumber
% = &
%         \frac{
%                 e^{
%                 s_i/\eta
%             }        
%         }{
%             \sum_{k=1}^N\,
%                 \frac{e^{s_k/\eta}[s^1+\eta-s^k]_+}{
%                     \sum_{m=1}^N\,
%                     [s^1+\eta-s^m]_+
%                 }
%         }
% \\
% \label{eq:optimizingQ__regularized__Renormalized____density_____END}
% = &
%         \Big(
%             \sum_{m=1}^N\,
%                 [s^1+\eta-s^m]_+
%         \Big)
%         \,
%         \frac{
%                 e^{
%                 s_i/\eta
%             }        
%         }{
%             \sum_{k=1}^N\,
%                 e^{s_k/\eta}[s^1+\eta-s^k]_+
%         }
% \end{align}
% for $i=1,\dots,N$.  Since $\mathbb{P}_{w^{\star}}$ is a minimizer of~\eqref{eq:optimizingQ__regularized__Renormalized} then we may deduce the expression for the optimal weights $w^{\star}$ by first noting that
% \allowdisplaybreaks
% \begin{align}
% \label{eq:optimizingQ__regularized___weights____P1}
%             \mathbb{P}_{w^{\star}} 
%         \eqdef 
%             \sum_{i=1}^N\, w^{\star}_i\delta_{\theta^\star_i}\,
%         = 
%             \sum_{i=1}^N\, 
%             \frac{d\mathbb{P}_{w^{\star}}}{d\bar{\mathbb{P}^{\eta}}}(\theta^\star_i)
%             \,
%             \left(
%                 \frac{
%                     [s^1+\eta-s^i]_+
%                 }{
%                     \sum_{j=1}^N\,
%                         [s^1+\eta-s^j]_+
%                 }
%             \right)
%             \,
%             \delta_{\theta^\star_i}\,
% .
% \end{align}
% Therefore,~\eqref{eq:optimizingQ__regularized__Renormalized____density_____BEGIN}-~\eqref{eq:optimizingQ__regularized__Renormalized____density_____END} and~\eqref{eq:optimizingQ__regularized___weights____P1} imply that, for each $i=1,\dots,N$, we have 
% \allowdisplaybreaks
% \begin{align}
%     \nonumber
% % \label{eq:optimizingQ__regularized___weights}
%         w^{\star}_i 
%     = & 
%             \frac{d\mathbb{P}_{w^{\star}}}{d\bar{\mathbb{P}^{\eta}}}(\theta^\star_i)
%             \,
%             \left(
%                 \frac{
%                     [s^1+\eta-s^i]_+
%                 }{
%                     \sum_{j=1}^N\,
%                         [s^1+\eta-s^j]_+
%                 }
%             \right)
%             \,
%     \\
%     \nonumber
%     = & 
%         \Big(
%             \sum_{m=1}^N\,
%                 [s^1+\eta-s^m]_+
%         \Big)
%         \,
%         \frac{
%                 e^{
%                 s_i/\eta
%             }        
%         }{
%             \sum_{k=1}^N\,
%                 e^{s_k/\eta}[s^1+\eta-s^k]_+
%         }
%         \,
%         \left(
%             \frac{
%                 [s^1+\eta-s^i]_+
%             }{
%                 \sum_{j=1}^N\,
%                     [s^1+\eta-s^j]_+
%             }
%         \right)
%     \\
%     \nonumber
%     = & 
%         \frac{
%                 e^{
%                 s_i/\eta
%             }   
%             \,
%             [s^1+\eta-s^i]_+
%         }{
%             \sum_{k=1}^N\,
%                 e^{s_k/\eta}[s^1+\eta-s^k]_+
%         }
% .
% \end{align}
% \end{proof}

% Next we now prove our main result, namely Theorem~\ref{thm:RegretOptimal_Dynamics__MainTextFormulation}. The result is first rewritten, in the optimal control-theoretic notation introduced in Section~\ref{s:Main_ss:Algorithm}.

% \begin{theorem}[The Regret-Optimal Algorithm - Control Theoretic Form]
% \label{thm:RegretOptimal_Dynamics}
% Suppose that Assumptions~\ref{assm:bddxy} and~\ref{assm:PD} hold.  Then, the optimal control problem 
% \eqref{eq:penalized_regret_functional} and \eqref{Theta-simple} admits a unique solution for $t=0, 1, ..., T-1$ such that 
% \allowdisplaybreaks\begin{align} 
%  \boldsymbol\alpha(t)  
%  = & -[(\lambda + \beta )I_{Np} + P(t+1)]^{-1} 
%  \big[ (\lambda I_{Np} + P(t+1)) \Theta(t) 
%  - \lambda  \Theta^\star + S(t+1)  \big] ,   \label{optimala} 
% \end{align} 
% and the resulting cost is 
% \begin{align} 
% L^\star(\boldsymbol\alpha; \mathcal{D}) 
% = \Theta^{\star \top} P(0) 
% \Theta^\star + 2 S^\top(0) \Theta^\star + r(0) .
% \label{optimalL} 
% \end{align} 
% The $P(t)$, $S(t)$, and $r(t)$ in \eqref{optimala} and \eqref{optimalL} are determined by the backward equation system on $t=1,\dots,T$:  
% \allowdisplaybreaks\begin{align} 
% & \begin{cases}
%    P(t)  =  \beta I_{Np} - \beta^2 [(\lambda+\beta) I_{Np} + P(t+1) ]^{-1} , \label{eqnP(t)} \\ 
%    P(T) =  [w^\star_1 I_p ,\cdots, w^\star_N I_p]^{\top} 
%  \big( \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|}   u^i_j u^{i\top}_j \big)  
%  [ w^\star_1 I_p, \cdots, w^\star_N I_p] ,  
% \end{cases}   \\
% %%%  
% & \begin{cases}
%   S(t) =  \beta \big[ (\lambda+\beta)I_{Np} + P(t+1) \big]^{-1} (S(t+1) - \lambda \Theta^\star )
%   \label{eqnS(t)} ,     \\ 
%    S(T) =  - [ w^\star_1 I_p, \cdots, w^\star_N I_p]^{\top} \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|}  {u^i_j} y^i_j ,    
% \end{cases} \\
% %\begin{align}
% %\begin{align} 
% &\begin{cases} 
%  r(t) =  - ( S(t+1) - \lambda \Theta^\star )^\top
%  [(\lambda+\beta)I_{Np} + P(t+1)]^{-1} \cdot ( S(t+1) - \lambda \Theta^\star )   \\  
%  \hspace{1.1cm}   + \lambda \| \Theta^\star \|_2^2 + r(t+1), 
%  \label{eqnr(t)} \\ r(T) = \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|} |y^i_j|^2 . 
%  \end{cases}  
% \end{align} 
% \end{theorem} 


% \begin{proof}[Proof of Theorem~\ref{thm:RegretOptimal_Dynamics} (and therefore of Theorem~\ref{thm:RegretOptimal_Dynamics__MainTextFormulation})]
% Let $V(t, \Theta)$ be the value function associated with the optimal control problem
% \eqref{eq:penalized_regret_functional} and \eqref{Theta-simple}. 
% By the dynamic programming principle, $V(t, \Theta)$  satisfies the equation 
% \allowdisplaybreaks\begin{align} 
% & V (t, \Theta) = \min_{\boldsymbol\alpha} 
%  \Big[   \lambda \left| \Theta + \boldsymbol\alpha - \Theta^\star \right|^2 
%  + \beta \left| \boldsymbol\alpha \right|^2  
%  + V (t+1, \Theta + \boldsymbol\alpha ) \Big] , \quad t=0, 1, ..., T-1 ,   \label{dpVw} \\  
%  & V(T, \Theta ) 
% = l (\theta^{w^\star}; \mathcal{D} ) .   \label{V(T,Theta)} 
% \end{align}


% The loss function can be written as a linear quadratic function of 
% $\Theta=[\theta_1^\top, \cdots, \theta_N^\top]^\top$ such that 
% \allowdisplaybreaks\begin{align} 
%  &  l (\theta^{w^\star}; \mathcal{D} ) \notag \\ 
%  = & 
%  \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|}  \Big[ u^{i\top}_j \sum_{k=1}^N w^\star_k \theta_k - y^i_j  \Big]^2 \notag \\ 
%  = &  \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|} 
%  \Big[ \sum_{k=1}^N w_k^{\star 2} \theta_k^\top u^i_j u^{i\top}_j \theta_k 
%  -2 \sum_{k=1}^N w_k^\star y^i_j u^{i \top}_j \theta_k + |y^i_j|^2 \Big]
%  \notag \\ 
% = &  \Big(\sum_{k=1}^N w^\star_k \theta_k^\top \Big) \Big( \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|}  u^i_j u^{i\top}_j  \Big) \Big(\sum_{k=1}^N w^\star_k  \theta_k\Big) 
%  - 2 \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|} y^i_j u^{i\top}_j \sum_{k=1}^N w^\star_k \theta_k  + \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|} | y^i_j |^2 \notag \\ 
% = & \Theta^\top [w^\star_1 I_p ,\cdots, w^\star_N I_p]^\top 
%  \Big( \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|}  u^i_j u^{i\top}_j \Big)  
%  [ w^\star_1 I_p, \cdots, w^\star_N I_p ] \Theta \notag \\ 
%  & - 2 \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|} y^i_j u^{i \top}_j   
%   [ w^\star_1 I_p, \cdots, w^\star_N I_p ] \Theta 
%  + \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|} | y^i_j |^2 . \label{lwT}  
% \end{align}



% We claim that $V(t, \Theta)$ takes the linear quadratic form 
% \allowdisplaybreaks\begin{align} 
%  V (t, \Theta) 
% =  \Theta^\top P(t) \Theta + 2 S^\top (t) \Theta + r(t) . \label{ansatzVw}
% \end{align} 
% To see this, note from \eqref{V(T,Theta)} and \eqref{lwT} that 
% $V(T, \Theta)$ takes the linear quadratic form of \eqref{ansatzVw}. By solving the dynamic programming equation \eqref{dpVw} at $t=T-1$ for the optimal $\boldsymbol\alpha$ and substituting it back into the equation, we obtain $V(T-1, \Theta)$ also taking the linear quadratic form of \eqref{ansatzVw}. By backward induction we have that $V(t,\Theta)$ takes the form of \eqref{ansatzVw} for all $t=0,...,T$.  


% \begin{remark} Here $r(t)$ is a constant term independent of the ``state variable'' $\Theta$, which we note exists because the cost $L^\star$ defined by \eqref{eq:penalized_regret_functional} contains terms independent of $\Theta(t)$.
% \end{remark}

% Combining \eqref{V(T,Theta)}, 
% \eqref{lwT}, and \eqref{ansatzVw}  verifies that $P(T)$ and $S(T)$ satisfy the terminal condition as given by \eqref{eqnP(t)} and \eqref{eqnS(t)}. 
% We substitute \eqref{ansatzVw} into \eqref{dpVw} and reorganize the terms to get 
% \begin{align} 
%  & \Theta^\top P(t) \Theta + 2 S^\top(t) \Theta + r(t)  \notag \\ 
%    = &  \min_{\boldsymbol\alpha} \Big\{  \boldsymbol\alpha^\top [(\lambda + \beta ) I_{Np} + P(t+1)] \boldsymbol\alpha  
%   + 2 [ \Theta^\top P(t+1)  
%  + S^\top (t+1) +\lambda (\Theta^\top - \Theta^{\star \top})]  \boldsymbol\alpha \notag \\ 
%  & \hspace{1cm} + \Theta^\top ( \lambda I_{Np} + P(t+1) )  \Theta 
%   + 2 ( S^\top(t+1) - \lambda \Theta^\star ) \Theta + \lambda |\Theta^\star|^2 + r(t+1) \Big\} . 
%   \label{DPVansatz}
% \end{align} 
% By the first order condition\footnote{NB, we can argue this way, since the problem is convexified upon fixing $w^{\star}$.  In fact, this is the control-theoretic motivation for using Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart} to decouple the optimization of $w$ and of $\theta_{\cdot}$ from one another, and not treating them as a single (non-convex if left coupled) control problem.} for the right-hand side of \eqref{DPVansatz} with respect to $\boldsymbol\alpha$, we have  
% \allowdisplaybreaks\begin{align} 
%  0 = &   [(\lambda+\beta) I_{Np} + P(t+1)] \boldsymbol\alpha  
%   +  [ ( \lambda I_{Np} + P(t+1) ) \Theta  
%  + S(t+1) - \lambda  \Theta^\star ]  . 
%  \label{1stOrdera}
% \end{align}
% % \Aurelien{I think there is a factor $2$ missing in front of second term.}
% % \Xuwei{
% % Taking the derivative of the right hand side of \eqref{DPVansatz} with respect to $\mathbf{a}$ and equating it to zero, we have 
% % \allowdisplaybreaks\begin{align} 
% %  0 = &   2 [(\lambda+1) I_{Np} + P(t+1)] \mathbf{a}  
% %   +  2 [ ( \lambda I_{Np} + P(t+1) ) \Theta  
% %  + S(t+1) - \lambda  \Theta^\star ]  . 
% %  \notag 
% % \end{align} 
% % Cancelling the common factor 2, we obtain \eqref{1stOrdera}. 
% % }
% By Assumption \ref{assm:PD}, we have 
% $P(T)+(\lambda+1)I_{Np} >0$, and therefore from \eqref{1stOrdera} we obtain the optimal $\boldsymbol{\alpha}$ taking the form of \eqref{optimala}. 





% % \Aurelien{I can not follow the derivation below. Would it be possible to add some intermediary steps?}\Anastasis{I agree some extra comments (just some words) would be good.}
% % \Xuwei{The proof is updated. The equations in the proof are reorganized and simplified.}
% % \Aurelien{Ok, I get it now, maybe we can add a few steps.
% % \begin{align} 
% %  & \Theta^\top  P(t) \Theta  + 2 S^\top(t) \Theta  + r(t) \notag \\ 
% %  = & - \big[ \Theta^\top (\lambda I_{Np} + P(t+1)) 
% %  + S^\top(t+1) - \lambda \Theta^{\star \top}  
% %  \big] \cdot \big[(\lambda + 1)I_{Np} + P(t+1)\big]^{-1} \cdot \notag \\ 
% %  & \big[  (\lambda I_{Np} + P(t+1)) \Theta  + S(t+1) 
% %   -  \lambda  \Theta^\star  \big]  
% %   + \Theta^\top (\lambda I_{Np} + P(t+1)) 
% %   \Theta \notag \\ 
% %  &  + 2 [ S^\top(t+1) - \lambda \Theta^{\star \top}]\Theta + \lambda |\Theta^\star|^2 + r(t+1) ,
% % \end{align} 
% % Let's isolate the term $\Theta^\top  P(t) \Theta$ to find $P(t)$:
% % \begin{align*} 
% % - \Theta^\top \underbrace{(\lambda I_{Np} + P(t+1)) \cdot \big[(\lambda + 1)I_{Np} + P(t+1)\big]^{-1} \cdot (\lambda I_{Np} + P(t+1))}_A \Theta
% % + \Theta^\top \underbrace{(\lambda I_{Np} + P(t+1))}_B \Theta
% % \end{align*} 
% % Focusing on the term $A$, we have
% % \begin{align*} 
% % & - ( (\lambda + 1 ) I_{Np} + P(t+1) - I_{Np}) \cdot \big[(\lambda + 1)I_{Np} + P(t+1)\big]^{-1} \cdot (\lambda I_{Np} + P(t+1)) \\
% % &= - (\lambda I_{Np} + P(t+1))
% % + \big[(\lambda + 1)I_{Np} + P(t+1)\big]^{-1} \cdot (\lambda I_{Np} + P(t+1))
% % \end{align*} 
% % %
% % Therefore,
% % \begin{align*}
% % A + B &= \big[(\lambda + 1)I_{Np} + P(t+1)\big]^{-1} \cdot (\lambda I_{Np} + P(t+1)) \\
% % &= \big[(\lambda + 1)I_{Np} + P(t+1)\big]^{-1} \cdot ((\lambda + 1) I_{Np} - I_{Np} + P(t+1)) \\
% % &= I_{Np} - \big[(\lambda + 1)I_{Np} + P(t+1)\big]^{-1}.
% % \end{align*}
% % } 
% % \Xuwei{Equations \eqref{eqn:P-unsimplified}, \eqref{eqn:P-simplified}, 
% % \eqref{eqn:S-unsimplified}, \eqref{eqn:S-simplified}, which integrate the Aurelien's steps above, are added to supplement more details of deriving equations \eqref{eqnP(t)} and \eqref{eqnS(t)} for $P$ and $S$. } 

% We further substitute $\boldsymbol{\alpha}$ of the form \eqref{optimala} into the right side of \eqref{DPVansatz} to obtain 
% \allowdisplaybreaks\begin{align} 
%  & \Theta^\top  P(t) \Theta  + 2 S^\top(t) \Theta  + r(t) \notag \\ 
%  = & - \big[ \Theta^\top (\lambda I_{Np} + P(t+1)) 
%  + S^\top(t+1) - \lambda \Theta^{\star \top}  
%  \big] \cdot \big[(\lambda + \beta )I_{Np} + P(t+1)\big]^{-1} \cdot \notag \\ 
%  & \big[  (\lambda I_{Np} + P(t+1)) \Theta  + S(t+1) 
%   -  \lambda  \Theta^\star  \big]  
%   + \Theta^\top (\lambda I_{Np} + P(t+1)) 
%   \Theta \notag \\ 
%  &  + 2 [ S^\top(t+1) - \lambda \Theta^{\star \top}]\Theta + \lambda |\Theta^\star|^2 + r(t+1) . 
%   \label{eqn:Vansatz}
% \end{align} 
% Reorganizing the terms on right side of \eqref{eqn:Vansatz}, we have 
% \begin{align} 
%  & \Theta^\top  P(t) \Theta  + 2 S^\top(t) \Theta  + r(t) \notag \\ 
%  = & - \Theta^\top   (\lambda I_{Np} + P(t+1) ) [(\lambda + \beta )I_{Np} + P(t+1)]^{-1} 
%  (\lambda I_{Np} + P(t+1))   \Theta \notag \\ 
%  & + \Theta^\top ( \lambda I_{Np} + P(t+1) ) \Theta + 2 [ S^\top(t+1) - \lambda \Theta^{\star \top}]\Theta  \notag \\  
%  & - 2 [S^\top(t+1) - \lambda \Theta^{\star \top}] 
%  [(\lambda +\beta )I_{Np} + P(t+1) ]^{-1} (\lambda I_{Np} + P(t+1)) \Theta \notag \\  
%  & - (S^\top(t+1) - \lambda \Theta^{\star\top}) [(\lambda + \beta )I_{Np} + P(t+1)]^{-1} (S(t+1) - \lambda \Theta^\star)  
%  \notag \\
%  & + \lambda |\Theta^\star|^2 + r(t+1) . 
%   \label{eqn:Vansatz-simplified} 
% \end{align} 
% %Since $\Theta$ is arbitrary, 
% Matching the coefficients of the quadratic terms of $\Theta$ on both sides of \eqref{eqn:Vansatz-simplified}, we obtain 
% \begin{align} 
%  P(t)  
%   = &  -  (\lambda I_{Np} + P(t+1) ) [(\lambda + \beta )I_{Np} + P(t+1)]^{-1} 
%  (\lambda I_{Np} + P(t+1))   \notag \\ 
%  & +   \lambda I_{Np} + P(t+1) .  
%  \label{eqn:P-unsimplified}
% \end{align} 
% The right side of 
% \eqref{eqn:P-unsimplified} further simplifies to  
% \begin{align} 
% & -  (\lambda I_{Np} + P(t+1) ) [(\lambda + \beta )I_{Np} + P(t+1)]^{-1} 
%  (\lambda I_{Np} + P(t+1))   
%   +  \lambda I_{Np} + P(t+1)   \notag \\ 
%  = &   -  [ ( \lambda + \beta ) I_{Np} + P(t+1) - \beta I_{Np} ]  [(\lambda + \beta )I_{Np} + P(t+1)]^{-1} 
%  (\lambda I_{Np} + P(t+1)) \notag \\
%  & +  \lambda I_{Np} + P(t+1)  \notag \\ 
%  = & -   ( \lambda  I_{Np} + P(t+1) )  + \beta [(\lambda + \beta )I_{Np} + P(t+1)]^{-1} 
%  (\lambda I_{Np} + P(t+1))  
%   +  \lambda I_{Np} + P(t+1) \notag \\ 
%   = & 
%   \beta [(\lambda + \beta )I_{Np} + P(t+1)]^{-1} 
%  (\lambda I_{Np} + P(t+1))  \notag \\ 
%  = & 
%   \beta [(\lambda + \beta )I_{Np} + P(t+1)]^{-1} 
%  [ ( \lambda + \beta ) I_{Np} + P(t+1) - \beta I_{Np} ] \notag  \\ 
%  = & \beta I_{Np} - \beta^2 [(\lambda + 1)I_{Np} + P(t+1)]^{-1} . 
%  \label{eqn:P-simplified}
% \end{align} 
% Combining \eqref{eqn:P-unsimplified}
% and \eqref{eqn:P-simplified} gives \eqref{eqnP(t)} for $t=T-1$. 

% Matching the coefficients of the linear terms of $\Theta$ on both sides of \eqref{eqn:Vansatz-simplified} and taking the transpose, we obtain  
% \begin{align} 
%  S(t) = & - (\lambda I_{Np} + P(t+1) ) [(\lambda + \beta )I_{Np} + P(t+1) ]^{-1} ( S(t+1) - \lambda \Theta^\star ) \notag \\ 
% & +  S(t+1) - \lambda \Theta^\star .  
%  \label{eqn:S-unsimplified} 
% \end{align} 
% The right side of \eqref{eqn:S-unsimplified} further simplifies to 
% \begin{align} 
% & - (\lambda I_{Np} + P(t+1) ) [(\lambda +  \beta )I_{Np} + P(t+1) ]^{-1} ( S(t+1) - \lambda \Theta^\star ) 
%  + S(t+1) - \lambda \Theta^\star 
%   \notag \\ 
% = &   - [ (\lambda + \beta ) I_{Np} + P(t+1) - \beta I_{Np} ] [(\lambda + \beta )I_{Np} + P(t+1) ]^{-1} ( S(t+1) - \lambda \Theta^\star ) \notag \\ 
% & + S(t+1) - \lambda \Theta^\star 
% \notag \\ 
%  = & - ( S(t+1) - \lambda \Theta^\star ) 
%   + \beta [(\lambda +\beta )I_{Np} + P(t+1) ]^{-1} ( S(t+1) - \lambda \Theta^\star ) 
%   + S(t+1) - \lambda \Theta^\star 
%   \notag \\ 
%  = &  \beta [(\lambda + \beta )I_{Np} + P(t+1) ]^{-1} ( S(t+1) - \lambda \Theta^\star ) . \label{eqn:S-simplified}
% \end{align}
% Combining \eqref{eqn:S-unsimplified} and \eqref{eqn:S-simplified} gives \eqref{eqnS(t)} for $t=T-1$. 

% Matching the terms independent of $\Theta$ on both sides of \eqref{eqn:Vansatz-simplified} gives 
% \begin{align} 
%  r(t) = &  - ( S(t+1) - \lambda \Theta^\star )^\top
%  [(\lambda+ \beta )I_{Np} + P(t+1)]^{-1} \cdot ( S(t+1) - \lambda \Theta^\star ) \notag    \\  
%  &  + \lambda |\Theta^\star|^2 + r(t+1) , \notag 
% \end{align} 
% which is \eqref{eqnr(t)} for $t=T-1$. 


% Since 
% $P(T) + (\lambda + \beta )I_{Np} > \beta I_{Np}$, 
% we have 
% \begin{align} 
% P(T-1) = \beta I_{Np} 
%  - \beta^2 [(\lambda + \beta )I_{Np} + P(T)]^{-1} > 0 . \notag 
% \end{align} 
% By backward induction on $t$, we can show that 
% $\boldsymbol{\alpha}$ takes the form of \eqref{optimala} for all $t=0, 1, ..., T-1$, and $P$ and $S$ satisfy the system \eqref{eqnP(t)} and \eqref{eqnS(t)}.  
% \end{proof} 

% \begin{corollary} 
% \label{cor:M(P)invbdd}
% Under Assumptions~\ref{assm:bddxy} and \ref{assm:PD}, the solution $P$ and $S$ of the system \eqref{eqnP(t)}-\eqref{eqnS(t)} satisfies that for all $t=1$, $2$, ..., $T$, 
% \begin{align} 
% & | [(\lambda + \beta) I_{Np} + P(t)]^{-1} |\leq  (\lambda + \beta)^{-1},  \label{M(P)invbd}  \\ 
%  & |S(t)| \leq C \cdot N 
%  \label{|S|bd} , 
% \end{align} 
% where $C> 0$ is a constant depending on $\lambda$, $\beta$, $(w_1^\star, ..., w_N^\star)$, $\Theta^\star$, $K_x$, $K_y$ and $T$. 
% \end{corollary} 


% \begin{proof}[Proof of Corollary~\ref{cor:M(P)invbdd}] 
% Let $\| \cdot \|$ be the spectral norm of a matrix such that $\|A\|\eqdef \sup_{x\neq 0} |Ax|/|x| $. 
% Since $P(t)$ is positive semi-definite, we have $(\lambda + \beta) I_{Np} + P(t) \geq (\lambda + \beta) I_{Np}$ and  
% \begin{align} 
% 0\leq [(\lambda + \beta) I_{Np} + P(t) ]^{-1} \leq (\lambda + \beta)^{-1} I_{Np}   ,  \notag 
% \end{align} 
% which, by the Courant-Fisher Theorem (see \cite{hornjohnson2012}), implies that $\|  [(\lambda + \beta) I_{Np} + P(t) ]^{-1} \| \leq \| (\lambda+\beta)^{-1} I_{Np} \| = (\lambda + \beta)^{-1}$. 
% Since all norms of finite dimensional normed spaces are equivalent, and in particular, $|\cdot|\le \|\cdot\|$ on the space of $N_p\times N_p$-matrices, then we find that
% \begin{align} 
%   \big| [(\lambda + \beta) I_{Np} + P(t) ]^{-1} \big| \leq \|  [(\lambda + \beta) I_{Np} + P(t) ]^{-1} \| , \notag 
% \end{align}  
% and thus $\big| [(\lambda + \beta) I_{Np} + P(t) ]^{-1} \big| \leq (\lambda + \beta)^{-1}$,  
% which proves \eqref{M(P)invbd}. 

% %\noindent 
% Next, we prove \eqref{|S|bd}. 
% By Lemmas~\ref{lm:|AB|<=|A||B|} and \ref{lm:|A1+An|2<=(|A1|2+|An|2)n}, and \eqref{eq:moredatasets_than_dataperdataset}, we obtain 
% \allowdisplaybreaks
% \begin{align} 
%  | S(T) |^2  
%  = & \Big( \sum_{i=1}^N w^{\star 2}_i \Big) 
%  \Big| \sum_{i=1}^N w^\star_i   \sum_{j=1}^{|\mathcal{D}_i|}  u^i_j y^i_j  \Big|^2  
%  \leq  \Big( \sum_{i=1}^N w^{\star 2}_i \Big) 
%  \sum_{i=1}^N w_i^\star  \Big| \sum_{j=1}^{|\mathcal{D}_i|}   u^i_j y^i_j \Big|^2  \notag  \\ 
%  \leq &  \Big( \sum_{i=1}^N w^{\star 2}_i \Big) 
%  \sum_{i=1}^N w_i^\star |\mathcal{D}_i|  \sum_{j=1}^{|\mathcal{D}_i|}   | u^i_j y^i_j |^2  
%  \leq  \Big( \sum_{i=1}^N w^{\star 2}_i \Big) \sum_{i=1}^N w_i^\star |\mathcal{D}_i|^2  K_x^2 K_y^2  \notag \\ 
%   \leq &  \Big( \sum_{i=1}^N w^{\star 2}_i \Big) \sum_{i=1}^N w_i^\star N^2  K_x^2 K_y^2 ,  
%   \label{eq:TBBounded} 
% \end{align} 
% and therefore the estimate \eqref{|S|bd} holds for $t=T$. 
% %By the relationship between the $\ell^1$ and $\ell^2$ norms on $\mathbb{R}^N$, 
% %we have that $\Big(\sum_{i=1}^N\,w_i^{\star \, 2}\Big)^{1/2}\le \sum_{i=1}^N\,|w_i^{\star}|$.  Since $(w^{\star}_i)_{i=1}^N$ belongs to the $N$-simplex then, by definition, $w_1^{\star},\dots,w_N^{\star}\ge 0$ and $\sum_{i=1}^n\,w_i^{\star}=1$.  Thus, 
% %\[
% %        \Big(\sum_{i=1}^N\,w_i^{\star \, 2}\Big)^{1/2}
% %    \le 
% %        \sum_{i=1}^N\,|w_i^{\star}|
% %    = 
% %        \sum_{i=1}^N\,w_i^{\star}
% %    =
% %        1
% %    .
% %\]
% %Consequentially, $\sum_{i=1}^N\,w_i^{\star \, 2}\le 1$; whence the right-hand side of the estimate~\eqref{eq:TBBounded} reduces %to
% %\allowdisplaybreaks
% %\begin{align} 
% % | S(T) |^2  
% % \le 
% % N^2  K_x^2 K_y^2  .
% %\end{align} 

% Assume by induction that \eqref{|S|bd} holds for $t=u$.  
% By \eqref{eqnS(t)}, Lemma~\ref{lm:|AB|<=|A||B|}, and the triangle inequality, we have 
% \begin{align} 
%  |S(u-1)| \leq &  \beta \big| \big[ (\lambda+\beta)I_{Np} + P(u) \big]^{-1} \big| \cdot \big| S(u) - \lambda \Theta^\star  \big| \notag \\ 
%   \leq & \beta \big| \big[ (\lambda+\beta)I_{Np} + P(u) \big]^{-1} \big| \cdot ( |S(u)| + \lambda | \Theta^\star | ) . 
%   \notag 
% \end{align} 
% The estimate \eqref{|S|bd} for $t=u-1$ then follows from \eqref{M(P)invbd} and the induction hypothesis. 
% Thus, by induction we have shown that \eqref{M(P)invbd} holds for all $t=1$, $2$, ..., $T$. 
% \end{proof} 


% We proceed to prove Theorem~\ref{thm:ComplexityAlgorithm} about the complexity of the regret-optimal algorithm. 
% To facilitate the proof, we introduce the following Lemma~\ref{lm:matCompComplexity} that summarizes complexities of matrix operations. 
% \begin{lemma} 
% \label{lm:matCompComplexity} 
% %Since we will be assuming that we work with \textit{floating-point arithmetic}, 
% Suppose all elementary arithmetic operations (e.g.\ addition, subtraction, multiplication) of two real numbers are of constant (i.e.\ $\mathcal{O}(1)$) complexity. Then elementary matrix computations have the following complexities: 

% \begin{enumerate}  
% \item[(i)] Adding two $n_1 \times n_2$ matrices has a complexity of $O(n_1 n_2)$. 

% \item[(ii)] Multiplying an $n_1 \times n_2$ matrices by a scalar has a complexity of $O(n_1 n_2)$. 

% \item[(iii)] Multiplying an $n_1 \times n_2$ matrix with an $n_2 \times n_3$ matrix has a complexity of $O(n_1 n_2 n_3)$. 
% In particular, multiplying two $n\times n$ matrices has a complexity of $\mathcal{O}(n^{2.373})$.  
% \end{enumerate} 
% \end{lemma} 

% \begin{proof} 
% Adding two $n_1\times n_2$ matrices involves adding each entry of one matrix with the corresponding entry of the other matrix, and each entry addition has a complexity of $\mathcal{O}(1)$. Hence the total complexity is $\mathcal{O}(n_1 n_2)$. 

% Multiplying an $n_1 \times n_2$ matrix by a scalar involves multiplying each entry by the scalar, and the scalar multiplication of each entry has a complexity of $\mathcal{O}(1)$. Hence the total complexity is $O(n_1 n_2)$. 

% Multiplication of an $n_1 \times n_2$ matrix and an $n_2 \times n_3$ matrix requires multiplying the $n_1$ row vectors of the first matrix by the $n_3$ column vectors of the second matrix, which needs a total of $n_1 n_3$ multiplications. Multiplication of two $n_2$-dimensional vectors has a complexity of $O(n_2)$. Therefore the total complexity is $O(n_1n_2n_3)$.  
% When multiplying two matrices of $n\times n$-dimension with an optimized CW-like algorithm the complexity is $\mathcal{O}(n^{2.373})$. 
% \end{proof} 


% %\Anastasis{Check complexity again with modificaitons.}
% \begin{proof}[{Proof of Theorem~\ref{thm:ComplexityAlgorithm}}] 
% \hfill\\
% \noindent\textbf{Complexity of Computing $P(T)$ is $\mathcal{O}\big(N^2p^3\big)$}\hfill\\
% Since $u^i_j \in \mathbb{R}^{p\times 1}$, computing each 
% $u^i_j u^{i\top}_j$ has $\mathcal{O}(p^2)$ complexity, by Lemma \ref{lm:matCompComplexity}-(iii). 
% Multiplying the $p\times p$ matrix $u^i_j u^{i\top}_j$ by the scalar $w^\star_i$ has a complexity of $\mathcal{O}(p^2)$, by Lemma~\ref{lm:matCompComplexity}-(iii).   
% %Adding two $n_1 \times n_2$ matrices has a complexity of $\mathcal{O}(n_1 n_2)$. 
% %Multiplying an $n_1\times n_2$ matrix by a scalar has a complexity of $\mathcal{O}(n_1 n_2)$.    
% Then computing the $p\times p$ matrix $\sum_{i=1}^N w^\star_i \sum_{j=1}^{S_i}\, u^i_j u^{i\top}_j$ by adding the $\bar{N}$ matrices of dimension $p\times p$ has complexity $\mathcal{O}(\bar{N}\,p^2)$, by Lemma \ref{lm:matCompComplexity}-(i).  
% Since $[w_1^\star I_p ,\cdots, w_N^\star I_p]^{\top}$ is $Np\times p$-dimensional, then computing the $np\times p$-dimensional product $[w_1^\star I_p ,\cdots, w_N^\star I_p]^{\top}\sum_{i=1}^N w^\star_i \sum_{j=1}^{S_i}\, u^i_j u^{i \top}_j$ has $\mathcal{O}(Np^3)$ complexity, by Lemma~\ref{lm:matCompComplexity}-(iii). 
% %Likewise, since the product $[w_1^\star I_p ,\cdots, w_N^\star I_p]^{\top}\sum_{i=1}^N\, w^\star_i \sum_{j=1}^{S_i}\,u^i_j 
% %u^{i\top}_j$ is $Np\times p$-dimensional 
% Likewise, the product 
% \[ 
%     \Big([w_1^\star I_p ,\cdots, w_N^\star I_p]^{\top}\sum_{i=1}^N  w^\star_i \sum_{j=1}^{S_i}\, u^i_j u^{i\top}_j \Big)[w_1^\star I_p ,\cdots, w_N^\star I_p]
% \]
% has a complexity of $\mathcal{O}(N^2p^3)$.  Therefore, computing $P(T)$ itself is of $\mathcal{O}\big(\bar{N}p^2+N^2p^3\big)$ complexity.  
% Assumption~\eqref{eq:moredatasets_than_dataperdataset} implies that $\bar{N}\leq N^2$; hence, the complexity of computing $P(T)$ is $\mathcal{O}\big(N^2p^3\big)$. 


% % \hfill\\
% \noindent
% \textbf{Complexity of Computing $S(T)$ is $\mathcal{O}\big(Np\max\{N,p\}\big)$}
% \hfill\\ 
% Since $u^i_j\in\mathbb{R}^{p\times 1}$ and $y^i_j\in \mathbb{R}$, 
% computing the product $u^i_j y_j^i$ has complexity $\mathcal{O}(p)$, by Lemma \ref{lm:matCompComplexity}-(iii). 
% And multiplying the $p\times 1$ dimensional vector $u^i_j y^i_j$ by the scalar $w^\star_i$ has complexity $\mathcal{O}(p)$, by Lemma \ref{lm:matCompComplexity}-(ii). Then the complexity of computing $\sum_{i=1}^N w^\star_i \sum_{j=1}^{S_i}\,u^i_j y_j^i$ by adding $\bar{N}$ vectors of dimension $p$ is $\mathcal{O}\big(\bar{N}p\big)$, by Lemma~\ref{lm:matCompComplexity}-(i). 
% Since $- [ w_1^\star I_p, \cdots, w_N^\star I_p]^{\top}$ is an $Np\times p$-dimensional matrix and $\sum_{i=1}^N w^\star_i \sum_{j=1}^{S_i}\, u^i_j y_j^i$ is a $p\times 1$-dimensional vector, then computing their $Np\times 1$ dimensional product has $\mathcal{O}(Np^2)$ complexity, according to Lemma~\ref{lm:matCompComplexity}-(iii).  
% Therefore, the computing $S(T)$ has a complexity of $\mathcal{O}(\bar{N}p + N P^2)$. 
% Since~\eqref{eq:moredatasets_than_dataperdataset} implies that $\bar{N}\le N^2$ then, computing $S(T)$ had a computational cost of $\mathcal{O}\big(Np\max\{N,p\}\big)$.


% % \hfill\\
% \noindent
% \textbf{Complexity of Computing $P(t)$ and $S(t)$ for $t=T-1,\dots, 1$ is $\mathcal{O}\big(T(Np)^{2.373}\big)$}
% \hfill\\
% The complexity of computing $(\lambda +\beta )I_{Np} + P(t+1)$ for each $t$ is $\mathcal{O}(Np)$, since we only need to add scalars on the matrix's \textit{diagonal}.  By \cite{LeGall_Complexity_CWLikeMatrixInversion_2014}, computing the matrix inverse $[(\lambda+\beta)I_{Np}+P(t+1)]^{-1}$ with a CW-like algorithm has a complexity of $\mathcal{O}\big((Np)^{2.373}\big)$.  
% Since the addition $\beta I_{Np} - \beta^2 [(\lambda+ \beta )I_{Np} + P(t+1) ]^{-1}$ only requires us to multiply all entries of $ [(\lambda+\beta)I_{Np} + P(t+1) ]^{-1}$ by $-\beta^2$ and add along the diagonal, then it has a complexity of $\mathcal{O}\big((Np)^2 + Np\big)$, by Lemma~\ref{lm:matCompComplexity}-(i) and (ii). 
% Performing the matrix addition $S(t+1)-\lambda \Theta^\star$ has complexity $\mathcal{O}(Np)$ by Lemma~\ref{lm:matCompComplexity}-(i).  
% Computing the $Np\times 1$-dimensional product 
% $[(\lambda+1)I_{Np} + P(t+1)]^{-1} (S(t+1) - \lambda \Theta^\star)$ 
% by multiplying an $Np\times Np$ matrix by an $Np\times 1$ matrix has complexity $\mathcal{O}(N^2 p^2)$, according to Lemma~\ref{lm:matCompComplexity}-(iii). 
% Therefore, computing each $P(t)$ and $S(t)$ for $t=T-1,\dots,1$, has complexity  $\mathcal{O}\big((Np)^{2.373}\big)$.  Since there are $T-1$ such matrices to compute, then the total cost of computing every $P(T-1),\dots,P(1)$ and $S(T-1)$, ..., $S(1)$ is $\mathcal{O}\big(T(Np)^{2.373}\big)$.



% % \hfill\\\noindent
% %\textbf{Complexity of Computing $S(t)$ for $t=1,\dots,T-1$ is $\mathcal{O}(T\,N^2p^2)$} \hfill\\ 
% %We fix $t\in\{1,\dots,T-1\}$ and assume $S(t+1)$ and $P(t+1)$ have already been computed.
% %The complexity of computing $(\lambda +\beta) I_{Np} + P(t+1)$ is $\mathcal{O}(Np)$ since we only need to add $(\lambda + \beta)$ to each diagonal element of $P(t+1)$.  The complexity of computing $[(\lambda+\beta)I_{Np} + P(t+1)]^{-1}$ is $\mathcal{O}\big(Np)^{2.373}\big)$ by \cite{LeGall_Complexity_CWLikeMatrixInversion_2014}. 
% %The complexity of performing the matrix addition $S(t+1)-\lambda \Theta^\star$ is $\mathcal{O}(Np)$. 
% %The complexity of performing the matrix multiplication $[(\lambda+1)I_{Np} + P(t+1)]^{-1} (S(t+1) - \lambda \Theta^\star)$ is $\mathcal{O}(N^2 p^2)$. 
% %Therefore, the complexity of computing $S(t)$ for $t=1,\dots,T-1$ is $\mathcal{O}(T\,N^2 p^2)$

% %The complexity of performing all the matrix multiplications $(M(P(t+1)))^{-1} \lambda I$, $ (M(P(t+1)))^{-1} \lambda I (M(P(t+1)))^{-1} P(t+1)$, and $(M(P(t+1)))^{-1} P(t) (M(P(t+1)))^{-1} \lambda I$ is $\mathcal{O}\big(N^3p^3\big)$; and the cost of adding their entries is of lower complexity namely $\mathcal{O}(N^2p^2)$.  Therefore, the cost of computing $M(P(t+1))^{-1}S(t+1)$ is $\mathcal{O}(N^2p^3)$. Since $\Theta^{\star}$ is a $Np\times p$-dimensional matrix then cost computing $H(P(t+1))\Theta^{\star}$ is $\mathcal{O}(N^2p^3)$.  Since all matrix additions involved in computing $S(t)$ are comparatively negligible, then the cost of computing $S(t)$ is $\mathcal{O}(N^3p^3)$ (nb, the most costly operation has been computing the matrix product $M(P(t+1))^{-1}M(P(t+1))^{-1}$).  Thus, the complexity of computing each $S(t)$ for $t=0,\dots,T-1$ is $\mathcal{O}(T\,N^3p^3)$.



% \noindent
% \textbf{The Cost of Computing Each $\Theta(t)$ is $\mathcal{O}(T\,N^2p^2)$}
% \hfill\\
% %Suppose that $P(t+1)$, $S(t+1)$, and $\Theta(t)$ have been computed.  
% To compute $\Theta(t)$ for all $t=1$, $\dots$, $T$, starting from $\Theta(0)=\Theta^\star$, 
% we need to compute $\mathbf{a}(t)$ given by \eqref{optimala} for $t=0$, $1$, $\dots$, $T-1$.  
% Hence we need to quantify the complexity of computing $\mathbf{a}(t)$. 
% %The complexity of computing $(\lambda + \beta)I_{Np} + P(t+1)$ is $\mathcal{O}(Np)$ since we only need to add $(\lambda+\beta)$ to each of $P(t+1)$'s diagonal elements. 
% %By~\cite{LeGall_Complexity_CWLikeMatrixInversion_2014}, the complexity of computing $-[(\lambda + \beta)I_{Np} + P(t+1)]^{-1}$ with a CW-like algorithm is $\mathcal{O}\big((Np)^{2.373}\big)$. 
% By \eqref{eqnP(t)}, we can obtain $-[(\lambda + \beta)I_{Np} + P(t+1)]^{-1}$ by computing 
% $\beta^{-2}(P(t)- \beta I_{Np})$, which involves adding a scalar to the diagonal of an $Np\times Np$ matrix, and then multiplying the matrix by a scalar. 
% The cost of computing the product
% $(\lambda I_{Np} + P(t+1)) \Theta(t)$ is $\mathcal{O}(N^2 p^2)$ and the cost of computing all sums in $(\lambda I_{Np} + P(t+1)) \Theta(t) 
%  - \lambda \Theta^\star + S(t+1)  $ are of lower order complexity.  Finally, the cost of computing the matrix-product between $-[(\lambda + \beta)I_{Np} + P(t+1)]^{-1} $ and $
%  \big[ (\lambda I_{Np} + P(t+1)) \Theta(t) 
%  - \lambda \Theta^\star + S(t+1)  \big]$ is $\mathcal{O}(N^2p^2)$, by Lemma~\ref{lm:matCompComplexity}-(iii). Therefore, the cost of computing each $\mathbf{a}(t)$ is $\mathcal{O}(N^2p^2)$, and therefore the cost of computing $\Theta(t)$ for all $t=1$, ..., $t=T$ from $\Theta(0)=\Theta^\star$ is $\mathcal{O}(T N^2 p^2)$.  
%  %have been computed is $\mathcal{O}(T\,N^2p^2)$.  

% \noindent
% \textbf{Tallying up Complexities: The Complexity of Computing $(\Theta(t))_{t=0}^T$ is 
% $\mathcal{O}( N^2 p^3 + T\, (N p)^{2.373})$.}
% \hfill\\
% Looking over all computations involved, we deduce that the cost of computing the sequence $(\Theta(t))_{t=1}^T$ is (in order) dominated by the computational complexity of computing the sequence $(P(t))_{t=1}^{T-1}$ and $P(T)$; whence it is 
% $\mathcal{O}( N^2 p^3 + T\, (N p)^{2.373})$. 
% %$\mathcal{O}(T\, N^{2.373}\, p^2)$.
% \end{proof}  




% The following Lemma~\ref{lem:stability_wrtData}, 
% Proposition~\ref{prop:stabilityControl}, and Corollary~\ref{cor:stabilityLast} are devoted to proving Theorem~\ref{thrm:adv_robust}, the adversarial robustness of Algorithm~\ref{alg:RegretOptimization}. 



% We introduce the linear map $M(\cdot): \mathbb{R}^{Np\times Np} \to \mathbb{R}^{Np\times Np}$ such that $M(Q) = (\lambda + \beta) I_{Np} + Q$ for any $Q\in \mathbb{R}^{Np\times Np}$. 
% \begin{lemma} 
% \label{lem:stability_wrtData}
% Given any two data sets $\mathcal{D}=\cup_{i=1}^N \mathcal{D}_i=\cup_{i=1}^N \cup_{j=1}^{|\mathcal{D}_i|} 
%  \{(x^i_j, y^i_j) \}$ and 
% $\widetilde{\mathcal{D}}=\cup_{i=1}^N \widetilde{\mathcal{D}}_i = \cup_{i=1}^N \cup_{j=1}^{|\mathcal{D}_i|}  \{(\tilde{x}^i_j, \tilde{y}^i_j) \}$ satisfying Assumption \ref{assm:bddxy}, let $(P, S)$ and $(\widetilde{P}, \widetilde{S})$ be the solutions of \eqref{eqnP(t)}-\eqref{eqnS(t)} corresponding to $\mathcal{D}$ and $\widetilde{\mathcal{D}}$, respectively. Then, for all $t=1, ..., T$, we have 
% \allowdisplaybreaks\begin{align}  
%     \big| P(t) - \widetilde{P}(t) \big| 
%  \le &
%      C \cdot \Big[ \sum_{i=1}^N w^\star_i |\mathcal{D}_i| \sum_{j=1}^{|\mathcal{D}_i|} | u^i_j - \tilde{u}^i_j |^2 \Big]^{1/2} , 
%  \label{eqn:estP-tildeP} 	 \\ 
%  %%%
%      \big| [ M(P(t)) ]^{-1} - [ M(\widetilde{P}(t)) ]^{-1} \big| 
%  \le&  
%      C \cdot \Big[ \sum_{i=1}^N w^\star_i |\mathcal{D}_i| \sum_{j=1}^{|\mathcal{D}_i|} | u^i_j - \tilde{u}^i_j |^2 \Big]^{1/2} ,  
%     \label{eqn:estM-tildeM} \\ 
% %%%
%         |S(t) - \widetilde{S}(t)| 
%     \le &
%       C \cdot \Big[ \sum_{i=1}^N w^\star_i |\mathcal{D}_i|  \sum_{j=1}^{|\mathcal{D}_i|} | u^i_j - \tilde{u}^i_j |^2 
%      + |y^i_j - \tilde{y}^i_j |^2 \Big]^{1/2} , 
% \label{eqn:estS-tildeS} 
% \end{align}
% where $C> 0$ is a constant depending on $\lambda$, $\beta$, $N$, $\bar{N}$, $(w_1^\star, ..., w_N^\star)$, $\Theta^\star$, $K_x$, $K_y$ and $T$. 
% \end{lemma}


% \begin{proof}%[{Proof of Lemma~\ref{lem:stability_wrtData}}]
% We let $C$ be a constant depending on $\lambda$, $\beta$, $N$, $\bar{N}$, $\Theta^\star$, $(w_1^\star, ..., w_N^\star)$, $K_x$, $K_y$, and $T$,  
% and allow $C$ to vary from place to place throughout the proof. 
% We employ backward induction starting from $t=T$ to prove \eqref{eqn:estM-tildeM}, \eqref{eqn:estP-tildeP}, and 
% \eqref{eqn:estS-tildeS}. 

% From \eqref{eqnP(t)}, the terminal condition $| P(T) - \widetilde{P}(T) |^2$ can be written as 
% \allowdisplaybreaks\begin{align} 
%  \big| P(T) - \widetilde{P}(T) \big|^2  
%  = &   \Big| [w_1^\star I_p ,\cdots, w_N^\star I_p ]^\top
%  \Big[ \sum_{i=1}^N w_i^\star  \sum_{j=1}^{|\mathcal{D}_i|}  ( u^i_j u^{i\top}_j  - \tilde{u}^i_j \tilde{u}^{i\top}_j  ) \Big]  
%  [ w_1^\star I_p, \cdots, 
%  w_N^\star I_p ]  \Big|^2 \notag \\ 
%  = & \sum_{k, l=1}^N 
%   w_k^{\star 2} 
%   w_l^{\star 2} 
%  \Big| \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|}  ( u^i_j u^{i\top}_j  - \tilde{u}^i_j \tilde{u}^{i\top}_j  ) \Big|^2 . \notag 
%  \end{align} 
% By Lemmas~\ref{lm:|AB|<=|A||B|} and \ref{lm:|A1+An|2<=(|A1|2+|An|2)n}, we have 
%  \begin{align} 
%  \big| P(T) - \widetilde{P}(T)  \big|^2  
%  \leq &   \sum_{k, l=1}^N w_k^{\star 2} w_l^{\star 2} 
%   \sum_{i=1}^N w_i^\star   
% \Big| \sum_{j=1}^{|\mathcal{D}_i|} 
%     (  u^i_j u^{i\top}_j  - \tilde{u}^i_j \tilde{u}^{i\top}_j  ) \Big|^2 
% \notag \\ 
%  \leq &   \sum_{k, l=1}^N w_k^{\star 2} w_l^{\star 2} 
%   \sum_{i=1}^N w_i^\star |\mathcal{D}_i|  \sum_{j=1}^{|\mathcal{D}_i|} 
%     \big| u^i_j u^{i\top}_j  - 
% \tilde{u}^i_j \tilde{u}^{i\top}_j  \big|^2 
% \notag \\ 
% %%% 
%  = &   \sum_{k, l=1}^N w_k^{\star 2} w_l^{\star 2} 
%   \sum_{i=1}^N 
%   w_i^\star |\mathcal{D}_i| \sum_{j=1}^{|\mathcal{D}_i|}  
% \big| ( u^i_j - \tilde{u}^i_j  )u^{i\top}_j  
%  + \tilde{u}^i_j (u^{i\top}_j - \tilde{u}^{i\top}_j)   \big|^2  \notag \\ 
% %%%
% \leq &   \sum_{k, l=1}^N w_k^{\star 2} w_l^{\star 2} 
%     \sum_{i=1}^N w_i^\star |\mathcal{D}_i| \sum_{j=1}^{|\mathcal{D}_i|}  
%  2 \big( \big|  u^i_j - \tilde{u}^i_j   \big|^2 \cdot \big| u^i_j \big|^2 
%  + \big| \tilde{u}^i_j \big|^2 \cdot \big| u^i_j - \tilde{u}^i_j  \big|^2 \big) 
%  \notag \\ 
%  \leq &   \sum_{k, l=1}^N w_k^{\star 2} w_l^{\star 2} 
%   \sum_{i=1}^N w_i^\star |\mathcal{D}_i|  \sum_{j=1}^{|\mathcal{D}_i|} 4 K_x^2 
% \big| u^i_j - \tilde{u}^i_j   \big|^2 
% . \label{estP(T)-tildeP(T)}   
% \end{align}
% %Combining \eqref{estP(T)-tildeP(T)} and \eqref{max|P-tildeP|<=|P(T)-tildeP(T)|}, we obtain the estimate \eqref{eqn:estM-tildeM}. 
% Therefore \eqref{eqn:estP-tildeP} holds for $t=T$. 



% Assume by induction that 
% \eqref{eqn:estP-tildeP} holds for $t=u$. We show that \eqref{eqn:estP-tildeP} also holds for $t=u-1$. 
% From \eqref{eqnP(t)}, we have  
% \allowdisplaybreaks\begin{align} 
%  P(u-1) - \widetilde{P}(u-1)  
% = & [ M( \widetilde{P}(u) ) ]^{-1} 
%  - [ M(P(u)) ]^{-1}\notag  \\ 
%  = & [ M( P(u) ) ]^{-1} ( P(u) - \widetilde{P}(u) )  
% [ M( \widetilde{P}(u) ) ]^{-1} ,  \notag 
% %\label{tildeP-Precursion}
% \end{align} 
% and by Lemma~\ref{lm:|AB|<=|A||B|} we further have 
% \allowdisplaybreaks  
% \begin{align} 
%  \big| P(u-1) - \widetilde{P}(u-1)  \big|  
%  \leq & \big| [ M( P(u) ) ]^{-1} 
%  \big| \cdot \big| P(u) - \widetilde{P}(u) \big| \cdot 
% \big| [ M( \widetilde{P}(u) ) ]^{-1} \big| . \label{|tildeP-P|recursion} 
% \end{align} 
% By Corollary~\ref{cor:M(P)invbdd} and the induction hypothesis for $t=u$,  
% \eqref{|tildeP-P|recursion} implies that \eqref{eqn:estP-tildeP} holds for $t=u-1$. 
% We have shown by induction that \eqref{eqn:estP-tildeP} holds for all $t=1$, ..., $T$. 


% Since 
% \begin{align} 
%   [M(P(t))]^{-1} - [M(\widetilde{P}(t))]^{-1} 
%   =  [ M( P(t) ) ]^{-1} (  \widetilde{P}(t) - P(t) )  
% [ M( \widetilde{P}(t) ) ]^{-1} ,   
% \notag 
% \end{align} 
% by Lemma~\ref{lm:|AB|<=|A||B|} we have   
% \begin{align} 
%  \big| [M(P(t))]^{-1} - [M(\widetilde{P}(t))]^{-1} \big| 
%   \leq  \big| [ M( P(t) ) ]^{-1} \big| \cdot  
%   \big|  \widetilde{P}(t) - P(t) \big| \cdot  
% \big| [ M( \widetilde{P}(t) ) ]^{-1} \big|  . 
% \label{eqn:M-tildeM<=P-tildeP}
% \end{align} 
% The estimate \eqref{eqn:estM-tildeM} then follows from \eqref{eqn:M-tildeM<=P-tildeP}, \eqref{eqn:estP-tildeP}, and Corollary~\ref{cor:M(P)invbdd}. 
% %the fact that $|[M(P(t))]^{-1}| \leq C$ and $[M(\widetilde{P}(t))]^{-1}\leq C$, 
 





% %For data sets $D$ and $\widetilde{D}$ satisfying Assumptions \ref{assm:bddxy} and \ref{assm:PD}, $P$ and $\widetilde{P}$ determined from \eqref{eqnP(t)} are positive-definite. Then $\big| [ M (P(t) ) ) ]^{-1} \big|$ is bounded by a constant depending on $K_x$, $(w^\star_1, \cdots, w^\star_N)$ and $T$. Similarly, $\big| [  M(\widetilde{P}(t) ) ]^{-1} \big|$ is bounded by a constant depending on $K_x$, $K_y$, $(w^\star_1, \cdots, w^\star_N)$ and $T$. 
 




% Now we establish the estimate \eqref{eqn:estS-tildeS}. 
% By \eqref{eqnS(t)}, the terminal condition $S(T)-\widetilde{S}(T)$ satisfies 
% \allowdisplaybreaks 
% \begin{align} 
%  | S(T) - \widetilde{S}(T) |^2 
%  = & 
%  \Big| [w_1^\star, \cdots, w_N^\star]^\top \sum_{i=1}^N w_i^\star \sum_{j=1}^{|\mathcal{D}_i|} 
%   ( u^i_j y^i_j - \tilde{u}^i_j \tilde{y}^i_j ) \Big|^2 \notag \\ 
%   =& \Big( \sum_{i=1}^N w^{\star 2}_i \Big) 
%  \Big| \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|} ( u^i_j y^i_j - \tilde{u}^i_j \tilde{y}^i_j ) \Big|^2 .  \notag
% \end{align} 
% By Lemmas~\ref{lm:|AB|<=|A||B|} and \ref{lm:|A1+An|2<=(|A1|2+|An|2)n}, we obtain 
% \allowdisplaybreaks
% \begin{align} 
%  | S(T) - \widetilde{S}(T) |^2  
%  \leq & \Big( \sum_{i=1}^N w^{\star 2}_i \Big) 
%  \sum_{i=1}^N w^\star_i  \Big| \sum_{j=1}^{|\mathcal{D}_i|} ( u^i_j y^i_j - \tilde{u}^i_j \tilde{y}^i_j ) \Big|^2  \notag  \\ 
%   \leq & \Big( \sum_{i=1}^N w^{\star 2}_i \Big) 
%  \sum_{i=1}^N w^\star_i |\mathcal{D}_i| \sum_{j=1}^{|\mathcal{D}_i|}  \big|  u^i_j y^i_j - \tilde{u}^i_j \tilde{y}^i_j \big|^2  \notag   \\ 
%  = & \Big( \sum_{i=1}^N w^{\star 2}_i \Big) 
%  \sum_{i=1}^N w^\star_i |\mathcal{D}_i| \sum_{j=1}^{|\mathcal{D}_i|}  \big|  (u^i_j - \tilde{u}^i_j) y^i_j + \tilde{u}^i_j (y^i_j - \tilde{y}^i_j) \big|^2  \notag \\ 
%   \leq & \Big( \sum_{i=1}^N w^{\star 2}_i \Big) 
%  \sum_{i=1}^N w^\star_i |\mathcal{D}_i| \cdot 2  \sum_{j=1}^{|\mathcal{D}_i|} \big[ \big|  (u^i_j - \tilde{u}^i_j) y^i_j \big|^2 
%  + \big|  \tilde{u}^i_j (y^i_j - \tilde{y}^i_j) \big|^2 \big]   \notag \\    
%  \leq & \Big( \sum_{i=1}^N w^{\star 2}_i \Big) 
%  \sum_{i=1}^N w^\star_i |\mathcal{D}_i| \cdot 2  \sum_{j=1}^{|\mathcal{D}_i|} \big[ |  u^i_j - \tilde{u}^i_j |^2 \cdot | y^i_j |^2 
%  + |  \tilde{u}^i_j |^2 \cdot | y^i_j - \tilde{y}^i_j  |^2 \big]   \notag\\ \leq & \Big( \sum_{i=1}^N w^{\star 2}_i \Big) 
%  \sum_{i=1}^N w^\star_i |\mathcal{D}_i| \cdot 2  \sum_{j=1}^{|\mathcal{D}_i|} \big[ K_y^2 \cdot |  u^i_j - \tilde{u}^i_j |^2  
%  + K_x^2 \cdot | y^i_j - \tilde{y}^i_j  |^2 \big]   \notag 
%  \\ 
%  \label{estST-tildeST} 
%  \leq & \Big( \sum_{i=1}^N w^{\star 2}_i \Big) 2 (K_x^2 + K_y^2)
%  \sum_{i=1}^N w^\star_i |\mathcal{D}_i|   \sum_{j=1}^{|\mathcal{D}_i|} \big[ |  u^i_j - \tilde{u}^i_j |^2  
%  +  | y^i_j - \tilde{y}^i_j  |^2 \big] , 
% \end{align} 
% and thus \eqref{eqn:estS-tildeS} holds for $t=T$. 
% Assume by induction that \eqref{eqn:estS-tildeS} holds for $t=u$, we show that \eqref{eqn:estS-tildeS} also holds for $t=u-1$. 
% From \eqref{eqnS(t)}, the difference $S(t)-\widetilde{S}(t)$ can be written as 
% \allowdisplaybreaks\begin{align} 
%  S(u-1) - \widetilde{S}(u-1) = & [ M(\widetilde{P}(u)) ]^{-1}[S(u) - \widetilde{S}(u) ]  \notag \\ 
%  & + \big[ ( M(P(u)) )^{-1} - 
%   ( M(\widetilde{P}(u)))^{-1} \big]  
%  ( S(u) - \lambda \Theta^\star ) , 
% \notag 
% \end{align} 
% and satisfies by Lemma~\ref{lm:|AB|<=|A||B|} and Corollary~\ref{cor:M(P)invbdd} that 
% \begin{align} 
% | S(u-1) - \widetilde{S}(u-1) | \leq &
%  \big| [ M(\widetilde{P}(u)) ]^{-1} \big| \cdot |S(u) - \widetilde{S}(u) |  \notag \\ 
%  & + \big| ( M(P(u)) )^{-1} - 
%   ( M(\widetilde{P}(u)))^{-1} \big| \cdot   
%  ( |S(u)| + \lambda | \Theta^\star | ) . 
%  \label{|tildeS-S|recursion} 
% \end{align} 
% By Corollary~\ref{cor:M(P)invbdd}, \eqref{eqn:estM-tildeM}, and the induction hypothesis, 
% \eqref{|tildeS-S|recursion} implies that 
% \eqref{eqn:estS-tildeS} holds for $t=u-1$.  
% We have shown by induction that \eqref{eqn:estS-tildeS} holds for all $t=1$, ..., $T$. 
% \end{proof} 

% \begin{proposition} 
% \label{prop:stabilityControl}
% For two arbitrary data sets $\mathcal{D}=\cup_{i=1}^N \mathcal{D}_i=\cup_{i=1}^N \cup_{j=1}^{|\mathcal{D}_i|} 
%  \{(x^i_j, y^i_j) \}$ and 
% $\widetilde{\mathcal{D}}=\cup_{i=1}^N \widetilde{\mathcal{D}}_i = \cup_{i=1}^N \cup_{j=1}^{|\mathcal{D}_i|}  \{(\tilde{x}^i_j, \tilde{y}^i_j) \}$ satisfying Assumption \ref{assm:bddxy}, 
% let $\boldsymbol\alpha =(\alpha_1^{\top}, \cdots, \alpha_N^{\top})^{\top}$ and 
% $\widetilde{\boldsymbol\alpha}=(\widetilde{\alpha}_1^{\top}, \cdots, \widetilde{\alpha}_N^{\top})^{\top}$ be the optimal controls for \eqref{eq:penalized_regret_functional} and \eqref{Theta-simple} corresponding to $\mathcal{D}$ and $\widetilde{\mathcal{D}}$, respectively. Then, we have
% \allowdisplaybreaks\begin{align} 
%  \sum_{t=0}^{T-1} |\boldsymbol\alpha(t) - \widetilde{\boldsymbol\alpha}(t) | 
%  \le C  \Big[ \sum_{i=1}^N w^{\star 2}_i |\mathcal{D}_i| \sum_{j=1}^{|\mathcal{D}_i|} | u^i_j - \tilde{u}^i_j |^2 
%  + |y^i_j - \tilde{y}^i_j|^2  \Big]^{1/2} , 
% \label{eqn:stabilityControl}
% \end{align} 
% where $C > 0$ is a constant depending on $\lambda$, $\beta$, $N$, $\bar{N}$, $\Theta^\star$, 
% $(w^\star_1, \cdots, w^\star_N)$, $K_x$, $K_y$, and $T$. 
% \end{proposition} 

% \begin{proof}[{Proof of Proposition~\ref{prop:stabilityControl}}]
% Let $C$ be a constant depending on $\lambda$, $\beta$, $N$, $\bar{N}$, $\Theta^\star$,  
% $(w^\star_1, \cdots, w^\star_N)$, $K_x$, $K_y$, and $T$,  
% and $C$ is allowed to vary from place to place throughout the proof. 
% By \eqref{optimala} and \eqref{Theta(t)Theta(0)}, the optimal control $\boldsymbol\alpha(t)$ along the optimal trajectory can be written as 
% \allowdisplaybreaks\begin{align} 
%   \boldsymbol\alpha(t) 
%  = & [ (M(P(t+1)))^{-1} - I_{Np} ]  \Big[ \Theta^\star 
%  + \sum_{u=0}^{t-1} \boldsymbol\alpha(u) \Big] \notag \\ 
%  & +  [ M(P(t+1)) ]^{-1} ( \lambda  \Theta^\star - S(t+1) ) ,   \notag 
% \end{align}
% and the difference $\boldsymbol{\alpha}(t)-\widetilde{\boldsymbol\alpha}(t)$ can be written as    
% \allowdisplaybreaks\begin{align}  
%   \boldsymbol\alpha(t) - \widetilde{\boldsymbol\alpha}(t) 
%  = &  \big[(M(P(t+1)))^{-1} - (M(\widetilde{P}(t+1)) )^{-1} \big] 
%  \Big[ \Theta^\star + \sum_{u=0}^{t-1}  \boldsymbol\alpha(u)   + \lambda \Theta^\star - S(t+1) \Big]  \notag \\ 
%  & + \big[ ( M(\widetilde{P}(t+1)) )^{-1} - I_{Np} \big] 
%  \sum_{u=0}^{t-1} (\boldsymbol\alpha(u) - \widetilde{\boldsymbol\alpha}(u)) \notag \\ 
% & + (M(\widetilde{P}(t+1)))^{-1} (S(t+1) - \widetilde{S}(t+1)) . 
% \label{a-tildea}
% \end{align} 


% For $t=0$, the difference $\boldsymbol\alpha(0)-\widetilde{\boldsymbol\alpha}(0)$ can be written as  
% \allowdisplaybreaks\begin{align} 
%   \boldsymbol\alpha(0) - \widetilde{\boldsymbol\alpha}(0)  
%  = & \big[ (M(P(1)))^{-1} - (M(\widetilde{P}(1)))^{-1}  \big] 
%  \big[ (\lambda + 1)   \Theta^\star - S(1) 
%  \big] \notag \\ 
%  & - [ M(\widetilde{P}(1)) ]^{-1} (S(1)-\widetilde{S}(1)) , \notag  
% \end{align} 
% and satisfies by Lemma~\ref{lm:|AB|<=|A||B|} that 
% \begin{align} 
% \big| \boldsymbol\alpha(0) - \widetilde{\boldsymbol\alpha}(0) \big|   
%  \leq &   \big| (M(P(1)))^{-1} - (M(\widetilde{P}(1)))^{-1}  \big| \cdot  
%  \big[ (\lambda + 1)   | \Theta^\star| +  | S(1) | 
%  \big] \notag \\ 
%  & +  \big| [ M(\widetilde{P}(1)) ]^{-1} \big| \cdot  \big| S(1)-\widetilde{S}(1) \big| .  \notag  
% \end{align} 
% It then follows from Corollary~\ref{cor:M(P)invbdd}, \eqref{eqn:estM-tildeM}, and \eqref{eqn:estS-tildeS} that 
% \allowdisplaybreaks\begin{align} 
%   \big| \boldsymbol\alpha(0) - \widetilde{\boldsymbol\alpha}(0) \big| \leq C 
%  \cdot \Big[ \sum_{i=1}^N w^\star_i |\mathcal{D}_i| \sum_{j=1}^{|\mathcal{D}_i|} | u^i_j 
%  - \tilde{u}^i_j |^2 
%  + |y^i_j - \tilde{y}^i_j|^2  \Big]^{1/2} . \notag   
% \end{align}
% Assume by induction that  
% \allowdisplaybreaks\begin{align} 
%  \sum_{u=0}^{t-1} \big| \boldsymbol\alpha(u) - \widetilde{\boldsymbol\alpha}(u) \big| \leq C 
%  \cdot \Big[ \sum_{i=1}^N w^\star_i |\mathcal{D}_i| \sum_{j=1}^{|\mathcal{D}_i|} | u^i_j - \tilde{u}^i_j |^2 
%  + |y^i_j - \tilde{y}^i_j |^2  \Big]^{1/2} .  \notag   
% \end{align} 
% By Lemma~\ref{lm:|AB|<=|A||B|}, \eqref{a-tildea} implies that   
% \allowdisplaybreaks\begin{align}  
%  & | \boldsymbol\alpha(t) - \widetilde{\boldsymbol\alpha}(t) | \notag \\ 
%  \leq &  \big| (M(P(t+1)))^{-1} - (M(\widetilde{P}(t+1)) )^{-1} \big| \cdot 
%  \Big[ |\Theta^\star| + \sum_{u=0}^{t-1}  | \boldsymbol\alpha(u) |   
%  + \lambda | \Theta^\star | +| S(t+1) | \Big]  \notag \\ 
%  & + \big| ( M(\widetilde{P}(t+1)) )^{-1} - I_{Np}  \big| 
%  \sum_{u=0}^{t-1} | \boldsymbol\alpha(u) - \widetilde{\boldsymbol\alpha}(u) | 
% + | (M(\widetilde{P}(t+1)))^{-1} | \cdot | S(t+1) - \widetilde{S}(t+1) | .  \notag   
% \end{align} 
% By \eqref{eqn:estM-tildeM},  \eqref{eqn:estS-tildeS}, and the induction hypothesis,
% the above inequality implies that that 
% \allowdisplaybreaks\begin{align}
%  |\boldsymbol\alpha(t) - \widetilde{\boldsymbol\alpha}(t)| 
%  \leq C  \Big[ \sum_{i=1}^N w^\star_i |\mathcal{D}_i| \sum_{j=1}^{|\mathcal{D}_i|} | u^i_j - \tilde{u}^i_j |^2 
%  + |y^i_j - \tilde{y}^i_j|^2  \Big]^{1/2} , \notag  
% \end{align} 
% and therefore 
% \allowdisplaybreaks\begin{align} 
%  \sum_{u=0}^{t} \big| \boldsymbol\alpha(u) - \widetilde{\boldsymbol\alpha}(u) \big| \leq C 
%  \cdot \Big[ \sum_{i=1}^N w^\star_i |\mathcal{D}_i| \sum_{j=1}^{|\mathcal{D}_i|} | u^i_j - \tilde{u}^i_j |^2 
%  + |y^i_j - \tilde{y}^i_j |^2  \Big]^{1/2} .  \notag   
% \end{align} 
% The estimate \eqref{eqn:stabilityControl} is then proved by induction.  
% \end{proof} 



% \begin{corollary} 
% \label{cor:stabilityLast}
% Under the hypothesis of Proposition \ref{prop:stabilityControl}, the costs \eqref{eq:penalized_regret_functional} under the optimal controls $\mathbf{a}$ 
% and $\widetilde{\mathbf{a}}$ satisfy the estimate 
% \allowdisplaybreaks\begin{align} 
%  \big| L^\star ( \boldsymbol\alpha ; \mathcal{D} ) 
%  -  L^\star (  \widetilde{\boldsymbol\alpha} ;  \widetilde{\mathcal{D}} )  \big|  
%  \leq  C \cdot \Big[ \sum_{i=1}^N w^\star_i |\mathcal{D}_i| \sum_{j=1}^{|\mathcal{D}_i|} | u^i_j - \tilde{x}^i_j |^2  + |y^i_j - \tilde{y}^i_j |^2 \Big]^{1/2} . 
%  \label{eqn:stabilityLast} 
% \end{align} 
% where $C>0$ is a constant depending on $\lambda$, $\beta$, $N$, $\bar{N}$, $\Theta^\star$, 
% $(w^\star_1, \cdots, w^\star_N)$, $K_x$, $K_y$, and $T$. 
% \end{corollary}


% \begin{proof}[{Proof of Corollary~\ref{cor:stabilityLast}}] 
% Throughout the proof $C$ is a constant depending on $\lambda$, $\beta$, $\bar{N}$, $\Theta^\star$, 
% $(w_1^\star, \cdots, w_N^\star)$, $K_x$, $K_y$ and $T$, and may vary from place to place.  
% By \eqref{ansatzVw} and \eqref{Theta-simple}, the difference of the costs can be written as 
% \allowdisplaybreaks\begin{align} 
%   L^\star ( \boldsymbol\alpha ; \mathcal{D} ) 
%  -  L^\star (  \widetilde{\boldsymbol\alpha} ;  \widetilde{\mathcal{D}} )  
% = & \Theta^\top (0) ( P(0) - \widetilde{P}(0) ) \Theta(0) 
%  + 2 ( S(0) - \widetilde{S}(0) )^\top \Theta(0) + r(0)-\widetilde{r}(0) ,  \notag \\ 
%   = & 
%    \Theta^{\star \top} ( P(0) - \widetilde{P}(0) ) \Theta^\star  
%  + 2 ( S(0) - \widetilde{S}(0) )^\top \Theta^\star + r(0)-\widetilde{r}(0) .  
%  \notag 
% \end{align} 
% By the triangular inequality, the difference satisfies  
% \allowdisplaybreaks\begin{align} 
%   \big| L^\star (  \boldsymbol\alpha ; \mathcal{D} ) 
%  -  L^\star (  \widetilde{\boldsymbol\alpha} ;  \widetilde{\mathcal{D}} ) \big|  
% \leq  |  P(0) - \widetilde{P}(0) | \cdot |\Theta^\star|^2  
%  + 2 | S(0) - \widetilde{S}(0) | \cdot | \Theta^\star | + | r(0)-\widetilde{r}(0) | . 
% \label{estLast-tildeLast} 
% \end{align}
% We claim that $r(0)-\widetilde{r}(0)$ satisfies the estimate 
% \allowdisplaybreaks\begin{align} 
%  | r(0)-\widetilde{r}(0) | \leq  C \cdot \Big[ \sum_{i=1}^N w^\star_i |\mathcal{D}_i| \sum_{j=1}^{|\mathcal{D}_i|} | u^i_j - \tilde{u}^i_j |^2 
%  + |y^i_j - \tilde{y}^i_j |^2 \Big]^{1/2} .  
% \label{eqn:estr-tilder(0)} 
% \end{align} 
% %where $C$ is a constant depending on $\Theta^\star$, $(w_1^\star, \cdots, w_N^\star)$, $K_x$, $K_y$ and $T$. 
% Then the desired estimate \eqref{eqn:stabilityLast} is established by \eqref{estLast-tildeLast}, \eqref{eqn:estP-tildeP}, 
% \eqref{eqn:estS-tildeS}  and \eqref{eqn:estr-tilder(0)}. 



% Now we prove the claim \eqref{eqn:estr-tilder(0)}. 
% From \eqref{eqnr(t)}, the difference $r-\widetilde{r}$ satisfies  
% \allowdisplaybreaks\begin{align} 
%  & r(t) - \widetilde{r}(t) =  r(t+1) - \widetilde{r}(t+1) 
%  - ( S(t+1) - \widetilde{S}(t+1) ) \big\{ (M(P(t+1)))^{-1} 
%  \big[ S(t+1) - 2 \lambda \Theta^\star \big]  \notag \\  
%  & \hspace{2cm} + (M(\widetilde{P}(t+1)))^{-1} \widetilde{S}(t+1) \big\}  \notag \\ 
%  &\hspace{2cm} - \widetilde{S}^\top(t+1) \big[ (M(P(t+1)))^{-1} 
%  - (M(\widetilde{P}(t+1)))^{-1} \big]  \big[ S(t+1) - 2 \lambda \Theta^\star \big]    \notag \\ 
%  &\hspace{2cm} - \Theta^{\star \top} \lambda  \big[ (M(P(t+1)))^{-1} 
%  - (M(\widetilde{P}(t+1)))^{-1} \big]  \lambda  \Theta^\star , \notag  \\ 
% %%% 
% & r(T) - \widetilde{r}(T) =   \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|} ( |y^i_j|^2 - |\widetilde{y}^i_j|^2 ) . \label{eqnr(t)-tilder(t)}  
% \end{align} 
% Inductively, $r(0)-\widetilde{r}(0)$ can be written in terms of $r(T)-\widetilde{r}(T)$ as   
% \allowdisplaybreaks\begin{align} 
%  & r(0) - \widetilde{r}(0) \notag \\ 
% = & r(T) - \widetilde{r}(T) 
%  - \sum_{t=1}^T \Big\{ ( S(t) - \widetilde{S}(t) ) \big[ (M(P(t)))^{-1} 
%  \big( S(t) - 2 \lambda \Theta^\star \big)    
%   + (M(\widetilde{P}(t)))^{-1} \widetilde{S}(t) \big]   \notag \\ 
%  & + \widetilde{S}^\top(t) \big[ (M(P(t)))^{-1} 
%  - (M(\widetilde{P}(t)))^{-1} \big]  \big[ S(t) - 2 \lambda  \Theta^\star \big]     
%   + \Theta^{\star \top} \lambda  \big[ (M(P(t)))^{-1} 
%  - (M(\widetilde{P}(t)))^{-1} \big]  \lambda \Theta^\star 
%   \Big\} . \notag  
% \end{align}
% By Lemma~\ref{lm:|AB|<=|A||B|}, we have  
% \allowdisplaybreaks\begin{align} 
% &   | r(0) - \widetilde{r}(0) | \notag \\ 
%  & \leq  | r(T) - \widetilde{r}(T) |
%   + \sum_{t=1}^T \Big\{ \big| S(t) - \widetilde{S}(t) \big| 
%  \cdot \Big[ \big| (M(P(t)))^{-1} \big| \cdot
%  \big(  | S(t) | + 2 \lambda | \Theta^\star| \big)    
%   + \big| (M(\widetilde{P}(t)))^{-1} \big| \cdot \big| \widetilde{S}(t) \big|  \Big]   \notag \\ 
%  & \hspace{2cm} +\big| (M(P(t)))^{-1} 
%  - (M(\widetilde{P}(t)))^{-1} \big|  \cdot  
%  \big( \big| \widetilde{S}(t) \big| \cdot \big| S(t) - 2 \lambda  \Theta^\star \big|     
%   +  \lambda | \Theta^\star |^2 \big) 
%   \Big\} . \label{estr(0)-tilder(0)}  
% \end{align}
% By \eqref{eqnr(t)-tilder(t)}, Lemma \ref{lm:|A1+An|2<=(|A1|2+|An|2)n}, and the Cauchy-Schwarz inequality, the terminal condition satisfies 
% \allowdisplaybreaks\begin{align} 
%   |r(T) - \widetilde{r}(T)| 
%   = &  \Big| \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|} 
%   ( y^i_j - \tilde{y}^i_j ) (y^i_j + \tilde{y}^i_j ) \Big| 
%   \leq \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|}  | (y^i_j - \tilde{y}^i_j) (y^i_j + \tilde{y}^i_j ) | \notag \\ 
%  \leq & \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|}  |y^i_j + \widetilde{y}^i_j| \cdot 
%  |y^i_ j - \widetilde{y}^i_j |  
%   \leq  2 K_y 
%  \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|}  |y^i_j -  \widetilde{y}^i_j| 
%   \notag \\ 
%  \leq & 2 K_y \Big( \sum_{i=1}^N w^\star_i  \sum_{j=1}^{|\mathcal{D}_i|}  |y^i_j - \widetilde{y}^i_j|^2 \Big)^{1/2} .  
%  \label{estr(T)-tilder(T)}  
% \end{align} 
% The estimate \eqref{eqn:estr-tilder(0)} then follows from 
% \eqref{estr(0)-tilder(0)}, \eqref{estr(T)-tilder(T)}, \eqref{eqn:estM-tildeM}, \eqref{eqn:estS-tildeS}, and \eqref{|S|bd}. 
% \end{proof}



% We may now derive the proof of Theorem~\ref{thrm:adv_robust} as a direct consequence of Corollary~\ref{cor:stabilityLast}.
% \begin{proof}[{Proof of Theorem~\ref{thrm:adv_robust}}]
% Fix $\widetilde{\mathcal{D}} \in \mathbb{D}^{p,\varepsilon}$ and let $I\subseteq \{(i,j):i=1,\dots,N,\,j=1,\dots,|\mathcal{D}_i|\}$ consist of all indices $(i,j)$ for which $\{(i,j):\, u^i_j\neq \widetilde{u}^i_j \mbox{ and } y^i_j\neq \widetilde{y}^i_j\}$.  By Corollary~\ref{cor:stabilityLast}, there is a constant $C>0$ which is independent of $\mathcal{D}$ such that
% \allowdisplaybreaks
% \allowdisplaybreaks\begin{align}
% \nonumber
%     \big| L^\star (  \boldsymbol\alpha ; \mathcal{D} ) 
%     -  L^\star (  \widetilde{\boldsymbol\alpha} ;  \widetilde{\mathcal{D}} )  \big|^2
%  \le &
%     \widetilde{C} \sum_{i=1}^N w_i^\star |\mathcal{D}_i| \sum_{j=1}^{|\mathcal{D}_i|} | u^i_j - \widetilde{u}^i_j |^2  + |y^i_j - \widetilde{y}^i_j |^2 
% \\ 
% \nonumber
% \le & 
% \widetilde{C} \cdot \sum_{(i,j)\in I}\, w_i^\star |\mathcal{D}_i|  ( | u^i_j - \widetilde{u}^i_j |^2  + |y^i_j - \widetilde{y}^i_j |^2 ) 
% \\ 
% \nonumber
% \le &
% \widetilde{C} \cdot \sum_{(i,j)\in I}\, w_i^\star |\mathcal{D}_i| \cdot \max\{| u^i_j - \widetilde{u}^i_j |^2, |y^i_j - \widetilde{y}^i_j |^2\}
% \\ 
% \nonumber
% = &
% \widetilde{C} \cdot \sum_{(i,j)\in I}\, w_i^\star |\mathcal{D}_i| \cdot \max\{| u^i_j - \widetilde{u}^i_j |, |y^i_j - \widetilde{y}^i_j |\}^2
% \\ 
% \nonumber
% \le &
% \widetilde{C} \cdot \sum_{(i,j)\in I}\, w_i^\star |\mathcal{D}_i| \cdot 2\varepsilon^2
% \\ 
% \nonumber
% \le &
% \widetilde{C} \#I\, p \, 2\varepsilon^2
%  ,
% \end{align}
% where we have set $\widetilde{C}\eqdef C^{1/2}$.
% \end{proof}



% %%%%%%%%%%%%%%%%%%%%%%%%%%%% 

% The computational complexity of the matrix-valued function $P(\cdot)$, as determined by \eqref{eqnP(t)}, does not primarily stem from the high dimensionality of the output matrices, but rather from their inherent lack of symmetries.
% As we will see later, such symmetry will allow us to efficiently encode $P(\cdot)$ into low-dimensional structures, therefore completely mitigating the high-dimensionality effect.


% We therefore introduce the following control, which is optimal for a ``symmetrized version'' of the control problem~\eqref{optimala} where $w^{\star}=(1/N,\dots,1/N)$.  This advantages this surrogate problem is that the associated $P$ function, which we denote by $\widehat{P}$, outputs highly symmetric\footnote{As formalized in Proposition~\ref{prop:P1/Nsubmat}.} Toeplitz matrices which are determined by exactly three factors. This allows us to encode the entire control problem into a control problem on $\mathbb{R}^{\tilde{O}(P)}$ whose dimension is independent of $N$. 
% Furthermore, the optimal controls of both problems can be related by stability estimates, depending only on the deviation of $(1/N,\dots,1/N)$ from $w^{\star}$, which allows us to infer the degree of sub-optimality of our $\widehat{P}$.  Therefore, we consider the control
% \begin{align} 
%  \widehat{\boldsymbol{\alpha}}(t)  
%  = & -[(\lambda + \beta )I_{Np} + \widehat{P}(t+1)]^{-1} 
%  \big[ (\lambda I_{Np} + \widehat{P}(t+1)) \Theta(t) 
%  - \lambda  \Theta^\star_{(N)} + \widehat{S}(t+1)  \big]   \label{hata} 
%  .
% \end{align} 
% We will show that the algorithm under control \eqref{hata} enjoys lower computational complexity in comparison with the regret-optimal algorithm \eqref{optimala}, whose computational complexity is summarized through Theorem~\ref{thm:ComplexityAlgorithm}. Furthermore, we will then establish the near-regret optimality of \eqref{hata}, stated in Theorem \ref{thrm:Epsilon_Efficiency}.

% The associated matrix-valued functions $\widehat{P}$ and $\widehat{S}$ are uniquely determined by 
% \allowdisplaybreaks\begin{align} 
% & \begin{cases}
%    \widehat{P}(t)  =  \beta I_{Np} - \beta^2 [(\lambda+\beta ) I_{Np} + \widehat{P}(t+1) ]^{-1} , \label{eqnhatP1/N(t)} \\ 
%    \widehat{P}(T) =  [ (1/N) I_p ,\cdots, (1/N) I_p]^{\top} 
%  \Big( \sum_{i=1}^N (1/N) \sum_{j=1}^{|\mathcal{D}_i|} u^i_j u^{i\top}_j  \Big)  
%  [ (1/N) I_p , \cdots, (1/N) I_p ] , 
% \end{cases} \\ 
% & \begin{cases}
%   \widehat{S}(t) =  
%   \beta [(\lambda + \beta ) I_{Np} + \widehat{P}(t+1) ]^{-1} 
%   \big( \widehat{S}(t+1) - \lambda \Theta^\star_{(N)} \big)
%   \label{eqnhatS1/N(t)} ,     \\ 
%         \widehat{S}(T) 
%     =  
%   - [(1/N)I_p, \cdots, (1/N)I_p ]^{\top} \sum_{i=1}^N(1/N)\sum_{j=1}^{|\mathcal{D}_i|}  u^i_j y^i_j  
%    ,  
% \end{cases} 
% \end{align} 
% where $[ I_p, \cdots, I_p ]$ denotes the $Np\times p$-dimensional matrix formed by concatenating $N$ copies of the $p\times p$-dimensional identity matrix $\frac{1}{N} I_p$.   The parameter $\Theta^\star_{(N)}$ is defined as 
% \allowdisplaybreaks\begin{align} 
%  \Theta^\star_{(N)} \eqdef [\theta_{(N)}^{\star \top}, \cdots, \theta_{(N)}^{\star \top}]^{\top} , \quad 
% \theta^\star_{(N)} \eqdef \frac{1}{N} \sum_{i=1}^N \theta^\star_i . \notag 
% \end{align}

% \begin{remark} 
% According to \eqref{Sum(uij)Tuij>=0} in Assumption \ref{assm:PD}, $\widehat{P}(T)\geq 0$ and therefore \eqref{eqnhatP1/N(t)} admits a unique solution. 
% \end{remark} 

% \begin{remark}
% \label{rmk:M(hatP)bdd}
% Similar to Corollary~\ref{cor:M(P)invbdd}, we have $\big| [ (\lambda+\beta)I_{Np} + \widehat{P}(t) ]^{-1} \big| \leq (\lambda + \beta)^{-1}$. By replacing $(w_1^\star, ..., w_N^\star)$ in the proof of Corollary~\ref{cor:M(P)invbdd} with $(1/N, ..., 1/N)$, we obtain 
% $|\widehat{S}(t)|\leq C \cdot N^{1/2}$ for all $t=1$, ..., $T$, 
% where $C>0$ is a constant depending on $\lambda$, $\beta$, $\Theta^\star$, $K_x$, $K_y$ and $T$.  
% \end{remark}


% \begin{lemma} 
% \label{lem:lemma_A}
%  Let $P$ and $\widehat{P}$ be the solutions of the systems \eqref{eqnP(t)} and \eqref{eqnhatP1/N(t)}, respectively. Then they satisfy that for all $t=1$, $2$, ..., $T$, 
% \allowdisplaybreaks
% \begin{align} 
%   \big| P(t) - \widehat{P}(t) \big| 
%  \leq  C \cdot \bar{N} N \max_{1\leq i, k, l \leq N} \Big| \frac{1}{N^3} -  w^\star_k w^\star_l w^\star_i \Big| ,  
% \label{estPw-P1/N} \\ 
%  \big| (M(P(t)))^{-1} - (M(\widehat{P}(t) ))^{-1} \big| 
%  \leq  C \cdot  \bar{N} N \max_{1\leq i, k, l \leq N} \Big| \frac{1}{N^3} -  w^\star_k w^\star_l w^\star_i \Big| ,  
% \label{estMPw-MP1/N}  
% \end{align}
% where $C>0$ is a constant depending on $\lambda$, $\beta$, $K_x$. 
% \end{lemma} 

% \begin{proof}[{Proof of Lemma~\ref{lem:lemma_A}}] 
% By \eqref{eqnhatP1/N(t)}, \eqref{eqnP(t)}, and Lemmas~\ref{lm:|AB|<=|A||B|} and \ref{lm:|A1+An|2<=(|A1|2+|An|2)n}, the difference 
% $\widehat{P}(T)-P(T)$ satisfies    
% \allowdisplaybreaks
% \begin{align} 
% |\widehat{P}(T) - P(T)|^2 = & \sum_{k,l=1}^N 
% \Big| \frac{1}{N^2} \sum_{k=1}^N \frac{1}{N} 
% \sum_{j=1}^{|\mathcal{D}_i|}  u^i_j u^{i\top}_j  - w^\star_k w^\star_l \sum_{i=1}^N w^\star_i  \sum_{j=1}^{|\mathcal{D}_i|} u^i_j u^{i\top}_j  \Big|^2 \notag \\ 
% \leq & N^2 \cdot \max_{1\leq k, l, i \leq N} \Big| \frac{1}{N^3} 
%   - w^\star_k w^\star_l 
%    w^\star_i \Big|^2 \cdot \Big| \sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|}  u^i_j u^{i\top}_j  \Big|^2  \notag \\  
%    \leq &   N^2 \cdot \max_{1\leq k, l, i \leq N} \Big| \frac{1}{N^3} 
%   -  w^\star_k w^\star_l 
%    w^\star_i \Big|^2 \cdot  \bar{N} \sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|}  | u^i_j |^4   \notag 
% \end{align} 
% and 
% \begin{align} 
% |\widehat{P}(T) - P(T)| 
%  \leq & \bar{N} N K_x^2 \cdot \max_{1\leq k, l, i \leq N} \Big| \frac{1}{N^3} 
%   -  w^\star_k w^\star_l 
%    w^\star_i \Big| . 
%    \label{|P(T)-hatP(T)|est}
% \end{align} 
% Therefore \eqref{estPw-P1/N} holds for $t=T$. 

% Assume by induction that \eqref{estPw-P1/N} holds for $t=u$. We show that \eqref{estPw-P1/N} also holds for $t=u-1$. 
% From \eqref{eqnhatP1/N(t)} and \eqref{eqnP(t)}, we have  
% \allowdisplaybreaks\begin{align} 
%  \widehat{P}(u-1) - P(u-1) 
% = & [ M(P(u)) ]^{-1}
%  -  [ M( \widehat{P}(u) ) ]^{-1}  \notag  \\ 
%  = & [ M( P(u) ) ]^{-1} (\widehat{P}(u) - P(u)) 
% [ M( \widehat{P}(u) ) ]^{-1} . 
% \label{hatP-Precursion}
% \end{align} 
% By Lemmas~\ref{lm:|AB|<=|A||B|} and \ref{lm:|A1+An|2<=(|A1|2+|An|2)n}, we further have 
% \allowdisplaybreaks\begin{align} 
%  | \widehat{P}(u-1) - P(u-1) | 
% = & | [ M(P(u)) ]^{-1} 
%  -  [ M( \widehat{P}(u) ) ]^{-1} | \notag  \\ 
%  \leq & | [ M( P(u) ) ]^{-1} | \cdot  | \widehat{P}(u) - P(u) | \cdot 
%  | [ M( \widehat{P}(u) ) ]^{-1} | . 
% \label{|hatP-P|recursion}
% \end{align} 
% By \eqref{|hatP-P|recursion}, Corollary~\ref{cor:M(P)invbdd}, Remark~\ref{rmk:M(hatP)bdd}, and the induction hypothesis, we have 
% that \eqref{estPw-P1/N} holds for $t=u-1$. By induction we have shown that \eqref{estPw-P1/N} holds for all $1\leq t\leq T$. 


% From \eqref{hatP-Precursion}, we have 
% \allowdisplaybreaks 
% \begin{align} 
% & \big| ( M(P(t)) )^{-1}
%  -  ( M( \widehat{P}(t) ) )^{-1} \big|   
%  \leq  \big| ( M( P(t) ) )^{-1} \big| \cdot  \big| \widehat{P}(t) - P(t) \big| \cdot   
% \big| ( M( \widehat{P}(t) ) )^{-1} 
% \big| ,  \notag 
% \end{align} 
% which, together with \eqref{estPw-P1/N}, Corollary~\ref{cor:M(P)invbdd}, and Remark~\ref{rmk:M(hatP)bdd}, establishes \eqref{estMPw-MP1/N}. 
% \end{proof}


% \begin{lemma}
% \label{lem:Lemma_B}
%  Let $S$ and $\widehat{S}$ be the solutions of \eqref{eqnS(t)} and \eqref{eqnhatS1/N(t)}, respectively. Then they satisfy that 
% for all $t=1$, ..., $T$, 
% \allowdisplaybreaks
% \begin{align} 
%  |S(t) - \widehat{S}(t)| \leq & 
% C \cdot \Big\{ \bar{N} N^{3/2} \max_{1\leq i, k, l \leq N} \Big| \frac{1}{N^3} -  w^\star_k w^\star_l w^\star_i \Big| 
%   \notag \\ 
% & \hspace{1cm} + \bar{N} N^{1/2} \max_{1\leq k, l\leq N} \Big| \frac{1}{N^2} - w^\star_k w^\star_l \Big|
% + |\Theta^\star - \Theta^\star_{(N)}| \Big\} , 
%  \label{sup|S-hatS|est}
% \end{align}
% where $C>0$ is a constant depending on $\lambda$, $\beta$, $\Theta^\star$, $K_x$, $K_y$, and $T$. 
% \end{lemma}

% \begin{proof}[{Proof of Lemma~\ref{lem:Lemma_B}}]
% By \eqref{eqnS(t)}, \eqref{eqnhatS1/N(t)}, and and Lemmas~\ref{lm:|AB|<=|A||B|} and \ref{lm:|A1+An|2<=(|A1|2+|An|2)n}, the terminal condition $S(T)-\widehat{S}(T)$ satisfies 
% \allowdisplaybreaks\begin{align} \Big|S(T)-\widehat{S}(T)\Big|^2 
% = & \sum_{k=1}^N \Big| 
%  \frac{1}{N} \sum_{i=1}^N \frac{1}{N} \sum_{j=1}^{|\mathcal{D}_i|} u^i_j y^i_j - w^\star_k 
%  \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|} u^i_j y^i_j 
% \Big|^2 \notag \\ 
% \leq & N \cdot \max_{1\leq k, l \leq N} \Big| \frac{1}{N^2} - w^\star_k w^\star_l \Big|^2 \cdot \Big| \sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|} u^i_j y^i_j \Big|^2  \notag \\ 
%  \leq & N \cdot \max_{1\leq k, l \leq N} \Big| \frac{1}{N^2} - w^\star_k w^\star_l \Big|^2 \cdot \bar{N} \sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|} | u^i_j|^2 \cdot |y^i_j|^2 ,  
%  \notag 
% \end{align} 
% which implies  
% \allowdisplaybreaks\begin{align} 
%  \big| S(T) - \widehat{S}(T) \big| 
%  \leq & \bar{N} N^{1/2} \max_{1\leq k, l\leq N} \Big| \frac{1}{N^2} - w^\star_k w^\star_l \Big| \cdot   K_x K_y . 
%   \label{|S(T)-hatS(T)|est}  
% \end{align} 
% Therefore \eqref{sup|S-hatS|est} holds for $t=T$. 

% Assume by induction that \eqref{sup|S-hatS|est} holds for $t=u$, we show that \eqref{sup|S-hatS|est} holds for $t=u-1$. 
% From \eqref{eqnS(t)} and \eqref{eqnhatS1/N(t)}, the difference $S(u-1)-\widehat{S}(u-1)$ can be written as 
% \allowdisplaybreaks\begin{align} 
%  S(u-1) - \widehat{S}(u-1) = & [ M(P(u)) ]^{-1}[S(u) - \widehat{S}(u) - \lambda (\Theta^\star - \Theta^\star_{(N)}) ] \notag \\ 
%  & - \big[ ( M(\widehat{P}(u)))^{-1} - ( M(P(u)) )^{-1} \big]  
%  (\widehat{S}(u) - \lambda \Theta^\star_{(N)}) , 
%  \label{S(t)-hatS(t)}
% \end{align} 
% and satisfies by 
% Lemma~\ref{lm:|AB|<=|A||B|} that  
% \begin{align} 
% |S(u-1) - \widehat{S}(u-1)| 
%  \leq & | [M(P(u))]^{-1} | \cdot 
% \big[  |S(u) - \widehat{S}(u)| + \lambda |\Theta^\star - \Theta^\star_{(N)}|
%  \big] \notag \\ 
%  & + \big| ( M(\widehat{P}(u)))^{-1} 
%   - ( M(P(u)) )^{-1} \big| \cdot  
%  \big( |\widehat{S}(u)| + \lambda |\Theta^\star_{(N)}| \big) . \label{|hatS-S|recursion}
% \end{align} 
% By \eqref{|hatS-S|recursion}, \eqref{estMPw-MP1/N}, Remark~\ref{rmk:M(hatP)bdd}, and the induction hypothesis, we have that 
% \eqref{sup|S-hatS|est} holds for $t=u-1$. By induction we have shown that \eqref{sup|S-hatS|est} holds for all $t=1$, ..., $T$. 


% \end{proof}


% We now obtain Theorem~\ref{thrm:Epsilon_Efficiency}; which is a direct consequence of the following Propositions \ref{prop:stabilityaw-a1/N} and \ref{prop:stabilityLw-L1/N}.

% \begin{proposition} 
% \label{prop:stabilityaw-a1/N}
% The controls
% \eqref{optimala} and \eqref{hata} satisfy $|\widehat{\boldsymbol{\alpha}}(t)| \leq C \cdot N^{1/2}$ for all $t=0$, $1$, ..., $T-1$, and  
% \allowdisplaybreaks\begin{align} 
%  \sum_{t=0}^{T-1} |\boldsymbol{\alpha}(t) - \widehat{\boldsymbol{\alpha}}(t)| 
%  \leq & C\cdot \Big\{ \bar{N} N^{3/2} \max_{1\leq i, k, l \leq N} \Big| \frac{1}{N^3} -  w^\star_k w^\star_l w^\star_i \Big| \notag \\ 
%  &\hspace{2cm} + \bar{N} N^{1/2} \cdot \max_{1\leq k, l\leq N} \Big| \frac{1}{N^2} - w^\star_k w^\star_l \Big| 
%  + |\Theta^\star - \Theta^\star_{(N)}| \Big\} , 
% \label{eqn:stabilityaw-a1/N}
% \end{align} 
% where $C>0$ is a constant depending on $\lambda$, $\beta$, $\Theta^\star$, $K_x$, $K_y$, and $T$. 
% \end{proposition} 

% \begin{proof}[{Proof of Proposition~\ref{prop:stabilityaw-a1/N}}]
% We let $C$ be a constant depending on $\lambda$, $\beta$, $\Theta^\star$, $K_x$, $K_y$, and $T$, 
% and $C$ is allowed to vary from place to place throughout the proof. 
% By \eqref{optimala}, \eqref{hata}, and \eqref{Theta(t)Theta(0)}, we can write $\boldsymbol{\alpha}$ and $\widehat{\boldsymbol\alpha}$ as   
% \allowdisplaybreaks\begin{align} 
%   \boldsymbol{\alpha}(t) 
%  = & [ (M(P(t+1)))^{-1} - I_{Np} ]  \Big[ \Theta^\star 
%  + \sum_{u=0}^{t-1} \boldsymbol{\alpha}(u) \Big]  
%   +  [ M(P(t+1)) ]^{-1} ( \lambda  \Theta^\star - S(t+1) ) ,   \notag \\ 
%   \widehat{\boldsymbol{\alpha}}(t) 
%  = & [ (M(\widehat{P}(t+1)))^{-1} - I_{Np} ]  \Big[ \Theta^\star 
%  + \sum_{u=0}^{t-1} \widehat{\boldsymbol{\alpha}}(u) \Big]  
%   +  [ M(\widehat{P}(t+1)) ]^{-1} ( \lambda  \Theta^\star_{(N)} - \widehat{S}(t+1) ) .   \notag 
% \end{align} 
% For $t=0$, we have 
% \begin{align} 
%  |\widehat{\boldsymbol{\alpha}}(0)| \leq  & | (M(\widehat{P}(1)))^{-1} - I_{Np} | \cdot |  \Theta^\star |   
%   + \big| [ M(\widehat{P}(1)) ]^{-1} \big| ( \lambda  |\Theta^\star_{(N)}| + |\widehat{S}(1)| ) ,  \notag 
% \end{align} 
% which implies $|\widehat{\boldsymbol{\alpha}}(0)| \leq C N^{1/2}$. 
% Assume by induction that $|\widehat{\boldsymbol{\alpha}}(u)| \leq C N^{1/2}$ for $u=0$, ..., $t-1$, then 
% \begin{align} 
% \widehat{\boldsymbol{\alpha}}(t) 
%  \leq & \big| (M(\widehat{P}(t+1)))^{-1} - I_{Np} \big|   \Big[ | \Theta^\star | 
%  + \sum_{u=0}^{t-1} | \widehat{\boldsymbol{\alpha}}(u) | \Big] \notag \\  
%  & + \big| [ M(\widehat{P}(t+1)) ]^{-1} \big| ( \lambda | \Theta^\star_{(N)} | + | \widehat{S}(t+1) | ) \notag 
% \end{align} 
% gives that $|\widehat{\boldsymbol{\alpha}}(t)|\leq CN^{1/2}$. By induction we have shown that 
% $|\widehat{\boldsymbol{\alpha}}(t)|\leq CN^{1/2}$ for all $t=0$, $1$, ..., $T-1$. 



% We further write the difference $\boldsymbol{\alpha} - \widehat{\boldsymbol\alpha}$ as    
% \allowdisplaybreaks\begin{align}  
%  & \boldsymbol{\alpha}(t) - \widehat{\boldsymbol\alpha}(t) \notag \\ 
%  = &  \big[(M(P(t+1)))^{-1} - (M(\widehat{P}(t+1)) )^{-1} \big] 
%  \Big[ (\lambda + 1)\Theta^\star + \sum_{u=0}^{t-1}  \boldsymbol{\alpha}(u)    - S(t+1) \Big]  \notag \\ 
%  & + \big[ ( M(\widehat{P}(t+1)) )^{-1} - I_{Np} \big] 
%  \sum_{u=0}^{t-1} (\boldsymbol{\alpha}(u) - \widehat{\boldsymbol{\alpha}}(u)) 
% + [ M(\widehat{P}(t+1)) ]^{-1} (\widehat{S}(t+1) - S(t+1))  \notag \\ 
%  & + \lambda [ M(\widehat{P}(t+1)) ]^{-1} ( \Theta^\star 
%  - \Theta^\star_{(N)} ) . \label{a-hata} 
% \end{align} 


% For $t=0$, the difference 
% \allowdisplaybreaks\begin{align} 
%   \boldsymbol{\alpha}(0) - \widehat{\boldsymbol{\alpha}}(0)  
%  = & \big[ (M(P(1)))^{-1} - (M(\widehat{P}(1)))^{-1}  \big] 
%  \big[ ( \lambda + 1 )   \Theta^\star_{(N)} - \widehat{S}(1)  \big] \notag \\ 
%  & + [ M(P(1)) ]^{-1} [ (\lambda+1) (\Theta^\star - \Theta^\star_{(N)} ) + \widehat{S}(1) - S(1) ]   \notag  
% \end{align} 
% satisfies 
% \allowdisplaybreaks\begin{align} 
%   \big| \boldsymbol{\alpha}(0) 
%    - \widehat{\boldsymbol{\alpha}}(0) \big| 
%   \leq & 
%   C  \cdot \Big\{ \bar{N} N^{3/2} \max_{1\leq i, k, l \leq N} \Big| \frac{1}{N^3} -  w^\star_k w^\star_l w^\star_i \Big| \notag \\ 
%  & \hspace{1cm} + \bar{N} N^{1/2} \max_{1\leq k, l\leq N} \Big| \frac{1}{N^2} - w^\star_k w^\star_l \Big|
%  + |\Theta^\star - \Theta^\star_{(N)}| \Big\} , \notag    
% \end{align} 
% due to \eqref{estMPw-MP1/N}, \eqref{sup|S-hatS|est}, Lemma~\ref{lm:|AB|<=|A||B|}, Corollary~\ref{cor:M(P)invbdd} and Remark~\ref{rmk:M(hatP)bdd}.  
% Assume by induction for all $0 \leq u\leq t-1$, 
% $\boldsymbol{\alpha}(u-1) - \widehat{\boldsymbol{\alpha}}(u-1)$ satisfies
% \allowdisplaybreaks\begin{align} 
%   \big| \boldsymbol{\alpha}(u-1) 
%   - \widehat{\boldsymbol{\alpha}}(u-1) \big| 
%   \leq & C   
%  \cdot \Big\{ \bar{N} N^{3/2} \max_{1\leq i, k, l \leq N} \Big| \frac{1}{N^3} -  w^\star_k w^\star_l w^\star_i \Big| \notag \\ 
% & \hspace{1cm} + \bar{N} N^{1/2} \max_{1\leq k, l\leq N} \Big| \frac{1}{N^2} - w^\star_k w^\star_l \Big| 
%  + |\Theta^\star - \Theta^\star_{(N)}| \Big\}  . \notag   
% \end{align} 
% By \eqref{a-hata} we have  
% \allowdisplaybreaks\begin{align}  
%  & | \boldsymbol{\alpha}(t) - \widehat{\boldsymbol{\alpha}}(t) | \notag \\ 
%  \leq &  \big| (M(P(t+1)))^{-1} - (M(\widehat{P}(t+1)) )^{-1} \big| \cdot 
%  \Big[ \sum_{u=0}^{t-1}  | \boldsymbol{\alpha}(u) |   
%  + | ( \lambda +1 ) \Theta^\star | 
%  +| S(t+1) | \Big]  \notag \\ 
%  & + \big| ( M(\widehat{P}(t+1)) )^{-1} - I_{Np}  \big| 
%  \sum_{u=0}^{t-1} | \boldsymbol{\alpha}(u) - \widehat{\boldsymbol{\alpha}}(u) | 
% + | (M(\widehat{P}(t+1)))^{-1} | \cdot | S(t+1) - \widehat{S}(t+1) | ,  \notag   \\ 
%  & + \big| [ M(\widehat{P}(t+1)) ]^{-1} \big| \cdot |\lambda | \cdot 
%   \big| \Theta^\star - \Theta^\star_{(N)} \big| . \notag  
% \end{align} 
% By the induction hypothesis, \eqref{estMPw-MP1/N}, 
% \eqref{sup|S-hatS|est}, and Remark~\ref{rmk:M(hatP)bdd},  the above inequality implies that  
% \allowdisplaybreaks\begin{align}
%  |\boldsymbol{\alpha}(t) - \widehat{\boldsymbol{\alpha}}(t)| 
%  \leq & C \cdot \Big\{ \bar{N} N^{3/2} \max_{1\leq i, k, l \leq N} \Big| \frac{1}{N^3} -  w^\star_k w^\star_l w^\star_i \Big| 
%   \notag \\
% & \hspace{1cm} + \bar{N} N^{1/2} \max_{1\leq k, l\leq N} \Big| \frac{1}{N^2} - w^\star_k w^\star_l \Big| 
%  + |\Theta^\star - \Theta^\star_{(N)}| \Big\}  . \label{|a(t)-hata(t)|est}  
% \end{align}
% We have shown by induction that \eqref{|a(t)-hata(t)|est} holds for all $t=0$, $1$, ..., $T-1$, 
% and therefore \eqref{eqn:stabilityaw-a1/N} follows.  
% \end{proof} 

% \begin{proposition} 
% \label{prop:stabilityLw-L1/N} 
% Under the hypothesis of Proposition \ref{prop:stabilityaw-a1/N}, the costs \eqref{eq:penalized_regret_functional} under the controls \eqref{optimala} 
% and \eqref{hata}, respectively, satisfy the estimate 
% \allowdisplaybreaks\begin{align} 
%  \big| L^\star (  \boldsymbol{\alpha} ; \mathcal{D} ) 
%  -  L^\star (  \widehat{\boldsymbol{\alpha}} ;  \mathcal{D} )  \big|  
%  \le &  C  \cdot \Big\{ \bar{N} N^3 \max_{1\leq i, k, l \leq N} \Big| \frac{1}{N^3} -  w^\star_k w^\star_l w^\star_i \Big| 
%   + \bar{N} N^{3/2} \max_{1\leq k, l\leq N} \Big| \frac{1}{N^2} - w^\star_k w^\star_l \Big| 
%   \notag \\
% & \hspace{3cm} 
%  + \bar{N} \max_{1\leq i \leq N} \Big|\frac{1}{N} - w_i^\star \Big|
%  + N |\Theta^\star - \Theta^\star_{(N)}| \Big\}  ,  
% \label{stabilityLw-L1/N} 
% \end{align} 
% where $C>0$ is a constant depending on $\lambda$, $\beta$, $\Theta^\star$, $(w_1^\star, ..., w_N^\star)$,  
% $K_x$, $K_y$ and $T$. 
% \end{proposition} 

% \begin{proof}[Proof of Proposition~\ref{prop:stabilityLw-L1/N} ] 
% Let $L^\star(\widehat{\boldsymbol{\alpha}}; \overline{1/N} , \mathcal{D})$, 
% $L^\star( \widehat{\boldsymbol{\alpha}}; w^\star, \mathcal{D})$, and
% $L^\star(\boldsymbol{\alpha}; w^\star , \mathcal{D})$ be as defined in 
% Lemmas~\ref{lm:|L(hata;1/N)-L(hata;w)|est} 
% and~\ref{lm:|L(a;w)-L(hata;1/N)|est}.   
% The difference $L^\star(\boldsymbol{\alpha}; \mathcal{D}) - L^\star( \widehat{\boldsymbol{\alpha}}; \mathcal{D})$ can be decomposed as 
% \begin{align} 
% L^\star(\boldsymbol{\alpha}; \mathcal{D}) - L^\star( \widehat{\boldsymbol{\alpha}}; \mathcal{D}) 
% = L^\star(\boldsymbol{\alpha}; w^\star, \mathcal{D}) - L^\star(\widehat{\boldsymbol{\alpha}}; \overline{1/N}, \mathcal{D}) 
%  + L^\star(\widehat{\boldsymbol{\alpha}}; \overline{1/N} , \mathcal{D}) 
%   - L^\star( \widehat{\boldsymbol{\alpha}}; w^\star, \mathcal{D}) ,\notag 
% \end{align}  
% and satisfies    
% \begin{align} 
%  | L^\star(\boldsymbol{\alpha}; \mathcal{D}) - L^\star( \widehat{\boldsymbol{\alpha}}; \mathcal{D}) | 
% \leq | L^\star(\boldsymbol{\alpha}; w^\star, \mathcal{D}) - L^\star(\widehat{\boldsymbol{\alpha}}; \overline{1/N}, \mathcal{D}) |
%  + | L^\star(\widehat{\boldsymbol{\alpha}}; \overline{1/N} , \mathcal{D}) 
%   - L^\star( \widehat{\boldsymbol{\alpha}}; w^\star, \mathcal{D}) | . \notag 
% \end{align} 
% The desired estimate \eqref{stabilityLw-L1/N} then follows from the above inequality and \eqref{|L(hata,1/N)-L(hata,w)|est} 
% and \eqref{|L(a,w)-L(hata,1/N)|est}. 
% \end{proof} 


% \begin{lemma}
% \label{lm:|L(hata;1/N)-L(hata;w)|est} 
% Let $L^\star(\widehat{\boldsymbol{\alpha}}; w^\star, \mathcal{D})$ be \eqref{eq:penalized_regret_functional} with 
% information sharing weights $w^\star=(w_1^\star, ..., w_N^\star)$ and $\Theta(t+1)-\Theta(t)=\widehat{\boldsymbol{\alpha}}(t)$, 
% and let $L^\star(\widehat{\boldsymbol{\alpha}}; \overline{1/N} , \mathcal{D})$ be \eqref{eq:penalized_regret_functional} with information sharing weights $\overline{1/N}=(1/N, ..., 1/N)$ and $\Theta(t+1)-\Theta(t)=\widehat{\boldsymbol{\alpha}}(t)$. 
% Then it satisfies 
% \begin{align} 
%  | L^\star(\widehat{\boldsymbol{\alpha}}; \overline{1/N} , \mathcal{D}) 
%   - L^\star( \widehat{\boldsymbol{\alpha}}; w^\star, \mathcal{D}) | \leq C  \cdot 
%   \Big\{ \bar{N} \max_{1\leq i \leq N} \Big|\frac{1}{N} - w_i^\star \Big| + N^{1/2} |\Theta^\star-\Theta^\star_{(N)}| \Big\} 
%   \label{|L(hata,1/N)-L(hata,w)|est} , 
% \end{align} 
% where $C>0$ is a constant depending on $\lambda$, $\beta$, $\Theta^\star$, 
% $(w^\star_1, \cdots, w^\star_N)$, $K_x$, $K_y$ and $T$. 
% \end{lemma} 
% \begin{proof} 
% By \eqref{eq:penalized_regret_functional} and \eqref{lwT}, we have 
% \begin{align} 
%    L^\star(\widehat{\boldsymbol{\alpha}}; \overline{1/N} , \mathcal{D}) 
%   - L^\star( \widehat{\boldsymbol{\alpha}}; w^\star, \mathcal{D}) 
%  = & \sum_{t=0}^{T-1} \big( |\Theta(t+1) - \Theta^\ast|^2 - |\Theta(t+1) - \Theta_{(N)}^\ast|^2 \big) \notag \\ 
%  & + l(\Theta(T), \overline{1/N}; \mathcal{D} ) - l(\Theta(T), w^\star ; \mathcal{D} ) .\notag  
% \end{align} 
% We have that
% \begin{equation}
% \label{|L(hata,1/N)-L(hata,w)|rcest} 
% \begin{aligned} 
%  &  \Big| \sum_{t=0}^{T-1} \big( |\Theta(t+1) - \Theta^\ast|^2 - |\Theta(t+1) - \Theta_{(N)}^\ast|^2 \big) \Big|  
%  \\
%  =&   \Big| \sum_{t=0}^{T-1} (\Theta^\star_{(N)} - \Theta^\star)^\top (2 \Theta(t+1) - \Theta^\star - \Theta^\star_{(N)}) \Big| \notag \\ 
%  \le & \sum_{t=0}^{T-1} | \Theta^\star_{(N)} - \Theta^\star | \cdot 
%  | 2 \Theta(t+1) - \Theta^\star - \Theta^\star_{(N)}|  
%  \leq C N^{1/2} \cdot  |\Theta^\star_{(N)} - \Theta^\star| ,  
% \end{aligned} 
% \end{equation}
% %where the last inequality is due to that $|\widehat{\boldsymbol{\alpha}}(t)|\leq C\cdot N$ for all $t=0$, $1$, ..., $T-1$ by %Proposition~\ref{prop:stabilityaw-a1/N}. 
% and 
% \begin{align} 
%  & l(\Theta(T), \overline{1/N}; \mathcal{D} ) - l(\Theta(T), w^\star ; \mathcal{D} )  \notag \\ 
%  = &  \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|}  \Big[ u^{i\top}_j \sum_{k=1}^N w^\star_k \theta_k - y^i_j  \Big]^2 
%  - \sum_{i=1}^N \frac{1}{N} \sum_{j=1}^{|\mathcal{D}_i|}  \Big[ u^{i\top}_j \sum_{k=1}^N \frac{1}{N} \theta_k - y^i_j  \Big]^2 
%   \notag \\ 
%   =& \sum_{i=1}^N (w^\star_i - 1/N) \sum_{j=1}^{|\mathcal{D}_i|}  \Big[ u^{i\top}_j \sum_{k=1}^N w^\star_k \theta_k - y^i_j  \Big]^2 \notag \\ 
%  &  + \sum_{i=1}^N \frac{1}{N} \sum_{j=1}^{|\mathcal{D}_i|}  
%  \Big[ u^{i\top}_j \sum_{k=1}^N (w^\star_k -1/N) \theta_k   \Big] 
%   \Big[ u^{i\top}_j \sum_{k=1}^N ( w^\star_k + 1/N ) \theta_k - 2 y^i_j  \Big]^2 , \notag 
% \end{align} 
% which implies that 
% \begin{align} 
%  | l(\Theta(T), \overline{1/N}; \mathcal{D} ) - l(\Theta(T), w^\star ; \mathcal{D} ) | 
%  \leq C \bar{N} \max_{1\leq i \leq N} |1/N - w_i^\star| . 
%  \label{|L(hata,1/N)-L(hata,w)|Test}
% \end{align} 
% The estimate \eqref{|L(hata,1/N)-L(hata,w)|est} then follows from 
% \eqref{|L(hata,1/N)-L(hata,w)|rcest}
% and \eqref{|L(hata,1/N)-L(hata,w)|Test}. 
% \end{proof} 


% \begin{lemma}
% \label{lm:|L(a;w)-L(hata;1/N)|est} 
% Let $L^\star(\alpha; w^\star, \mathcal{D})$ be \eqref{eq:penalized_regret_functional} with 
% information sharing weights $w^\star=(w_1^\star, ..., w_N^\star)$ and $\Theta(t+1)-\Theta(t)= \boldsymbol{\alpha}(t)$, 
% and let $L^\star(\widehat{\boldsymbol{\alpha}}; \overline{1/N} , \mathcal{D})$ be \eqref{eq:penalized_regret_functional} with information sharing weights $\overline{1/N}=(1/N, ..., 1/N)$ and $\Theta(t+1)-\Theta(t)=\widehat{\boldsymbol{\alpha}}(t)$. 
% Then it satisfies 
% \begin{align} 
%  & | L^\star(\boldsymbol{\alpha}; w^\star , \mathcal{D}) 
%   - L^\star( \widehat{\boldsymbol{\alpha}}; \overline{1/N}, \mathcal{D}) | 
%   \leq   
%    C \cdot  \Big\{ \bar{N} N^3 \cdot \max_{1\leq i, k, l \leq N} \Big| \frac{1}{N^3} -  w^\star_k w^\star_l w^\star_i \Big| 
%   \notag \\
% & \hspace{1.5cm} 
% +\bar{N} N^{3/2} \max_{1\leq k, l\leq N} \Big| \frac{1}{N^2} - w^\star_k w^\star_l \Big|  + \bar{N} \cdot \max_{1\leq i \leq N} \Big| \frac{1}{N} - w_i^\star \Big|
% + N |\Theta^\star - \Theta^\star_{(N)}| \Big\} , 
%   \label{|L(a,w)-L(hata,1/N)|est}
% \end{align} 
% where $C$ is a constant depending on $\lambda$, $\beta$, $\Theta^\star$, 
% $(w^\star_1, \cdots, w^\star_N)$, $K_x$, $K_y$ and $T$. 
% \end{lemma} 

% \begin{proof} 
% By the similar argument for \eqref{ansatzVw}, we have 
% \begin{align} 
%  L^\star( \widehat{\boldsymbol{\alpha}}; \overline{1/N}, \mathcal{D}) 
%   = \Theta^{\star\top}  \widehat{P}(0)  \Theta^\star 
%  + 2\widehat{S}(0)^\top \Theta^\star + \widehat{r}(0) . \label{ansatzV1/N} 
% \end{align} 
% By \eqref{ansatzVw} and \eqref{ansatzV1/N}, the difference $L^\star(\boldsymbol{\alpha}; w^\star, \mathcal{D}) - L^\star( \widehat{\boldsymbol{\alpha}}; \overline{1/N}, \mathcal{D})$ can be written as 
% \allowdisplaybreaks\begin{align} 
%   L^\star(\boldsymbol{\alpha}; w^\star, \mathcal{D}) - L^\star( \widehat{\boldsymbol{\alpha}}; \overline{1/N}, \mathcal{D}) 
% = \Theta^{\star\top} ( P(0) - \widehat{P}(0) ) \Theta^\star 
%  + 2 ( S(0) - \widehat{S}(0) )^\top \Theta^\star + r(0)-\widehat{r}(0) ,  
%  \notag 
% \end{align} 
% and by Lemma~\ref{lm:|AB|<=|A||B|}, the difference satisfies  
% \allowdisplaybreaks\begin{align} 
%   \big| L^\star (  \boldsymbol{\alpha} ; w^\star, \mathcal{D} ) 
%  -  L^\star (  \widehat{\boldsymbol{\alpha}} ; \overline{1/N} , \mathcal{D} ) \big|  
% \le & |\Theta^\star|^2 \cdot |  P(0) - \widehat{P}(0) |  
%  + 2 | S(0) - \widehat{S}(0) | \cdot | \Theta^\star| 
%  \nonumber
%  \\ 
%  & + | r(0)-\widehat{r}(0) | . \label{|L(a,w)-L(hata,1/N)|leqQudratic}
% %\label{estLast-tildeLast} 
% \end{align}
% We claim that $r(0)-\widehat{r}(0)$ has the estimate 
% \allowdisplaybreaks\begin{align} 
%  | r(0)-\widehat{r}(0) | \le &  C  \cdot  \Big\{ \bar{N} N^3 \cdot \max_{1\leq i, k, l \leq N} \Big| \frac{1}{N^3} -  w^\star_k w^\star_l w^\star_i \Big| 
%  +\bar{N} N^{3/2} \max_{1\leq k, l\leq N} \Big| \frac{1}{N^2} - w^\star_k w^\star_l \Big| 
%   \notag \\
% & \hspace{2cm} 
%  + \bar{N} \cdot \max_{1\leq i \leq N} \Big| \frac{1}{N} - w_i^\star \Big|
% + N \cdot |\Theta^\star - \Theta^\star_{(N)}| \Big\}  , 
% \label{eqn:estrw-tilder1/N} 
% \end{align} 
% where $C$ is a constant depending on $\lambda$, $\beta$, $\Theta^\star$, 
% $(w^\star_1, \cdots, w^\star_N)$, $K_x$, $K_y$ and $T$. 
% Then the desired estimate \eqref{|L(a,w)-L(hata,1/N)|est} is established by \eqref{|L(a,w)-L(hata,1/N)|leqQudratic}, \eqref{estPw-P1/N}, \eqref{sup|S-hatS|est} and \eqref{eqn:estrw-tilder1/N}. 



% Now we prove the claim \eqref{eqn:estrw-tilder1/N}. 
% From \eqref{eqn:Vansatz} and \eqref{lwT}, we obtain the equation that $\widehat{r}$ satisfies on $0\leq t \leq T$: 
% \begin{align} 
% &\begin{cases} 
%  \widehat{r}(t) =  - ( \widehat{S}(t+1) - \lambda \Theta_{(N)}^\star )^\top
%  [(\lambda+\beta)I_{Np} + \widehat{P}(t+1)]^{-1} \cdot ( \widehat{S}(t+1) - \lambda \Theta_{(N)}^\star )   \\  
%  \hspace{1.1cm}   + \lambda \| \Theta_{(N)}^\star \|_2^2 + \widehat{r}(t+1), 
%  \label{eqnhatr(t)} \\ \widehat{r}(T) = \sum_{i=1}^N (1/N) \sum_{j=1}^{|\mathcal{D}_i|} |y^i_j|^2 . 
%  \end{cases}  
% \end{align} 
% %\allowdisplaybreaks\begin{align} 
% %\begin{cases}
% %  r(t) =  r(t+1) - S^\top(t+1) (M(P(t+1)))^{-1} S(t+1)  
% % + 2 \lambda S^\top(t+1) (M(P(t+1)))^{-1}  \Theta^\star  \\ 
% %  \hspace{1cm} + \Theta^{\star \top} \big[ \lambda I_{Np} - \lambda^2 (M(P(t+1)))^{-1}  \big] \Theta^\star  ,  \\ 
% %%% 
% %  r(T) = \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|} |y^i_j|^2 .    
% %\end{cases} 
% %\notag 
% %\label{eqnr(t)}
% %\end{align} 
% Then $r-\widehat{r}$ satisfies the equation on $0\leq t \leq T$
% \allowdisplaybreaks\begin{align} 
%  & r(t) - \widehat{r}(t) \notag \\ 
% = &  r(t+1) - \widehat{r}(t+1) + \lambda (\Theta^\star - \Theta^\star_{(N)}) (\Theta^\star + \Theta^\star_{(N)}) \notag \\  
% & - (S(t+1) - \lambda \Theta^\star)^\top \big[ (M(P(t+1)))^{-1} - (M(\widehat{P}(t+1)))^{-1} \big] (S(t+1)-\lambda \Theta^\star) \notag \\ 
% & - \big[ S(t+1) - \widehat{S}(t+1) - \lambda (\Theta^\star - \Theta_{(N)}^\star ) \big] 
%  (M(\widehat{P}(t+1)))^{-1} 
%  \cdot 
% \\
% \notag
% & \qquad
% \big[ S(t+1) + \widehat{S}(t+1) - \lambda (\Theta^\star + \Theta_{(N)}^\star ) \big] , \notag \\ 
% %%% 
% & r(T) - \widehat{r}(T) = \sum_{i=1}^N (w_i^\star - 1/N) \sum_{j=1}^{|\mathcal{D}_i|} |y^i_j|^2 . \notag  
% \end{align} 
% Inductively, we have  
% \allowdisplaybreaks\begin{align} 
%   r(0) - \widehat{r}(0)  
% = &   r(T) - \widehat{r}(T) + T \lambda (\Theta^\star - \Theta^\star_{(N)}) (\Theta^\star + \Theta^\star_{(N)})   \notag \\  
%  & - \sum_{t=1}^T (S(t) - \lambda \Theta^\star)^\top \big[ (M(P(t)))^{-1} - (M(\widehat{P}(t)))^{-1} \big] (S(t)-\lambda \Theta^\star)   \notag  \\  
% %%% 
% &  - \sum_{t=1}^T \big[ S(t) - \widehat{S}(t) - \lambda (\Theta^\star - \Theta_{(N)}^\star ) \big] 
%  (M(\widehat{P}(t)))^{-1} \big[ S(t) + \widehat{S}(t) - \lambda (\Theta^\star + \Theta_{(N)}^\star ) \big] . \notag 
% \end{align}
% By Lemma~\ref{lm:|AB|<=|A||B|}, we have 
% \allowdisplaybreaks\begin{align} 
%  & | r(0) - \widehat{r}(0) | \leq |r(T) - \widehat{r}(T)| 
%   + T \lambda | \Theta^\star - \Theta^\star_{(N)} | \cdot | \Theta^\star + \Theta^\star_{(N)} |   \notag \\ 
% &  + \sum_{t=1}^T  \big| (M(P(t)))^{-1} - (M(\widehat{P}(t)))^{-1} \big| \cdot 
%  \big| S(t)-\lambda \Theta^\star \big|^2   \notag  \\  
% %%% 
% &  + \sum_{t=1}^T \big[ | S(t) - \widehat{S}(t) | + \lambda | \Theta^\star - \Theta_{(N)}^\star | \big] \cdot 
%  \big| (M(\widehat{P}(t)))^{-1} \big| \cdot \big| S(t) + \widehat{S}(t) - \lambda (\Theta^\star + \Theta_{(N)}^\star ) \big| .  \label{estrw(0)-tilder1/N(0)}  
% \end{align}
% Then the estimate \eqref{eqn:estrw-tilder1/N} follows from 
% \eqref{estrw(0)-tilder1/N(0)}, \eqref{estMPw-MP1/N}, 
% \eqref{sup|S-hatS|est}, and Remark~\ref{rmk:M(hatP)bdd}. 
% \end{proof}

%     \begin{proof}[{Proof of Theorem~\ref{thrm:Epsilon_Efficiency}}]
%         Under Assumptions~\ref{assm:bddxy} and~\ref{assm:PD}, the existence of the regret-optimal algorithm $\theta_{\cdot}$ is implied by Theorem~\ref{thm:RegretOptimal_Dynamics}.  The first claim follows from Proposition~\ref{prop:stabilityaw-a1/N} upon noting that the constant ``$C_w$'' therein is bounded as a function of $w$; whence we take the constant $C$ hidden by $\mathcal{O}$ to be $C\eqdef \sup_{w\in [0,1]^N\,\sum_{i=1}^N\,w_i=1}\, C_w$.  Likewise, the second statement follows directly from Corollary~\ref{cor:stabilityLast} upon defining the constant hidden by $\mathcal{O}$ as before.  
%     \end{proof}



% Further investigation of the ``symmetrized system'' \eqref{eqnhatP1/N(t)} reveals a symmetric form of $\widehat{P}$, which suggests that  $\widehat{P}$ can be decomposed into homogeneous submatrices of lower dimensions. 
% Specifically, if we decompose the high dimensional $Np\times Np$ matrix $\widehat{P}$ into $N\times N$ submatrices of dimensions $p\times p$ each,  and either exchange two submatrices symmetrically positioned with respect to the diagonal of $\widehat{P}$ or exchange two submatrices on the diagonal, the system \eqref{eqnhatP1/N(t)} is invariant. 
% This suggests that all the submatrices on the diagonal are homogeneous and all the off-diagonal submatrices are homogeneous.
% %%%%%%%%%%
% \begin{proposition}[Symmetries in $\widehat{P}$] 
% \label{prop:P1/Nsubmat}
% The solution of \eqref{eqnhatP1/N(t)} has the following submatrix decomposition  
% \begin{align} 
%  \widehat{P} = \begin{bmatrix} \pi_1 & \pi_2 & \cdots & \pi_2 \\ 
%  \pi_2 & \pi_1 & \cdots &\pi_2 \\ 
% \vdots & \vdots & \ddots & \vdots \\ 
%  \pi_2 & \pi_2 & \cdots & \pi_1 
%  \end{bmatrix} \in \mathbb{R}^{Np\times Np}, 
% \quad \pi_1 \in \mathbb{R}^{p\times p}, \quad 
% \pi_2 \in \mathbb{R}^{p\times p} , 
% \label{hatPpi12}
% \end{align} 
% and the submatrices $\pi_1$ and $\pi_2$ are uniquely determined by the system   
% \allowdisplaybreaks\begin{align}  
% \begin{cases}
%   \pi_1(t) =  \beta I_p - \beta^2 \gamma_1(t+1)  ,  
% \label{eqnpi1pi2}  \\ 
%    \pi_2(t) =  - \beta^2 \gamma_2(t+1) ,  \quad 1\leq t \leq T-1 , \\
%  \pi_1(T) = \pi_2(T) = (1/N^3)\sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|} u^i_j u^{i\top}_j ,   
% \end{cases} 
% \end{align}
% where $\gamma_1(\cdot)$ and $\gamma_2(\cdot)$ are defined as 
% \eqref{gamma1} and \eqref{gamma2}. 
% \end{proposition} 


% We argue analogously to \cite[Lemmata 1]{huang2021linear} in deriving the following submatrix decomposition of $\widehat{P}$. 
% \begin{proof}[{Proof of Proposition~\ref{prop:P1/Nsubmat}}]
% We decompose the $Np\times Np$ identity matrix into $N\times N$ submatrices
% $I=(I_{ij})_{1\leq i, j \leq N}$ with each 
% $I_{ij}\in \mathbb{R}^{p\times p}$.  
% For each $1\leq i, j \leq N$, by $E_{ij} $we denote the $Np\times Np$ elementary matrix by exchanging the $i$th and $j$th rows of submatrices of the $Np\times Np$ identity matrix $I=(I_{ij})_{1\leq i, j \leq N}$. Note that $E_{ij}=E_{ij}^{-1}=E_{ij}^T$. 
% Multiplying both sides of \eqref{eqnP(t)} from the left by $E_{ij}$ and from the right by $E_{ij}$, we obtain  
% \allowdisplaybreaks\begin{align} 
% & \begin{cases}
%    E_{ij} \widehat{P}(t) E_{ij}  
% =  \beta I_{Np} - \beta^2 [(\lambda+\beta ) I_{Np} + E_{ij} \widehat{P}(t+1) E_{ij} ]^{-1} ,  \\ 
%   E_{ij} \widehat{P}(T) E_{ij} =  [ (1/N) I_p ,\cdots, (1/N) I_p ]^\top 
%  \Big( \sum_{i=1}^N \frac{1}{N} \sum_{j=1}^{|\mathcal{D}_i|}  u^i_j u^{i\top}_j  \Big)  
%  [ (1/N) I_p , \cdots, (1/N) I_p ] .   
% \end{cases}   \label{eqnEijtildePEij}
% \end{align} 
% Comparing \eqref{eqnEijtildePEij} and \eqref{eqnhatP1/N(t)} reveals that 
%  $\widehat{P}(t)$ and $E_{ij} \widehat{P}(t) E_{ij}$ satisfy the same ODE for all $1\leq i, j \leq N$. This observation implies that 
% \allowdisplaybreaks\begin{align} 
%  \widehat{P}_{ii} = \widehat{P}_{jj}, \quad \widehat{P}_{ij} = \widehat{P}_{ji} , \quad \widehat{P}_{ik}= \widehat{P}_{jk}, \quad 
% \widehat{P}_{ki} = \widehat{P}_{kj}, \quad \forall 1\leq i, j \leq N, \quad \forall k \neq i, j , \notag 
% \end{align} 
% and the first assertion of the proposition is proved. 


% Since $\widehat{P}$ takes the form \eqref{hatPpi12}, 
% it is straight forward to verify that $[(\lambda+\beta)I_{Np} + \widehat{P}]^{-1}$ takes the form 
% \allowdisplaybreaks\begin{align} 
%  [(\lambda+\beta) I_{Np} + \widehat{P}]^{-1} = \begin{bmatrix} \gamma_1 & \gamma_2 & \cdots & \gamma_2 \\ 
%  \gamma_2 & \gamma_1 & \cdots &\gamma_2 \\ 
% \vdots & \vdots & \ddots & \vdots \\ 
%  \gamma_2 & \gamma_2 & \cdots & \gamma_1 
%  \end{bmatrix} , \label{[(lambda+1)I+P]inv}
% \end{align} 
% with $\gamma_1$ and $\gamma_2$ given by \eqref{gamma1} and \eqref{gamma2}. 

% We substitute \eqref{hatPpi12} and \eqref{[(lambda+1)I+P]inv} into \eqref{eqnhatP1/N(t)} to obtain the equations \eqref{eqnpi1pi2}.  
% \end{proof}

% Upon substituting $\widehat{P}$  into \eqref{eqnhatS1/N(t)}, we find that the $Np\times 1$ matrix $\widehat{S}$ can be decomposed into homogeneous submatrices of dimensions $p\times 1$ each.  
% \begin{proposition} \label{prop:SubmatrixReduction}
% The solution of \eqref{eqnhatS1/N(t)} can be decomposed into submatrices 
% \begin{align} 
% \widehat{S}=(\pi_3^\top, \cdots, \pi_3^\top )^\top \in \mathbb{R}^{Np\times 1}, 
% \quad \pi_3 \in \mathbb{R}^{p\times 1} , 
% \label{hatSpi3}
% \end{align} 
% and $\pi_3$ satisfies
% \allowdisplaybreaks\begin{align} 
% \begin{cases}
%   \pi_3(t) = \beta \big[ \gamma_1(t+1) + (N-1) \gamma_2(t+1)  \big] 
%   ( \pi_3(t+1) - \lambda \theta^\star_{(N)} )   , \\   
%  \pi_3(T) = - (1/N^2) \sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|}  u^i_j y^i_j . 
% \end{cases}   \label{eqnpi3}
% \end{align} 
% \end{proposition}

% \begin{proof}[{Proof of Proposition~\ref{prop:SubmatrixReduction}}]
% We multiply both sides of \eqref{eqnhatS1/N(t)} from the left by $E_{ij}$ defined in the proof of Proposition \ref{prop:P1/Nsubmat}, 
% \allowdisplaybreaks\begin{align} 
%  E_{ij} \widehat{S}(t) = &  E_{ij} \beta [(\lambda + \beta )I_{Np} + \widehat{P}(t+1)]^{-1} (\widehat{S}(t+1) - \lambda \Theta^\star_{(N)})
% \notag \\ 
% = &    E_{ij} \beta [(\lambda + \beta )I_{Np} + \widehat{P}(t+1)]^{-1} E_{ij} E_{ij}(\widehat{S}(t+1) - \lambda \Theta^\star_{(N)}) \notag \\ 
% = &    \beta [(\lambda + \beta )I_{Np} + E_{ij} \widehat{P}(t+1)E_{ij}]^{-1}  ( E_{ij}\widehat{S}(t+1) - \lambda \Theta^\star_{(N)}) 
% \label{EijtildeS1/N(t)}
% \end{align}
% and 
% \allowdisplaybreaks\begin{align} 
%   E_{ij}\widehat{S}(T) = &  - E_{ij}[ (1/N) I_p, \cdots, (1/N) I_p ]^\top \sum_{i=1}^N \frac{1}{N} \sum_{j=1}^{|\mathcal{D}_i|}  u^i_j y^i_j \notag \\ 
% = &  - [ (1/N) I_p, \cdots, (1/N) I_p ]^\top \sum_{i=1}^N \frac{1}{N} \sum_{j=1}^{|\mathcal{D}_i|}  u^i_j y^i_j .   
% \label{EijtildeS1/N(T)} 
% \end{align}
% From \eqref{EijtildeS1/N(t)} and \eqref{EijtildeS1/N(t)}, we have that $E_{ij}\widehat{S}$ also satisfies \eqref{eqnhatS1/N(t)} for all 
% $1\leq i, j \leq N$. This proves that all submatrices of $\widehat{S}=(\widehat{S}_i)_{1\leq i \leq N}$ are equal on $0\leq t \leq T$. 
% We further substitute \eqref{hatPpi12}, \eqref{[(lambda+1)I+P]inv} and 
% $\widehat{S} = [\pi_3^\top, \cdots, \pi_3^\top]^\top$ into \eqref{eqnhatS1/N(t)} to obtain \eqref{eqnpi3}. 
% \end{proof} 



% \begin{corollary} 
% \label{cor:ComplexityAlgorithm__Heuristic}
% Fix a data set $\mathcal{D}$ and assume that \eqref{eq:moredatasets_than_dataperdataset} holds. Then the computational complexity of computing the sequence $\big( \theta(t) \big)_{t=0}^T$ by \eqref{hata} is 
% $\mathcal{O}(Tp^2 \max\{N, p^{0.373}\})$. 
% %$\mathcal{O}(TNp\max\{N,p\}))$. 
% \end{corollary}

% \begin{proof}[{Proof of Corollary~\ref{cor:ComplexityAlgorithm__Heuristic}}]
% \hfill\\ 
% \noindent \textbf{Complexity of computing $\pi_1(T)$, $\pi_2(T)$, and $\pi_3(T)$ is $O(N^2 p^2)$} \\ 
% Computing $u^i_j u^{i\top}_j$ has complexity $O(p^2)$ by Lemma~\ref{lm:matCompComplexity}-(iii) and computing the sum\\
% $\sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|} u^i_j u^{i\top}_j$ has a complexity of $O( N^2 p^2)$ by Lemma~\ref{lm:matCompComplexity}-(i). 
% Moreover, multiplying the $p\times p$ matrix $\sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|} u^i_j u^{i\top}_j$ by the scalar $1/N^3$ has complexity $O(p^2)$. Hence the computing $\pi_1(T)$ and $\pi_2(T)$ has complexity $\mathcal{O}(N^2 p^2)$. 
% Computing the product $u^i_j y^i_j$ has a complexity of $O(p)$ by Lemma~\ref{lm:matCompComplexity}-(iii), and summing $\sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|} u^i_j y^i_j$ has complexity $O(N^2 p)$ by Lemma~\ref{lm:matCompComplexity}-(i). Multiplying the $p\times 1$ vector $\sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|} u^i_j y^i_j$
% by the scalar $1/N^2$ has a complexity of $O(p)$. 
% Therefore computing $\pi_3(T)$ has complexity $O(N^2 p)$, and the complexity of computing $\pi_1(T)$, $\pi_2(T)$, and $\pi_3(T)$ is $\mathcal{O}(N^2 p)$.  

% \noindent\textbf{Complexity of Computing $\gamma_1(T)$ and $\gamma_2(T)$ is $O(p^{2.373})$} 
% \\
% With $\pi_1(T)$ and $\pi_2(T)$ obtained, we can compute $\gamma_1(T)$ and $\gamma_2(T)$ by \eqref{gamma1} and \eqref{gamma2}.  
% From \eqref{gamma1} and \eqref{gamma2}, computing $\gamma_1(\cdot)$ and $\gamma_2(\cdot)$ from $\pi_1(\cdot)$ and $\pi_2(\cdot)$ involves multiplication and addition of $p \times p$ matrices, scalar multiplication of $p\times p$-dimensional matrices, multiplication of a $p\times p$ matrix and a $p\times 1$ vector, and inversion of a $p \times p$ matrix. 
% By Lemma~\ref{lm:matCompComplexity}, multiplication of two $p\times p$ matrices has the dominant complexity of $\mathcal{O}(p^{2.373})$ among the above matrix operations. 
% Moreover, inverting a $p\times p$ matrix has complexity $\mathcal{O}(p^{2,373})$. 
% Hence, computing $\gamma_1(T)$ and $\gamma_2(T)$ has a complexity of $O(p^{2.373})$. 
% %\Anastasis{@Xuwei, multiplication of two \textit{square} $p\times p$ matrices has $\mathcal{O}(p^{2.373})$ complexity}.



% \noindent \textbf{Complexity of computing $\pi_1(t)$, $\pi_2(t)$, $\pi_3(t)$, $\gamma_1(t)$ and $\gamma_2(t)$ for $t=T-1$, $T-2$, ..., $1$ has complexity $\mathcal{O}(T p^{2.373})$.}
% \\ 
% %For each $t=T-1$, $T-2$, ..., $1$ fixed, suppose $\pi_1(t+1)$, $\pi_2(t+1)$, $\pi_3(t+1)$, $\gamma_1(t+1)$ and $\gamma_2(t+1)$ have been obtained. 
% Similar to computing $\gamma_1(T)$ and $\gamma_2(T)$, computing $\gamma_1(t)$ and $\gamma_2(t)$ from $\pi_1(t+1)$ and $\pi_2(t+1)$ has complexity $\mathcal{O}(p^{2.373})$. 
% According to \eqref{eqnpi1pi2}, computing $\pi_1(t)$ and $\pi_2(t)$ from $\gamma_1(t+1)$ and $\gamma_2(t+1)$ involves scalar multiplication and addition along diagonal of $p\times p$ matrices, and therefore has complexity $O(p^2)$ by Lemma~\ref{lm:matCompComplexity}-(i) and (ii), 
% According to \eqref{eqnpi3}, computing $\pi_3(t)$ from $\gamma_1(t+1)$, $\gamma_2(t+1)$, and $\pi_3(t+1)$ involves scalar multiplication and addition of $p\times p$ matrices, scalar multiplication and addition of $p\times 1$ matrices, 
% and multiplication of a $p\times p$ matrix with a $p\times 1$ matrix. By Lemma~\ref{lm:matCompComplexity}, the dominant complexity of these operations is $\mathcal{O}(p^2)$.   
% Summing up the above argument, computing $\pi_1(t)$, $\pi_2(t)$, $\pi_3(t)$, $\gamma_1(t)$ and $\gamma_2(t)$ for each $t$ has a complexity of $\mathcal{O}(p^{2.373})$, and therefore has a complexity of $\mathcal{O}(T p^{2.373})$ for all $t=T-1$, $T-2$,..., $1$. 


% \noindent\textbf{The Cost of Computing Each $\Theta(t)$ is $O(Tp^2 \max\{N, p^{0.373}\})$.}
% \\
% By \eqref{Theta-simple}, the cost of updating from $\Theta(t)$ to $\Theta(t+1)$ is equal to the complexity of computing $\widehat{\boldsymbol{\alpha}}(t)=(\widehat{\alpha}_1^\top(t), \cdots \widehat{\alpha}_N^\top(t))^\top$ for $t=0, 1, ..., T-1$. 

% By \eqref{eq:RegretOptimizationHeuristic_Helper__1}, $\widehat\alpha_i(t)$ for all $i=1$, ..., $N$ share the common term 
% \allowdisplaybreaks 
% \begin{align} 
%  & - \big\{ \gamma_1(t+1) \pi_2(t+1) + \gamma_2(t+1) [ \lambda I_p + \pi_1(t+1) + (N-2)\pi_2(t+1) ] \big\} \sum_{k=1}^N \theta_k(t) 
%  \notag \\ 
%  & - \big[ \gamma_1(t+1) + (N-1) \gamma_2(t+1) \big] (\pi_3(t+1) - \lambda \theta^\star_{(N)}) ,  \notag 
% \end{align} 
% and computing the common term involves matrix multiplication, addition, and scalar multiplication of $p\times p$ matrices, 
% matrix addition and scalar multiplication of $p\times 1$ matrices, 
% and multiplication of a $p\times p$ matrix and a $p\times 1$ matrix.  
% By Lemma~\ref{lm:matCompComplexity}, these operations have complexity $O(Np + p^{2.373})$, where $Np$ is due to adding the $N$ $p$-dimensional vectors $\sum_{k=1}^N \theta_k(t)$, and $p^{2.373}$ is due to multiplication of two $p\times p$ matrices by a CW-like algorithm. 


% Computing the individual terms 
% \allowdisplaybreaks
% \begin{align} 
%  - (\gamma_1(t+1) - \gamma_2(t+1) ) (\lambda I_p + \pi_1(t+1) - \pi_2(t+1) ) \theta_i(t) \notag 
% \end{align} 
% for $\widehat\alpha_i(t)$, $i=1$, ..., $N$ involves addition, scalar multiplication, and matrix multiplication of $p\times p$ matrices, and multiplication of a $p\times p$ matrix and a $p\times 1$ matrix. 
% By Lemma~\ref{lm:matCompComplexity}, these operations have complexity of $\mathcal{O}(p^{2.373} + Np)$, where $p^{2.373}$ is due to multiplication of two $p\times p$ matrices by a CW-like algorithm and $Np$ is due to multiplying a $p\times p$ matrix by the $p$-dimensional vector $\theta_i(t)$ for $i=1$, ..., $N$. 
% Hence the complexity of computing $\widehat{\boldsymbol{\alpha}}(t)$ for $t=0, 1, ..., T-1$ is $\mathcal{O}(T p^2\max\{N, p^{0.373} \} )$. 


% \noindent\textbf{The complexity of computing $(\Theta(t))_{t=0}^T$ is $\mathcal{O}(T p^2 \max\{N,p^{0.373}\})$} \\ 
% Looking over all computations involved, we deduce that the complexity of computing the sequence 
% $(\Theta(t))_{t=1}^T$ starting from $\Theta(0)=\Theta^\star$ has a complexity of $\mathcal{O}(T p^2 \max\{N,p^{0.373}\})$. 
% \end{proof}

% We may now deduce Theorem~\ref{thrm:accelertion_heuristic_regret_optimal_algorithm} and Theorem~\ref{thrm:regretoptimality_SymmetricCase}.  
% \begin{proof}[{Proof of Theorem~\ref{thrm:accelertion_heuristic_regret_optimal_algorithm}}]
%     The result directly follows from Theorem~\ref{thm:ComplexityAlgorithm} and Corollary~\ref{cor:ComplexityAlgorithm__Heuristic}.  
% \end{proof}


% \begin{proof}[{Proof of Theorem~\ref{thrm:regretoptimality_SymmetricCase}}]
% Direct consequence of Propositions~\ref{prop:P1/Nsubmat} and~\ref{prop:SubmatrixReduction}.
% \end{proof}







% \section{Background}
% \label{s:Background}
% In this paper, we consider regret-optimal memoryless training dynamics for \textit{\textbf{f}inite-rank \textbf{k}ernel \textbf{r}idge \textbf{r}egressors} (fKRR) trained from $N$ finite datasets drawn from $N$ (possibly) different data-generating distributions.
% We are considering a scenario in which these datasets can originate from $N$ distinct tasks or be adversarially generated perturbations of the initial dataset, and we aim for our fKRR to exhibit robustness towards them.

% Any continuous \textit{feature map} $\phi:\mathbb{R}^d\rightarrow \mathbb{R}^p$, induces a hypothesis of fKRR $f_{\theta}:\mathbb{R}^d\rightarrow \mathbb{R}$ each of which is uniquely determined by a \textit{trainable parameter} $\theta\in \mathbb{R}^p$ via
% \begin{equation}
% \label{eq:FRKR 1}
% f_{\theta}(x)=\phi(x)^\top\theta;
% \end{equation}
% where all vectors are represented as column-vectors and not row vectors.

% The hypothesis class $\mathcal{H}$ possesses a natural reproducing kernel Hilbert space (RKHS) structure with inner-product given for $f_{\theta},f_{\tilde{\theta}}\in \mathcal{H}$ by $\langle f_{\theta},f_{\tilde{\theta}}\rangle_{\phi}\eqdef \sum_{k=1}^p\, \theta_k\tilde{\theta}_k$.  This RKHS structure suggests an optimal selection criterion to decide which hypothesis in $\mathcal{H}$ best describes a \textit{single} training set $\mathcal{D}_1\eqdef \{(x^1_j,y^1_j)\}_{j=1}^{S^1}$ of $S^1\in \mathbb{N}_+$, by solving the penalized least-squares problem

% \begin{align} 
% \label{eq:FRKR 2}
%  \theta^\star_1 \in \argmin_{\theta \in \mathbb{R}^p } \big\| \Phi(x^1) \theta  - y^1  \big\|_2^2 
%   + \kappa \big\| \theta \big\|_2^2 , 
% \end{align} 
% where 
% \begin{align} 
% \Phi(x^1) \eqdef 
% \big( \phi(x^1_1), \ 
% \phi(x^1_2), \ \cdots , \ 
%  \phi(x^1_{S^1}) \big)^\top \in \mathbb{R}^{S^1 \times p} , \ 
% y^1 \eqdef (y^1_1, y^1_2, \cdots, y^1_{S^1})^\top 
%  \in \mathbb{R}^{S^1} , \notag  
% \end{align} 
% and $\kappa>0$ is a fixed hyperparameter.  In this classical case, the Representer Theorem \cite{KimeldorfWahba__Representer_OriginalI,KimeldorfWahba__Representer_OriginalII} states that the optimal choice of $f_{\theta}$ to the convex optimization problem~\eqref{eq:FRKR 2} is parameterized by
% \begin{equation} 
% \label{eq:loss_one_dataset}
%  \theta^\star_1 = 
%  ( \Phi^\top(x^1) \Phi(x^1)  
%   + \kappa I_p )^{-1} 
%   \Phi^\top(x^1) y^1 ,
% \end{equation} 
% Alternatively, the optimal parameter choice $\theta^\star_1$ can be arrived at via \textit{gradient descent} since~\eqref{eq:FRKR 2} has a strictly convex loss with a Lipschitz gradient.
% The training of fKRR on a single dataset is very-well understood.  Likewise, other aspects of fKRR are well understood; namely, their statistical properties \cite{KRRExactTestError}, their in-sample behaviour in \cite{amini2022target}, and even the approximation power and risk of randomly generated fKRR are respectively known \cite{gonon2022approximation} and \cite{gonon2020risk}.

% Using the fKRR \eqref{eq:FRKR 1}, the joint terminal time objective \eqref{eq:terminal_time_objective} simplifies to
% \allowdisplaybreaks\begin{align} 
% \label{eq:terminal_time_objective__fKRR}
% \begin{aligned}
%         l(\theta_1,\dots,\theta_N, w;\,\mathcal{D} )  
%     \eqdef & 
%         \sum_{i=1}^N 
%         w_i
%         \biggl(
%             \sum_{j=1}^{S_i} 
%                 \big| 
%                 \langle 
%                     u^i_j
%                     ,
%                     \theta^{w}
%                 \rangle - y^i_j  \big|^2 
%         \biggr)
%     \\
%     % \,\,
%     \mbox{ s.t. }
%     \,%\,
%     \theta^w\eqdef & \sum_{i=1}^N \theta_i
%         w_i
%  ,
% \end{aligned}
% \end{align} 
% where $\langle\cdot,\cdot\rangle$ denotes the Euclidean inner-product, $u^i_j\eqdef \phi(x^i_j)$ and, as in~\eqref{eq:terminal_time_objective}, $w = (w_1, \cdots, w_N) \in [0,1]^N$ with $\sum_{i=1}^N\,w_i=1$.










% \end{document}



==> OLD/TMLRVersion.tex <==
% %%%%%%%% NeurIPS 2020 EXAMPLE LATEX SUBMISSION FILE %%%%%%%%%%%%%%%%%
% % \documentclass{article}
% % to avoid loading the natbib package, add option nonatbib:
% % \usepackage{Formatting/neurips_2020}

% %%%%%%%% ICML 2021 EXAMPLE LATEX SUBMISSION FILE %%%%%%%%%%%%%%%%%
% % \documentclass[preprint]{article}


% % \usepackage{xcolor} 
% % \usepackage{amsthm}
% % \usepackage{neurips_2020}

% % \documentclass[jair,twoside,11pt,theapa]{article}
% \documentclass[10pt]{article} % For LaTeX2e
% \usepackage{tmlr}

% % \usepackage{jair, theapa, rawfonts}
% \usepackage{svg}
% \usepackage{csvsimple}

% % \jairheading{1}{1993}{1-15}{6/91}{9/91}
% % \ShortHeadings{Regret-Optimal Federated Transfer Learning - KRR}{Yang, Kratsios, Krach, Grasselli, \& Lucchi}
% \title{Regret-Optimal Federated Transfer Learning for Kernel Regressions – with Applications in American Option Pricing}
% % \title{Regret-Optimal Transfer Learning \add{from Pretrained} Kernel Regressors -- with Applications to American Option Pricing}


% % Authors must not appear in the submitted version. They should be hidden
% % as long as the tmlr package is used without the [accepted] or [preprint] options.
% % Non-anonymous submissions will be rejected without review.

% \author{\name Xuwei Yang \email yangx212@mcmaster.ca \\
%       \addr Department of Mathematics\\
%       McMaster University
%       \AND
%       \name Anastasis Kratsios \email kratsioa@mcmaster.ca \\
%       \addr Department of Mathematics\\
%       McMaster University and Vector Institute
%       \AND
%       \name Florian Krach \email florian.krach@math.ethz.ch\\
%       \addr Department of Mathematics\\
%       ETH Z\"{u}rich
%       \AND Matheus Grasselli \email grassel@mcmaster.ca\\
%       \addr Department of Mathematics\\
%       McMaster University
%        \AND Aurelien Lucchi \email aurelien.lucchi@unibas.ch\\
%     \addr Department of Mathematics and Informatics\\
%       University of Basel}


% % \def\month{MM}  % Insert correct month for camera-ready version
% % \def\year{YYYY} % Insert correct year for camera-ready version
% % \def\openreview{\url{https://openreview.net/forum?id=XXXX}} % Insert correct link to OpenReview for camera-ready version

% \usepackage{amsthm}
% \newtheorem{proposition}{Proposition}%[section]
% \newtheorem{lemma}{Lemma}%[section]
% \newtheorem{definition}{Definition}%[section]
% \newtheorem{theorem}{Theorem}%[section]
% \newtheorem{remark}{Remark}%[section] 
% \newtheorem{assumption}{Assumption} 
% \newtheorem{corollary}{Corollary}
% \newtheorem{experiment}{Experiment}


% \newcommand{\com}[1]{{\color{orange}{#1}}}


% %To display labels in the PDF. Comment at the end!
% % Code
% \usepackage{algpseudocode}
% \usepackage[linesnumbered,lined,boxed,commentsnumbered,ruled,longend]{algorithm2e}
%     \RestyleAlgo{ruled}
% \newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
% \SetCommentSty{mycommfont}

% % TABLE Formatting
% \raggedbottom
% \newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
% % \setlength\heavyrulewidth{0.3ex}
% \usepackage{lscape}



% % Packages and Macros
% \input{Formatting/macros}
% % For Annotating + Commenting
% \input{Formatting/comment}

% % Code link:
% \newcommand{\code}{%
%     %\url{https://github.com/FlorianKrach/RegretOptimalFederatedTransferLearning} %
%     \url{https://github.com/???}%
% }



% \begin{document}

% % \title{Regret-Optimal Federated Transfer Learning for Kernel Regression -- with Applications in American Option Pricing}

% % \author{\name Xuwei Yang \email yangx212@mcmaster.ca \\
% %        \name Anastasis Kratsios \email kratsioa@mcmaster.ca \\
% %         \name Florian Krach \email florian.krach@math.ethz.ch\\
% %         \name Matheus Grasselli \email grassel@mcmaster.ca\\
% %        \name Aurelien Lucchi \email aurelien.lucchi@unibas.ch}



% \maketitle

% \begin{abstract}
% Several pre-trained machine learning models operate by aggregating, fine-tuning, and adapting a (set of) models which have been pre-trained on a set of relevant tasks to any given novel task.  
% This paper exhibits a theoretically regret-optimal iterative scheme for performing this aggregation for pre-trained finite-rank kernel ridge regression models using a fixed and finite number of training iterations.
% % We propose an optimal iterative scheme for transfer learning, where a central planner has access to datasets ${\cal D}_1,\dots,{\cal D}_N$ for the same learning model $f_{\theta}$.
% % Our objective is to minimize the cumulative deviation of the generated parameters $\{\theta_i(t)\}_{t=0}^T$ across all $T$ iterations from the specialized parameters $\theta^\star_{1},\ldots,\theta^\star_N$ obtained for each dataset while respecting the loss function for the model $f_{\theta(T)}$ produced by the algorithm upon halting.  
% % We only allow for continual communication between each of the specialized models (nodes/agents) and the central planner (server) at each iteration (round).  For the case where the model $f_{\theta}$ is a finite-rank kernel regression, we derive explicit updates for the regret-optimal algorithm.  
% We investigate the properties of our algorithm, including its computational complexity and its adversarial robustness.  We show that an adversary which perturbs $q$ training pairs by at most $\varepsilon>0$, across all training sets, cannot reduce the regret-optimal algorithm's regret by more than $\mathcal{O}(\varepsilon q \bar{N}^{1/2})$, where $\bar{N}$ is the aggregate number of training pairs. 
% Additionally, by leveraging symmetries within the regret-optimal algorithm, we further develop a nearly regret-optimal heuristic that runs with $\mathcal{O}(Np^2)$ fewer elementary operations, where $p$ is the dimension of the parameter space and $N$ is the total number of training instances.  
% To validate our theoretical findings, we conduct numerical experiments in the context of American option pricing, utilizing a randomly generated finite-rank kernel. 
% \end{abstract}

% % Intro
% \section{Introduction}
% \label{s:Intro}

% %% Motivation
% A core challenge in machine learning is identifying a set of parameters that optimize the performance of a learning model on a single dataset $\mathcal{D}_1$ by empirical risk minimization.
% Often, especially in transfer learning, one does not have access to only a single dataset but \textit{several relevant datasets} $\mathcal{D}_1,\dots,\mathcal{D}_N$ whose data can be integrated into the training scheme. 
% Comparable datasets naturally arise in instances of meta-learning \citep{finn2017model,pavasovic2022mars}), in multi-task learning \citep{kumar2012learning,NEURIPS2020_3fe78a8a}, in quantitative finance due to natural market cycles \citep{lowry2002ipo}, or in robust finance approaches to model uncertainty resulting in several plausible stochastic time-series models wherewith data can be simulated \citep{hou2018robust,aksamit2019robust,prashanth2022wasserstein}.


% This paper considers the problem of optimally selecting a deterministic training algorithm which maximizes the performance of any given finite-rank kernel ridge regressor on a primary dataset $\mathcal{D}_1$ while incorporating the information present in $N$ \textit{pretrained} kernel ridge regressors, each trained on one of the datasets $\mathcal{D}_1,\dots,\mathcal{D}_N$.  
% %%%%
% The optimality of a training algorithm is quantified by minimizing a performance metric, the trajectory generated by the optimization algorithm after a fixed number $(T)$ of iterations.  

% We focus on the rich class of finite-rank kernel ridge regressor (fKRR) since they subsume all deep neural networks whose hidden layers have been pre-trained (or randomly generated) and frozen, and only the final linear layer can be trained on the relevant novel task; see e.g.~\cite{herrera2023optimal,gonon2021random}.  Furthermore, fKRRs are also known to provide analytically tractable approximations to the training dynamics of deep neural networks under certain conditions~\cite{jacot2018neural,jacot2020implicit,arora2019fine,bordelon2021spectrum}.

% %% Problem Formulation
% \subsection{Problem Formulation}
% Fix positive integers $d$, $N$, $p$, and $T$.
% A finite-rank kernel regressor is a map $f_{\theta}:\mathbb{R}^d\rightarrow \mathbb{R}$ which is linear in its trainable parameter%%
% \footnote{We emphasize that all vectors are represented as column vectors, not row vectors.} 
% %%%%%%
% $\theta\in \mathbb{R}^p$ but typically \textit{non-linear} in its inputs $x\in \mathbb{R}^d$ through
% a feature map $\phi:\mathbb{R}^d\rightarrow \mathbb{R}^p$
% \begin{equation}
% \label{eq:FRKR}
% f_{\theta}(x)=\phi(x)^\top\theta
% ;
% \end{equation}
% typically with $p\gg d$.  
% The kernel associated to $f$ is given by $\kappa(x,\tilde{x}) = \phi(x)^{\top}\phi(x)$.   One example would be a pre-trained deep neural network where only the final linear layer $\theta$ is fine-tuned and the frozen hidden layers define the feature map $\phi$; see Section~\ref{s:Experiments_n_Validation} for details.

% We are provided with $N$ non-empty datasets $\mathcal{D}_1,\dots,\mathcal{D}_N\subseteq \mathbb{R}^d\times \mathbb{R}$, of which $\mathcal{D}_1$ is distinguished as describing the principal (supervised) regression task.  
% Each of the $i=1,\dots,N$ pre-trained fKRRs $f_{\theta^n}$ optimizes their respective penalized empirical minimization problem defined over their respective dataset $\mathcal{D}_i$
% \begin{equation}
% \label{eq:Regression_Klassische0}
%     \inf_{\theta \in \Theta}\, 
%             \sum_{(x,y)\in \mathcal{D}_i}\,
%                 (f_\theta(x)-y)^2
%         +
%             \kappa \,
%                 \|\theta\|_2
% ;
% \end{equation}
% where the hyperparameter $\kappa > 0$ controls the regularity of the model by modulating the magnitude of Euclidean norm $\|\theta\|_2$ of its weight vector. 
% The minimizer $\theta_i^{\star}$ of~\eqref{eq:Regression_Klassische0} for each $i$ is called a \emph{finite-rank kernel ridge regressor} (fKRR) and is available in closed-form, see Appendix~\ref{s:Background}.
% % Other regularizers are available~\cite{VDG_Sara_HighDimenisonalGLMsandLassi_AnnStat,simon2013sparse,AdcockAnyiBrugiapaglia_2019_NumerischeMath}.  

% Fix a set of weights $w \in \Delta_N\eqdef \{[0,1]^N:\,\sum_{i=1}^N\,w_i=1\}$, to be optimized.  We extend the summed squared error (SSE) loss function in~\eqref{eq:Regression_Klassische0} in the case $n=1$ to incorporate the influence of other datasets into the primary regression task
% \allowdisplaybreaks\begin{align} 
% \label{eq:terminal_time_objective}
% \begin{aligned}
%         l(\Theta, w;\,\mathcal{D} )  
%     \eqdef 
%         \sum_{i=1}^N 
%         w_i
%             \sum_{j=1}^{|\mathcal{D}_i|} 
%                 (
%                 f_{\theta^w}(x_j^i)
%                 - y^i_j  
%                 )^2,
% \end{aligned}
% \end{align} 
% where $\Theta\eqdef (\theta_1^{\top}, \cdots, \theta_N^{\top})^\top\in \mathbb{R}^{Np \times 1}$ and $\theta^w\eqdef\sum_{i=1}^N w_i\,\theta_i$.  The optimal weights $w$ are selected in a PAC-Bayesian fashion, see~\cite{alquier2021user} for an overview of PAC-Bayesian bounds, in such a way that they prioritize the influence of datasets which are similar to $\mathcal{D}_1$ while automatically removing sufficiently different datasets.

% Since the optimizer of~\eqref{eq:terminal_time_objective} need not be available in closed-form, we must optimize it iteratively.  Upon fixing a maximal number of iterations $T$ and an initial parameter choice $\theta_0\in \mathbb{R}^p$, we follow~\cite{casgrain2021optimizing} and identify every deterministic training algorithm for~\eqref{eq:terminal_time_objective} with a sequence in $\mathbb{R}^{Np}$ of length $1+T$
% \begin{equation}
% \label{eq:algorithms}
%     \theta^{0\cdots T}\eqdef \left\{\theta(t)\right\}_{t=0}^T, 
%     \qquad 
%     \theta(0)=\theta_0
% .
% \end{equation}

% \paragraph{Regret Optimality}
% We seek the algorithms which aim to minimize~\eqref{eq:terminal_time_objective} while biasing their iterates towards the parameters $\theta_1^{\star},\dots,\theta_N^{\star}$ which are optimal for the pre-trained models, weighted by $w$.  To this end, minimize the following \textit{penalized regret functional} over the class of deterministic algorithms, i.e.\ of the form~\eqref{eq:algorithms},
% \begin{equation}
% \label{eq:penalized_regret_functional__REGRETFORM}
% \begin{aligned}
%     \mathcal{R}(\Theta^{0\cdots T})
% \eqdef &
%         \underbrace{
%         l (\Theta(T), w;\,\mathcal{D} ) 
%         }_{\text{Prediction}}
%     -
%                   \,\,  l^{\star}
%     +
%         \sum_{t=0}^{T-1}  
%         \,
%              \big(
%                     \underbrace{
%                         \lambda \left\| \Theta(t+1) - \Theta^\star \right\|_2^2    
%                     }_{\text{Transfer Learning}}
%                 + 
%                     \underbrace{
%                         \beta  \left\| \Delta \Theta(t) \right\|_2^2 
%                     }_{\text{Algo.\ Stability}}
%                 \big) 
%     ,
% \end{aligned}
% \end{equation} 
% where $\Theta^\star\eqdef (\theta_1^{\star \top}, \cdots, \theta_N^{\star\top})^\top \in \mathbb{R}^{Np \times 1}$ records the optimal parameters of each pretrained fKRR, $\Delta \Theta(t)\eqdef \Theta(t+1)-\Theta(t)$ quantifies the magnitude of each training update, and $
%         l^{\star}
%     \eqdef 
%         \min_{\Xi \in \mathbb{R}^{Np\times 1}}\, 
%             l(\Xi,w; \mathcal{D})
% $ is the minimal value of the loss function~\eqref{eq:terminal_time_objective}.  
% Thus, the formulation of regret in~\eqref{eq:penalized_regret_functional__REGRETFORM} is \textit{specific to the setting of training a fKRR from multiple datasets}.  The first term \textit{(prediction)} in~\eqref{eq:penalized_regret_functional__REGRETFORM} emphasizes that any ``good'' optimization algorithm must minimize the regression loss function~\eqref{eq:terminal_time_objective}.  The second term \textit{(transfer learning)} encodes the degree to which an optimization algorithm encodes information from similar datasets into its iterates.  Finally, the third (algo.\ stability) term biases towards algorithms whose iterative updates do not change too rapidly, similar to controlling the learning rate in gradient descent.  
% A game theoretic interpretation of $\mathcal{R}$ is given in Appendix~\ref{s:GameTheoreticInterpretation}.

% The primary objective of this paper is to exhibit a \textit{regret optimal optimization algorithm}, meaning a sequence $\Theta^{0\dots T}$ minimizing $\mathcal{R}$ across all deterministic algorithms with $T$ iterations; i.e.\ all elements of $\mathbb{R}^{(1+T)Np}$.  Further, our objective is to explicitly establish the existence of a regret-optimal algorithm, i.e.\ the algorithm minimizing~\eqref{eq:penalized_regret_functional__REGRETFORM}, and to investigate its theoretical properties such as adversarial robustness and computational complexity.




% \subsection{Contributions}
% \label{s:Introduction_Contrib}
% We exhibit a \textit{regret optimal} algorithm, by which we mean an optimizer of~\eqref{eq:penalized_regret_functional__REGRETFORM}.
% % when $f_{\theta}:\mathbb{R}^d\rightarrow \mathbb{R}$ is linear in its trainable parameter%%
% % \footnote{We emphasize that all vectors are represented as column-vectors and not row vectors.} %%
% % $\theta\in \mathbb{R}^p$ but non-linear in its inputs $x\in \mathbb{R}^d$ through
% % a feature map $\phi:\mathbb{R}^d\rightarrow \mathbb{R}^p$, typically with $p\gg d$, namely 
% % \begin{equation}
% % \label{eq:FRKR}
% % f_{\theta}(x)=\phi(x)^\top\theta.
% % \end{equation}
% % In this case, $f_\theta$ is called a \emph{finite-rank kernel ridge regressor} (fKRR) and a closed-form solution to the ridge-regression problem \eqref{eq:Regression_Klassische1} exists and is given by \eqref{eq:loss_one_dataset} in Appendix~\ref{s:Background}.
% Aligned with the recent trends in optimization \cite{casgrain2019latent,JMLR:v18:17-653}, we leverage techniques from optimal control theory to characterize the regret-optimal algorithm.  We show that this is possible due to the observation that minimizers of~\eqref{eq:penalized_regret_functional__REGRETFORM} coincide with the minimizers of the energy functional 
% \allowdisplaybreaks\begin{align} 
% \label{eq:penalized_regret_functional}
%     {\cal L}(\Theta^{0\cdots T})
% \eqdef &
%     \underbrace{
%         \sum_{t=0}^{T-1}  
%         \,
%              \left[  
%                     \lambda \left\| \Theta(t+1) - \Theta^\star \right\|_2^2    
%                 + 
%                     \beta \left\| \Delta \Theta(t) \right\|_2^2 
%             \right] 
%     }_{\text{
%         Running-Cost
%     }}
%     + 
%     \underbrace{
%         l (\Theta(T), w;\,\mathcal{D} ) 
%     }_{\text{
%     Terminal Cost
%     }}
% .
% \end{align} 
% From this control-theoretic perspective, every algorithm~\eqref{eq:algorithms} can be regarded as driven by a ``control'', and the functional ${\cal L}$ has the form of a ``cost function'' of an optimal control problem,  decomposable into the sum of a ``running/operational cost'' and a ``terminal/objective cost''.  This allows us to leverage tools from optimal control \citep{touzi2013optimal} to derive a  closed-form expression of the unique regret-optimal algorithm driven by the unique ``optimal control'' as defined in Algorithm~\ref{alg:RegretOptimization}.  

% We prove that this procedure is adversarially robust, meaning that the value of~\eqref{eq:penalized_regret_functional} varies by $\mathcal{O}(\varepsilon \sqrt{\bar{N}}q)$ if a malicious adversary can perturb at most $1/q$ percent of all the data in each of the dataset $\mathcal{D}_i$ by at-most $\varepsilon\ge 0$, where $\bar{N}=\sum_{i=1}^N |\mathcal{D}_i|$.  
% Furthermore, we show that our regret-optimal algorithm has a computational complexity of $\mathcal{O}(N^2p^3 + T\,(Np)^{2.373})$.  
% Moreover, we characterize the optimal choice of the weights $w$ 
% % defining~\eqref{eq:terminal_time_objective} 
% which the central planner must use to maximize the selected model's performance on the primary/focal dataset $\mathcal{D}_1$.  

% Finally, we show that if all the datasets $\mathcal{D}_1$, $\dots$, $\mathcal{D}_N$ are equally dissimilar (but not necessarily similar) then the regret-optimal algorithm can be accelerated.  This acceleration requires $\mathcal{O}(N\,p^2)$ fewer elementary operations.  We also show that if this ``accelerated'' algorithm is used in situations when the datasets differ by a little, then it does not deviate far from the regret-optimal algorithm.  Thus, it is an accelerated heuristic.  

% We emphasize that this problem has not previously been studied.  Therefore, there are no available benchmarks for the proposed algorithm.  Hence, our numerical experiments consist of ablation studies where the proposed models are benchmarked against various natural alternatives to the regret-optimal algorithm.

% \subsection*{Outline}   
% The paper is organized as follows. In Section~\ref{s:Main}, we introduce the regret-optimal algorithm and demonstrate the optimality, computational complexity, and adversarial robustness of the algorithm. We  further introduce an accelerated algorithm of lower computational complexity that can achieve near-regret optimality. 
% In Section~\ref{s:Experiments_n_Validation}, we conduct a convergence analysis of the regret-optimal algorithm and compare it to the standard gradient descent approach. Then we show the transfer learning capabilities of the algorithm for American option pricing.  

% A game theoretic interpretation of $\mathcal{R}$ is given in Appendix~\ref{s:GameTheoreticInterpretation}. Appendix~\ref{s:Proofs_TechnicalLemmata} is devoted to proving the optimality, adversarial robustness, and computational complexity of the regret-optimal algorithm. The near-regret optimality and computational complexity of the accelerated algorithm are also proven. Appendix~\ref{s:Background} briefly introduces the background of finite-rank kernel ridge regressors.   


% \subsection{Related Work}
% \label{s:Introduction__sss:RelatedWork}

% Examples of $f_\theta$ of the form \eqref{eq:FRKR} include extreme learning machine \citep{gonon2020risk,gonon2022approximation,ghorbani2022linearized,MeiMontanari_CommPaAMath_2022__DoubleDescent} or any finite-rank kernel ridge regressor (fKRR) \citep{Amini_2021_EJS_SpectrallyTruncatedKernel,amini2022target}.  Random feature models, and finite-rank ridge regressors, are typical in contemporary quantitative finance \citep{gonon2021random,herrera2023optimal} or reservoir computing \citep{cuchiero2021discrete}, where it is favourable to rapidly deploy a deep learning model due to time or computing-power limitations/constraints.  Finite-rank kernel ridge regressors are also typical in the setting of standard transfer \citep{howard2018universal} and multi-task learning \citep{ren2018cross,jia2019leveraging} pipelines where one often has a pre-trained deep neural network model and, for any novel task, the user freezes the hidden layers in the deep neural network model and only fine-tunes/trains the deep neural network's final linear layer.  
% This is useful, since the hidden layers of most deep neural network architectures are known to process general, cruder features and the final layer of any such model captures finer, task-specific features \citep{zeiler2014visualizing,yosinski2014transferable}.


% The optimization of a model trained from multiple data sources lies at the heart of multi-task learning.  In  \cite{SenerKoltun_MultiTaskLEarningMultiObjectiveOptimization__NeurIPS2018}, the authors cast the task of optimizing~\eqref{eq:terminal_time_objective} as a multi-objective optimization problem.  They propose to solve it via a multi-gradient descent algorithm which, under mild conditions, converges to a Pareto stationary point; i.e.\ which is essentially a critical point of each of the $i$-th player's penalized SSE.  
% Though iterative schemes for multi-objective optimization can efficiently reach critical points \citep{fliege2019complexity}, this problem's critical point is not necessarily a minimum since the problem~\eqref{eq:terminal_time_objective} is not convex when $w$ is shared amongst all $N$ players.  

% This proposed algorithm reflects the ideas of the federated stochastic gradient descent (FedSGD) algorithm of \cite{SINGHZHU_FedSGD_2018} and of its online counterpart FedOGD which is an online federated version of online gradient descent\footnote{See \cite[Chapter 3]{hazan2016introduction} for details on online gradient descent} and more efficient online versions thereof such as \cite{kwon2022tighter}.  From the federated learning perspective, the problem of training individual fKRR on each dataset, and then centralizing them by optimizing the mixing parameter $w$ in~\eqref{eq:terminal_time_objective} and its origins date back to local gradient descent introduced in the optimization and control literature in \cite{Mangasarian_1995_localGD}.  Though several authors (e.g. \cite{TighterTheoryLocalSGD}) have proposed various progressive improvements of federated gradient-descent-type algorithms for training a learner from several data sources, the problem of studying \textit{the} most efficient iterative federated learning algorithm for regret minimization has not yet been tackled.  

% We note that (stochastic) optimal control tools have revealed new insights into machine learning.  Examples include an optimal step-size control \citep{li2017stochastic} and batch-size control \citep{zhao2022batch}, developing online subgradient methods that adapt to the data's observed geometry \citep{DuchiHazanSinger_2011_JMLR_adaptiveSGOnlineOptim}, developing new maximum principle-based training algorithms for deep neural networks \citep{JMLR:v18:17-653}, or unifying (stochastic) optimization frameworks \citep{Casgrain_LatentVarStochOptim_2019}.

% \subsection*{Notation}
% We briefly introduce some additional notation.
% Each dataset has a finite number of samples which we write as $\mathcal{D}_i = \{ (x_j^i, y_j^i) \, | \, 1 \leq j \leq |\mathcal{D}_i| \}$. We assume that some feature map $\phi$ is fixed and denote the features of each sample of $\mathcal{D}_i$ as 
% $$u_j^i \eqdef \phi(x_j^i).$$ 
% Moreover, we denote the joint inputs and outputs for each dataset as 
% \begin{align}
%     X^i \eqdef \left( x^i_1, \cdots , x^i_{|\mathcal{D}_i|} \right)^\top \in \mathbb{R}^{|\mathcal{D}_i| \times d} \quad \text{ and } \quad
%     Y^i \eqdef (y^i_1, \cdots, y^i_{|\mathcal{D}_i|})^\top \in \R^{|\mathcal{D}_i|}, \notag 
% \end{align}
% and the joint features as
% \begin{align} 
% U^i \eqdef \Phi(X^i) \eqdef 
% \left( \phi(x^i_1), \cdots , \ 
%  \phi(x^i_{|\mathcal{D}_i|}) \right)^\top \in \mathbb{R}^{|\mathcal{D}_i| \times p}. \notag  
% \end{align} 
% Finally, we use $I_p$ to denote a $p\times p$ identity matrix. 

% \section{Main Results}
% \label{s:Main}

% This section contains the description of the \textit{unique} regret-optimal algorithm and an analysis of its theoretical properties. Throughout our manuscript, we maintain the following two assumptions.  
% \begin{assumption}[$\mathcal{D}$-Boundedness]
% \label{assm:bddxy} 
% There are constants $K_x,K_y>0$ such that all 
% $(x^i_j, y^i_j) \in \mathcal{D}$ satisfy $\|u^i_j\|_2 \leq K_x$ and $|y^i_j|^2 \leq K_y$, where $u^i_j = \phi (x^i_j)$. 
% \end{assumption}
% % \begin{assumption}[$\mathcal{D}$-Boundedness]
% % \label{assm:bddxy} 
% % There are constants $K_x,K_y>0$ such that all 
% % $(u^i_j, y^i_j) \in \cup_{i=1}^N \mathcal{D}_i$ are norm-bounded
% % $\|u^i_j\|_2 \leq K_x$ and $\|y^i_j\|_2 \leq K_y$. 
% % \end{assumption}
% \begin{assumption}[$(w^{\star},\mathcal{D})$-Compatibility]
% \label{assm:PD}
% The data ${\cal D} = \cup_{i=1}^N\,\mathcal{D}_i$ and the weights $w^{\star}$ satisfy 
% \allowdisplaybreaks
% \begin{align} 
%  & \sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|} u^i_j u^{i\top}_j \geq 0 , 
%  \label{Sum(uij)Tuij>=0}\\  
% & [w^\star_1 I_p ,\cdots, w^\star_N I_p]^{\top} 
%  \left( \sum_{i=1}^N
%  w^\star_i \,
%  \sum_{j=1}^{|\mathcal{D}_i|}  u^i_j u^{i\top}_j \right)  
%  [ w^\star_1 I_p, \cdots, w^\star_N I_p ] \geq 0 . 
%  \label{WeightedSum(uij)Tuij>=0}
%  \end{align} 
% \end{assumption}
% With the notation introduced before, the 
% object $[w_1^\star I_p, \cdots, w_N^\star I_p ]$ above is a $p \times Np$ matrix.



% \subsection{The Algorithms}
% \label{s:Main_ss:Algorithm}

% \begin{figure}[H]%[ht!]%
%     \centering
%      \begin{subfigure}[b]{0.45\textwidth}
%      \centering
%         \includegraphics[width=0.75\textwidth]{Graphics/Information_Sharing.pdf}
%     \caption{Step 1: Adaptive ``Prior'' Sharing: The $i^{th}$ dataset $\mathcal{D}_i$ is shared with the main dataset $\mathcal{D}_1$ if the best model $f_{\theta^\star_i}$, optimizing~\eqref{eq:Regression_Klassische1} on dataset $\mathcal{D}_i$, can outperform the optimal model trained on the main dataset, up to a slack factor $\eta>0$.  The relative importance of each dataset is proportional to $f_{\theta^\star_i}$'s performance relative to the training performance of the best model trained on the main dataset.
%     When $\eta$ is small, sharing is unlikely; when $\eta$ is large, nearly all datasets are pooled together with approximately the same relative importance.}
%         \label{fig:information_sharing_prior}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.45\textwidth}
%          \includegraphics[width=0.6\textwidth]{Graphics/Information_Sharing_inhomogeneous.pdf}
%     \caption{Step 2: Optimized ``Posterior'' Sharing: We then optimize the relative importance/weights given to the shared datasets from the naive adaptive sharing.  The optimization is a closed-form update of the adaptive ``prior'' weights which optimize a certain maximum expected performance criterion subject to a relative entropy penalization against the weights obtained from adaptive prior sharing.}
%     \label{fig:information_sharing_posterior}
%      \end{subfigure}
%     \caption{Visual Summary of Optimal Information Sharing (Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart}).}
%     \label{fig:information_sharing}
% \end{figure}

% We begin by describing our procedure for determining the optimal mixture weights defining the cooperative objective function \eqref{eq:terminal_time_objective} used in ~\eqref{eq:penalized_regret_functional__REGRETFORM}.  This procedure is illustrated graphically in Figure~\ref{fig:information_sharing} and detailed in Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart}.   


% \begin{algorithm}[ht!]%[H]%
% \caption{{Optimal Information Sharing - Initialization to Algorithm~\ref{alg:RegretOptimization}}}
% %\label{alg:RegretOptimization}
% \label{alg:RegretOptimizationHeuristic__WarmStart}
% \begin{algorithmic}
% \SetAlgoLined
% \Require Datasets $\mathcal{D}_1,\dots,\mathcal{D}_N$, finite-rank kernel $\phi$, hyperparameters\footnote{Different ridge hyperparameters $\kappa$ can be used to define each regressor in Algorithm ~\ref{alg:RegretOptimizationHeuristic__WarmStart}} $\kappa,\eta>0$.
% \DontPrintSemicolon
%     \State \tcp{Initialize Locally-Optimal Learners and Record Scores on Main Dataset}  
%     %\tcc{Initialize Locally-Optimal Learners and Record Scores on Main Dataset} 
%     \State \SetKwBlock{ForParallel}{For $i:1,\dots,N$ in parallel}{end}
%         \ForParallel{\State 
%         $\theta^\star_i \leftarrow  
%  ( \Phi^\top(X^i) \Phi(X^i)  
%   + \kappa I_p )^{-1} 
%   \Phi^\top(X^i) Y^i$ 
%             \tcp*{Optimize each fKRR}
%         \State $s^i
%             \leftarrow  
%         \frac1{|\mathcal{D}_1|}\sum_{j=1}^{|\mathcal{D}_1|}\,
%                 \big\|
%                         f_{\theta^\star_i}(u_j^1)
%                     -  y_j^1
%                 \big\|_2^2
%         $
%         % \State 
%         \tcp*{Score predictive power of fKRR on main dataset}
%         } 
%         \State \tcp{Get Adaptive Prior} 
%         \State \SetKwBlock{ForParallel}{For $i:1,\dots,N$ in parallel}{end} 
%         \ForParallel{\State $
%             w_i
%                 \leftarrow 
%             \frac{   
%                 [s^1+\eta-s^i]_+
%             }{ \sum_{j=1}^N\, [s^1+\eta-s^j]_+ }
%         $}
%         \State \tcp{Get Optimized Posterior} 
% \State \SetKwBlock{ForParallel}{For $i:1,\dots,N$ in parallel}{end} 
%         \ForParallel{\State $
%             w^\star_i
%                 \leftarrow 
%             \frac{
%                     e^{
%                     s_i/\eta
%                 }   
%                 \,
%                 [s^1+\eta-s^i]_+
%             }{
%                 \sum_{j=1}^N\,
%                     e^{s_j/\eta}[s^1+\eta-s^j]_+
%             }
%         $}
%     \State \Return Optimal Weights $w^\star$ and Locally-Optimal fKRR Parameters $\theta^\star_1,\dots,\theta^\star_N$.
% \end{algorithmic}
% \end{algorithm}

% \vspace{0.2in}

% Suppose now that we have used Algorithm \ref{alg:RegretOptimizationHeuristic__WarmStart} to compute weights $w^\star=(w^\star_1, \cdots, w^\star_N)$ and the locally optimal fKRR parameters $\theta^\star_1$, ..., $\theta^\star_N$, and $w^{\star}$. The key novelty in the next algorithm follows a similar spirit to \cite{JMLR_MaximumBasedDL_LiChenTaiCheng} and \cite{casgrain2021optimizing}, by casting the problem of constructing a regret-optimal algorithm as an optimal control problem. 

% As before, denote 
% \allowdisplaybreaks\begin{align} 
%  & \Theta(t)\eqdef [ \theta_1^{\top}(t), \cdots, \theta_N^{\top}(t) ]^{\top}, \quad 
%  \Theta^\star \eqdef [ \theta^{\star \top}_1, \cdots, \theta^{\star \top}_N ]^{\top} , 
%  \notag \\ 
%  & \boldsymbol\alpha(t) \eqdef [\alpha_1^{\top}(t), \cdots, \alpha_N^{\top}(t)]^{\top}, \notag   
% \end{align} 
% which are all elements of $\R^{Np}$, and introduce the dynamics that $\Theta$ follows    \allowdisplaybreaks\begin{align} 
% & \Theta(0)=\Theta^\star, 
% \quad 
% \Theta(t+1) = \Theta(t) + \boldsymbol\alpha(t) , 
% \quad 0\leq t \leq T-1 ,   
% \label{Theta-simple}  
% \end{align} 
% which is equivalently written as   \allowdisplaybreaks\begin{align} 
%  \Theta(t+1) = \Theta^\star + \sum_{u=0}^{t} \boldsymbol\alpha(u) , \quad 0\leq t \leq 
%   T-1 . 
% \label{Theta(t)Theta(0)} 
% \end{align}

% Then, since the optimizers of the energy~\eqref{eq:penalized_regret_functional} coincide with the optimizers of the systemic regret functional~\eqref{eq:penalized_regret_functional__REGRETFORM}, searching for a regret-optimal algorithm reduces to solving for an optimal control $\mathbf{\alpha}$ to minimize the cost 
% \eqref{eq:penalized_regret_functional} subject to \eqref{Theta-simple}.  
% The optimal control problem 
% \eqref{eq:penalized_regret_functional} and \eqref{Theta-simple} is a discrete-time linear quadratic optimal control problem, and can be solved by dynamic programming methods that are standard in the literature. For instance, by \cite[Proposition 5.1]{BO1998}, we obtain the solution for the regret-optimal algorithm in closed-form as solutions of a system of Riccati equations \eqref{eqnP(t) 0} and \eqref{eqnS(t) 0}, given in
% Theorem~\ref{thm:RegretOptimal_Dynamics__MainTextFormulation}. 

% Algorithm~\ref{alg:RegretOptimization} below implements the optimal control approach in two steps. In Step 1, we solve the equation system \eqref{eqnP(t) 0} and \eqref{eqnS(t) 0} backwards for $t=T$, $T-1$, ..., $1$. Then in Step 2, we obtain the optimal control $\boldsymbol\alpha(t)$ and update the parameter $\Theta(t)$ for $t=0$, $1$, ... $T$. 

% %by Algorithm~\ref{alg:RegretOptimization}.
% \begin{algorithm}[ht]%[H]
% \caption{Regret-Optimal Optimization Algorithm}
% \label{alg:RegretOptimization}
% \begin{algorithmic}
% \SetAlgoLined
% \Require Datasets $\mathcal{D}_1,\dots,\mathcal{D}_N$, $N$.\ Iterations $T\in \mathbb{N}_+$, finite-rank kernel $\phi$ and hyperparameters $\lambda, \beta, \kappa, \eta >0$.
% \DontPrintSemicolon
%     \State 
%     \tcp{Get Initialize Weights and Locally-Optimal fKRR Parameters}
%     %%%% Externalized
%         \State $\theta^\star_1,\dots,\theta^\star_N,w^{\star}$ $\leftarrow$ Run: Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart} with $\mathcal{D}_1,\dots,\mathcal{D}_N$, $\phi$, and $\kappa,\eta$.
   
%     \State 
%     \tcp{Initialize Updates}
%     \State $P(T) 
%     = [w_1^\star I_p , \cdots, w_N^\star I_p ]^\top \left(\sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|}  u^i_j u_j^{i\top}\right) [w_1^\star I_p, \cdots, w_N^\star I_p ] $ 

% \State $S(T) = -[w_1^\star I_p , \cdots, w_N^\star I_p ]^\top \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|}  u^i_j y^i_j$ 

% \State $\Theta(0) = \Theta^\star \eqdef (\theta_1^{\star \top}, \cdots, \theta_N^{\star \top} )^\top$ 

%     \State \tcp{Generate Iterates}
%     \State \For{$t=T-1,\dots,1$}{
%         \State \tcp{Update Driving Parameters} 

% \State $P(t)= \beta I_{Np} - \beta^2 [(\lambda+\beta)I_{Np} + P(t+1)]^{-1}$

% \State $S(t) = \beta [(\lambda + \beta )I_{Np} + P(t+1)]^{-1} (S(t+1) - \lambda \Theta^\star)$
% }


% \State\For{$t=0, ..., T-1$}{
%   \State\tcp{Update Control} 

% \State 
% $\boldsymbol{\alpha}(t) = -[(\lambda+\beta )I_{Np} + P(t+1)]^{-1} 
% [(\lambda I_{Np} + P(t+1))\Theta(t) - \lambda \Theta^\star + S(t+1) ]$

% \State 
% $\Theta(t+1)=\Theta(t)+\boldsymbol{\alpha}(t)$
% }

% \State \Return Return the Optimized fKRR $f_{\theta^{w^\star}}$
% \end{algorithmic}
% \end{algorithm} 

% In the next subsections, we state our primary results, whose proofs are presented in Appendix \ref{s:Proofs_TechnicalLemmata}. We first quantify the optimality of Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart}. Next, we establish the optimality, complexity, and adversarial robustness of Algorithm~\ref{alg:RegretOptimization}.  

% \subsection{{Properties of Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart}}}
% \label{s:Main_Algorithm_2}

% By decoupling the optimization of the ``dataset-relevant weights'' $w$ in Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart} from the optimization of the parameter $\theta$ in Algorithm ~\ref{alg:RegretOptimization}, we avoid open-loop forward-backward iterations, which iterate between optimizing $w$ and $\theta$.  We now study the optimality of the weight $w^{\star}$ generated by Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart}.  The weights $w^{\star}$ represent the optimal probability distributions of randomly selecting amongst the $N$ optimized regressors $\{ f_{\theta^\star_i} \}_{i=1}^N$, each optimized locally on their dataset $\mathcal{D}_i$ by solving~\eqref{eq:Regression_Klassische1}.  Here, optimality is quantified in terms of the best-expected prediction on the focal dataset $\mathcal{D}_1$ subject to a penalty for deviating too far from a reference distribution.  This reference distribution serves to automatically delete models whose datasets are too dissimilar to $\mathcal{D}_1$.  Inspired by most meta-learning problems, e.g. \cite{pavasovic2022mars}, similarity is quantified by extracting a ``similarity score'' from each learner.  


% Let $\mathcal{P}(\{\theta^\star_i\}_{i=1}^N)$ consist of all probability measures on the set $\{\theta^\star_i \}_{i=1}^N$.  Any probability measure $\mathbb{P}_w$ in $\mathcal{P}(\{\theta^\star_ i\}_{i=1}^N)$ is uniquely determined by a weight $w$ in the $N$-simplex; consisting of all $w\in [0,1]^N$ whose entries sum to $1$.  Let $\theta$ be a random variable with law $\mathbb{P}_{w}$, for some $\mathbb{P}_w\in \mathcal{P}(\{\theta^\star_i \}_{i=1}^N)$.  The average performance of the random learner $f_{\theta}$ on the dataset $\mathcal{D}_1$ is
% \begin{equation}
% \label{eq:optimizingQ}
%     \mathbb{E}_{\theta \sim \mathbb{P}_w}\,
%         \left[
%             \frac1{|\mathcal{D}_1|}\sum_{j=1}^{|\mathcal{D}_1|}\,
%             \big\|
%                     f_{\theta}(u_j^1)
%                 -
%                     y_j^1
%             \big\|_2^2
%         \right]
%     =
%         \sum_{i=1}^N\,
%             w_i
%             %%% Score
%             \underbrace{
%             \biggl[
%                 \frac1{|\mathcal{D}_1|}\sum_{j=1}^{|\mathcal{D}_1|}\,
%                 \big\|
%                         f_{\theta^\star_i}(u_j^1)
%                     -
%                         y_j^1
%                 \big\|_2^2
%             \biggl]
%             }_{i^{th} \mbox{ learner's score }(s_i)} .
% \end{equation}


% Fix an \textit{information sharing level} $ \eta > 0$.  The information sharing level $\eta$ adaptively determines which of the datasets in $\mathcal{D}$ are implicitly shared with the principle dataset $\mathcal{D}_1$.  The information sharing is formalized through the probability measure 
% \[
% \bar{\mathbb{P}}^{\eta}(\theta^\star_i) \eqdef 
% \frac{
% [s^1+\eta -s^i]_+
% }{
% \sum_{i=1}^N\, [s^1 + \eta - s^i]_+
% }
% .
% \]
% on the set of $N$ learners, or equivalently on the parameters $\theta^\star_1,\dots,\theta^\star_N$.  
% The measure $\bar{\mathbb{P}}^{\eta}$ thus allows us to minimize the regularized version of the loss in~\eqref{eq:optimizingQ},
% \begin{equation}
% \label{eq:optimizingQ__regularized}
%     \min_{
%         \mathbb{P}_w
%     }
%     \,
%     \,
%     \underbrace{
%     \mathbb{E}_{\theta \sim \mathbb{P}_w}\biggl[
%         % \Big[
%             \frac1{|\mathcal{D}_1|}\sum_{j=1}^{|\mathcal{D}_1|}\,
%             % w_i\,
%             \big\|
%                     f_{\theta}(u_j^1)
%                 -
%                     y_j^1
%             \big\|_2^2
%     \biggr]
%     }_{i^{th} \mbox{ learner's score }(s_i)}
%     +
%     \underbrace{
%         % (1-\eta)
%         \eta\,
%         \operatorname{D}_{\operatorname{KL}}\big(
%             \mathbb{P}_w
%         \|
%             \bar{\mathbb{P}}^{\eta}
%         \big)
%     }_{
%     \underset{\mbox{information sharing}}{\mbox{Inhomogeneity of}}
%     }
% ,
% \end{equation}
% where the infimum is taken over all $\mathbb{P}_w$ in $\mathcal{P}(\{\theta^\star_i\}_{i=1}^N)$ and  $\operatorname{D}_{\operatorname{KL}}$ denotes the \textit{Kulbeck-Leibler divergence with respect to $\bar{P}^{\eta}$} given for any probability measure $\mathbb{P}_w$ on $\{\theta^\star_i\}_{i=1}^N$, namely 
% \[
%         \operatorname{D}_{\operatorname{KL}}\big(\mathbb{P}_w\| \bar{\mathbb{P}}^{\eta})
%     \eqdef 
%         % \begin{cases}
%             \sum_{i=1}^N\,
%                 w_i\,
%                 % \Biggl(
%                     \log\biggl(
%                         % \sum_{j=1}^N\,[s^1+\eta-s^j]_+
%                         \frac{w_i}{
%                         [s^1+\eta-s^i]_+
%                         }
%                         % \Big)
%                     % +
%                     % \log\big(
%                         % \sum_{j=1}^N\,[s^1+\eta-s^j]_+
%                         C_{\eta}
%                     % \big)
%                     \biggr)
%                 % \Biggr)
%         %         & \mbox{ if } \mathbb{P}\ll \mathbb{Q} \\
%         %     \infty & \mbox{ otherwise } 
%         % \end{cases}
% ,
% \]
% where $C_{\eta}\eqdef  \sum_{j=1}^N\,[s^1+\eta-s^j]_+$, if $\mathbb{P}_w$ is absolutely continuous with respect to $\bar{\mathbb{P}}^{\eta}$ and otherwise $\operatorname{D}_{\operatorname{KL}}\big(\mathbb{P}_w\| \bar{\mathbb{P}}^{\eta})=\infty$.  
% There is a unique probability measure optimizing the penalized functional~\eqref{eq:optimizingQ__regularized} determined by the weight $w^{\star}$ in Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart}.
% %%
% %%
% %%
% \begin{theorem}[Optimality of Weights $w^{\star}$ in Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart}]
% \label{prop:Optimal_Bayes_Weighting}
% Fix $\eta>0$.  The unique weights $w^{\star}_i$ on the $N$-simplex minimizing~\eqref{eq:optimizingQ__regularized} are given by 
% \begin{equation}
% \label{eq:prop:Optimal_Bayes_Weighting__OptimalWeights}
% \begin{aligned}
%     w^{\star}_i
% = 
%         \frac{
%                 e^{
%                 s^i/\eta
%             }   
%             \,
%             [s^1+\eta-s^i]_+
%         }{
%             \sum_{j=1}^N\,
%                 e^{s^j/\eta}[s^1+\eta-s^j]_+
%         }
% , \qquad  i=1,\dots,N.
% \end{aligned}
% \end{equation}

% \end{theorem}


% \subsection{Guarantees for Algorithm~\ref{alg:RegretOptimization}}
% \label{s:GuaranteesTheoretical__ss:Algo_1}



% %Our first result shows that Algorithm~\ref{alg:RegretOptimizationHeuristic}, and its iterates, are near-regret optimal.  Moreover, the degree of near-optimality depends only on the data, through the mixing parameter $w^{\star}$.  

% Our next result shows that Algorithm~\ref{alg:RegretOptimization}, and its iterates, are regret-optimal. 

% \begin{theorem}[Algorithm~\ref{alg:RegretOptimization} Computes the Unique Regret-Optimal Algorithm]
% \label{thm:RegretOptimal_Dynamics__MainTextFormulation}
% Suppose that Assumptions~\ref{assm:bddxy} and~\ref{assm:PD} hold and fix $\Theta^{\star}\in \mathbb{R}^{N\,p}$ as in \eqref{Theta_star}.  Then, the systemic regret functional $\mathcal{R}$ defined in~\eqref{eq:penalized_regret_functional__REGRETFORM} admits a unique minimizer $\hat\Theta_{\cdot}\eqdef (\hat\Theta(t))_{t=0}^T$ of the form~\eqref{Theta-simple__nocontrol} with $\hat\Theta(0) = \Theta^{\star}$ aand increments
% \allowdisplaybreaks\begin{align} 
%  \Delta \hat\Theta(t)  
%  = & -[(\lambda + \beta )I_{Np} + P(t+1)]^{-1} 
%  \big[ (\lambda I_{Np} + P(t+1)) \hat\Theta(t) 
%  - \lambda  \Theta^\star + S(t+1)  \big] ,   \label{optimala 0} 
% \end{align} 
% where, for $t=1,\dots,T$,  the matrices $P(t)$ and $S(t)$ in \eqref{optimala 0} are determined by
% \allowdisplaybreaks\begin{align} 
% & \begin{cases}
%  P(T) =  [w^\star_1 I_p ,\cdots, w^\star_N I_p]^{\top} 
%  \left( \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|}   u^i_j u^{i\top}_j \right)  
%  [ w^\star_1 I_p, \cdots, w^\star_N I_p] \\
%    P(t)  =  \beta I_{Np} - \beta^2 [(\lambda+\beta) I_{Np} + P(t+1) ]^{-1}  \label{eqnP(t) 0} 
% \end{cases},   \\
% %%%  
% & \begin{cases}
%  S(T) =  - [ w^\star_1 I_p, \cdots, w^\star_N I_p]^{\top} \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|}  {u^i_j} y^i_j \\
%   S(t) =  \beta \big[ (\lambda+\beta)I_{Np} + P(t+1) \big]^{-1} (S(t+1) - \lambda \Theta^\star )
%   \label{eqnS(t) 0}    
% \end{cases} .
% %\begin{align} 
% \end{align} 
% In particular, for each $t=0,\dots,T-1$ 
% \[
%         \Delta \hat\Theta(t) 
%     = 
%         \boldsymbol{\alpha}(t)
% ,
% \]
% where $\boldsymbol{\alpha}$ is as in Algorithm~\ref{alg:RegretOptimization}. 
% \end{theorem}
% \begin{remark}
%     Instead of the sums we can equivalently use our matrix notation to write $\sum_{j=1}^{|\mathcal{D}_i|} u^i_j u^{i\top}_j = {U^i}^\top U^i$ and $\sum_{j=1}^{|\mathcal{D}_i|}  {u^i_j} y^i_j = U^{i\top} Y^i$. 
% \end{remark}

% The explicit update rules for the regret-optimal optimization algorithm presented above permit us to compute its complexity.  Since we will be assuming that we work with \textit{floating-point arithmetic}, all elementary arithmetic operations (e.g.\ addition, subtraction, multiplication) are of constant (i.e.\ $\mathcal{O}(1)$) complexity.  We are most interested in the regime where the number of datasets is much larger than the typical number of instances/data per dataset; i.e.\ when
% \begin{equation}
% \label{eq:moredatasets_than_dataperdataset}
%         \frac1{N}\sum_{i=1}^N\,|\mathcal{D}_i| 
%     \le 
%         N
% .
% \end{equation}
% %%
% %%%
% %% 
% \begin{theorem}[Complexity of Regret-Optimal Algorithm]
% %\label{cor:ComplexityAlgorithm}
% \label{thm:ComplexityAlgorithm}
% In the setting of Theorem~\ref{thm:RegretOptimal_Dynamics__MainTextFormulation}, the computational complexity\footnote{We emphasize that we have assumed that computational complexity of all elementary arithmetic operations (e.g.\ addition, subtraction, multiplication) is $\mathcal{O}(1)$.} of computing the sequence $(\hat \Theta(t))_{t=0}^T$ defining the regret-optimal algorithm is $
%     \mathcal{O}\big( N^2 p^3 +
%         T
%         \, 
%         (Np)^{2.373}
%         %N^{2.373}\, p^2
%     \big)
% .
% $
% \end{theorem}




% Next, we quantify the sensitivity of Algorithm~\ref{alg:RegretOptimization} to adversarial attacks.  We study the robustness of Algorithm~\ref{alg:RegretOptimization} with respect to a family of perturbations that switch a given percentage $0\le q\le 1$ of all training data by selecting fake data points at a distance of at-most $\varepsilon\ge 0$ for any perturbed datapoint.  Thus, for a fixed set of datasets 
% $\{ \mathcal{D}_i \}_{i=1}^N$, and $q,\varepsilon$ as above, 
% we define the class $\mathbb{D}^{q,\varepsilon}$ of \textit{adversarially generated datasets} of ``magnitude'' $(q,\varepsilon)$ as all sets of datasets 
% $\{ \widetilde{\mathcal{D}}_i \}_{i=1}^N$, $\widetilde{\mathcal{D}}_i=\{ \{(\tilde{x}^i_j,\tilde{y}^i_j) \, | \, 1 \leq j \leq |\mathcal{D}_i| \}\subseteq \mathbb{R}^{d}\times \mathbb{R}$ satisfying Assumptions~\ref{assm:bddxy} and~\ref{assm:PD}, as well as
% % we define the class $\mathbb{D}^{q,\varepsilon}\subseteq \mathbb{R}^{d}\times \mathbb{R}^d$ of \textit{adversarially generated datasets} of ``magnitude'' $(q,\varepsilon)$ as all sets of datasets $\widetilde{\mathcal{D}}=\{ \{(\tilde{x}^i_j,\tilde{y}^i_j) \, | \, 1 \leq j \leq |\mathcal{D}_i| \} \, | \, 1 \leq i \leq N\}$ satisfying Assumptions~\ref{assm:bddxy} and~\ref{assm:PD}, as well as
% \[
%         %%%% Number of Perturbed Instances
%         \underbrace{
%                     \frac{
%                         \#\{
%                             (i,j):\, u^i_j\neq \tilde{u}^i_j \mbox{ or } y^i_j\neq \tilde{y}^i_j
%                         \}
%                     }{
%                         \sum_{i=1}^N\,|\mathcal{D}_i|
%                     }
%                 \le 
%                     q
%         }_{\mbox{Attack Persistence}}
%     \mbox{ and }
%             %%%% Maximum Magnitude of Adversarial Perturbations
%         \underbrace{
%                     \max_{i,j} \left\{ \,
%                         \max\left(
%                             \|u^i_j-\tilde{u}^i_j\|_2 
%                         ,
%                             |y^i_j-\tilde{y}^i_j|^2
%                         \right) \right\}
%                 \le 
%                     \varepsilon
%         }_{\mbox{Attack Severity}}
% ,
% \]
% where the indices $(i,j)$ run over $\{(i,j) \, | \, 1 \leq i \leq N,\,1 \leq j \leq |\mathcal{D}_i|\}$ and $\tilde{u}^i_j\eqdef \phi(\tilde{x}^i_j)$.

% In view of Theorem~\ref{thm:RegretOptimal_Dynamics__MainTextFormulation}, the updates of the unique regret-optimal algorithm $\hat \Theta^{0\cdots T}$ are determined by the sequence $\boldsymbol{\alpha}_{\cdot}\eqdef (\boldsymbol{\alpha}(t))_{t=0}^T$ computed by Algorithm~\ref{alg:RegretOptimization}.  It is convenient to emphasize this connection on $\boldsymbol{\alpha}_{\cdot}$ and the connection with the dataset $\mathcal{D}$ when expressing the following theorem, with the energy~\eqref{eq:penalized_regret_functional} determining the value of the systematic regret functional $\mathcal{R}$.  We therefore write $
%     {\cal L}(\boldsymbol{\alpha};\mathcal{D})
%         \eqdef 
%     {\cal L}(\hat\Theta^{0\cdots T})
% .$
% \begin{theorem}[Adversarial Robustness]
% \label{thrm:adv_robust}
% Fix a $\mathcal{D}$ satisfying Assumptions~\ref{assm:bddxy} and~\ref{assm:PD}.  For any level of ``attack persistence'' $0\le q\le 1$ and any degree of ``attack severity'' $\varepsilon\ge 0$ we have that
% \[
%         \big| {\cal L} (  \boldsymbol\alpha ; \mathcal{D} ) 
%         -  
%         {\cal L}(  \widetilde{\boldsymbol\alpha} ;  \widetilde{\mathcal{D}} )  \big|
%     \le 
%         \mathcal{O}\Big(
%             \varepsilon
%             \sqrt{\bar{N}\,q}
%         \Big)
% ,
% \]
% where 
% $\widetilde{\boldsymbol\alpha}$ is the output of Algorithm~\ref{alg:RegretOptimization} for any given adversarially-generated set of datasets 
% $\{ \widetilde{\mathcal{D}}_i \}_{i=1}^N\in \mathbb{D}^{q,\varepsilon}$ and $\bar{N}=\sum_{i=1}^N |\mathcal{D}_i|$.  Here $\mathcal{O}$ hides a constant depending only on Assumption~\ref{assm:bddxy}.  
% \end{theorem}



% \subsection{An Accelerated Heuristic}
% \label{s:Main__ss:AcceleratedHeuristic}
% We now discuss a situation in which the computational complexity of the regret-optimal algorithm can be reduced.  This is achieved by exploiting symmetries in the optimal policy computed by Algorithm~\ref{alg:RegretOptimization}.

% Examining the explicit update rules, we notice that \textit{if} the weights $w$ defining the energy~\eqref{eq:penalized_regret_functional} were to be $\overline{1/N}\eqdef (1/N,\dots,1/N)$ then the matrices defining the optimal policy/control's updates would become highly symmetric Toeplitz matrices, depending on exactly three $p$-dimensional block sub-matrices.  This allows us to parameterize the entire regret-optimal algorithm, for the sub-optimal weights $\overline{1/N}$, using only three low-dimensional systems whose dimension is \textit{independent} of the number of datasets $N$.  In line with this, Algorithm~\ref{alg:RegretOptimizationHeuristic} implements the regret-optimal algorithm for the weight specification $\overline{1/N}$ by only keeping track of these three optimal low-dimensional systems, and then efficiently recombining them by leveraging the Toeplitz structure defining the optimal policy/control.  These low-dimensional systems are defined using \textit{helper functions}, listed in equations \eqref{gamma1}-\eqref{eq:RegretOptimizationHeuristic_Helper__1}.

% The approximate near-optimality of Algorithm~\ref{alg:RegretOptimizationHeuristic} only depends on the stability of the optimal policy/control, defining the algorithm's updates as a function of the weights $w$.  If the optimal weights defining the systemic regret functional~\eqref{eq:penalized_regret_functional__REGRETFORM} are close to $\overline{1/N}$, then Algorithm~\ref{alg:RegretOptimizationHeuristic} is nearly regret-optimal.  Otherwise, the sub-optimality it incurs in favor of computational efficiency is explicitly quantifiable and depends only on the difference between the optimal weights computed in Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart} and the symmetric weights $\overline{1/N}$.


% Note now record, the matrix-valued functions $\gamma_1(\cdot)$ and $\gamma_2(\cdot)$ used to define the updates in Algorithm~\ref{alg:RegretOptimizationHeuristic}.  

% \begin{algorithm}[htp!]%
% \caption{Accelerated (Nearly) Regret-Optimal Algorithm}
% \label{alg:RegretOptimizationHeuristic}
% \begin{algorithmic}
% \SetAlgoLined
% \Require Datasets  $\mathcal{D}_1,\dots,\mathcal{D}_N$, $N$.\ Iterations $T\in \mathbb{N}_+$, finite-rank kernel $\phi$, hyperparameters $\lambda, \beta, \kappa, \eta >0$.
% \DontPrintSemicolon
%     \State  
% \tcp{Get Initialize Weights and Locally-Optimal fRKR Parameters}
%     %%%% Externalized
%        \State $\theta^\star_1,\dots,\theta^\star_N,w^{\star}$ $\leftarrow$ Run: Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart} with $\mathcal{D}_1,\dots,\mathcal{D}_N$, $\phi$, and $\kappa,\eta$.
%     \State 
%   \tcp{Initialize Updates}
%     \State $\pi_1(T) 
%     = \pi_2(T) 
%     = (1/N^3) \sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|}  u^i_j u^{i\top}_j$
%     \State $\pi_3(T) 
%     =  - (1/N^2) \sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|}  {u^i_j} y^i_j $
%  \State $\theta_1(0) = \theta^\star_1$, $\theta_2(0) = \theta^\star_2$, $\dots$, $\theta_N(0) =\theta^\star_N$
% \State $\theta^\star_{(N)} = \frac{1}{N} \sum_{i=1}^N \theta^\star_i .$
%     \State \tcp{Generate Iterates}
%     \State \For{$t=T-1,\dots,0$}{
%         \State \tcp{Update Low-Dimensional Driving Parameters} 

% \State$\pi_1(t)= \beta I_p- \beta^2 \gamma_1(t+1)$ 
% \tcp{$\gamma_1(\cdot)$ is defined by \eqref{gamma1}}

% \State $\pi_2(t) = - \beta^2 \gamma_2(t+1)$ 
% \tcp{$\gamma_2(\cdot)$ is defined by \eqref{gamma2}}

% \State $\pi_3(t)
% = \beta \big[ \gamma_1(t+1)
% + (N-1) \gamma_2(t+1)
% \big] ( \pi_3(t+1) -\lambda \theta^\star_{(N)})$ }

% \State\For{$t=0, ..., T-1$}{ 
%   \State \tcp{Update Low-Dimensional Control} 
%  \State \For{$i=1, ..., N$}{
%   \State $\widehat{\alpha}_i(t)
%   =  \widehat{\alpha}\big(\theta_i(t) ,\ 
%  (\theta_j(t))_{j = 1,j\neq i}^N ,\ (\gamma_i(t+1))_{i=1}^2, 
%    \ (\pi_i(t+1))_{i=1}^3 \big)$ 
   
%  \State $\theta_i(t+1) =\theta_i(t) + \widehat{\alpha}_i(t)$ } } 
 
%  \State \Return Synchronized fKRR 
% $f_{\theta^{w^\star}}$
% \end{algorithmic}
% \end{algorithm} 

% The matrix-valued functions $\gamma_1(\cdot)$ and $\gamma_2(\cdot)$ in Algorithm~\ref{alg:RegretOptimizationHeuristic} are defined as 
% \allowdisplaybreaks 
% \begin{align} 
% & \gamma_1(\cdot) \eqdef 
% \big\{ (\lambda+\beta )I_p
% +\pi_1(\cdot) \notag \\
% & \hspace{2cm} - (N-1) \pi_2(\cdot)\big[ (\lambda+ \beta )
% I_p + \pi_1(\cdot) 
% + (N-2)\pi_2(\cdot)]^{-1} \pi_2(\cdot) \big\}^{-1} , 
% \label{gamma1} \\ 
%  & \gamma_2(\cdot)  \eqdef 
%  - \gamma_1(\cdot) \pi_2(\cdot) 
%  \big[ (\lambda+\beta )I_p + \pi_1(\cdot) 
%  + (N-2)\pi_2(\cdot) \big]^{-1},  \label{gamma2}
% \end{align} 
% where 
% \begin{align*}
%     \pi_1(T) = \pi_2(T) = \frac{1}{N^3} \sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|}  u^i_j u^{i\top}_j 
%     \qquad 
%     \mbox{ and }
%     \qquad
%     \pi_3(T) =  - \frac{1}{N^2} \sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|}  {u^i_j} y^i_j 
% \end{align*}
% and, for $t=T-1,\dots,0$,
% \begin{align*}
%   \pi_1(t) &= \beta I_p- \beta^2 \gamma_1(t+1) \\ 
%   \pi_2(t) &= - \beta^2 \gamma_2(t+1) \\
%   \pi_3(t) &= \beta \big[ \gamma_1(t+1)
% + (N-1) \gamma_2(t+1)
% \big] \left( \pi_3(t+1) -\lambda \theta^\star_{(N)}\right)
% \end{align*}
% where $\theta^\star_{(N)} = \frac{1}{N} \sum_{i=1}^N \theta^\star_i$.

% The updates of the low-dimensional systems which Algorithm~\ref{alg:RegretOptimizationHeuristic} exploits are implemented via the helper function $\hat \alpha$, defined as 
% \allowdisplaybreaks 
% \begin{align} 
% \label{eq:RegretOptimizationHeuristic_Helper__1}
%   \widehat{\alpha}\big( \theta_i, ((\theta_j)_{j=1,j\neq i}^N) , (\gamma_i)_{i=1}^2,(\pi_i)_{i=1}^3 \big)  \eqdef &  
%  - (\gamma_1-\gamma_2)(\lambda I_p + \pi_1 - \pi_2 )\theta_i \notag \\ & 
%  - \big\{ \gamma_1 \pi_2 + \gamma_2 [ \lambda I_p + \pi_1 + (N-2)\pi_2 ] \big\} \sum_{j=1}^N \theta_j \notag \\ 
%  & - \big[ \gamma_1 + (N-1) \gamma_2 \big] 
%  (\pi_3 - \lambda \theta^\star_{(N)}) . 
%  \end{align}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% \vspace{0.2in} 
% The degree to which Algorithm~\ref{alg:RegretOptimizationHeuristic} is nearly regret-optimal depends on how far the weights $w$ determined by Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart} are from the equal weighting $\overline{1/N}$.  This is precisely quantified by the following results.

% \begin{theorem}[Near-Regret Optimality]\label{thrm:Epsilon_Efficiency}
% Suppose that $\mathcal{D}$ satisfies Assumptions~\ref{assm:bddxy} and~\ref{assm:PD}.  and let $\hat\Theta^{0\cdots T}$ denote the unique regret-optimal algorithm\footnote{That is, the unique optimizer of~\eqref{eq:penalized_regret_functional}} computed according to Algorithm \ref{alg:RegretOptimization}. Then, the output $\vartheta^{0\cdots T}$ of Algorithm~\ref{alg:RegretOptimizationHeuristic} satisfies
% \vspace{0.2in}
% \begin{enumerate}
%     \item[(i)] \textbf{Near-Optimality:} The difference $\big|
%             {\cal L}(\Theta^{0\cdots T})
%             -
%             {\cal L}(\vartheta^{0\cdots T})
%         \big|$ is of the order
%     \begin{align}
%     %    & \big|
%     %         {\cal L}(\Theta^{0\cdots T})
%     %         -
%     %         {\cal L}(\vartheta^{0\cdots T})
%     %     \big|
%     % \in 
%     &
%         \mathcal{O}\Big(
%                    \bar{N} N^3 \max_{1\leq i, k, l \leq N} \Big| \frac{1}{N^3} -  w^\star_k w^\star_l w^\star_i\Big| 
%                   + \bar{N} N^{3/2} \max_{1\leq k, l\leq N} \Big| \frac{1}{N^2} - w^\star_k w^\star_l \Big| 
%                   \notag \\ 
% & \hspace{5cm} + \bar{N}  \max_{1\leq i \leq N} \Big|\frac{1}{N} - w_i^\star \Big| 
%  + N \big\|\Theta^\star - \Theta^\star_{(N)} \big\|_2 
%         \Big)
%         \notag
%     ,
%     \end{align}
%     \item[(ii)] \textbf{Near-Optimal Increments:} The difference $\|\Delta \Theta^{0\cdots T-1}-\Delta \vartheta^{0\cdots T-1} \|_{\ell^1}$ is of the order
%     \begin{align} 
%        & 
%     %    \|\Delta \Theta^{0\cdots T-1}-\Delta \vartheta^{0\cdots T-1} \|_{\ell^1}
%     % \in 
%         \mathcal{O}\Big(
%                 \bar{N} N^{3/2} \max_{1\leq i, k, l \leq N} \Big| \frac{1}{N^3} -  w^\star_k w^\star_l w^\star_i \Big| \notag \\  
%  & %\hspace{5cm} 
%  + \bar{N} N^{1/2} \max_{1\leq k, l\leq N} \Big| \frac{1}{N^2} - w^\star_k w^\star_l \Big| 
%   +  \big\|\Theta^\star - \Theta^\star_{(N)}\big\|_2
%         \Big),
%         \notag
%     \end{align}
% \end{enumerate}
% where $\mathcal{O}$ hides a constant depending only on $\lambda$, $\beta$, 
% $\Theta^{\star}$, $(w_1^\star, ..., w_N^\star)$, $T$, $K_x$, and in $K_y$.  
% \end{theorem}

% The next result shows that Algorithm~\ref{alg:RegretOptimizationHeuristic} accelerates the regret-optimal algorithm by a linear factor in $N$ and by a quadratic factor in $p$, when $N$ is large.  
% %%%
% \begin{theorem}[$\mathcal{O}\big(N\,p^2\big)$-Acceleration over Regret-Optimal Algorithm]
% \label{thrm:accelertion_heuristic_regret_optimal_algorithm}
% With the convention that floating-point arithmetic operations are $\mathcal{O}(1)$, we have that:
% \begin{enumerate}
%     \item[(i)] \textbf{Complexity:} Algorithm~\ref{alg:RegretOptimizationHeuristic} has a complexity of $\mathcal{O}(TNp\max\{N,p\}))$
%     \item[(ii)] \textbf{Acceleration over Regret-Optimal Algorithm:} The regret-optimal algorithm has a complexity of $\mathcal{O}\big(TN^3 p^3\big)$.
% \end{enumerate}
% When $N\ge p$, Algorithm~\ref{alg:RegretOptimizationHeuristic} requires $\mathcal{O}(N\,p^2)$ fewer operations than the regret-optimal algorithm.  
% \end{theorem}

% % \Anastasis{I added this to held the reader understand Algo 1's solution:}\hfill\\
% % {\color{violet}{
% Finally, we establish that Algorithm~\ref{alg:RegretOptimizationHeuristic} is the regret-optimal algorithm, optimizing the systemic regret functional~\eqref{eq:penalized_regret_functional}, in the ``symmetric'' case where the optimal weights $w^{\star}$ are all $(1/N,\dots,1/N)$.  
% \begin{theorem}[Regret-Optimality in the Symmetric Case]
% \label{thrm:regretoptimality_SymmetricCase}
% Suppose that $w^{\star}_i=1/N$ for $i=1,\dots,N.$  Then, $\hat\Theta^{0\cdots T}=\vartheta^{0\cdots T}$.  
% \end{theorem}
% % }}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % We now examine the empirical performance of our algorithm.

% \section{Experiments}
% \label{s:Experiments_n_Validation}
% We now experimentally verify our theoretical results, with a focus on quantitative finance.
% In particular, we implemented the regret-optimal algorithm as well as its accelerated version and provide them together with the code for all experiments described in this section at \code.

% First, we conduct a convergence analysis of our regret-optimal algorithm, comparing it to standard gradient descent. We then demonstrate the transfer learning capabilities of our algorithm in the context of American option pricing.  
% We use the randomized neural networks approach of \cite{herrera2023optimal} as our fKRR model, since it best balances computational efficiency and expressiveness amongst the available non-linear versions of the \cite{longstaff2001valuing} algorithm for American option pricing.


% \subsection{Convergence of the Regret-Optimal Algorithm}
% \label{sec:Convergence of the Regret Optimal Algorithm}
% We first study the evolution of the energy functional  \eqref{eq:penalized_regret_functional} and loss \eqref{eq:terminal_time_objective} achieved in each iteration by our regret-optimal Algorithm~\ref{alg:RegretOptimization} with weights initialized by Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart}. That is to say, we compute ${\cal L}(\Theta^{0\cdots t})$ as defined in \eqref{eq:penalized_regret_functional} but for intermediate iterations $t$, as well as the loss $l(\Theta(t), w;\,\mathcal{D})$. 
% % the sum over the weights stops at $t-1$ and for the loss $l(\Theta(t), w;\,\mathcal{D})$ of the current weights is used. 
% We compare the regret-optimal algorithm with its accelerated version, given by Algorithm~\ref{alg:RegretOptimizationHeuristic} with weights given by Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart}, where we use $\Theta(0) = \Theta^\star_{(N)}$ and replace $\Theta^\star$ by $\Theta^\star_{(N)}$ in \eqref{eq:penalized_regret_functional}.
% Moreover, we compare to the results when using gradient descent to optimize the loss \eqref{eq:terminal_time_objective} directly.
% For all algorithms we use a ridge coefficient $\kappa=0$, regret coefficients $\lambda = 0$, $\beta=1$  and Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart} with information sharing level $\eta=10$ to get the corresponding optimal weights $w^\star$ and to initialize $\Theta(0)$ with the locally optimal parameters.
% We note that the comparison of our algorithms to gradient descent optimizing the loss \eqref{eq:terminal_time_objective} only makes sense in the $\lambda=0$ regime, since otherwise the objectives and therefore the behaviour are different. On the other hand, using $\beta > 0$ doesn't change the objective, but only forces our algorithm to make equally sized steps $\Delta \Theta (t)$, where the step size depends on $\beta$ and $T$.

% For our convergence analysis we use $N=5$ randomly generated datasets. In particular, each dataset $\mathcal{D}_i$ corresponds to a neural network $g_{\omega_i}$ with fixed randomly-generated hidden weights and biases.  Here $\omega_i$ denotes the vector of all these hidden weights and bias parameters. The networks have $d=5$ dimensional input, one hidden layer with $10$ hidden nodes, $\operatorname{ReLU}$ activation function and map to a $1$-dimensional output. The dataset is generated by sampling $S_i = 100$ inputs $x^i_j$ from a $d$-dimensional standard normal distribution and the corresponding target values are given by $g_{\omega_i}(x^i_j)$, i.e.,
% \begin{equation*}
%     \mathcal{D}_i = \{ (x^i_j, g_{\omega_i}(x^i_j)) \, | \, 1 \leq i \leq S_i, x^i_j \sim N(0,I_d) \}.
% \end{equation*}

% Our feature map $\phi$ in~\eqref{eq:FRKR} is a randomized neural network%
% \footnote{Also called a random feature model or an extreme learning machine} %
% with one hidden layer, $500$ hidden nodes and $\operatorname{ReLU}$ activation as studied by \cite{mei2021generalization,gonon2020risk,gonon2021random}. In particular, the weights of the hidden layers are randomly initialized and fixed and only the weights of the last layer, corresponding to $\theta$ in \eqref{eq:FRKR}, are optimized. We note that by our choice for the number of hidden nodes to equal the total number of samples, the algorithms can in principle learn to have perfect replication on the training set, i.e., loss $l(\Theta(t), w;\,\mathcal{D}) = 0$.
% For a fair comparison between the algorithms, we use the same randomly generated datasets and the same randomized neural networks for each of the methods.

% Figure~\ref{fig:convergence analysis} shows the averaged results for 10 runs each with a different set of randomly generated datasets and a different randomized neural network as fKRR. For the regret-optimal algorithm and for its accelerated version we use $T=10^3$ iterations, while we use $10^5$ steps for gradient descent with learning rate $7 \cdot 10^{-5}$. We note that for learning rates $\geq 8 \cdot 10^{-5}$ the training becomes unstable such that the loss explodes. 
% The gradient descent method gradually but slowly reduces the loss.
% Since the gradient descent method makes so small parameter updates (and since $\lambda=0)$, the regret is nearly $0$ and the energy ${\cal L}$ nearly equal to the loss. Even though it runs $100$ times the number of iterations of our algorithms, it would still need much more training to achieve the same loss.
% On the other hand, the regret-optimal algorithm and its accelerated version behave nearly indistinguishably, reducing the loss nearly to $0$ and piling up a little bit of regret. We note that by increasing the number of iterations, our algorithms could reduce the loss further by making smaller parameter updates and therefore piling up less regret, allowing them to focus even more on reducing the loss.

% \begin{figure}[!ht]%[H]
%         \centering            
%         \includegraphics[width=0.32\textwidth]{Graphics/conv_analysis-1}
%         \includegraphics[width=0.32\textwidth]{Graphics/conv_analysis-2}
%         \includegraphics[width=0.32\textwidth]{Graphics/conv_analysis-3}
%         \caption{Loss and energy ${\cal L}$ for gradient descent (GD), the regret-optimal algorithm (RO) and the accelerated regret-optimal algorithm (ARO). Means and standard deviations over 10 runs are shown. Left: all iterations; middle: first 1000 iterations; right: iterations 500 to 1000 for our algorithms.}
%         \label{fig:convergence analysis}
% \end{figure}

% In the regime where $\lambda > 0$ the behaviour of the algorithm changes drastically. In particular, since deviating from $\Theta(0) = \Theta^\star$ is penalised, the algorithm remains at the starting point in the initial steps and only starts to converge when approaching $T$. The exact behaviour depends on the choice of $\lambda$ (and is additionally influenced by the choice of $\beta$). In Figure~\ref{fig:convergence analysis 2} we compare the behaviour for $\lambda=10^{-4}$ and $\lambda = 2$ while otherwise using the same setup as before.  For the smaller value of $\lambda$, the algorithm starts the decent earlier and decreases the loss by more compared to the larger value for $\lambda$, where the algorithm deviates from $\Theta^\star$ only in the very last steps. 
% \begin{figure}[!ht]%[H]
%         \centering            
%         \includegraphics[width=0.48\textwidth]{Graphics/conv_analysis-4}
%         \includegraphics[width=0.48\textwidth]{Graphics/conv_analysis-5}
%         \caption{Loss and energy ${\cal L}$ for the regret-optimal algorithm (RO) and the accelerated regret-optimal algorithm (ARO). Means and standard deviations over 10 runs are shown. Left: $\lambda = 10^{-4}$; right: $\lambda=2$.}
%         \label{fig:convergence analysis 2}
% \end{figure}







% \subsection{American Option Pricing}
% \label{sec:American Option Pricing}
% We test our algorithm in the context of the optimal stopping problem for American option pricing, a computationally highly challenging problem which has recently become tractable also in higher dimensional settings through deep learning \citep{PatrickDOSJMLR_2019,Ruimeng_QF_OptimStopping,Timo_DOS_2021,herrera2023optimal}. This is a good example for our purpose for two reasons. 
% On the one hand, \cite{herrera2023optimal} did show that randomized neural networks, which are one class of fKRR, are well suited to (approximately) solve these optimal stopping problems. Moreover, it was shown that using randomized neural networks can heavily improve the computation time, which is also of importance to us since we need to solve several optimizations problems for a potentially large number of datasets.
% On the other hand, to solve the optimal stopping problem one needs to generate synthetic datasets. Hence, this problem allows us to generate multiple synthetic datasets of different sizes and varying similarity on which we can test the transfer-learning capabilities of our algorithm. The performance can be measured by comparing the achieved prices with those of several baseline methods.

% We first provide a short recap of the optimal stopping problem in American option pricing and then present our transfer-learning experiments.

% \subsubsection{Background: American Option Pricing and Optimal Stopping}\label{sec:Recap: American Option Pricing and Optimal Stopping}
% An American option is a financial derivative that gives its owner the right to execute a certain predetermined trade at any time between the start date and the maturity of the option. For example, a call (put) option gives its owner the right to buy (sell) a certain stock from the writer of the option for a fixed price $K$, called the strike. If the current stock price $X_t$ is higher (lower) than $K$ then the option owner can make a profit of $(X_t - K)_+$ (or $(K - X_t)_+$ respectively) by directly selling (buying) the stock again in the open market after having exercised their right to buy (sell) from the option writer. 
% While American options allow for continuous-in-time execution, it is common practice to approximate them via Bermudan options, which can be executed on a predetermined time grid $t_0 < \dotsb t_M$. We briefly overview the American option pricing problem, details of which can be found in \citep[Chapter 25]{PeshirShiryaev_FreeBoundaryProblems_2006Book}.


% In order to capture the computational challenges posed by the American option pricing problem in higher dimensions, we consider a stochastic process $(X_t)_{t=0}^M \in (\R^d)^{(M+1)}$ describing the price of $d$ stocks on the time grid 
% % Let $(X_t)_{t=0}^M \in \R^{(M+1)}$ be a stochastic process describing the price of a stock on the time grid
% and let $(Z_t)_{t=0}^M \in \R^{(M+1)}$ be the corresponding discounted payoff process of an American option written on a one-dimensional process obtained from $X_t$ (e.g. the largest price among the $d$ stocks). We define the filtration $\mathbb{F} = (\mathcal{F}_t)_{t=0}^M$ generated by $X$ via $\mathcal{F}_t = \sigma(X_s | s\leq t)$. Then the price of the American option is given by the starting value $U_0$ of the \emph{Snell envelope} \citep{SnellOGPaper_1952_SemiMartingaleOptimalStopping}, given by
% \begin{equation}\label{equ:snell envelope 2}
% U_m = \operatorname{sup}_{\tau \in \mathcal{T}_m} \E[ Z_{\tau} \, | \, \mathcal{F}_m ],
% \end{equation}
% where $\mathcal{T}_m$ is the set of all stopping times $\tau \geq m$. 
% The smallest optimal stopping time is
% \begin{align}\label{equ: optimal stopping time}
% \tau_M &:= M, \\
% \tau_m &:= \begin{cases}
% m, & \text{if } Z_m \geq \E[U_{m+1}  \, | \, \mathcal{F}_m],\\
% \tau_{m+1}, & \text{otherwise},
% \end{cases} \nonumber
% \end{align}
% hence, to compute the price of the American option it suffices to compute the \emph{continuation values} $\E[U_{m+1}  \, | \, \mathcal{F}_m]$ for all $m$. 
% In the following, we will use the \textit{randomized least squares Monte Carlo} (RLSM) algorithm of \cite{herrera2023optimal}, which utilises randomized neural networks to approximate the continuation values via backward induction (note the backward recursive scheme that \eqref{equ:snell envelope 2} and \eqref{equ: optimal stopping time} imply).
% In particular, this leads to $M$ backward-recursively defined regression problems that need to be solved sequentially. Since \eqref{equ:snell envelope 2} is a maximisation problem and since we only approximate the optimal stopping time, we compute lower bounds of the price $U_0$.
% The standard procedure is to fix some law for the process $X$ and to sample a dataset of $\nu = \nu_1+\nu_2$ i.i.d.\ paths of $X$, where $\nu_1$ of them are used for training the randomized neural networks (approximating the continuation value functions) and $\nu_2$ of them are used to evaluate the resulting price $U_0$ (using these trained networks). 
% Through the independence of the two parts of the dataset it is clear that any over-fitting bias the networks might learn will \emph{not} lead to prices that are too large. This is important, since the quality of a method can therefore be evaluated by the resulting price, using a higher price indicating a a better result. 
% % For more details we refer the interested reader to \cite{herrera2023optimal}.


% \subsubsection{Transfer Learning in American Option Pricing}\label{sec:Transfer Learning in American Option Pricing}
% In order to test the transfer learning capabilities of our algorithm, we do not generate a very large dataset of the most plausible distribtution of $X$ as is standard practice. Instead we generate many smaller, more or less similar datasets $\mathcal{D}_1, \dotsc, \mathcal{D}_N$ out of which  $\mathcal{D}_1$ is considered our main dataset on which we evaluate the performance.

% We always use the RLSM algorithm to price the American options and only vary the optimization method used internally by RLSM to solve the $M$ recursive regression problems arising at the exercise dates. Depending on the chosen optimisation method only one, multiple or all datasets are taken into account to compute the parameters of the randomized neural network at the given exercise date. 
% We compare our regret-optimal (RO) optimisation method of Theorem~\ref{thm:RegretOptimal_Dynamics__MainTextFormulation} to the following baselines.
% \begin{itemize}
%     \item \textbf{Local optimizer (LO-$i$).} The local optimizers $\theta^\star_i$ solves the individual optimisation problem on the datasets $\mathcal{D}_i$ without considering the other datasets.
%     \item \textbf{Mean Local optimizer (MLO).} The mean of the local optimizers $ \bar{\theta}^\star = \frac{1}{N} \sum_{i=1}^N \theta^\star_i$ is the bagging aggregation.
%     \item \textbf{Joint optimizer (JO).} The joint optimizer ${\theta}^\star_{\mathcal{N}}$ with $\mathcal{N}=\{ 1, \dotsc, N\}$ solves the optimisation problem of the pooled regime $\mathcal{D} = \cup_{i=1}^N \mathcal{D}_i$.
%     \item \textbf{Joint Subset optimizer.} This is the joint optimizer for any subset $\mathcal{I} \subset \mathcal{N}$ of the datasets $\mathcal{D}_{\mathcal{I}} = \cup_{i \in \mathcal{I}} \mathcal{D}_i$.
% \end{itemize}
% In this application we are only interested in the terminal parameters $\Theta(T)$. We know that our algorithm yields the parameters optimising \eqref{eq:penalized_regret_functional} for any $T\geq 1$ since there exists a closed-form solution. Hence, we choose $T=1$ which is most specialized on minimizing \eqref{eq:terminal_time_objective}, while the influence of the running costs \eqref{eq:penalized_regret_functional__REGRETFORM___Individual} can be controlled via the choice of $\lambda$ and $\beta$. Additionally, this minimizes the computation time for our algorithm.

% As fKRR we use the same randomized neural networks as in Section~\ref{sec:Convergence of the Regret Optimal Algorithm}.
% The random weights of the randomized neural networks, as well as the randomly sampled paths both introduce some randomness into the pricing problem. Therefore we follow \cite{herrera2023optimal} by always running the experiments $n_{runs} = 100$ times with different seeds and taking means over the prices. For easier comparison, we then consider the relative performance ($RP$) on our main dataset, computed as the mean price of any given method divided by the mean price of the local optimizer on the main dataset.
% Additionally, we compute asymptotically valid (by the central limit theorem) $95\%$-confidence-intervals as $RP \pm z_{0.975}\hat\sigma/\sqrt{n_{runs}}$, where $z_{0.975}$ is the $0.975$-quantile of the standard normal distribution and $\hat\sigma$ is the standard deviation  of $RP$ (computed as the sample standard deviation of the prices over the runs divided by the mean price of the local optimizer on the main dataset).
% To make the results comparable between the optimization methods, we use the same seeds for all of them, such that run $i$ always uses the exact same paths and the exact same random weights in the randomized neural network, independently of the chosen method.
% Moreover, we always use $\nu_2 \geq 50,000$ evaluation paths, such that the noise of the Monte Carlo approximation of the expectations is relatively small when evaluating the prices, even if we use much smaller training set sizes $\nu_1$.

% In the first experiment we study the ability of our method to transfer knowledge of those datasets, out a large number of small equally-sized datasets, benefiting the main task.

% \begin{experiment}\label{exp:1}{\rm 
%     In this experiment we generate $13$ different datasets, all of a Heston model with $\nu_1 = 100$ training samples but with different parameters.
%     The Heston model is defined as
%     \begin{equation}\label{equ:heston model}
%     \begin{split}
%     d X_t &= (r - \delta) X_t dt + \sqrt{v_t} X_t d W_t, \\
%     d v_t &= -k (v_t - v_{\infty}) dt + \sigma \sqrt{v_t}d B_t,
%     \end{split}
%     \end{equation}
%     where $W$ and $B$ are two Brownian motions with correlation $\rho \in [-1,1]$.
%     The main dataset $\mathcal{D}_1$ has the parameters $r=0.05$, $\delta=0.1$, $k=2$, $v_{\infty}=0.01$, $\sigma=0.2$, $\rho=-0.3$ and starting values $X_0=100$ and $v_0=v_\infty$.
%     The other datasets are define as all combinations of $r \in \{0.05, 0.5\}$, $\sigma \in \{ 0.15, 0.2, 0.25 \}$, $v_{\infty} \in \{ 0.005, 0.015 \}$ and otherwise the same parameters as the main dataset.
%     For all datasets we use a max call option with strike $K=100$ on $d=2$ i.i.d.\ stocks of the given model with $M=9$ equidistant exercise dates until the maturity $T_{mat} = 3$. The discounting factor is $e^{-r\,T_{mat}\,t/M}$ for $0\leq t \leq M$.
%     Moreover, we use a randomized neural network with one hidden layer with $300$ nodes and all methods use the ridge coefficient $\kappa=2$ and, where applicable, regret coefficients $\lambda=2, \beta=1$.
    
%     We report the results in Table~\ref{table:results exp 1}.
%     For our regret-optimal method (RO) we use information sharing levels $\eta \in \{  10, 100, 500\}$ and see that $\eta=100$ leads to the best result outperforming the local optimizer of the main dataset (LO-1) by $9\%$. It also outperforms all other local optimizers (LO-$i$), the mean local optimizer (MLO) and the joint optimizer (JO).
%     For $\eta=10$ we have similar performance as LO-1 and for $\eta=500$ we also have significant outperformance, though smaller than for $\eta=100$. 
    
%     The 6 datasets with $r=0.05$ (LO-2, $\dotsc$, LO-7) are relatively similar to the main dataset (with $RP \geq 0.96$), while the other 6 (LO-8, $\dotsc$, LO-13) are quite different (with $RP < 0.73$).
%     Therefore, we claim that our algorithm should mainly transfer knowledge from those 6 datasets with $r=0.05$ while avoiding to learn something wrong from the others.
%     In line with this we provide results of the joint optimizer on the 7 datasets with $r=0.05$, which performs better than the other baselines and outperforms LO-1 by $6.2\%$. In particular, this confirms that the datasets with $r=0.05$ are those to transfer knowledge from, since the joint optimizer for all datasets performs worse than LO-1. The joint subset optimizer is significantly outperformed by our regret-optimal algorithm RO ($\eta=100$) by about $3\%$, which shows that our method constitutes a better way for transfer learning than simply selecting the datasets most similar to $\mathcal{D}_1$.
    
%     We additionally compare our method to the local optimizer for the main dataset which uses either $700$ (the number of training samples in the 7 similar datasets with $r=0.05$) or $50,000$ training samples. Importantly, both are just references that would not be available in a real world setting where the datasets are limited.
%     The first one only leads to a slight increase in $RP$ of about $1\%$, which shows that our method extracts nearly as much knowledge out of the (same amount of) samples of the similar datasets with $r=0.05$. 
%     The second one (which is considered a good proxy for the true American option price on the main dataset) has about $10\%$ better performance. This also shows the limitations of our method, in particular, it can only transfer as much knowledge as available in the other datasets.}
% \end{experiment}

% \begin{table}[hbt]
%     \centering
%     \caption{Relative performance (RP) and $95\%$-confidence-intervals for different optimization methods in Experiment~\ref{exp:1}. We compare the local optimizers on the different datasets (LO-$n$), with the mean local optimizer (MLO), the joint optimizer (JO) and our regret-optimal method (RO). The ``oracle'' local optimizer on the main dataset with additional training samples (standard: $100$ samples per dataset) is included.  
%     \hfill\\
%     When the information sharing parameter $\eta$ is set to $100$, the regret-optimal (RO) algorithm outperforms all ``non-oracle'' baselines. }
%     % \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{@{}ccc@{}}
%     \cmidrule[0.3ex](){1-3}
%     method &  $RP$ &  $95\%$-CI \\
%     \midrule
%     \csvreader[head to column names, late after line=\\]
%     {Tables/training_overview-1-1.csv}{}%
%     {  \name & \RP & \CI }%
%     \midrule
%     \csvreader[head to column names, late after line=\\]
%     {Tables/training_overview-1-2.csv}{}%
%     {  \name & \RP & \CI }%
%     \bottomrule
%     \end{tabular}
%     % }% END Resize box
%     \label{table:results exp 1}
%     \end{table}
    


% In the second experiment we test the ability of our method to transfer knowledge from a small dataset which is similar to the small main dataset, even if it is confronted with a very different and much larger (dominating in terms of samples) dataset.

% \begin{experiment}\label{exp:2}{\rm 
%     In this experiment we generate 3 different datasets. The main dataset is generated from a rough Heston model
%     \begin{align*}
%     dX_t &=  (r - \delta) X_t dt +  \sqrt{v_t} X_t dW_t, \\
%     v_t &= v_0 + \int_0^t \frac{(t-s)^{H-1/2} }{\Gamma(H + 1/2)} \kappa (v_\infty - v_s)ds + \int_0^t \frac{(t-s)^{H-1/2} }{\Gamma(H + 1/2)} \sigma \sqrt{v_s}dB_s,
%     \end{align*}
%     which is similar to the Heston model except that the volatility is  a rough process with Hurst parameter $H\in(0,1/2]$, where the case $H=1/2$ coincides with the standard Heston model. 
%     We use $H=0.1$ and otherwise the same parameters as for the main dataset in Experiment~\ref{exp:1}. The second and third dataset generated from standard Heston model (i.e.\  $H=1/2$), with the same parameters, except for the drift $r=0.5$ for the second dataset.
%     In particular, dataset 3 is the closest non-rough dataset to the main dataset, while dataset 2 is quite different.
%     For datasets 1 and 3 we use $\nu_1=100$ training samples, while we use $\nu_1=50,000$ for dataset 2, such that it dominates the others in its size.
%     All the other choices are the same as in Experiment~\ref{exp:1}.

%     The results are reported in Table~\ref{table:results exp 2}. The baselines MLO and  JO perform significantly worse than the LO on the main dataset. As expected, the JO suffers much more from the dominating dataset 2 than the MLO. Indeed, the MLO would suffer more from a large number of datasets that are quite different from the main dataset, no matter their sample size.
%     In contrast to this, our regret optimal method with $\eta \in\{50,100\}$ outperforms the LO-1 by $4\%$, showing that also a quite different dataset dominating in sample size is not a problem.}
% \end{experiment}

%     \begin{table*}[!htb]
%     \centering
%     \caption{Relative performance (RP) and $95\%$-confidence-intervals for different optimization methods in Experiment~\ref{exp:2}. We compare the local optimizers on the different datasets (LO-$n$), the mean local optimizer (MLO), the joint optimizer (JO) and our regret-optimal method (RO). With $\eta=100$ RO outperforms all baselines. }
%     \begin{tabular}{@{}ccc@{}}
%     \cmidrule[0.3ex](){1-3}
%     method &  $RP$ &  $95\%$-CI \\
%     \midrule
%     \csvreader[head to column names, late after line=\\]
%     {Tables/training_overview-2.csv}{}%
%     {  \name & \RP & \CI }%
%     \bottomrule
%     \end{tabular}
%     % }% END Resize box
%     \label{table:results exp 2}
%     \end{table*} 
    


% Both of these experiments show that our regret optimal method is well suited for automatic (up to the hyper-parameter $\eta$) dataset selection in transfer learning tasks that have potentially large numbers of datasets and do not allow a (manual) pre-selection. 
% In particular, neither a large number of ``bad'' datasets (of which the MLO suffers) nor some ``bad'' datasets that dominate in sample size (of which the JO suffers) constitute a problem for our regret-optimal method.
% Moreover, the sample efficiency when transferring knowledge from similar datasets to the main task is very high (outperforming the JO on the respective subset of similar datasets and nearly being on par with the LO on the main dataset using a larger training sample), as we saw in Experiment~\ref{exp:1}.





































% \section{Conclusion}
% In this work we presented a regret-optimal algorithm for federated transfer learning based on finite-rank kernel ridge-regressors (fKRR). 
% Besides the theoretical properties of this algorithm, we also provided experiments demonstrating the transfer learning capabilities of our method in the context of American option pricing.

% One possible future research direction is to apply our transfer learning method to real world datasets, where the similarity between the datasets is a priori not easy to quantify.
% From the theoretical side we would like to extend our method to regression models that do not necessarily permit a closed-form solution.



% % \acks{}
% % \section*{Acknowledgments}
% % AK acknowledges financial support from an NSERC Discovery Grant No.\ RGPIN-2023-04482 and their McMaster Startup Funds. 
% % MG acknowledges support from an NSERC Discovery Grant No.\ RGPIN-2013-276671.



% \bibliography{Formatting/References}
% \bibliographystyle{icml2021}


% \appendix

% \section{Game Theoretic Interpretation of Regret-Optimal Algorithm}
% \label{s:GameTheoreticInterpretation}

% We now offer a game-theoretic interpretation of the regret functional, as defined in~\eqref{eq:penalized_regret_functional}.  This interpretation views the user as a central planner whose objective is to organize a system of individual agents, representing the pretrained KRR models, to maximize the singular goal of identifying a parameter optimizing~\eqref{eq:penalized_regret_functional__REGRETFORM}.  
% We now interpret the roles and interactions of the central planner and each agent as defined by our regret-optimization problem.
% % %%
% % In classical regression analysis, one typically selects a regression model $f:\Theta \times \mathbb{R}^d\rightarrow \mathbb{R}$ by optimizing a performance criterion on a (finite) training dataset $\mathcal{D}_1\subset \mathbb{R}^d\times \mathbb{R}$. The model $f$ is parameterized by $\Theta\subseteq \mathbb{R}^p$, with $p,d\in \mathbb{N}_+$, and for fixed $\theta \in \Theta$ we write $f_\theta \eqdef f(\theta, \cdot)$ for the function that maps the input $x\in \mathbb{R}^d$ to the model's output $y\in \mathbb{R}$.
% % Selecting a regression model then amounts to identifying a \textit{parameter vector} $\theta_1 \in \Theta$ which is typically chosen to minimize the penalized sum-of-squares errors (SSE) on the given dataset
% % \begin{equation}
% % \label{eq:Regression_Klassische0}
% %     \inf_{\theta \in \Theta}\, 
% %             \sum_{(x,y)\in \mathcal{D}_1}\,
% %                 (f_\theta(x)-y)^2
% %         +
% %             \kappa \,
% %                 \|\theta\|_2.
% % \end{equation}
% % Here, $\kappa \geq 0$ is a hyperparameter controlling the regularity of the model, which is often implicitly reflected by the Euclidean norm of its parameter vector $\|\theta\|_2$, though other regularizers are available, for example in \cite{VDG_Sara_HighDimenisonalGLMsandLassi_AnnStat,simon2013sparse,AdcockAnyiBrugiapaglia_2019_NumerischeMath}.  Even if each output $y$ is obscured by ``noise'', there is an underlying homogeneity assumption underpinning~\eqref{eq:Regression_Klassische0}, namely that the training data all belongs to the same dataset and the elements of that dataset represent the same task.  Typically (see e.g.~\cite{bartlett2002rademacher,ZouAdaptiveLassoOracle_AnnStat_2006}), one assumes that there is a suitable, yet unknown, ``target'' function $f^\star:\mathbb{R}^d\rightarrow \mathbb{R}$ and a ``noise'' generating probability distribution $\mu$ on $\mathbb{R}$ such that for every $(x,y)$ in the training dataset $\mathcal{D}_1$ one has $y=f^{\star}(x)+\varepsilon_y$ where $\{\varepsilon_y\}_{(x,y)\in \mathcal{D}_1}$ are i.i.d.\ random variables with law $\mu$.
 
% % A parameter vector optimizing~\eqref{eq:Regression_Klassische0} need not be available in closed-form.  Instead, provided it exists, it is typically identified approximately via an iterative gradient descent-type procedure.  Even if a closed-form expression exists, it is often more computationally efficient to resort to iterative algorithms \citep{YaoRosascoCoponnetto_2007_CA}.  A \textit{deterministic} iterative algorithm initialized at $\theta_0\in\mathbb{R}^p$ and running for $T\in\mathbb{N}_+$ iterations is characterized by its iterates.  Thus, any such iterative deterministic algorithm is identifiable with a sequence in $\mathbb{R}^p$ of length $1+T$; i.e.
% % \begin{equation}
% % \label{eq:algorithms}
% %     \theta^{0\cdots T}\eqdef \left\{\theta(t)\right\}_{t=0}^T, 
% %     \qquad 
% %     \theta(0)=\theta_0.
% % \end{equation}
% % % \begin{equation}
% % % \label{eq:algorithms}
% % %     \theta_{\cdot}\eqdef (\theta(0),\dots,\theta(T)) 
% % %     \qquad 
% % %     \theta(0)=\theta_0.
% % % \end{equation}
% % With this identification and a measure of algorithmic efficiency, e.g.\ \textit{regret}, one can characterize the most efficient algorithm as in \cite{casgrain2019latent,casgrain2021optimizing}.

% % The situation becomes more complicated in modern machine learning, where one often has access to large amounts of data, typically drawn from several \textit{similar}, yet \textit{distinct} sources.  
% % These types of comparable datasets arise in meta-learning \citep{finn2017model,pavasovic2022mars}), in multi-task learning \citep{kumar2012learning,NEURIPS2020_3fe78a8a}, in quantitative finance due to natural market cycles \citep{lowry2002ipo}, or in robust finance approaches to model uncertainty resulting in several plausible stochastic time-series models wherewith data can be simulated \citep{hou2018robust,aksamit2019robust,prashanth2022wasserstein}.

% % This paper focuses on the optimization aspect of the regression problem under multi-sourced data, with a focus on applications in mathematical finance, instead of the more often explored questions of learning-theoretic nature such as the risk of a federated learning procedure as in \cite{hu2023generalization,sun2023fedspeed}.  Specifically, we construct a \textit{regret-optimal federated optimization algorithm}, as defined shortly, under no communication restrictions between the server (central planner) and the local nodes (agents) at each round. 


% % \paragraph{Optimizing with Multi-Sourced Data:}
% % In situations where we have access to several distinct \emph{additional} datasets $\mathcal{D}_2,\dots,\mathcal{D}_N$ whose information we wish to leverage, we can improve the predictive performance of our regression model past what can be achieved using the focal or \textit{primary} dataset $\mathcal{D}_1$ in the classical approach~\eqref{eq:Regression_Klassische0}.
% % Here, the underpinning assumption is that the datasets $\mathcal{D}_i$, for $i\neq 1$, are generated by a different, but comparable, mechanism from which $\mathcal{D}_1$ was generated.  

% % The introduction of \textit{multi-sourced data} yields a spectrum of interpretations of optimality extending~\eqref{eq:Regression_Klassische0}, which can be naturally organized from a game-theoretic point of view.  In this perspective, we can consider several \textit{agents} (or nodes), each representing the influence of a dataset $\mathcal{D}_i$ on the model selection problem, who propose parameter vectors $\theta_1,\dots,\theta_N$ optimized for their own datasets. The agents are then  assumed to be organized by a \textit{central planner} (or server), representing the user. The objective of this central planner is to maximize the predictive power of the selected model on new data sampled from the same process which generated the focal dataset $\mathcal{D}_1$.  
% \paragraph{The Central Planner:}
% The purpose of the central planner is to avoid the situation whereby the structure of the different datasets is ignored in the model selection problem, by merging them into a single dataset $\mathcal{D}\eqdef \cup_{i=1}^N\,\mathcal{D}_i$ and thereby reducing the problem to~\eqref{eq:Regression_Klassische0}. Though intuitively simple, such merging  approach can be particularly disadvantageous in the presence of heterogeneity among the datasets, since a dataset that is potentially very different from the focal dataset $\mathcal{D}_1$ would be equally influential in the regression problem~\eqref{eq:Regression_Klassische0}.  
% Instead, the user, acting as a central planner, organizes the model selection problem through a cooperative objective
% \allowdisplaybreaks\begin{align} 
% \label{eq:terminal_time_objective appendix}
% \begin{aligned}
%         l(\Theta, w;\,\mathcal{D} )  
%     \eqdef & 
%         \sum_{i=1}^N 
%         w_i
%             \sum_{j=1}^{|\mathcal{D}_i|} 
%                 (
%                 f_{\theta^w}(x_j^i)
%                 - y^i_j  
%                 )^2,
%     \\
%     \mbox{ with }
%     \,
%     \theta^w\eqdef & \sum_{i=1}^N 
%         w_i\,\theta_i
%  ,
% \end{aligned}
% \end{align} 
% where $\Theta\eqdef (\theta_1^{\top}, \cdots, \theta_N^{\top})^\top\in \mathbb{R}^{Np \times 1}$. Here, the central planner \textit{ascribes} the influence of each agent on the model selection problem through the weight vector $w=(w_1, \cdots, w_N)\in [0,1]^N$ with $\sum_{i=1}^N\,w_i=1$.  
% As can be seen in \eqref{eq:terminal_time_objective appendix}, this influence is two-fold: on the one hand, it impacts the cooperative objective $l$ in the aggregation of the SSE of each player; on the other hand, it affects the proportion of each player's preferred parameter choice entering into the collectively selected parameter $\theta^{w}$.
% %
% The choice of $w$ is approached in different ways in the literature, e.g.\ by bagging 
% % $\frac1{N}\sum_{i=1}^N\, \theta^\star_i$ 
% reminiscent of mean-field games \citep{carmona2018probabilistic}, by data-driven weighting procedures \citep{Baxter_2000_JAIR__AmodelIndutvieBiasLearning}, Bayesian aggregation \citep{MR2280214,PACOH_rothfuss_2021,pavasovic2022mars}, or with dictionaries \citep{argyriou2006multi}.  

% \paragraph{The Agents:}
% When acting in isolation, each agent's preferred model is determined by optimizing a version of ~\eqref{eq:Regression_Klassische0} using only their dataset.  Under mild conditions\footnote{E.g.\ coercivity and lower semi-continuity in $\theta$.} on $f$, this corresponds to an {\em individual} parameter selection
% \begin{align}
%     \theta^{\star}_i \in 
%     \operatorname{argmin}_{\theta \in \Theta}
%         \, 
%             \sum_{(x,y)\in \mathcal{D}_i}\,
%                 (f_\theta(x)-y)^2
%         +
%             \kappa \,
%                 \|\theta\|_2, 
% \label{eq:Regression_Klassische1}
% \end{align}
% for $i=1,\dots,N$, which we assume to be fixed and known to all agents prior to their {\em collective} parameter selection. Taking into account the other agents, each agent \textit{acts} by specifying an iterative deterministic algorithm of the form~\eqref{eq:algorithms}, with the intent of maximizing their influence on the joint model selection problem~\eqref{eq:terminal_time_objective appendix}.  Thus, the $i^{th}$ player wants the jointly selected model, specified by $\theta^{w}(T)=\sum_{n=1}^N\, w_i\,\theta_i(T)$, to be as close to $\theta_i^{\star}$ as possible, thereby maximally encoding the characteristics of the $i^{th}$ dataset into the selected model $f_{\theta^w(T)}$. The accumulated \textit{regret} which the $i^{th}$ player incurs by deploying an algorithm $\theta^{0\cdots T}_{i}$ that deviates from their preferred selection $\theta^*_i$ is measured by
% \begin{equation}
% \label{eq:penalized_regret_functional__REGRETFORM___Individual}
% \begin{aligned}
%     %     \mathcal{R}_i(\theta^{0\cdots T}_{i})
%     % \eqdef &
%             \sum_{t=0}^{T-1}  
%             \,
%                 \underbrace{
%                     \lambda \,
%                     \left\| \theta_i(t+1) - \theta^\star_{i} \right\|_2^2
%                 }_{\text{Preference Strength}}
%             + 
%                 \underbrace{
%                       \beta \, \left\| \Delta \theta_i(t) \right\|_2^2 
%                 }_{\text{Algorithm Stability}}
% ,
% \end{aligned}
% \end{equation}
% % \begin{equation}
% % \label{eq:penalized_regret_functional__REGRETFORM___Individual}
% % \begin{aligned}
% %         \mathcal{R}_i(\theta_{\cdot})
% %     \eqdef &
% %             \sum_{t=0}^{T-1}  
% %             \,
% %                 \underbrace{
% %                     \lambda \,
% %                     \left\| \theta(t+1) - \theta^\star_{i} \right\|_2^2
% %                 }_{\text{Preference Strength}}
% %             + 
% %                 \underbrace{
% %                       \beta \, \left\| \Delta \theta(t) \right\|_2^2 
% %                 }_{\text{Algorithm Stability}}
% % ,
% % \end{aligned}
% % \end{equation} 
% % \begin{align} 
% %  \frac{1}{|\mathcal{D}_i|} \sum_{(x,y)\in \mathcal{D}_i}\,
% %                 (f(\theta,x)-y)^2
% %         +
% %             \kappa \,
% %                 \|\theta\|_2 + \sum_{t=0}^T 
% %  \lambda \|\theta_i(t+1) - \theta_i^\star \|_2^2 
% %  + \beta\|\Delta \theta_i(t) \|_2^2
% % \end{align}
% where $\lambda>0$ is a hyperparameter quantifying the player's \textit{attachment} towards their preferred model choice $\theta^{\star}_i$ and the hyperparameter $\beta > 0$ quantifies the the stability of the algorithm during the iterations, where  $\Delta \theta_i(t)\eqdef \theta_i(t+1)-\theta_i(t)$.  
% % The regularization term $\sum_{t=0}^{T-1}\, \left\| \Delta \theta_i(t) \right\|_2^2$, in~\eqref{eq:penalized_regret_functional__REGRETFORM___Individual}, prohibits unstable algorithms from being deployed which ``teleport/jump'' to $\theta_i^{\star}$ and to their terminal position $\theta_i(T)$.  
% % \Anastasis{@Aurelien can you add a reference here, in the context of optimization for the quadratic term.}
% % \Aurelien{Can probably cite Convex Optimization Algorithms Dimitri P. Bertsekas} 


% The central planner then organizes the action $\Theta^{0\cdots T}\eqdef 
% \left\{\Theta(t)\right\}_{t=0}^{T}$ of the system of $N$ players to reach the objective~\eqref{eq:terminal_time_objective appendix} while encoding their individual regrets~\eqref{eq:penalized_regret_functional__REGRETFORM___Individual}, where
% \begin{equation}
% \Theta (t) = (\theta_1(t)^\top,\ldots,\theta_N(t)^\top)^\top \in \mathbb{R}^{Np \times 1}. \notag 
% \end{equation}

% This is achieved by coupling the individual agent's regret functionals~\eqref{eq:penalized_regret_functional__REGRETFORM___Individual} through the \textit{systemic regret functional}
% \begin{equation}
% \label{eq:penalized_regret_functional__REGRETFORM appendix}
% \begin{aligned}
%     \mathcal{R}(\Theta^{0\cdots T})
% \eqdef &
%         \underbrace{
%         l (\Theta(T), w;\,\mathcal{D} ) 
%         }_{\text{Cooperative Objective}}
%     -
%                   \,\,  l^{\star}
%     +
%         \sum_{t=0}^{T-1}  
%         \,
%              \big(
%                     \underbrace{
%                         \lambda \left\| \Theta(t+1) - \Theta^\star \right\|_2^2    
%                     }_{\text{Preference Strength}}
%                 + 
%                     \underbrace{
%                         \beta  \left\| \Delta \Theta(t) \right\|_2^2 
%                     }_{\text{Algo. Stability}}
%                 \big) 
%     ,
% \end{aligned}
% \end{equation} 
% where
% \begin{equation}
%     \label{Theta_star}
%     \Theta^\star\eqdef (\theta_1^{\star \top}, \cdots, \theta_N^{\star\top})^\top
%     \in \mathbb{R}^{Np \times 1}
% \end{equation}
% encodes the individual preferences of the players,
% % is a \textit{fixed initial condition} and the $N$-player system evolves according to 
% % \allowdisplaybreaks
% % \begin{align}
% % & \Theta(0)=\Theta^\star, 
% % \quad 
% % \Theta(t+1) = \Theta(t) + \Delta \Theta(t), 
% % \label{Theta-simple__nocontrol}
% % \end{align} 
% % for $\quad 0\leq t \leq T-1$, where 
% % $\Theta(0)=(\theta_1(0)^\top, \cdots, \theta_N(0)^\top)^\top \in \mathbb{R}^{Np\times 1}$, $\Theta(t)=(\theta_1^\top(t),\dots,\theta_N^\top(t))^\top$ is matrix notation, and 
% \begin{equation}
%     \Delta \Theta(t)\eqdef \Theta(t+1)-\Theta(t) 
%     \label{Theta-simple__nocontrol}
% \end{equation}
% quantifies the integrative updates of any candidate optimizing sequence $\Theta^{0\cdots T}$, and the \textit{ideal terminal loss} is 
% \[
%         l^{\star}
%     \eqdef 
%         \underbrace{
%             \min_{\Xi \in \mathbb{R}^{Np\times 1}}\, 
%                 l(\Xi,w; \mathcal{D}) 
%                 % + \lambda \|\Xi - \Theta^{\star} \|_2
%         }_{\text{Cooperative Sub-optimality}}
%     .
% \]
% The term $(l(\cdot,\cdot;\cdot)-l^{\star})$ measures the central planner's regret in failing to optimize~\eqref{eq:terminal_time_objective appendix}.  The algorithm stability term in~\eqref{eq:penalized_regret_functional__REGRETFORM appendix} appears in forward-backward proximal splitting algorithms with quadratic objectives (e.g. \cite{MR3619041,MR4490614}) and several standard proximal algorithms (see \cite[Section 5.1]{bertsekas2015convex}).

% The systemic regret functional~\eqref{eq:penalized_regret_functional__REGRETFORM appendix} acts as a performance criterion for any optimization algorithm, played by $N$ players, initialized at an arbitrary $\Theta(0)$, and running for $T$ iterations.  
% In what follows, we take the initial condition of the algorithm as $\Theta(0)=\Theta^\star$ for simplicity, but other choices are possible. In other words, the regret of each player is initialized at zero, as they all start from their individually preferred parameter $\theta^\star_i$, and starts to accumulate as the system moves away from $\Theta^\star$ towards the optimizer of  \eqref{eq:penalized_regret_functional__REGRETFORM appendix}.       


% \section{Proofs and Technical Results}
% \label{s:Proofs_TechnicalLemmata}



% \begin{remark}
% \label{rem:Notation_InnerProduct}
% We keep our notation light and use $u^{\top}v$ to implement the Euclidean inner-product between any two vectors $u,v\in \mathbb{R}^k$ for any $k\in \mathbb{N}_+$. 
% We use $| \cdot |$ to denote the Euclidean norm of a vector or Fr\"{o}benius norm of a matrix, whichever is applicable. 
% For two square matrices $A$ and $B$, $A\leq B$ ($A<B$, resp.) means that $B-A$ is positive semi-definite (positive definite, resp.); see \citep[page 146 - Equation (7)]{LaxBookLinearAlgebra_2007} for details.
% \end{remark} 

% Lemmas~\ref{lm:|AB|<=|A||B|} and \ref{lm:|A1+An|2<=(|A1|2+|An|2)n} give some elementary properties of matrix algebra, which will be used repeatedly in the subsequent proofs. 
% \begin{lemma} 
% \label{lm:|AB|<=|A||B|}
% The Euclidean norm $|\cdot|$ of matrices has the following properties: 

% \noindent\emph{i)}. For any matrices $A\in \mathbb{R}^{n_1 \times n_2}$ and $B\in\mathbb{R}^{n_2\times n_3}$, we have that
% $|AB| \leq |A|\cdot |B|$;   

% \noindent\emph{ii)}. For any matrices $A$, $B\in \mathbb{R}^{n_1 \times n_2}$, we have $|A+B| \leq |A|+|B|$.  
% \end{lemma} 
% \begin{proof}  
% Denote $A=(A_{ij})_{1\leq i\leq n_1 , 1\leq j \leq n_2}$ and $B=(B_{jk})_{1\leq j \leq n_2, 1\leq k \leq n_3}$. 
% %Further denote the $k$-th column vector of $B$ by $b_{\cdot k}$. 
% By the Cauchy-Schwarz inequality, we have for each column vector $B_{\cdot k}$ of $B$ that 
% \begin{align} 
%  |A B_{\cdot k}|^2 = \sum_{i=1}^{n_1} \big( \sum_{j=1}^{n_2} A_{ij} B_{jk} \big)^2 
%   \leq \sum_{i=1}^{n_1} \big( \sum_{j=1}^{n_2} A_{ij}^2 \sum_{j=1}^{n_2} B_{jk}^2 \big) 
%   = \big( \sum_{i=1}^{n_1} \sum_{j=1}^{n_2} A_{ij}^2 \big) \sum_{j=1}^{n_2} B_{jk}^2 
%   = |A|^2 \sum_{j=1}^{n_2} B_{jk}^2 . 
%   \notag 
% \end{align} 
% It then follows that 
% \begin{align} 
%  |AB|^2 = & |(A B_{\cdot 1}, A B_{\cdot 2}, ..., A B_{\cdot n_3} ) |^2 
%  = |A B_{\cdot 1}|^2 + |A B_{\cdot 2}|^2 + \cdots + |A B_{\cdot n_3}|^2 \notag \\ 
%  \leq & |A|^2 \sum_{j=1}^{n_2} \sum_{k=1}^{n_3} B_{jk}^2 = |A|^2 |B|^2 , \notag 
% \end{align} 
% and assertion i) is proved. 

% For $A$, $B\in \mathbb{R}^{n_1\times n_1}$, we have 
% \begin{align} 
% |A+B|^2 = & \sum_{i=1}^{n_1} \sum_{j=1}^{n_2} (A_{ij} + B_{ij})^2  
%  =   \sum_{i=1}^{n_1} \sum_{j=1}^{n_2} A_{ij}^2 + \sum_{i=1}^{n_1} \sum_{j=1}^{n_2} B_{ij}^2 
%  + 2 \sum_{i=1}^{n_1} \sum_{j=1}^{n_2} A_{ij} B_{ij} \notag \\ 
%  \leq & |A|^2 + |B|^2 + 2 |A|^2 |B|^2 
%   = (|A|+|B|)^2 , \notag 
% \end{align} 
% which proves assertion ii). 
% \end{proof} 








% \begin{lemma} 
% \label{lm:|A1+An|2<=(|A1|2+|An|2)n} 
% Let $w_1$, $w_2$, ..., $w_n$ be positive numbers such that $\sum_{k=1}^n w_k = 1$. 
% For any $n$ matrices $A_1$, ..., $A_n\in \mathbb{R}^{n_1 \times n_2}$, it satisfies that 
% $\big| \sum_{k=1}^n w_k A_k \big|^2 \leq \sum_{k=1}^n w_k |A_k|^2$; 
% particularly, when $w_1=w_2=\cdots = w_n=1/n$, we have 
% $\big|\sum_{k=1}^n  A_k \big|^2 \leq n \sum_{k=1}^n |A_k|^2$ . 
% \end{lemma} 
% \begin{proof} 
% Denote $A_k = ( A_{k, ij})_{1\leq i\leq n_1,  1\leq j \leq n_2}$, $k=1$, ..., $n$. 
% By the Jensen's inequality, we have 
% \begin{align} 
%  ( w_1 A_{1, ij} + \cdots + w_n A_{n, ij})^2 \leq  w_1 A_{1, ij}^2 + \cdots + w_n A_{n, ij}^2  . \notag 
% \end{align}  
% It then follows that 
% \begin{align} 
%  |w_1 A_1 + \cdots + w_n A_n|^2 = & \sum_{i=1}^{n_1} \sum_{j=1}^{n_2} (w_1 A_{1, ij} + \cdots + w_n A_{n, ij})^2 
%  \leq  \sum_{i=1}^{n_1} \sum_{j=1}^{n_2} w_1 A_{1, ij}^2 + \cdots + w_n A_{n, ij}^2   \notag \\ 
%   = &   w_1 \sum_{i=1}^{n_1} \sum_{j=1}^{n_2} A_{1, ij}^2 + \cdots + w_n \sum_{i=1}^{n_1} \sum_{j=1}^{n_2} A_{n, ij}^2  \notag \\ 
%   = &   w_1 |A_1|^2 + \cdots + w_n |A_n|^2  .   
%   \notag 
% \end{align} 


% \end{proof} 

% We begin with the relatively short proof of Theorem \ref{prop:Optimal_Bayes_Weighting} establishing the optimality of the weights obtained in Algorithm \ref{alg:RegretOptimizationHeuristic__WarmStart}. 

% \begin{proof}[{Proof of Theorem~\ref{prop:Optimal_Bayes_Weighting}}]
% For $i=1,\dots,N$, consider the probability measure 
% \[
% \bar{\mathbb{P}}^{\eta}
% \eqdef 
% \sum_{i=1}^N\,
% \frac{
% [s^1+\eta -s^i]_+
% }{
% \sum_{k=1}^N\, [s^1 + \eta - s^k]_+
% }
% \,
% \delta_{\theta^\star_i}
% \] 
% on the discrete space $\{\theta^\star_i\}_{i=1}^N$ topologized by the discrete metric.
% % Since arg-minima are invariant under multiplication by positive constants, then i
% Any minimizer of~\eqref{eq:optimizingQ__regularized} is a minimizer of the following problem, and vice-versa
% \begin{align}
% \nonumber
% &
%     \min_{
%         \mathbb{P}_w \in \mathcal{P}(\{\theta^\star_i\}_{i=1}^N)
%     }\,
%             \frac1{|\mathcal{D}_1|}\sum_{j=1}^{|\mathcal{D}_1|}\,
%             \big\|
%                     f_{\theta}(u_j^1)
%                 -
%                     y_j^1
%             \big\|_2^2
%     +
%         \eta\,
%         % \frac{(1-\eta)}{\eta}
%         \operatorname{D}_{\operatorname{KL}}\big(
%             \mathbb{P}_w
%         \|
%             \bar{\mathbb{P}}^{\eta}
%         \big)
%     % +\iota(\mathbb{P}_w \ll \bar{P}^{\eta})
% \\
% \nonumber
% & =
%     \min_{
%         \mathbb{P}_w \in \mathcal{P}(\{\theta^\star_i\}_{i=1}^N)
%     }\,
%         \mathbb{E}_{\theta \sim \mathbb{P}_w}\,
%         \Biggl[
%             \frac1{|\mathcal{D}_1|}\sum_{j=1}^{|\mathcal{D}_1|}\,
%             \big\|
%                     f_{\theta}(u_j^1)
%                 -
%                     y_j^1
%             \big\|_2^2
%         \Biggr]
%     +
%         % \frac{(1-\eta)}{\eta}
%         \eta\,
%         \operatorname{D}_{\operatorname{KL}}\big(
%             \mathbb{P}_w
%         \|
%             \bar{\mathbb{P}}^{\eta}
%         \big)
%     +
%     \iota(\mathbb{P}_w \ll \bar{P}^{\eta})
% \\
% \label{eq:optimizingQ__regularized__Renormalized}
% & =
%     \min_{
%         \mathbb{P}_w \in \mathcal{P}(\{\theta^\star_i\}_{i=1}^N)
%     }\,
%         \mathbb{E}_{\theta \sim \mathbb{P}_w}\,
%         \biggl[
%         \sum_{i=1}^N\,
%         I_{\theta = \theta^\star_i}
%             s_i
%         \biggl]
%     +
%         % \frac{(1-\eta)}{\eta}
%         \eta\,
%         \operatorname{D}_{\operatorname{KL}}\big(
%             \mathbb{P}_w
%         \|
%             \bar{\mathbb{P}}^{\eta}
%         \big)
%     +
%     \iota(\mathbb{P}_w \ll \bar{P}^{\eta})
% ,
% \end{align}
% where the map $\iota(\mathbb{P}_w \ll \bar{P}^{\eta})$ is an ``indicator function in the sense of convex analysis''; that is, $\iota(\mathbb{P}_w \ll \bar{P}^{\eta})=0$ if $\mathbb{P}_w$ is absolutely continuous with respect to $\bar{P}^{\eta}$ and $\infty$ otherwise.  
% We may now apply \citep[Proposition 1]{WangHyndmanKratsios_EMT_2020}\footnote{This result is an extension of \citep[Proposition 2.3]{DaiPraMenghiniRunggaldier_ConnectionStochControlDynGames__1996__MathControlSigSys} which allows us to vary the influence of the regulative-entropy term in~\eqref{eq:optimizingQ__regularized__Renormalized}.} to~\eqref{eq:optimizingQ__regularized__Renormalized} deducing that it admits a minimizer $\mathbb{P}_{w^{\star}}=\sum_{i=1}^N\,w_i^{\star}\,\delta_{\theta^\star_i}$ and its Radon-Nikodym derivative with respect to the measure $\bar{\mathbb{P}}^{\eta}$ is 
% \allowdisplaybreaks
% \begin{align}
% \label{eq:optimizingQ__regularized__Renormalized____density_____BEGIN}
%     \frac{
%         d\mathbb{P}_{w^{\star}}
%     }{
%         \bar{\mathbb{P}}^{\eta}
%     }
%     (\theta^\star_i)
% = &
%         \frac{
%                 e^{
%                 \sum_{l=1}^N \, I_{\theta^\star_l=\theta^\star_i}
%                 s_i/\eta
%             }        
%         }{
%             \mathbb{E}_{\bar{\mathbb{P}^{\eta}}}\biggl[
%              \exp\big(
%                 \sum_{i=1}^N\,
%                 I_{\theta = \theta^\star_i}
%                     s_i
%                 \big)    
%             \biggr]
%         }
% \\
% \nonumber
% = &
%         \frac{
%                 e^{
%                 s_i/\eta
%             }        
%         }{
%             \sum_{k=1}^N\,
%                 \frac{e^{s_k/\eta}[s^1+\eta-s^k]_+}{
%                     \sum_{m=1}^N\,
%                     [s^1+\eta-s^m]_+
%                 }
%         }
% \\
% \label{eq:optimizingQ__regularized__Renormalized____density_____END}
% = &
%         \Big(
%             \sum_{m=1}^N\,
%                 [s^1+\eta-s^m]_+
%         \Big)
%         \,
%         \frac{
%                 e^{
%                 s_i/\eta
%             }        
%         }{
%             \sum_{k=1}^N\,
%                 e^{s_k/\eta}[s^1+\eta-s^k]_+
%         }
% \end{align}
% for $i=1,\dots,N$.  Since $\mathbb{P}_{w^{\star}}$ is a minimizer of~\eqref{eq:optimizingQ__regularized__Renormalized} then we may deduce the expression for the optimal weights $w^{\star}$ by first noting that
% \allowdisplaybreaks
% \begin{align}
% \label{eq:optimizingQ__regularized___weights____P1}
%             \mathbb{P}_{w^{\star}} 
%         \eqdef 
%             \sum_{i=1}^N\, w^{\star}_i\delta_{\theta^\star_i}\,
%         = 
%             \sum_{i=1}^N\, 
%             \frac{d\mathbb{P}_{w^{\star}}}{d\bar{\mathbb{P}^{\eta}}}(\theta^\star_i)
%             \,
%             \left(
%                 \frac{
%                     [s^1+\eta-s^i]_+
%                 }{
%                     \sum_{j=1}^N\,
%                         [s^1+\eta-s^j]_+
%                 }
%             \right)
%             \,
%             \delta_{\theta^\star_i}\,
% .
% \end{align}
% Therefore,~\eqref{eq:optimizingQ__regularized__Renormalized____density_____BEGIN}-~\eqref{eq:optimizingQ__regularized__Renormalized____density_____END} and~\eqref{eq:optimizingQ__regularized___weights____P1} imply that, for each $i=1,\dots,N$, we have 
% \allowdisplaybreaks
% \begin{align}
%     \nonumber
% % \label{eq:optimizingQ__regularized___weights}
%         w^{\star}_i 
%     = & 
%             \frac{d\mathbb{P}_{w^{\star}}}{d\bar{\mathbb{P}^{\eta}}}(\theta^\star_i)
%             \,
%             \left(
%                 \frac{
%                     [s^1+\eta-s^i]_+
%                 }{
%                     \sum_{j=1}^N\,
%                         [s^1+\eta-s^j]_+
%                 }
%             \right)
%             \,
%     \\
%     \nonumber
%     = & 
%         \Big(
%             \sum_{m=1}^N\,
%                 [s^1+\eta-s^m]_+
%         \Big)
%         \,
%         \frac{
%                 e^{
%                 s_i/\eta
%             }        
%         }{
%             \sum_{k=1}^N\,
%                 e^{s_k/\eta}[s^1+\eta-s^k]_+
%         }
%         \,
%         \left(
%             \frac{
%                 [s^1+\eta-s^i]_+
%             }{
%                 \sum_{j=1}^N\,
%                     [s^1+\eta-s^j]_+
%             }
%         \right)
%     \\
%     \nonumber
%     = & 
%         \frac{
%                 e^{
%                 s_i/\eta
%             }   
%             \,
%             [s^1+\eta-s^i]_+
%         }{
%             \sum_{k=1}^N\,
%                 e^{s_k/\eta}[s^1+\eta-s^k]_+
%         }
% .
% \end{align}
% \end{proof}

% Next we now prove our main result, namely Theorem~\ref{thm:RegretOptimal_Dynamics__MainTextFormulation}. The result is first rewritten, in the optimal control-theoretic notation introduced in Section~\ref{s:Main_ss:Algorithm}.

% \begin{theorem}[The Regret-Optimal Algorithm - Control Theoretic Form]
% \label{thm:RegretOptimal_Dynamics}
% Suppose that Assumptions~\ref{assm:bddxy} and~\ref{assm:PD} hold.  Then, the optimal control problem 
% \eqref{eq:penalized_regret_functional} and \eqref{Theta-simple} admits a unique solution for $t=0, 1, ..., T-1$ such that 
% \allowdisplaybreaks\begin{align} 
%  \boldsymbol\alpha(t)  
%  = & -[(\lambda + \beta )I_{Np} + P(t+1)]^{-1} 
%  \big[ (\lambda I_{Np} + P(t+1)) \Theta(t) 
%  - \lambda  \Theta^\star + S(t+1)  \big] ,   \label{optimala} 
% \end{align} 
% and the resulting cost is 
% \begin{align} 
% L^\star(\boldsymbol\alpha; \mathcal{D}) 
% = \Theta^{\star \top} P(0) 
% \Theta^\star + 2 S^\top(0) \Theta^\star + r(0) .
% \label{optimalL} 
% \end{align} 
% The $P(t)$, $S(t)$, and $r(t)$ in \eqref{optimala} and \eqref{optimalL} are determined by the backward equation system on $t=1,\dots,T$:  
% \allowdisplaybreaks\begin{align} 
% & \begin{cases}
%    P(t)  =  \beta I_{Np} - \beta^2 [(\lambda+\beta) I_{Np} + P(t+1) ]^{-1} , \label{eqnP(t)} \\ 
%    P(T) =  [w^\star_1 I_p ,\cdots, w^\star_N I_p]^{\top} 
%  \big( \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|}   u^i_j u^{i\top}_j \big)  
%  [ w^\star_1 I_p, \cdots, w^\star_N I_p] ,  
% \end{cases}   \\
% %%%  
% & \begin{cases}
%   S(t) =  \beta \big[ (\lambda+\beta)I_{Np} + P(t+1) \big]^{-1} (S(t+1) - \lambda \Theta^\star )
%   \label{eqnS(t)} ,     \\ 
%    S(T) =  - [ w^\star_1 I_p, \cdots, w^\star_N I_p]^{\top} \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|}  {u^i_j} y^i_j ,    
% \end{cases} \\
% %\begin{align}
% %\begin{align} 
% &\begin{cases} 
%  r(t) =  - ( S(t+1) - \lambda \Theta^\star )^\top
%  [(\lambda+\beta)I_{Np} + P(t+1)]^{-1} \cdot ( S(t+1) - \lambda \Theta^\star )   \\  
%  \hspace{1.1cm}   + \lambda \| \Theta^\star \|_2^2 + r(t+1), 
%  \label{eqnr(t)} \\ r(T) = \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|} |y^i_j|^2 . 
%  \end{cases}  
% \end{align} 
% \end{theorem} 


% \begin{proof}[Proof of Theorem~\ref{thm:RegretOptimal_Dynamics} (and therefore of Theorem~\ref{thm:RegretOptimal_Dynamics__MainTextFormulation})]
% Let $V(t, \Theta)$ be the value function associated with the optimal control problem
% \eqref{eq:penalized_regret_functional} and \eqref{Theta-simple}. 
% By the dynamic programming principle, $V(t, \Theta)$  satisfies the equation 
% \allowdisplaybreaks\begin{align} 
% & V (t, \Theta) = \min_{\boldsymbol\alpha} 
%  \Big[   \lambda \left| \Theta + \boldsymbol\alpha - \Theta^\star \right|^2 
%  + \beta \left| \boldsymbol\alpha \right|^2  
%  + V (t+1, \Theta + \boldsymbol\alpha ) \Big] , \quad t=0, 1, ..., T-1 ,   \label{dpVw} \\  
%  & V(T, \Theta ) 
% = l (\theta^{w^\star}; \mathcal{D} ) .   \label{V(T,Theta)} 
% \end{align}


% The loss function can be written as a linear quadratic function of 
% $\Theta=[\theta_1^\top, \cdots, \theta_N^\top]^\top$ such that 
% \allowdisplaybreaks\begin{align} 
%  &  l (\theta^{w^\star}; \mathcal{D} ) \notag \\ 
%  = & 
%  \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|}  \Big[ u^{i\top}_j \sum_{k=1}^N w^\star_k \theta_k - y^i_j  \Big]^2 \notag \\ 
%  = &  \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|} 
%  \Big[ \sum_{k=1}^N w_k^{\star 2} \theta_k^\top u^i_j u^{i\top}_j \theta_k 
%  -2 \sum_{k=1}^N w_k^\star y^i_j u^{i \top}_j \theta_k + |y^i_j|^2 \Big]
%  \notag \\ 
% = &  \Big(\sum_{k=1}^N w^\star_k \theta_k^\top \Big) \Big( \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|}  u^i_j u^{i\top}_j  \Big) \Big(\sum_{k=1}^N w^\star_k  \theta_k\Big) 
%  - 2 \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|} y^i_j u^{i\top}_j \sum_{k=1}^N w^\star_k \theta_k  + \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|} | y^i_j |^2 \notag \\ 
% = & \Theta^\top [w^\star_1 I_p ,\cdots, w^\star_N I_p]^\top 
%  \Big( \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|}  u^i_j u^{i\top}_j \Big)  
%  [ w^\star_1 I_p, \cdots, w^\star_N I_p ] \Theta \notag \\ 
%  & - 2 \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|} y^i_j u^{i \top}_j   
%   [ w^\star_1 I_p, \cdots, w^\star_N I_p ] \Theta 
%  + \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|} | y^i_j |^2 . \label{lwT}  
% \end{align}



% We claim that $V(t, \Theta)$ takes the linear quadratic form 
% \allowdisplaybreaks\begin{align} 
%  V (t, \Theta) 
% =  \Theta^\top P(t) \Theta + 2 S^\top (t) \Theta + r(t) . \label{ansatzVw}
% \end{align} 
% To see this, note from \eqref{V(T,Theta)} and \eqref{lwT} that 
% $V(T, \Theta)$ takes the linear quadratic form of \eqref{ansatzVw}. By solving the dynamic programming equation \eqref{dpVw} at $t=T-1$ for the optimal $\boldsymbol\alpha$ and substituting it back into the equation, we obtain $V(T-1, \Theta)$ also taking the linear quadratic form of \eqref{ansatzVw}. By backward induction we have that $V(t,\Theta)$ takes the form of \eqref{ansatzVw} for all $t=0,...,T$.  


% \begin{remark} Here $r(t)$ is a constant term independent of the ``state variable'' $\Theta$, which we note exists because the cost $L^\star$ defined by \eqref{eq:penalized_regret_functional} contains terms independent of $\Theta(t)$.
% \end{remark}

% Combining \eqref{V(T,Theta)}, 
% \eqref{lwT}, and \eqref{ansatzVw}  verifies that $P(T)$ and $S(T)$ satisfy the terminal condition as given by \eqref{eqnP(t)} and \eqref{eqnS(t)}. 
% We substitute \eqref{ansatzVw} into \eqref{dpVw} and reorganize the terms to get 
% \begin{align} 
%  & \Theta^\top P(t) \Theta + 2 S^\top(t) \Theta + r(t)  \notag \\ 
%    = &  \min_{\boldsymbol\alpha} \Big\{  \boldsymbol\alpha^\top [(\lambda + \beta ) I_{Np} + P(t+1)] \boldsymbol\alpha  
%   + 2 [ \Theta^\top P(t+1)  
%  + S^\top (t+1) +\lambda (\Theta^\top - \Theta^{\star \top})]  \boldsymbol\alpha \notag \\ 
%  & \hspace{1cm} + \Theta^\top ( \lambda I_{Np} + P(t+1) )  \Theta 
%   + 2 ( S^\top(t+1) - \lambda \Theta^\star ) \Theta + \lambda |\Theta^\star|^2 + r(t+1) \Big\} . 
%   \label{DPVansatz}
% \end{align} 
% By the first order condition\footnote{NB, we can argue this way, since the problem is convexified upon fixing $w^{\star}$.  In fact, this is the control-theoretic motivation for using Algorithm~\ref{alg:RegretOptimizationHeuristic__WarmStart} to decouple the optimization of $w$ and of $\theta_{\cdot}$ from one another, and not treating them as a single (non-convex if left coupled) control problem.} for the right-hand side of \eqref{DPVansatz} with respect to $\boldsymbol\alpha$, we have  
% \allowdisplaybreaks\begin{align} 
%  0 = &   [(\lambda+\beta) I_{Np} + P(t+1)] \boldsymbol\alpha  
%   +  [ ( \lambda I_{Np} + P(t+1) ) \Theta  
%  + S(t+1) - \lambda  \Theta^\star ]  . 
%  \label{1stOrdera}
% \end{align}
% % \Aurelien{I think there is a factor $2$ missing in front of second term.}
% % \Xuwei{
% % Taking the derivative of the right hand side of \eqref{DPVansatz} with respect to $\mathbf{a}$ and equating it to zero, we have 
% % \allowdisplaybreaks\begin{align} 
% %  0 = &   2 [(\lambda+1) I_{Np} + P(t+1)] \mathbf{a}  
% %   +  2 [ ( \lambda I_{Np} + P(t+1) ) \Theta  
% %  + S(t+1) - \lambda  \Theta^\star ]  . 
% %  \notag 
% % \end{align} 
% % Cancelling the common factor 2, we obtain \eqref{1stOrdera}. 
% % }
% By Assumption \ref{assm:PD}, we have 
% $P(T)+(\lambda+1)I_{Np} >0$, and therefore from \eqref{1stOrdera} we obtain the optimal $\boldsymbol{\alpha}$ taking the form of \eqref{optimala}. 





% % \Aurelien{I can not follow the derivation below. Would it be possible to add some intermediary steps?}\Anastasis{I agree some extra comments (just some words) would be good.}
% % \Xuwei{The proof is updated. The equations in the proof are reorganized and simplified.}
% % \Aurelien{Ok, I get it now, maybe we can add a few steps.
% % \begin{align} 
% %  & \Theta^\top  P(t) \Theta  + 2 S^\top(t) \Theta  + r(t) \notag \\ 
% %  = & - \big[ \Theta^\top (\lambda I_{Np} + P(t+1)) 
% %  + S^\top(t+1) - \lambda \Theta^{\star \top}  
% %  \big] \cdot \big[(\lambda + 1)I_{Np} + P(t+1)\big]^{-1} \cdot \notag \\ 
% %  & \big[  (\lambda I_{Np} + P(t+1)) \Theta  + S(t+1) 
% %   -  \lambda  \Theta^\star  \big]  
% %   + \Theta^\top (\lambda I_{Np} + P(t+1)) 
% %   \Theta \notag \\ 
% %  &  + 2 [ S^\top(t+1) - \lambda \Theta^{\star \top}]\Theta + \lambda |\Theta^\star|^2 + r(t+1) ,
% % \end{align} 
% % Let's isolate the term $\Theta^\top  P(t) \Theta$ to find $P(t)$:
% % \begin{align*} 
% % - \Theta^\top \underbrace{(\lambda I_{Np} + P(t+1)) \cdot \big[(\lambda + 1)I_{Np} + P(t+1)\big]^{-1} \cdot (\lambda I_{Np} + P(t+1))}_A \Theta
% % + \Theta^\top \underbrace{(\lambda I_{Np} + P(t+1))}_B \Theta
% % \end{align*} 
% % Focusing on the term $A$, we have
% % \begin{align*} 
% % & - ( (\lambda + 1 ) I_{Np} + P(t+1) - I_{Np}) \cdot \big[(\lambda + 1)I_{Np} + P(t+1)\big]^{-1} \cdot (\lambda I_{Np} + P(t+1)) \\
% % &= - (\lambda I_{Np} + P(t+1))
% % + \big[(\lambda + 1)I_{Np} + P(t+1)\big]^{-1} \cdot (\lambda I_{Np} + P(t+1))
% % \end{align*} 
% % %
% % Therefore,
% % \begin{align*}
% % A + B &= \big[(\lambda + 1)I_{Np} + P(t+1)\big]^{-1} \cdot (\lambda I_{Np} + P(t+1)) \\
% % &= \big[(\lambda + 1)I_{Np} + P(t+1)\big]^{-1} \cdot ((\lambda + 1) I_{Np} - I_{Np} + P(t+1)) \\
% % &= I_{Np} - \big[(\lambda + 1)I_{Np} + P(t+1)\big]^{-1}.
% % \end{align*}
% % } 
% % \Xuwei{Equations \eqref{eqn:P-unsimplified}, \eqref{eqn:P-simplified}, 
% % \eqref{eqn:S-unsimplified}, \eqref{eqn:S-simplified}, which integrate the Aurelien's steps above, are added to supplement more details of deriving equations \eqref{eqnP(t)} and \eqref{eqnS(t)} for $P$ and $S$. } 

% We further substitute $\boldsymbol{\alpha}$ of the form \eqref{optimala} into the right side of \eqref{DPVansatz} to obtain 
% \allowdisplaybreaks\begin{align} 
%  & \Theta^\top  P(t) \Theta  + 2 S^\top(t) \Theta  + r(t) \notag \\ 
%  = & - \big[ \Theta^\top (\lambda I_{Np} + P(t+1)) 
%  + S^\top(t+1) - \lambda \Theta^{\star \top}  
%  \big] \cdot \big[(\lambda + \beta )I_{Np} + P(t+1)\big]^{-1} \cdot \notag \\ 
%  & \big[  (\lambda I_{Np} + P(t+1)) \Theta  + S(t+1) 
%   -  \lambda  \Theta^\star  \big]  
%   + \Theta^\top (\lambda I_{Np} + P(t+1)) 
%   \Theta \notag \\ 
%  &  + 2 [ S^\top(t+1) - \lambda \Theta^{\star \top}]\Theta + \lambda |\Theta^\star|^2 + r(t+1) . 
%   \label{eqn:Vansatz}
% \end{align} 
% Reorganizing the terms on right side of \eqref{eqn:Vansatz}, we have 
% \begin{align} 
%  & \Theta^\top  P(t) \Theta  + 2 S^\top(t) \Theta  + r(t) \notag \\ 
%  = & - \Theta^\top   (\lambda I_{Np} + P(t+1) ) [(\lambda + \beta )I_{Np} + P(t+1)]^{-1} 
%  (\lambda I_{Np} + P(t+1))   \Theta \notag \\ 
%  & + \Theta^\top ( \lambda I_{Np} + P(t+1) ) \Theta + 2 [ S^\top(t+1) - \lambda \Theta^{\star \top}]\Theta  \notag \\  
%  & - 2 [S^\top(t+1) - \lambda \Theta^{\star \top}] 
%  [(\lambda +\beta )I_{Np} + P(t+1) ]^{-1} (\lambda I_{Np} + P(t+1)) \Theta \notag \\  
%  & - (S^\top(t+1) - \lambda \Theta^{\star\top}) [(\lambda + \beta )I_{Np} + P(t+1)]^{-1} (S(t+1) - \lambda \Theta^\star)  
%  \notag \\
%  & + \lambda |\Theta^\star|^2 + r(t+1) . 
%   \label{eqn:Vansatz-simplified} 
% \end{align} 
% %Since $\Theta$ is arbitrary, 
% Matching the coefficients of the quadratic terms of $\Theta$ on both sides of \eqref{eqn:Vansatz-simplified}, we obtain 
% \begin{align} 
%  P(t)  
%   = &  -  (\lambda I_{Np} + P(t+1) ) [(\lambda + \beta )I_{Np} + P(t+1)]^{-1} 
%  (\lambda I_{Np} + P(t+1))   \notag \\ 
%  & +   \lambda I_{Np} + P(t+1) .  
%  \label{eqn:P-unsimplified}
% \end{align} 
% The right side of 
% \eqref{eqn:P-unsimplified} further simplifies to  
% \begin{align} 
% & -  (\lambda I_{Np} + P(t+1) ) [(\lambda + \beta )I_{Np} + P(t+1)]^{-1} 
%  (\lambda I_{Np} + P(t+1))   
%   +  \lambda I_{Np} + P(t+1)   \notag \\ 
%  = &   -  [ ( \lambda + \beta ) I_{Np} + P(t+1) - \beta I_{Np} ]  [(\lambda + \beta )I_{Np} + P(t+1)]^{-1} 
%  (\lambda I_{Np} + P(t+1)) \notag \\
%  & +  \lambda I_{Np} + P(t+1)  \notag \\ 
%  = & -   ( \lambda  I_{Np} + P(t+1) )  + \beta [(\lambda + \beta )I_{Np} + P(t+1)]^{-1} 
%  (\lambda I_{Np} + P(t+1))  
%   +  \lambda I_{Np} + P(t+1) \notag \\ 
%   = & 
%   \beta [(\lambda + \beta )I_{Np} + P(t+1)]^{-1} 
%  (\lambda I_{Np} + P(t+1))  \notag \\ 
%  = & 
%   \beta [(\lambda + \beta )I_{Np} + P(t+1)]^{-1} 
%  [ ( \lambda + \beta ) I_{Np} + P(t+1) - \beta I_{Np} ] \notag  \\ 
%  = & \beta I_{Np} - \beta^2 [(\lambda + 1)I_{Np} + P(t+1)]^{-1} . 
%  \label{eqn:P-simplified}
% \end{align} 
% Combining \eqref{eqn:P-unsimplified}
% and \eqref{eqn:P-simplified} gives \eqref{eqnP(t)} for $t=T-1$. 

% Matching the coefficients of the linear terms of $\Theta$ on both sides of \eqref{eqn:Vansatz-simplified} and taking the transpose, we obtain  
% \begin{align} 
%  S(t) = & - (\lambda I_{Np} + P(t+1) ) [(\lambda + \beta )I_{Np} + P(t+1) ]^{-1} ( S(t+1) - \lambda \Theta^\star ) \notag \\ 
% & +  S(t+1) - \lambda \Theta^\star .  
%  \label{eqn:S-unsimplified} 
% \end{align} 
% The right side of \eqref{eqn:S-unsimplified} further simplifies to 
% \begin{align} 
% & - (\lambda I_{Np} + P(t+1) ) [(\lambda +  \beta )I_{Np} + P(t+1) ]^{-1} ( S(t+1) - \lambda \Theta^\star ) 
%  + S(t+1) - \lambda \Theta^\star 
%   \notag \\ 
% = &   - [ (\lambda + \beta ) I_{Np} + P(t+1) - \beta I_{Np} ] [(\lambda + \beta )I_{Np} + P(t+1) ]^{-1} ( S(t+1) - \lambda \Theta^\star ) \notag \\ 
% & + S(t+1) - \lambda \Theta^\star 
% \notag \\ 
%  = & - ( S(t+1) - \lambda \Theta^\star ) 
%   + \beta [(\lambda +\beta )I_{Np} + P(t+1) ]^{-1} ( S(t+1) - \lambda \Theta^\star ) 
%   + S(t+1) - \lambda \Theta^\star 
%   \notag \\ 
%  = &  \beta [(\lambda + \beta )I_{Np} + P(t+1) ]^{-1} ( S(t+1) - \lambda \Theta^\star ) . \label{eqn:S-simplified}
% \end{align}
% Combining \eqref{eqn:S-unsimplified} and \eqref{eqn:S-simplified} gives \eqref{eqnS(t)} for $t=T-1$. 

% Matching the terms independent of $\Theta$ on both sides of \eqref{eqn:Vansatz-simplified} gives 
% \begin{align} 
%  r(t) = &  - ( S(t+1) - \lambda \Theta^\star )^\top
%  [(\lambda+ \beta )I_{Np} + P(t+1)]^{-1} \cdot ( S(t+1) - \lambda \Theta^\star ) \notag    \\  
%  &  + \lambda |\Theta^\star|^2 + r(t+1) , \notag 
% \end{align} 
% which is \eqref{eqnr(t)} for $t=T-1$. 


% Since 
% $P(T) + (\lambda + \beta )I_{Np} > \beta I_{Np}$, 
% we have 
% \begin{align} 
% P(T-1) = \beta I_{Np} 
%  - \beta^2 [(\lambda + \beta )I_{Np} + P(T)]^{-1} > 0 . \notag 
% \end{align} 
% By backward induction on $t$, we can show that 
% $\boldsymbol{\alpha}$ takes the form of \eqref{optimala} for all $t=0, 1, ..., T-1$, and $P$ and $S$ satisfy the system \eqref{eqnP(t)} and \eqref{eqnS(t)}.  
% \end{proof} 

% \begin{corollary} 
% \label{cor:M(P)invbdd}
% Under Assumptions~\ref{assm:bddxy} and \ref{assm:PD}, the solution $P$ and $S$ of the system \eqref{eqnP(t)}-\eqref{eqnS(t)} satisfies that for all $t=1$, $2$, ..., $T$, 
% \begin{align} 
% & | [(\lambda + \beta) I_{Np} + P(t)]^{-1} |\leq  (\lambda + \beta)^{-1},  \label{M(P)invbd}  \\ 
%  & |S(t)| \leq C \cdot N 
%  \label{|S|bd} , 
% \end{align} 
% where $C> 0$ is a constant depending on $\lambda$, $\beta$, $(w_1^\star, ..., w_N^\star)$, $\Theta^\star$, $K_x$, $K_y$ and $T$. 
% \end{corollary} 


% \begin{proof}[Proof of Corollary~\ref{cor:M(P)invbdd}] 
% Let $\| \cdot \|$ be the spectral norm of a matrix such that $\|A\|\eqdef \sup_{x\neq 0} |Ax|/|x| $. 
% Since $P(t)$ is positive semi-definite, we have $(\lambda + \beta) I_{Np} + P(t) \geq (\lambda + \beta) I_{Np}$ and  
% \begin{align} 
% 0\leq [(\lambda + \beta) I_{Np} + P(t) ]^{-1} \leq (\lambda + \beta)^{-1} I_{Np}   ,  \notag 
% \end{align} 
% which, by the Courant-Fisher Theorem (see \cite{hornjohnson2012}), implies that $\|  [(\lambda + \beta) I_{Np} + P(t) ]^{-1} \| \leq \| (\lambda+\beta)^{-1} I_{Np} \| = (\lambda + \beta)^{-1}$. 
% Since all norms of finite dimensional normed spaces are equivalent, and in particular, $|\cdot|\le \|\cdot\|$ on the space of $N_p\times N_p$-matrices, then we find that
% \begin{align} 
%   \big| [(\lambda + \beta) I_{Np} + P(t) ]^{-1} \big| \leq \|  [(\lambda + \beta) I_{Np} + P(t) ]^{-1} \| , \notag 
% \end{align}  
% and thus $\big| [(\lambda + \beta) I_{Np} + P(t) ]^{-1} \big| \leq (\lambda + \beta)^{-1}$,  
% which proves \eqref{M(P)invbd}. 

% %\noindent 
% Next, we prove \eqref{|S|bd}. 
% By Lemmas~\ref{lm:|AB|<=|A||B|} and \ref{lm:|A1+An|2<=(|A1|2+|An|2)n}, and \eqref{eq:moredatasets_than_dataperdataset}, we obtain 
% \allowdisplaybreaks
% \begin{align} 
%  | S(T) |^2  
%  = & \Big( \sum_{i=1}^N w^{\star 2}_i \Big) 
%  \Big| \sum_{i=1}^N w^\star_i   \sum_{j=1}^{|\mathcal{D}_i|}  u^i_j y^i_j  \Big|^2  
%  \leq  \Big( \sum_{i=1}^N w^{\star 2}_i \Big) 
%  \sum_{i=1}^N w_i^\star  \Big| \sum_{j=1}^{|\mathcal{D}_i|}   u^i_j y^i_j \Big|^2  \notag  \\ 
%  \leq &  \Big( \sum_{i=1}^N w^{\star 2}_i \Big) 
%  \sum_{i=1}^N w_i^\star |\mathcal{D}_i|  \sum_{j=1}^{|\mathcal{D}_i|}   | u^i_j y^i_j |^2  
%  \leq  \Big( \sum_{i=1}^N w^{\star 2}_i \Big) \sum_{i=1}^N w_i^\star |\mathcal{D}_i|^2  K_x^2 K_y^2  \notag \\ 
%   \leq &  \Big( \sum_{i=1}^N w^{\star 2}_i \Big) \sum_{i=1}^N w_i^\star N^2  K_x^2 K_y^2 ,  
%   \label{eq:TBBounded} 
% \end{align} 
% and therefore the estimate \eqref{|S|bd} holds for $t=T$. 
% %By the relationship between the $\ell^1$ and $\ell^2$ norms on $\mathbb{R}^N$, 
% %we have that $\Big(\sum_{i=1}^N\,w_i^{\star \, 2}\Big)^{1/2}\le \sum_{i=1}^N\,|w_i^{\star}|$.  Since $(w^{\star}_i)_{i=1}^N$ belongs to the $N$-simplex then, by definition, $w_1^{\star},\dots,w_N^{\star}\ge 0$ and $\sum_{i=1}^n\,w_i^{\star}=1$.  Thus, 
% %\[
% %        \Big(\sum_{i=1}^N\,w_i^{\star \, 2}\Big)^{1/2}
% %    \le 
% %        \sum_{i=1}^N\,|w_i^{\star}|
% %    = 
% %        \sum_{i=1}^N\,w_i^{\star}
% %    =
% %        1
% %    .
% %\]
% %Consequentially, $\sum_{i=1}^N\,w_i^{\star \, 2}\le 1$; whence the right-hand side of the estimate~\eqref{eq:TBBounded} reduces %to
% %\allowdisplaybreaks
% %\begin{align} 
% % | S(T) |^2  
% % \le 
% % N^2  K_x^2 K_y^2  .
% %\end{align} 

% Assume by induction that \eqref{|S|bd} holds for $t=u$.  
% By \eqref{eqnS(t)}, Lemma~\ref{lm:|AB|<=|A||B|}, and the triangle inequality, we have 
% \begin{align} 
%  |S(u-1)| \leq &  \beta \big| \big[ (\lambda+\beta)I_{Np} + P(u) \big]^{-1} \big| \cdot \big| S(u) - \lambda \Theta^\star  \big| \notag \\ 
%   \leq & \beta \big| \big[ (\lambda+\beta)I_{Np} + P(u) \big]^{-1} \big| \cdot ( |S(u)| + \lambda | \Theta^\star | ) . 
%   \notag 
% \end{align} 
% The estimate \eqref{|S|bd} for $t=u-1$ then follows from \eqref{M(P)invbd} and the induction hypothesis. 
% Thus, by induction we have shown that \eqref{M(P)invbd} holds for all $t=1$, $2$, ..., $T$. 
% \end{proof} 


% We proceed to prove Theorem~\ref{thm:ComplexityAlgorithm} about the complexity of the regret-optimal algorithm. 
% To facilitate the proof, we introduce the following Lemma~\ref{lm:matCompComplexity} that summarizes complexities of matrix operations. 
% \begin{lemma} 
% \label{lm:matCompComplexity} 
% %Since we will be assuming that we work with \textit{floating-point arithmetic}, 
% Suppose all elementary arithmetic operations (e.g.\ addition, subtraction, multiplication) of two real numbers are of constant (i.e.\ $\mathcal{O}(1)$) complexity. Then elementary matrix computations have the following complexities: 

% \begin{enumerate}  
% \item[(i)] Adding two $n_1 \times n_2$ matrices has a complexity of $O(n_1 n_2)$. 

% \item[(ii)] Multiplying an $n_1 \times n_2$ matrices by a scalar has a complexity of $O(n_1 n_2)$. 

% \item[(iii)] Multiplying an $n_1 \times n_2$ matrix with an $n_2 \times n_3$ matrix has a complexity of $O(n_1 n_2 n_3)$. 
% In particular, multiplying two $n\times n$ matrices has a complexity of $\mathcal{O}(n^{2.373})$.  
% \end{enumerate} 
% \end{lemma} 

% \begin{proof} 
% Adding two $n_1\times n_2$ matrices involves adding each entry of one matrix with the corresponding entry of the other matrix, and each entry addition has a complexity of $\mathcal{O}(1)$. Hence the total complexity is $\mathcal{O}(n_1 n_2)$. 

% Multiplying an $n_1 \times n_2$ matrix by a scalar involves multiplying each entry by the scalar, and the scalar multiplication of each entry has a complexity of $\mathcal{O}(1)$. Hence the total complexity is $O(n_1 n_2)$. 

% Multiplication of an $n_1 \times n_2$ matrix and an $n_2 \times n_3$ matrix requires multiplying the $n_1$ row vectors of the first matrix by the $n_3$ column vectors of the second matrix, which needs a total of $n_1 n_3$ multiplications. Multiplication of two $n_2$-dimensional vectors has a complexity of $O(n_2)$. Therefore the total complexity is $O(n_1n_2n_3)$.  
% When multiplying two matrices of $n\times n$-dimension with an optimized CW-like algorithm the complexity is $\mathcal{O}(n^{2.373})$. 
% \end{proof} 


% %\Anastasis{Check complexity again with modificaitons.}
% \begin{proof}[{Proof of Theorem~\ref{thm:ComplexityAlgorithm}}] 
% \hfill\\
% \noindent\textbf{Complexity of Computing $P(T)$ is $\mathcal{O}\big(N^2p^3\big)$}\hfill\\
% Since $u^i_j \in \mathbb{R}^{p\times 1}$, computing each 
% $u^i_j u^{i\top}_j$ has $\mathcal{O}(p^2)$ complexity, by Lemma \ref{lm:matCompComplexity}-(iii). 
% Multiplying the $p\times p$ matrix $u^i_j u^{i\top}_j$ by the scalar $w^\star_i$ has a complexity of $\mathcal{O}(p^2)$, by Lemma~\ref{lm:matCompComplexity}-(iii).   
% %Adding two $n_1 \times n_2$ matrices has a complexity of $\mathcal{O}(n_1 n_2)$. 
% %Multiplying an $n_1\times n_2$ matrix by a scalar has a complexity of $\mathcal{O}(n_1 n_2)$.    
% Then computing the $p\times p$ matrix $\sum_{i=1}^N w^\star_i \sum_{j=1}^{S_i}\, u^i_j u^{i\top}_j$ by adding the $\bar{N}$ matrices of dimension $p\times p$ has complexity $\mathcal{O}(\bar{N}\,p^2)$, by Lemma \ref{lm:matCompComplexity}-(i).  
% Since $[w_1^\star I_p ,\cdots, w_N^\star I_p]^{\top}$ is $Np\times p$-dimensional, then computing the $np\times p$-dimensional product $[w_1^\star I_p ,\cdots, w_N^\star I_p]^{\top}\sum_{i=1}^N w^\star_i \sum_{j=1}^{S_i}\, u^i_j u^{i \top}_j$ has $\mathcal{O}(Np^3)$ complexity, by Lemma~\ref{lm:matCompComplexity}-(iii). 
% %Likewise, since the product $[w_1^\star I_p ,\cdots, w_N^\star I_p]^{\top}\sum_{i=1}^N\, w^\star_i \sum_{j=1}^{S_i}\,u^i_j 
% %u^{i\top}_j$ is $Np\times p$-dimensional 
% Likewise, the product 
% \[ 
%     \Big([w_1^\star I_p ,\cdots, w_N^\star I_p]^{\top}\sum_{i=1}^N  w^\star_i \sum_{j=1}^{S_i}\, u^i_j u^{i\top}_j \Big)[w_1^\star I_p ,\cdots, w_N^\star I_p]
% \]
% has a complexity of $\mathcal{O}(N^2p^3)$.  Therefore, computing $P(T)$ itself is of $\mathcal{O}\big(\bar{N}p^2+N^2p^3\big)$ complexity.  
% Assumption~\eqref{eq:moredatasets_than_dataperdataset} implies that $\bar{N}\leq N^2$; hence, the complexity of computing $P(T)$ is $\mathcal{O}\big(N^2p^3\big)$. 


% % \hfill\\
% \noindent
% \textbf{Complexity of Computing $S(T)$ is $\mathcal{O}\big(Np\max\{N,p\}\big)$}
% \hfill\\ 
% Since $u^i_j\in\mathbb{R}^{p\times 1}$ and $y^i_j\in \mathbb{R}$, 
% computing the product $u^i_j y_j^i$ has complexity $\mathcal{O}(p)$, by Lemma \ref{lm:matCompComplexity}-(iii). 
% And multiplying the $p\times 1$ dimensional vector $u^i_j y^i_j$ by the scalar $w^\star_i$ has complexity $\mathcal{O}(p)$, by Lemma \ref{lm:matCompComplexity}-(ii). Then the complexity of computing $\sum_{i=1}^N w^\star_i \sum_{j=1}^{S_i}\,u^i_j y_j^i$ by adding $\bar{N}$ vectors of dimension $p$ is $\mathcal{O}\big(\bar{N}p\big)$, by Lemma~\ref{lm:matCompComplexity}-(i). 
% Since $- [ w_1^\star I_p, \cdots, w_N^\star I_p]^{\top}$ is an $Np\times p$-dimensional matrix and $\sum_{i=1}^N w^\star_i \sum_{j=1}^{S_i}\, u^i_j y_j^i$ is a $p\times 1$-dimensional vector, then computing their $Np\times 1$ dimensional product has $\mathcal{O}(Np^2)$ complexity, according to Lemma~\ref{lm:matCompComplexity}-(iii).  
% Therefore, the computing $S(T)$ has a complexity of $\mathcal{O}(\bar{N}p + N P^2)$. 
% Since~\eqref{eq:moredatasets_than_dataperdataset} implies that $\bar{N}\le N^2$ then, computing $S(T)$ had a computational cost of $\mathcal{O}\big(Np\max\{N,p\}\big)$.


% % \hfill\\
% \noindent
% \textbf{Complexity of Computing $P(t)$ and $S(t)$ for $t=T-1,\dots, 1$ is $\mathcal{O}\big(T(Np)^{2.373}\big)$}
% \hfill\\
% The complexity of computing $(\lambda +\beta )I_{Np} + P(t+1)$ for each $t$ is $\mathcal{O}(Np)$, since we only need to add scalars on the matrix's \textit{diagonal}.  By \cite{LeGall_Complexity_CWLikeMatrixInversion_2014}, computing the matrix inverse $[(\lambda+\beta)I_{Np}+P(t+1)]^{-1}$ with a CW-like algorithm has a complexity of $\mathcal{O}\big((Np)^{2.373}\big)$.  
% Since the addition $\beta I_{Np} - \beta^2 [(\lambda+ \beta )I_{Np} + P(t+1) ]^{-1}$ only requires us to multiply all entries of $ [(\lambda+\beta)I_{Np} + P(t+1) ]^{-1}$ by $-\beta^2$ and add along the diagonal, then it has a complexity of $\mathcal{O}\big((Np)^2 + Np\big)$, by Lemma~\ref{lm:matCompComplexity}-(i) and (ii). 
% Performing the matrix addition $S(t+1)-\lambda \Theta^\star$ has complexity $\mathcal{O}(Np)$ by Lemma~\ref{lm:matCompComplexity}-(i).  
% Computing the $Np\times 1$-dimensional product 
% $[(\lambda+1)I_{Np} + P(t+1)]^{-1} (S(t+1) - \lambda \Theta^\star)$ 
% by multiplying an $Np\times Np$ matrix by an $Np\times 1$ matrix has complexity $\mathcal{O}(N^2 p^2)$, according to Lemma~\ref{lm:matCompComplexity}-(iii). 
% Therefore, computing each $P(t)$ and $S(t)$ for $t=T-1,\dots,1$, has complexity  $\mathcal{O}\big((Np)^{2.373}\big)$.  Since there are $T-1$ such matrices to compute, then the total cost of computing every $P(T-1),\dots,P(1)$ and $S(T-1)$, ..., $S(1)$ is $\mathcal{O}\big(T(Np)^{2.373}\big)$.



% % \hfill\\\noindent
% %\textbf{Complexity of Computing $S(t)$ for $t=1,\dots,T-1$ is $\mathcal{O}(T\,N^2p^2)$} \hfill\\ 
% %We fix $t\in\{1,\dots,T-1\}$ and assume $S(t+1)$ and $P(t+1)$ have already been computed.
% %The complexity of computing $(\lambda +\beta) I_{Np} + P(t+1)$ is $\mathcal{O}(Np)$ since we only need to add $(\lambda + \beta)$ to each diagonal element of $P(t+1)$.  The complexity of computing $[(\lambda+\beta)I_{Np} + P(t+1)]^{-1}$ is $\mathcal{O}\big(Np)^{2.373}\big)$ by \cite{LeGall_Complexity_CWLikeMatrixInversion_2014}. 
% %The complexity of performing the matrix addition $S(t+1)-\lambda \Theta^\star$ is $\mathcal{O}(Np)$. 
% %The complexity of performing the matrix multiplication $[(\lambda+1)I_{Np} + P(t+1)]^{-1} (S(t+1) - \lambda \Theta^\star)$ is $\mathcal{O}(N^2 p^2)$. 
% %Therefore, the complexity of computing $S(t)$ for $t=1,\dots,T-1$ is $\mathcal{O}(T\,N^2 p^2)$

% %The complexity of performing all the matrix multiplications $(M(P(t+1)))^{-1} \lambda I$, $ (M(P(t+1)))^{-1} \lambda I (M(P(t+1)))^{-1} P(t+1)$, and $(M(P(t+1)))^{-1} P(t) (M(P(t+1)))^{-1} \lambda I$ is $\mathcal{O}\big(N^3p^3\big)$; and the cost of adding their entries is of lower complexity namely $\mathcal{O}(N^2p^2)$.  Therefore, the cost of computing $M(P(t+1))^{-1}S(t+1)$ is $\mathcal{O}(N^2p^3)$. Since $\Theta^{\star}$ is a $Np\times p$-dimensional matrix then cost computing $H(P(t+1))\Theta^{\star}$ is $\mathcal{O}(N^2p^3)$.  Since all matrix additions involved in computing $S(t)$ are comparatively negligible, then the cost of computing $S(t)$ is $\mathcal{O}(N^3p^3)$ (nb, the most costly operation has been computing the matrix product $M(P(t+1))^{-1}M(P(t+1))^{-1}$).  Thus, the complexity of computing each $S(t)$ for $t=0,\dots,T-1$ is $\mathcal{O}(T\,N^3p^3)$.



% \noindent
% \textbf{The Cost of Computing Each $\Theta(t)$ is $\mathcal{O}(T\,N^2p^2)$}
% \hfill\\
% %Suppose that $P(t+1)$, $S(t+1)$, and $\Theta(t)$ have been computed.  
% To compute $\Theta(t)$ for all $t=1$, $\dots$, $T$, starting from $\Theta(0)=\Theta^\star$, 
% we need to compute $\mathbf{a}(t)$ given by \eqref{optimala} for $t=0$, $1$, $\dots$, $T-1$.  
% Hence we need to quantify the complexity of computing $\mathbf{a}(t)$. 
% %The complexity of computing $(\lambda + \beta)I_{Np} + P(t+1)$ is $\mathcal{O}(Np)$ since we only need to add $(\lambda+\beta)$ to each of $P(t+1)$'s diagonal elements. 
% %By~\cite{LeGall_Complexity_CWLikeMatrixInversion_2014}, the complexity of computing $-[(\lambda + \beta)I_{Np} + P(t+1)]^{-1}$ with a CW-like algorithm is $\mathcal{O}\big((Np)^{2.373}\big)$. 
% By \eqref{eqnP(t)}, we can obtain $-[(\lambda + \beta)I_{Np} + P(t+1)]^{-1}$ by computing 
% $\beta^{-2}(P(t)- \beta I_{Np})$, which involves adding a scalar to the diagonal of an $Np\times Np$ matrix, and then multiplying the matrix by a scalar. 
% The cost of computing the product
% $(\lambda I_{Np} + P(t+1)) \Theta(t)$ is $\mathcal{O}(N^2 p^2)$ and the cost of computing all sums in $(\lambda I_{Np} + P(t+1)) \Theta(t) 
%  - \lambda \Theta^\star + S(t+1)  $ are of lower order complexity.  Finally, the cost of computing the matrix-product between $-[(\lambda + \beta)I_{Np} + P(t+1)]^{-1} $ and $
%  \big[ (\lambda I_{Np} + P(t+1)) \Theta(t) 
%  - \lambda \Theta^\star + S(t+1)  \big]$ is $\mathcal{O}(N^2p^2)$, by Lemma~\ref{lm:matCompComplexity}-(iii). Therefore, the cost of computing each $\mathbf{a}(t)$ is $\mathcal{O}(N^2p^2)$, and therefore the cost of computing $\Theta(t)$ for all $t=1$, ..., $t=T$ from $\Theta(0)=\Theta^\star$ is $\mathcal{O}(T N^2 p^2)$.  
%  %have been computed is $\mathcal{O}(T\,N^2p^2)$.  

% \noindent
% \textbf{Tallying up Complexities: The Complexity of Computing $(\Theta(t))_{t=0}^T$ is 
% $\mathcal{O}( N^2 p^3 + T\, (N p)^{2.373})$.}
% \hfill\\
% Looking over all computations involved, we deduce that the cost of computing the sequence $(\Theta(t))_{t=1}^T$ is (in order) dominated by the computational complexity of computing the sequence $(P(t))_{t=1}^{T-1}$ and $P(T)$; whence it is 
% $\mathcal{O}( N^2 p^3 + T\, (N p)^{2.373})$. 
% %$\mathcal{O}(T\, N^{2.373}\, p^2)$.
% \end{proof}  




% The following Lemma~\ref{lem:stability_wrtData}, 
% Proposition~\ref{prop:stabilityControl}, and Corollary~\ref{cor:stabilityLast} are devoted to proving Theorem~\ref{thrm:adv_robust}, the adversarial robustness of Algorithm~\ref{alg:RegretOptimization}. 



% We introduce the linear map $M(\cdot): \mathbb{R}^{Np\times Np} \to \mathbb{R}^{Np\times Np}$ such that $M(Q) = (\lambda + \beta) I_{Np} + Q$ for any $Q\in \mathbb{R}^{Np\times Np}$. 
% \begin{lemma} 
% \label{lem:stability_wrtData}
% Given any two data sets $\mathcal{D}=\cup_{i=1}^N \mathcal{D}_i=\cup_{i=1}^N \cup_{j=1}^{|\mathcal{D}_i|} 
%  \{(x^i_j, y^i_j) \}$ and 
% $\widetilde{\mathcal{D}}=\cup_{i=1}^N \widetilde{\mathcal{D}}_i = \cup_{i=1}^N \cup_{j=1}^{|\mathcal{D}_i|}  \{(\tilde{x}^i_j, \tilde{y}^i_j) \}$ satisfying Assumption \ref{assm:bddxy}, let $(P, S)$ and $(\widetilde{P}, \widetilde{S})$ be the solutions of \eqref{eqnP(t)}-\eqref{eqnS(t)} corresponding to $\mathcal{D}$ and $\widetilde{\mathcal{D}}$, respectively. Then, for all $t=1, ..., T$, we have 
% \allowdisplaybreaks\begin{align}  
%     \big| P(t) - \widetilde{P}(t) \big| 
%  \le &
%      C \cdot \Big[ \sum_{i=1}^N w^\star_i |\mathcal{D}_i| \sum_{j=1}^{|\mathcal{D}_i|} | u^i_j - \tilde{u}^i_j |^2 \Big]^{1/2} , 
%  \label{eqn:estP-tildeP} 	 \\ 
%  %%%
%      \big| [ M(P(t)) ]^{-1} - [ M(\widetilde{P}(t)) ]^{-1} \big| 
%  \le&  
%      C \cdot \Big[ \sum_{i=1}^N w^\star_i |\mathcal{D}_i| \sum_{j=1}^{|\mathcal{D}_i|} | u^i_j - \tilde{u}^i_j |^2 \Big]^{1/2} ,  
%     \label{eqn:estM-tildeM} \\ 
% %%%
%         |S(t) - \widetilde{S}(t)| 
%     \le &
%       C \cdot \Big[ \sum_{i=1}^N w^\star_i |\mathcal{D}_i|  \sum_{j=1}^{|\mathcal{D}_i|} | u^i_j - \tilde{u}^i_j |^2 
%      + |y^i_j - \tilde{y}^i_j |^2 \Big]^{1/2} , 
% \label{eqn:estS-tildeS} 
% \end{align}
% where $C> 0$ is a constant depending on $\lambda$, $\beta$, $N$, $\bar{N}$, $(w_1^\star, ..., w_N^\star)$, $\Theta^\star$, $K_x$, $K_y$ and $T$. 
% \end{lemma}


% \begin{proof}%[{Proof of Lemma~\ref{lem:stability_wrtData}}]
% We let $C$ be a constant depending on $\lambda$, $\beta$, $N$, $\bar{N}$, $\Theta^\star$, $(w_1^\star, ..., w_N^\star)$, $K_x$, $K_y$, and $T$,  
% and allow $C$ to vary from place to place throughout the proof. 
% We employ backward induction starting from $t=T$ to prove \eqref{eqn:estM-tildeM}, \eqref{eqn:estP-tildeP}, and 
% \eqref{eqn:estS-tildeS}. 

% From \eqref{eqnP(t)}, the terminal condition $| P(T) - \widetilde{P}(T) |^2$ can be written as 
% \allowdisplaybreaks\begin{align} 
%  \big| P(T) - \widetilde{P}(T) \big|^2  
%  = &   \Big| [w_1^\star I_p ,\cdots, w_N^\star I_p ]^\top
%  \Big[ \sum_{i=1}^N w_i^\star  \sum_{j=1}^{|\mathcal{D}_i|}  ( u^i_j u^{i\top}_j  - \tilde{u}^i_j \tilde{u}^{i\top}_j  ) \Big]  
%  [ w_1^\star I_p, \cdots, 
%  w_N^\star I_p ]  \Big|^2 \notag \\ 
%  = & \sum_{k, l=1}^N 
%   w_k^{\star 2} 
%   w_l^{\star 2} 
%  \Big| \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|}  ( u^i_j u^{i\top}_j  - \tilde{u}^i_j \tilde{u}^{i\top}_j  ) \Big|^2 . \notag 
%  \end{align} 
% By Lemmas~\ref{lm:|AB|<=|A||B|} and \ref{lm:|A1+An|2<=(|A1|2+|An|2)n}, we have 
%  \begin{align} 
%  \big| P(T) - \widetilde{P}(T)  \big|^2  
%  \leq &   \sum_{k, l=1}^N w_k^{\star 2} w_l^{\star 2} 
%   \sum_{i=1}^N w_i^\star   
% \Big| \sum_{j=1}^{|\mathcal{D}_i|} 
%     (  u^i_j u^{i\top}_j  - \tilde{u}^i_j \tilde{u}^{i\top}_j  ) \Big|^2 
% \notag \\ 
%  \leq &   \sum_{k, l=1}^N w_k^{\star 2} w_l^{\star 2} 
%   \sum_{i=1}^N w_i^\star |\mathcal{D}_i|  \sum_{j=1}^{|\mathcal{D}_i|} 
%     \big| u^i_j u^{i\top}_j  - 
% \tilde{u}^i_j \tilde{u}^{i\top}_j  \big|^2 
% \notag \\ 
% %%% 
%  = &   \sum_{k, l=1}^N w_k^{\star 2} w_l^{\star 2} 
%   \sum_{i=1}^N 
%   w_i^\star |\mathcal{D}_i| \sum_{j=1}^{|\mathcal{D}_i|}  
% \big| ( u^i_j - \tilde{u}^i_j  )u^{i\top}_j  
%  + \tilde{u}^i_j (u^{i\top}_j - \tilde{u}^{i\top}_j)   \big|^2  \notag \\ 
% %%%
% \leq &   \sum_{k, l=1}^N w_k^{\star 2} w_l^{\star 2} 
%     \sum_{i=1}^N w_i^\star |\mathcal{D}_i| \sum_{j=1}^{|\mathcal{D}_i|}  
%  2 \big( \big|  u^i_j - \tilde{u}^i_j   \big|^2 \cdot \big| u^i_j \big|^2 
%  + \big| \tilde{u}^i_j \big|^2 \cdot \big| u^i_j - \tilde{u}^i_j  \big|^2 \big) 
%  \notag \\ 
%  \leq &   \sum_{k, l=1}^N w_k^{\star 2} w_l^{\star 2} 
%   \sum_{i=1}^N w_i^\star |\mathcal{D}_i|  \sum_{j=1}^{|\mathcal{D}_i|} 4 K_x^2 
% \big| u^i_j - \tilde{u}^i_j   \big|^2 
% . \label{estP(T)-tildeP(T)}   
% \end{align}
% %Combining \eqref{estP(T)-tildeP(T)} and \eqref{max|P-tildeP|<=|P(T)-tildeP(T)|}, we obtain the estimate \eqref{eqn:estM-tildeM}. 
% Therefore \eqref{eqn:estP-tildeP} holds for $t=T$. 



% Assume by induction that 
% \eqref{eqn:estP-tildeP} holds for $t=u$. We show that \eqref{eqn:estP-tildeP} also holds for $t=u-1$. 
% From \eqref{eqnP(t)}, we have  
% \allowdisplaybreaks\begin{align} 
%  P(u-1) - \widetilde{P}(u-1)  
% = & [ M( \widetilde{P}(u) ) ]^{-1} 
%  - [ M(P(u)) ]^{-1}\notag  \\ 
%  = & [ M( P(u) ) ]^{-1} ( P(u) - \widetilde{P}(u) )  
% [ M( \widetilde{P}(u) ) ]^{-1} ,  \notag 
% %\label{tildeP-Precursion}
% \end{align} 
% and by Lemma~\ref{lm:|AB|<=|A||B|} we further have 
% \allowdisplaybreaks  
% \begin{align} 
%  \big| P(u-1) - \widetilde{P}(u-1)  \big|  
%  \leq & \big| [ M( P(u) ) ]^{-1} 
%  \big| \cdot \big| P(u) - \widetilde{P}(u) \big| \cdot 
% \big| [ M( \widetilde{P}(u) ) ]^{-1} \big| . \label{|tildeP-P|recursion} 
% \end{align} 
% By Corollary~\ref{cor:M(P)invbdd} and the induction hypothesis for $t=u$,  
% \eqref{|tildeP-P|recursion} implies that \eqref{eqn:estP-tildeP} holds for $t=u-1$. 
% We have shown by induction that \eqref{eqn:estP-tildeP} holds for all $t=1$, ..., $T$. 


% Since 
% \begin{align} 
%   [M(P(t))]^{-1} - [M(\widetilde{P}(t))]^{-1} 
%   =  [ M( P(t) ) ]^{-1} (  \widetilde{P}(t) - P(t) )  
% [ M( \widetilde{P}(t) ) ]^{-1} ,   
% \notag 
% \end{align} 
% by Lemma~\ref{lm:|AB|<=|A||B|} we have   
% \begin{align} 
%  \big| [M(P(t))]^{-1} - [M(\widetilde{P}(t))]^{-1} \big| 
%   \leq  \big| [ M( P(t) ) ]^{-1} \big| \cdot  
%   \big|  \widetilde{P}(t) - P(t) \big| \cdot  
% \big| [ M( \widetilde{P}(t) ) ]^{-1} \big|  . 
% \label{eqn:M-tildeM<=P-tildeP}
% \end{align} 
% The estimate \eqref{eqn:estM-tildeM} then follows from \eqref{eqn:M-tildeM<=P-tildeP}, \eqref{eqn:estP-tildeP}, and Corollary~\ref{cor:M(P)invbdd}. 
% %the fact that $|[M(P(t))]^{-1}| \leq C$ and $[M(\widetilde{P}(t))]^{-1}\leq C$, 
 





% %For data sets $D$ and $\widetilde{D}$ satisfying Assumptions \ref{assm:bddxy} and \ref{assm:PD}, $P$ and $\widetilde{P}$ determined from \eqref{eqnP(t)} are positive-definite. Then $\big| [ M (P(t) ) ) ]^{-1} \big|$ is bounded by a constant depending on $K_x$, $(w^\star_1, \cdots, w^\star_N)$ and $T$. Similarly, $\big| [  M(\widetilde{P}(t) ) ]^{-1} \big|$ is bounded by a constant depending on $K_x$, $K_y$, $(w^\star_1, \cdots, w^\star_N)$ and $T$. 
 




% Now we establish the estimate \eqref{eqn:estS-tildeS}. 
% By \eqref{eqnS(t)}, the terminal condition $S(T)-\widetilde{S}(T)$ satisfies 
% \allowdisplaybreaks 
% \begin{align} 
%  | S(T) - \widetilde{S}(T) |^2 
%  = & 
%  \Big| [w_1^\star, \cdots, w_N^\star]^\top \sum_{i=1}^N w_i^\star \sum_{j=1}^{|\mathcal{D}_i|} 
%   ( u^i_j y^i_j - \tilde{u}^i_j \tilde{y}^i_j ) \Big|^2 \notag \\ 
%   =& \Big( \sum_{i=1}^N w^{\star 2}_i \Big) 
%  \Big| \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|} ( u^i_j y^i_j - \tilde{u}^i_j \tilde{y}^i_j ) \Big|^2 .  \notag
% \end{align} 
% By Lemmas~\ref{lm:|AB|<=|A||B|} and \ref{lm:|A1+An|2<=(|A1|2+|An|2)n}, we obtain 
% \allowdisplaybreaks
% \begin{align} 
%  | S(T) - \widetilde{S}(T) |^2  
%  \leq & \Big( \sum_{i=1}^N w^{\star 2}_i \Big) 
%  \sum_{i=1}^N w^\star_i  \Big| \sum_{j=1}^{|\mathcal{D}_i|} ( u^i_j y^i_j - \tilde{u}^i_j \tilde{y}^i_j ) \Big|^2  \notag  \\ 
%   \leq & \Big( \sum_{i=1}^N w^{\star 2}_i \Big) 
%  \sum_{i=1}^N w^\star_i |\mathcal{D}_i| \sum_{j=1}^{|\mathcal{D}_i|}  \big|  u^i_j y^i_j - \tilde{u}^i_j \tilde{y}^i_j \big|^2  \notag   \\ 
%  = & \Big( \sum_{i=1}^N w^{\star 2}_i \Big) 
%  \sum_{i=1}^N w^\star_i |\mathcal{D}_i| \sum_{j=1}^{|\mathcal{D}_i|}  \big|  (u^i_j - \tilde{u}^i_j) y^i_j + \tilde{u}^i_j (y^i_j - \tilde{y}^i_j) \big|^2  \notag \\ 
%   \leq & \Big( \sum_{i=1}^N w^{\star 2}_i \Big) 
%  \sum_{i=1}^N w^\star_i |\mathcal{D}_i| \cdot 2  \sum_{j=1}^{|\mathcal{D}_i|} \big[ \big|  (u^i_j - \tilde{u}^i_j) y^i_j \big|^2 
%  + \big|  \tilde{u}^i_j (y^i_j - \tilde{y}^i_j) \big|^2 \big]   \notag \\    
%  \leq & \Big( \sum_{i=1}^N w^{\star 2}_i \Big) 
%  \sum_{i=1}^N w^\star_i |\mathcal{D}_i| \cdot 2  \sum_{j=1}^{|\mathcal{D}_i|} \big[ |  u^i_j - \tilde{u}^i_j |^2 \cdot | y^i_j |^2 
%  + |  \tilde{u}^i_j |^2 \cdot | y^i_j - \tilde{y}^i_j  |^2 \big]   \notag\\ \leq & \Big( \sum_{i=1}^N w^{\star 2}_i \Big) 
%  \sum_{i=1}^N w^\star_i |\mathcal{D}_i| \cdot 2  \sum_{j=1}^{|\mathcal{D}_i|} \big[ K_y^2 \cdot |  u^i_j - \tilde{u}^i_j |^2  
%  + K_x^2 \cdot | y^i_j - \tilde{y}^i_j  |^2 \big]   \notag 
%  \\ 
%  \label{estST-tildeST} 
%  \leq & \Big( \sum_{i=1}^N w^{\star 2}_i \Big) 2 (K_x^2 + K_y^2)
%  \sum_{i=1}^N w^\star_i |\mathcal{D}_i|   \sum_{j=1}^{|\mathcal{D}_i|} \big[ |  u^i_j - \tilde{u}^i_j |^2  
%  +  | y^i_j - \tilde{y}^i_j  |^2 \big] , 
% \end{align} 
% and thus \eqref{eqn:estS-tildeS} holds for $t=T$. 
% Assume by induction that \eqref{eqn:estS-tildeS} holds for $t=u$, we show that \eqref{eqn:estS-tildeS} also holds for $t=u-1$. 
% From \eqref{eqnS(t)}, the difference $S(t)-\widetilde{S}(t)$ can be written as 
% \allowdisplaybreaks\begin{align} 
%  S(u-1) - \widetilde{S}(u-1) = & [ M(\widetilde{P}(u)) ]^{-1}[S(u) - \widetilde{S}(u) ]  \notag \\ 
%  & + \big[ ( M(P(u)) )^{-1} - 
%   ( M(\widetilde{P}(u)))^{-1} \big]  
%  ( S(u) - \lambda \Theta^\star ) , 
% \notag 
% \end{align} 
% and satisfies by Lemma~\ref{lm:|AB|<=|A||B|} and Corollary~\ref{cor:M(P)invbdd} that 
% \begin{align} 
% | S(u-1) - \widetilde{S}(u-1) | \leq &
%  \big| [ M(\widetilde{P}(u)) ]^{-1} \big| \cdot |S(u) - \widetilde{S}(u) |  \notag \\ 
%  & + \big| ( M(P(u)) )^{-1} - 
%   ( M(\widetilde{P}(u)))^{-1} \big| \cdot   
%  ( |S(u)| + \lambda | \Theta^\star | ) . 
%  \label{|tildeS-S|recursion} 
% \end{align} 
% By Corollary~\ref{cor:M(P)invbdd}, \eqref{eqn:estM-tildeM}, and the induction hypothesis, 
% \eqref{|tildeS-S|recursion} implies that 
% \eqref{eqn:estS-tildeS} holds for $t=u-1$.  
% We have shown by induction that \eqref{eqn:estS-tildeS} holds for all $t=1$, ..., $T$. 
% \end{proof} 

% \begin{proposition} 
% \label{prop:stabilityControl}
% For two arbitrary data sets $\mathcal{D}=\cup_{i=1}^N \mathcal{D}_i=\cup_{i=1}^N \cup_{j=1}^{|\mathcal{D}_i|} 
%  \{(x^i_j, y^i_j) \}$ and 
% $\widetilde{\mathcal{D}}=\cup_{i=1}^N \widetilde{\mathcal{D}}_i = \cup_{i=1}^N \cup_{j=1}^{|\mathcal{D}_i|}  \{(\tilde{x}^i_j, \tilde{y}^i_j) \}$ satisfying Assumption \ref{assm:bddxy}, 
% let $\boldsymbol\alpha =(\alpha_1^{\top}, \cdots, \alpha_N^{\top})^{\top}$ and 
% $\widetilde{\boldsymbol\alpha}=(\widetilde{\alpha}_1^{\top}, \cdots, \widetilde{\alpha}_N^{\top})^{\top}$ be the optimal controls for \eqref{eq:penalized_regret_functional} and \eqref{Theta-simple} corresponding to $\mathcal{D}$ and $\widetilde{\mathcal{D}}$, respectively. Then, we have
% \allowdisplaybreaks\begin{align} 
%  \sum_{t=0}^{T-1} |\boldsymbol\alpha(t) - \widetilde{\boldsymbol\alpha}(t) | 
%  \le C  \Big[ \sum_{i=1}^N w^{\star 2}_i |\mathcal{D}_i| \sum_{j=1}^{|\mathcal{D}_i|} | u^i_j - \tilde{u}^i_j |^2 
%  + |y^i_j - \tilde{y}^i_j|^2  \Big]^{1/2} , 
% \label{eqn:stabilityControl}
% \end{align} 
% where $C > 0$ is a constant depending on $\lambda$, $\beta$, $N$, $\bar{N}$, $\Theta^\star$, 
% $(w^\star_1, \cdots, w^\star_N)$, $K_x$, $K_y$, and $T$. 
% \end{proposition} 

% \begin{proof}[{Proof of Proposition~\ref{prop:stabilityControl}}]
% Let $C$ be a constant depending on $\lambda$, $\beta$, $N$, $\bar{N}$, $\Theta^\star$,  
% $(w^\star_1, \cdots, w^\star_N)$, $K_x$, $K_y$, and $T$,  
% and $C$ is allowed to vary from place to place throughout the proof. 
% By \eqref{optimala} and \eqref{Theta(t)Theta(0)}, the optimal control $\boldsymbol\alpha(t)$ along the optimal trajectory can be written as 
% \allowdisplaybreaks\begin{align} 
%   \boldsymbol\alpha(t) 
%  = & [ (M(P(t+1)))^{-1} - I_{Np} ]  \Big[ \Theta^\star 
%  + \sum_{u=0}^{t-1} \boldsymbol\alpha(u) \Big] \notag \\ 
%  & +  [ M(P(t+1)) ]^{-1} ( \lambda  \Theta^\star - S(t+1) ) ,   \notag 
% \end{align}
% and the difference $\boldsymbol{\alpha}(t)-\widetilde{\boldsymbol\alpha}(t)$ can be written as    
% \allowdisplaybreaks\begin{align}  
%   \boldsymbol\alpha(t) - \widetilde{\boldsymbol\alpha}(t) 
%  = &  \big[(M(P(t+1)))^{-1} - (M(\widetilde{P}(t+1)) )^{-1} \big] 
%  \Big[ \Theta^\star + \sum_{u=0}^{t-1}  \boldsymbol\alpha(u)   + \lambda \Theta^\star - S(t+1) \Big]  \notag \\ 
%  & + \big[ ( M(\widetilde{P}(t+1)) )^{-1} - I_{Np} \big] 
%  \sum_{u=0}^{t-1} (\boldsymbol\alpha(u) - \widetilde{\boldsymbol\alpha}(u)) \notag \\ 
% & + (M(\widetilde{P}(t+1)))^{-1} (S(t+1) - \widetilde{S}(t+1)) . 
% \label{a-tildea}
% \end{align} 


% For $t=0$, the difference $\boldsymbol\alpha(0)-\widetilde{\boldsymbol\alpha}(0)$ can be written as  
% \allowdisplaybreaks\begin{align} 
%   \boldsymbol\alpha(0) - \widetilde{\boldsymbol\alpha}(0)  
%  = & \big[ (M(P(1)))^{-1} - (M(\widetilde{P}(1)))^{-1}  \big] 
%  \big[ (\lambda + 1)   \Theta^\star - S(1) 
%  \big] \notag \\ 
%  & - [ M(\widetilde{P}(1)) ]^{-1} (S(1)-\widetilde{S}(1)) , \notag  
% \end{align} 
% and satisfies by Lemma~\ref{lm:|AB|<=|A||B|} that 
% \begin{align} 
% \big| \boldsymbol\alpha(0) - \widetilde{\boldsymbol\alpha}(0) \big|   
%  \leq &   \big| (M(P(1)))^{-1} - (M(\widetilde{P}(1)))^{-1}  \big| \cdot  
%  \big[ (\lambda + 1)   | \Theta^\star| +  | S(1) | 
%  \big] \notag \\ 
%  & +  \big| [ M(\widetilde{P}(1)) ]^{-1} \big| \cdot  \big| S(1)-\widetilde{S}(1) \big| .  \notag  
% \end{align} 
% It then follows from Corollary~\ref{cor:M(P)invbdd}, \eqref{eqn:estM-tildeM}, and \eqref{eqn:estS-tildeS} that 
% \allowdisplaybreaks\begin{align} 
%   \big| \boldsymbol\alpha(0) - \widetilde{\boldsymbol\alpha}(0) \big| \leq C 
%  \cdot \Big[ \sum_{i=1}^N w^\star_i |\mathcal{D}_i| \sum_{j=1}^{|\mathcal{D}_i|} | u^i_j 
%  - \tilde{u}^i_j |^2 
%  + |y^i_j - \tilde{y}^i_j|^2  \Big]^{1/2} . \notag   
% \end{align}
% Assume by induction that  
% \allowdisplaybreaks\begin{align} 
%  \sum_{u=0}^{t-1} \big| \boldsymbol\alpha(u) - \widetilde{\boldsymbol\alpha}(u) \big| \leq C 
%  \cdot \Big[ \sum_{i=1}^N w^\star_i |\mathcal{D}_i| \sum_{j=1}^{|\mathcal{D}_i|} | u^i_j - \tilde{u}^i_j |^2 
%  + |y^i_j - \tilde{y}^i_j |^2  \Big]^{1/2} .  \notag   
% \end{align} 
% By Lemma~\ref{lm:|AB|<=|A||B|}, \eqref{a-tildea} implies that   
% \allowdisplaybreaks\begin{align}  
%  & | \boldsymbol\alpha(t) - \widetilde{\boldsymbol\alpha}(t) | \notag \\ 
%  \leq &  \big| (M(P(t+1)))^{-1} - (M(\widetilde{P}(t+1)) )^{-1} \big| \cdot 
%  \Big[ |\Theta^\star| + \sum_{u=0}^{t-1}  | \boldsymbol\alpha(u) |   
%  + \lambda | \Theta^\star | +| S(t+1) | \Big]  \notag \\ 
%  & + \big| ( M(\widetilde{P}(t+1)) )^{-1} - I_{Np}  \big| 
%  \sum_{u=0}^{t-1} | \boldsymbol\alpha(u) - \widetilde{\boldsymbol\alpha}(u) | 
% + | (M(\widetilde{P}(t+1)))^{-1} | \cdot | S(t+1) - \widetilde{S}(t+1) | .  \notag   
% \end{align} 
% By \eqref{eqn:estM-tildeM},  \eqref{eqn:estS-tildeS}, and the induction hypothesis,
% the above inequality implies that that 
% \allowdisplaybreaks\begin{align}
%  |\boldsymbol\alpha(t) - \widetilde{\boldsymbol\alpha}(t)| 
%  \leq C  \Big[ \sum_{i=1}^N w^\star_i |\mathcal{D}_i| \sum_{j=1}^{|\mathcal{D}_i|} | u^i_j - \tilde{u}^i_j |^2 
%  + |y^i_j - \tilde{y}^i_j|^2  \Big]^{1/2} , \notag  
% \end{align} 
% and therefore 
% \allowdisplaybreaks\begin{align} 
%  \sum_{u=0}^{t} \big| \boldsymbol\alpha(u) - \widetilde{\boldsymbol\alpha}(u) \big| \leq C 
%  \cdot \Big[ \sum_{i=1}^N w^\star_i |\mathcal{D}_i| \sum_{j=1}^{|\mathcal{D}_i|} | u^i_j - \tilde{u}^i_j |^2 
%  + |y^i_j - \tilde{y}^i_j |^2  \Big]^{1/2} .  \notag   
% \end{align} 
% The estimate \eqref{eqn:stabilityControl} is then proved by induction.  
% \end{proof} 



% \begin{corollary} 
% \label{cor:stabilityLast}
% Under the hypothesis of Proposition \ref{prop:stabilityControl}, the costs \eqref{eq:penalized_regret_functional} under the optimal controls $\mathbf{a}$ 
% and $\widetilde{\mathbf{a}}$ satisfy the estimate 
% \allowdisplaybreaks\begin{align} 
%  \big| L^\star ( \boldsymbol\alpha ; \mathcal{D} ) 
%  -  L^\star (  \widetilde{\boldsymbol\alpha} ;  \widetilde{\mathcal{D}} )  \big|  
%  \leq  C \cdot \Big[ \sum_{i=1}^N w^\star_i |\mathcal{D}_i| \sum_{j=1}^{|\mathcal{D}_i|} | u^i_j - \tilde{x}^i_j |^2  + |y^i_j - \tilde{y}^i_j |^2 \Big]^{1/2} . 
%  \label{eqn:stabilityLast} 
% \end{align} 
% where $C>0$ is a constant depending on $\lambda$, $\beta$, $N$, $\bar{N}$, $\Theta^\star$, 
% $(w^\star_1, \cdots, w^\star_N)$, $K_x$, $K_y$, and $T$. 
% \end{corollary}


% \begin{proof}[{Proof of Corollary~\ref{cor:stabilityLast}}] 
% Throughout the proof $C$ is a constant depending on $\lambda$, $\beta$, $\bar{N}$, $\Theta^\star$, 
% $(w_1^\star, \cdots, w_N^\star)$, $K_x$, $K_y$ and $T$, and may vary from place to place.  
% By \eqref{ansatzVw} and \eqref{Theta-simple}, the difference of the costs can be written as 
% \allowdisplaybreaks\begin{align} 
%   L^\star ( \boldsymbol\alpha ; \mathcal{D} ) 
%  -  L^\star (  \widetilde{\boldsymbol\alpha} ;  \widetilde{\mathcal{D}} )  
% = & \Theta^\top (0) ( P(0) - \widetilde{P}(0) ) \Theta(0) 
%  + 2 ( S(0) - \widetilde{S}(0) )^\top \Theta(0) + r(0)-\widetilde{r}(0) ,  \notag \\ 
%   = & 
%    \Theta^{\star \top} ( P(0) - \widetilde{P}(0) ) \Theta^\star  
%  + 2 ( S(0) - \widetilde{S}(0) )^\top \Theta^\star + r(0)-\widetilde{r}(0) .  
%  \notag 
% \end{align} 
% By the triangular inequality, the difference satisfies  
% \allowdisplaybreaks\begin{align} 
%   \big| L^\star (  \boldsymbol\alpha ; \mathcal{D} ) 
%  -  L^\star (  \widetilde{\boldsymbol\alpha} ;  \widetilde{\mathcal{D}} ) \big|  
% \leq  |  P(0) - \widetilde{P}(0) | \cdot |\Theta^\star|^2  
%  + 2 | S(0) - \widetilde{S}(0) | \cdot | \Theta^\star | + | r(0)-\widetilde{r}(0) | . 
% \label{estLast-tildeLast} 
% \end{align}
% We claim that $r(0)-\widetilde{r}(0)$ satisfies the estimate 
% \allowdisplaybreaks\begin{align} 
%  | r(0)-\widetilde{r}(0) | \leq  C \cdot \Big[ \sum_{i=1}^N w^\star_i |\mathcal{D}_i| \sum_{j=1}^{|\mathcal{D}_i|} | u^i_j - \tilde{u}^i_j |^2 
%  + |y^i_j - \tilde{y}^i_j |^2 \Big]^{1/2} .  
% \label{eqn:estr-tilder(0)} 
% \end{align} 
% %where $C$ is a constant depending on $\Theta^\star$, $(w_1^\star, \cdots, w_N^\star)$, $K_x$, $K_y$ and $T$. 
% Then the desired estimate \eqref{eqn:stabilityLast} is established by \eqref{estLast-tildeLast}, \eqref{eqn:estP-tildeP}, 
% \eqref{eqn:estS-tildeS}  and \eqref{eqn:estr-tilder(0)}. 



% Now we prove the claim \eqref{eqn:estr-tilder(0)}. 
% From \eqref{eqnr(t)}, the difference $r-\widetilde{r}$ satisfies  
% \allowdisplaybreaks\begin{align} 
%  & r(t) - \widetilde{r}(t) =  r(t+1) - \widetilde{r}(t+1) 
%  - ( S(t+1) - \widetilde{S}(t+1) ) \big\{ (M(P(t+1)))^{-1} 
%  \big[ S(t+1) - 2 \lambda \Theta^\star \big]  \notag \\  
%  & \hspace{2cm} + (M(\widetilde{P}(t+1)))^{-1} \widetilde{S}(t+1) \big\}  \notag \\ 
%  &\hspace{2cm} - \widetilde{S}^\top(t+1) \big[ (M(P(t+1)))^{-1} 
%  - (M(\widetilde{P}(t+1)))^{-1} \big]  \big[ S(t+1) - 2 \lambda \Theta^\star \big]    \notag \\ 
%  &\hspace{2cm} - \Theta^{\star \top} \lambda  \big[ (M(P(t+1)))^{-1} 
%  - (M(\widetilde{P}(t+1)))^{-1} \big]  \lambda  \Theta^\star , \notag  \\ 
% %%% 
% & r(T) - \widetilde{r}(T) =   \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|} ( |y^i_j|^2 - |\widetilde{y}^i_j|^2 ) . \label{eqnr(t)-tilder(t)}  
% \end{align} 
% Inductively, $r(0)-\widetilde{r}(0)$ can be written in terms of $r(T)-\widetilde{r}(T)$ as   
% \allowdisplaybreaks\begin{align} 
%  & r(0) - \widetilde{r}(0) \notag \\ 
% = & r(T) - \widetilde{r}(T) 
%  - \sum_{t=1}^T \Big\{ ( S(t) - \widetilde{S}(t) ) \big[ (M(P(t)))^{-1} 
%  \big( S(t) - 2 \lambda \Theta^\star \big)    
%   + (M(\widetilde{P}(t)))^{-1} \widetilde{S}(t) \big]   \notag \\ 
%  & + \widetilde{S}^\top(t) \big[ (M(P(t)))^{-1} 
%  - (M(\widetilde{P}(t)))^{-1} \big]  \big[ S(t) - 2 \lambda  \Theta^\star \big]     
%   + \Theta^{\star \top} \lambda  \big[ (M(P(t)))^{-1} 
%  - (M(\widetilde{P}(t)))^{-1} \big]  \lambda \Theta^\star 
%   \Big\} . \notag  
% \end{align}
% By Lemma~\ref{lm:|AB|<=|A||B|}, we have  
% \allowdisplaybreaks\begin{align} 
% &   | r(0) - \widetilde{r}(0) | \notag \\ 
%  & \leq  | r(T) - \widetilde{r}(T) |
%   + \sum_{t=1}^T \Big\{ \big| S(t) - \widetilde{S}(t) \big| 
%  \cdot \Big[ \big| (M(P(t)))^{-1} \big| \cdot
%  \big(  | S(t) | + 2 \lambda | \Theta^\star| \big)    
%   + \big| (M(\widetilde{P}(t)))^{-1} \big| \cdot \big| \widetilde{S}(t) \big|  \Big]   \notag \\ 
%  & \hspace{2cm} +\big| (M(P(t)))^{-1} 
%  - (M(\widetilde{P}(t)))^{-1} \big|  \cdot  
%  \big( \big| \widetilde{S}(t) \big| \cdot \big| S(t) - 2 \lambda  \Theta^\star \big|     
%   +  \lambda | \Theta^\star |^2 \big) 
%   \Big\} . \label{estr(0)-tilder(0)}  
% \end{align}
% By \eqref{eqnr(t)-tilder(t)}, Lemma \ref{lm:|A1+An|2<=(|A1|2+|An|2)n}, and the Cauchy-Schwarz inequality, the terminal condition satisfies 
% \allowdisplaybreaks\begin{align} 
%   |r(T) - \widetilde{r}(T)| 
%   = &  \Big| \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|} 
%   ( y^i_j - \tilde{y}^i_j ) (y^i_j + \tilde{y}^i_j ) \Big| 
%   \leq \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|}  | (y^i_j - \tilde{y}^i_j) (y^i_j + \tilde{y}^i_j ) | \notag \\ 
%  \leq & \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|}  |y^i_j + \widetilde{y}^i_j| \cdot 
%  |y^i_ j - \widetilde{y}^i_j |  
%   \leq  2 K_y 
%  \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|}  |y^i_j -  \widetilde{y}^i_j| 
%   \notag \\ 
%  \leq & 2 K_y \Big( \sum_{i=1}^N w^\star_i  \sum_{j=1}^{|\mathcal{D}_i|}  |y^i_j - \widetilde{y}^i_j|^2 \Big)^{1/2} .  
%  \label{estr(T)-tilder(T)}  
% \end{align} 
% The estimate \eqref{eqn:estr-tilder(0)} then follows from 
% \eqref{estr(0)-tilder(0)}, \eqref{estr(T)-tilder(T)}, \eqref{eqn:estM-tildeM}, \eqref{eqn:estS-tildeS}, and \eqref{|S|bd}. 
% \end{proof}



% We may now derive the proof of Theorem~\ref{thrm:adv_robust} as a direct consequence of Corollary~\ref{cor:stabilityLast}.
% \begin{proof}[{Proof of Theorem~\ref{thrm:adv_robust}}]
% Fix $\widetilde{\mathcal{D}} \in \mathbb{D}^{p,\varepsilon}$ and let $I\subseteq \{(i,j):i=1,\dots,N,\,j=1,\dots,|\mathcal{D}_i|\}$ consist of all indices $(i,j)$ for which $\{(i,j):\, u^i_j\neq \widetilde{u}^i_j \mbox{ and } y^i_j\neq \widetilde{y}^i_j\}$.  By Corollary~\ref{cor:stabilityLast}, there is a constant $C>0$ which is independent of $\mathcal{D}$ such that
% \allowdisplaybreaks
% \allowdisplaybreaks\begin{align}
% \nonumber
%     \big| L^\star (  \boldsymbol\alpha ; \mathcal{D} ) 
%     -  L^\star (  \widetilde{\boldsymbol\alpha} ;  \widetilde{\mathcal{D}} )  \big|^2
%  \le &
%     \widetilde{C} \sum_{i=1}^N w_i^\star |\mathcal{D}_i| \sum_{j=1}^{|\mathcal{D}_i|} | u^i_j - \widetilde{u}^i_j |^2  + |y^i_j - \widetilde{y}^i_j |^2 
% \\ 
% \nonumber
% \le & 
% \widetilde{C} \cdot \sum_{(i,j)\in I}\, w_i^\star |\mathcal{D}_i|  ( | u^i_j - \widetilde{u}^i_j |^2  + |y^i_j - \widetilde{y}^i_j |^2 ) 
% \\ 
% \nonumber
% \le &
% \widetilde{C} \cdot \sum_{(i,j)\in I}\, w_i^\star |\mathcal{D}_i| \cdot \max\{| u^i_j - \widetilde{u}^i_j |^2, |y^i_j - \widetilde{y}^i_j |^2\}
% \\ 
% \nonumber
% = &
% \widetilde{C} \cdot \sum_{(i,j)\in I}\, w_i^\star |\mathcal{D}_i| \cdot \max\{| u^i_j - \widetilde{u}^i_j |, |y^i_j - \widetilde{y}^i_j |\}^2
% \\ 
% \nonumber
% \le &
% \widetilde{C} \cdot \sum_{(i,j)\in I}\, w_i^\star |\mathcal{D}_i| \cdot 2\varepsilon^2
% \\ 
% \nonumber
% \le &
% \widetilde{C} \#I\, p \, 2\varepsilon^2
%  ,
% \end{align}
% where we have set $\widetilde{C}\eqdef C^{1/2}$.
% \end{proof}



% %%%%%%%%%%%%%%%%%%%%%%%%%%%% 

% The computational complexity of the matrix-valued function $P(\cdot)$, as determined by \eqref{eqnP(t)}, does not primarily stem from the high dimensionality of the output matrices, but rather from their inherent lack of symmetries.
% As we will see later, such symmetry will allow us to efficiently encode $P(\cdot)$ into low-dimensional structures, therefore completely mitigating the high-dimensionality effect.


% We therefore introduce the following control, which is optimal for a ``symmetrized version'' of the control problem~\eqref{optimala} where $w^{\star}=(1/N,\dots,1/N)$.  This advantages this surrogate problem is that the associated $P$ function, which we denote by $\widehat{P}$, outputs highly symmetric\footnote{As formalized in Proposition~\ref{prop:P1/Nsubmat}.} Toeplitz matrices which are determined by exactly three factors. This allows us to encode the entire control problem into a control problem on $\mathbb{R}^{\tilde{O}(P)}$ whose dimension is independent of $N$. 
% Furthermore, the optimal controls of both problems can be related by stability estimates, depending only on the deviation of $(1/N,\dots,1/N)$ from $w^{\star}$, which allows us to infer the degree of sub-optimality of our $\widehat{P}$.  Therefore, we consider the control
% \begin{align} 
%  \widehat{\boldsymbol{\alpha}}(t)  
%  = & -[(\lambda + \beta )I_{Np} + \widehat{P}(t+1)]^{-1} 
%  \big[ (\lambda I_{Np} + \widehat{P}(t+1)) \Theta(t) 
%  - \lambda  \Theta^\star_{(N)} + \widehat{S}(t+1)  \big]   \label{hata} 
%  .
% \end{align} 
% We will show that the algorithm under control \eqref{hata} enjoys lower computational complexity in comparison with the regret-optimal algorithm \eqref{optimala}, whose computational complexity is summarized through Theorem~\ref{thm:ComplexityAlgorithm}. Furthermore, we will then establish the near-regret optimality of \eqref{hata}, stated in Theorem \ref{thrm:Epsilon_Efficiency}.

% The associated matrix-valued functions $\widehat{P}$ and $\widehat{S}$ are uniquely determined by 
% \allowdisplaybreaks\begin{align} 
% & \begin{cases}
%    \widehat{P}(t)  =  \beta I_{Np} - \beta^2 [(\lambda+\beta ) I_{Np} + \widehat{P}(t+1) ]^{-1} , \label{eqnhatP1/N(t)} \\ 
%    \widehat{P}(T) =  [ (1/N) I_p ,\cdots, (1/N) I_p]^{\top} 
%  \Big( \sum_{i=1}^N (1/N) \sum_{j=1}^{|\mathcal{D}_i|} u^i_j u^{i\top}_j  \Big)  
%  [ (1/N) I_p , \cdots, (1/N) I_p ] , 
% \end{cases} \\ 
% & \begin{cases}
%   \widehat{S}(t) =  
%   \beta [(\lambda + \beta ) I_{Np} + \widehat{P}(t+1) ]^{-1} 
%   \big( \widehat{S}(t+1) - \lambda \Theta^\star_{(N)} \big)
%   \label{eqnhatS1/N(t)} ,     \\ 
%         \widehat{S}(T) 
%     =  
%   - [(1/N)I_p, \cdots, (1/N)I_p ]^{\top} \sum_{i=1}^N(1/N)\sum_{j=1}^{|\mathcal{D}_i|}  u^i_j y^i_j  
%    ,  
% \end{cases} 
% \end{align} 
% where $[ I_p, \cdots, I_p ]$ denotes the $Np\times p$-dimensional matrix formed by concatenating $N$ copies of the $p\times p$-dimensional identity matrix $\frac{1}{N} I_p$.   The parameter $\Theta^\star_{(N)}$ is defined as 
% \allowdisplaybreaks\begin{align} 
%  \Theta^\star_{(N)} \eqdef [\theta_{(N)}^{\star \top}, \cdots, \theta_{(N)}^{\star \top}]^{\top} , \quad 
% \theta^\star_{(N)} \eqdef \frac{1}{N} \sum_{i=1}^N \theta^\star_i . \notag 
% \end{align}

% \begin{remark} 
% According to \eqref{Sum(uij)Tuij>=0} in Assumption \ref{assm:PD}, $\widehat{P}(T)\geq 0$ and therefore \eqref{eqnhatP1/N(t)} admits a unique solution. 
% \end{remark} 

% \begin{remark}
% \label{rmk:M(hatP)bdd}
% Similar to Corollary~\ref{cor:M(P)invbdd}, we have $\big| [ (\lambda+\beta)I_{Np} + \widehat{P}(t) ]^{-1} \big| \leq (\lambda + \beta)^{-1}$. By replacing $(w_1^\star, ..., w_N^\star)$ in the proof of Corollary~\ref{cor:M(P)invbdd} with $(1/N, ..., 1/N)$, we obtain 
% $|\widehat{S}(t)|\leq C \cdot N^{1/2}$ for all $t=1$, ..., $T$, 
% where $C>0$ is a constant depending on $\lambda$, $\beta$, $\Theta^\star$, $K_x$, $K_y$ and $T$.  
% \end{remark}


% \begin{lemma} 
% \label{lem:lemma_A}
%  Let $P$ and $\widehat{P}$ be the solutions of the systems \eqref{eqnP(t)} and \eqref{eqnhatP1/N(t)}, respectively. Then they satisfy that for all $t=1$, $2$, ..., $T$, 
% \allowdisplaybreaks
% \begin{align} 
%   \big| P(t) - \widehat{P}(t) \big| 
%  \leq  C \cdot \bar{N} N \max_{1\leq i, k, l \leq N} \Big| \frac{1}{N^3} -  w^\star_k w^\star_l w^\star_i \Big| ,  
% \label{estPw-P1/N} \\ 
%  \big| (M(P(t)))^{-1} - (M(\widehat{P}(t) ))^{-1} \big| 
%  \leq  C \cdot  \bar{N} N \max_{1\leq i, k, l \leq N} \Big| \frac{1}{N^3} -  w^\star_k w^\star_l w^\star_i \Big| ,  
% \label{estMPw-MP1/N}  
% \end{align}
% where $C>0$ is a constant depending on $\lambda$, $\beta$, $K_x$. 
% \end{lemma} 

% \begin{proof}[{Proof of Lemma~\ref{lem:lemma_A}}] 
% By \eqref{eqnhatP1/N(t)}, \eqref{eqnP(t)}, and Lemmas~\ref{lm:|AB|<=|A||B|} and \ref{lm:|A1+An|2<=(|A1|2+|An|2)n}, the difference 
% $\widehat{P}(T)-P(T)$ satisfies    
% \allowdisplaybreaks
% \begin{align} 
% |\widehat{P}(T) - P(T)|^2 = & \sum_{k,l=1}^N 
% \Big| \frac{1}{N^2} \sum_{k=1}^N \frac{1}{N} 
% \sum_{j=1}^{|\mathcal{D}_i|}  u^i_j u^{i\top}_j  - w^\star_k w^\star_l \sum_{i=1}^N w^\star_i  \sum_{j=1}^{|\mathcal{D}_i|} u^i_j u^{i\top}_j  \Big|^2 \notag \\ 
% \leq & N^2 \cdot \max_{1\leq k, l, i \leq N} \Big| \frac{1}{N^3} 
%   - w^\star_k w^\star_l 
%    w^\star_i \Big|^2 \cdot \Big| \sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|}  u^i_j u^{i\top}_j  \Big|^2  \notag \\  
%    \leq &   N^2 \cdot \max_{1\leq k, l, i \leq N} \Big| \frac{1}{N^3} 
%   -  w^\star_k w^\star_l 
%    w^\star_i \Big|^2 \cdot  \bar{N} \sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|}  | u^i_j |^4   \notag 
% \end{align} 
% and 
% \begin{align} 
% |\widehat{P}(T) - P(T)| 
%  \leq & \bar{N} N K_x^2 \cdot \max_{1\leq k, l, i \leq N} \Big| \frac{1}{N^3} 
%   -  w^\star_k w^\star_l 
%    w^\star_i \Big| . 
%    \label{|P(T)-hatP(T)|est}
% \end{align} 
% Therefore \eqref{estPw-P1/N} holds for $t=T$. 

% Assume by induction that \eqref{estPw-P1/N} holds for $t=u$. We show that \eqref{estPw-P1/N} also holds for $t=u-1$. 
% From \eqref{eqnhatP1/N(t)} and \eqref{eqnP(t)}, we have  
% \allowdisplaybreaks\begin{align} 
%  \widehat{P}(u-1) - P(u-1) 
% = & [ M(P(u)) ]^{-1}
%  -  [ M( \widehat{P}(u) ) ]^{-1}  \notag  \\ 
%  = & [ M( P(u) ) ]^{-1} (\widehat{P}(u) - P(u)) 
% [ M( \widehat{P}(u) ) ]^{-1} . 
% \label{hatP-Precursion}
% \end{align} 
% By Lemmas~\ref{lm:|AB|<=|A||B|} and \ref{lm:|A1+An|2<=(|A1|2+|An|2)n}, we further have 
% \allowdisplaybreaks\begin{align} 
%  | \widehat{P}(u-1) - P(u-1) | 
% = & | [ M(P(u)) ]^{-1} 
%  -  [ M( \widehat{P}(u) ) ]^{-1} | \notag  \\ 
%  \leq & | [ M( P(u) ) ]^{-1} | \cdot  | \widehat{P}(u) - P(u) | \cdot 
%  | [ M( \widehat{P}(u) ) ]^{-1} | . 
% \label{|hatP-P|recursion}
% \end{align} 
% By \eqref{|hatP-P|recursion}, Corollary~\ref{cor:M(P)invbdd}, Remark~\ref{rmk:M(hatP)bdd}, and the induction hypothesis, we have 
% that \eqref{estPw-P1/N} holds for $t=u-1$. By induction we have shown that \eqref{estPw-P1/N} holds for all $1\leq t\leq T$. 


% From \eqref{hatP-Precursion}, we have 
% \allowdisplaybreaks 
% \begin{align} 
% & \big| ( M(P(t)) )^{-1}
%  -  ( M( \widehat{P}(t) ) )^{-1} \big|   
%  \leq  \big| ( M( P(t) ) )^{-1} \big| \cdot  \big| \widehat{P}(t) - P(t) \big| \cdot   
% \big| ( M( \widehat{P}(t) ) )^{-1} 
% \big| ,  \notag 
% \end{align} 
% which, together with \eqref{estPw-P1/N}, Corollary~\ref{cor:M(P)invbdd}, and Remark~\ref{rmk:M(hatP)bdd}, establishes \eqref{estMPw-MP1/N}. 
% \end{proof}


% \begin{lemma}
% \label{lem:Lemma_B}
%  Let $S$ and $\widehat{S}$ be the solutions of \eqref{eqnS(t)} and \eqref{eqnhatS1/N(t)}, respectively. Then they satisfy that 
% for all $t=1$, ..., $T$, 
% \allowdisplaybreaks
% \begin{align} 
%  |S(t) - \widehat{S}(t)| \leq & 
% C \cdot \Big\{ \bar{N} N^{3/2} \max_{1\leq i, k, l \leq N} \Big| \frac{1}{N^3} -  w^\star_k w^\star_l w^\star_i \Big| 
%   \notag \\ 
% & \hspace{1cm} + \bar{N} N^{1/2} \max_{1\leq k, l\leq N} \Big| \frac{1}{N^2} - w^\star_k w^\star_l \Big|
% + |\Theta^\star - \Theta^\star_{(N)}| \Big\} , 
%  \label{sup|S-hatS|est}
% \end{align}
% where $C>0$ is a constant depending on $\lambda$, $\beta$, $\Theta^\star$, $K_x$, $K_y$, and $T$. 
% \end{lemma}

% \begin{proof}[{Proof of Lemma~\ref{lem:Lemma_B}}]
% By \eqref{eqnS(t)}, \eqref{eqnhatS1/N(t)}, and and Lemmas~\ref{lm:|AB|<=|A||B|} and \ref{lm:|A1+An|2<=(|A1|2+|An|2)n}, the terminal condition $S(T)-\widehat{S}(T)$ satisfies 
% \allowdisplaybreaks\begin{align} \Big|S(T)-\widehat{S}(T)\Big|^2 
% = & \sum_{k=1}^N \Big| 
%  \frac{1}{N} \sum_{i=1}^N \frac{1}{N} \sum_{j=1}^{|\mathcal{D}_i|} u^i_j y^i_j - w^\star_k 
%  \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|} u^i_j y^i_j 
% \Big|^2 \notag \\ 
% \leq & N \cdot \max_{1\leq k, l \leq N} \Big| \frac{1}{N^2} - w^\star_k w^\star_l \Big|^2 \cdot \Big| \sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|} u^i_j y^i_j \Big|^2  \notag \\ 
%  \leq & N \cdot \max_{1\leq k, l \leq N} \Big| \frac{1}{N^2} - w^\star_k w^\star_l \Big|^2 \cdot \bar{N} \sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|} | u^i_j|^2 \cdot |y^i_j|^2 ,  
%  \notag 
% \end{align} 
% which implies  
% \allowdisplaybreaks\begin{align} 
%  \big| S(T) - \widehat{S}(T) \big| 
%  \leq & \bar{N} N^{1/2} \max_{1\leq k, l\leq N} \Big| \frac{1}{N^2} - w^\star_k w^\star_l \Big| \cdot   K_x K_y . 
%   \label{|S(T)-hatS(T)|est}  
% \end{align} 
% Therefore \eqref{sup|S-hatS|est} holds for $t=T$. 

% Assume by induction that \eqref{sup|S-hatS|est} holds for $t=u$, we show that \eqref{sup|S-hatS|est} holds for $t=u-1$. 
% From \eqref{eqnS(t)} and \eqref{eqnhatS1/N(t)}, the difference $S(u-1)-\widehat{S}(u-1)$ can be written as 
% \allowdisplaybreaks\begin{align} 
%  S(u-1) - \widehat{S}(u-1) = & [ M(P(u)) ]^{-1}[S(u) - \widehat{S}(u) - \lambda (\Theta^\star - \Theta^\star_{(N)}) ] \notag \\ 
%  & - \big[ ( M(\widehat{P}(u)))^{-1} - ( M(P(u)) )^{-1} \big]  
%  (\widehat{S}(u) - \lambda \Theta^\star_{(N)}) , 
%  \label{S(t)-hatS(t)}
% \end{align} 
% and satisfies by 
% Lemma~\ref{lm:|AB|<=|A||B|} that  
% \begin{align} 
% |S(u-1) - \widehat{S}(u-1)| 
%  \leq & | [M(P(u))]^{-1} | \cdot 
% \big[  |S(u) - \widehat{S}(u)| + \lambda |\Theta^\star - \Theta^\star_{(N)}|
%  \big] \notag \\ 
%  & + \big| ( M(\widehat{P}(u)))^{-1} 
%   - ( M(P(u)) )^{-1} \big| \cdot  
%  \big( |\widehat{S}(u)| + \lambda |\Theta^\star_{(N)}| \big) . \label{|hatS-S|recursion}
% \end{align} 
% By \eqref{|hatS-S|recursion}, \eqref{estMPw-MP1/N}, Remark~\ref{rmk:M(hatP)bdd}, and the induction hypothesis, we have that 
% \eqref{sup|S-hatS|est} holds for $t=u-1$. By induction we have shown that \eqref{sup|S-hatS|est} holds for all $t=1$, ..., $T$. 


% \end{proof}


% We now obtain Theorem~\ref{thrm:Epsilon_Efficiency}; which is a direct consequence of the following Propositions \ref{prop:stabilityaw-a1/N} and \ref{prop:stabilityLw-L1/N}.

% \begin{proposition} 
% \label{prop:stabilityaw-a1/N}
% The controls
% \eqref{optimala} and \eqref{hata} satisfy $|\widehat{\boldsymbol{\alpha}}(t)| \leq C \cdot N^{1/2}$ for all $t=0$, $1$, ..., $T-1$, and  
% \allowdisplaybreaks\begin{align} 
%  \sum_{t=0}^{T-1} |\boldsymbol{\alpha}(t) - \widehat{\boldsymbol{\alpha}}(t)| 
%  \leq & C\cdot \Big\{ \bar{N} N^{3/2} \max_{1\leq i, k, l \leq N} \Big| \frac{1}{N^3} -  w^\star_k w^\star_l w^\star_i \Big| \notag \\ 
%  &\hspace{2cm} + \bar{N} N^{1/2} \cdot \max_{1\leq k, l\leq N} \Big| \frac{1}{N^2} - w^\star_k w^\star_l \Big| 
%  + |\Theta^\star - \Theta^\star_{(N)}| \Big\} , 
% \label{eqn:stabilityaw-a1/N}
% \end{align} 
% where $C>0$ is a constant depending on $\lambda$, $\beta$, $\Theta^\star$, $K_x$, $K_y$, and $T$. 
% \end{proposition} 

% \begin{proof}[{Proof of Proposition~\ref{prop:stabilityaw-a1/N}}]
% We let $C$ be a constant depending on $\lambda$, $\beta$, $\Theta^\star$, $K_x$, $K_y$, and $T$, 
% and $C$ is allowed to vary from place to place throughout the proof. 
% By \eqref{optimala}, \eqref{hata}, and \eqref{Theta(t)Theta(0)}, we can write $\boldsymbol{\alpha}$ and $\widehat{\boldsymbol\alpha}$ as   
% \allowdisplaybreaks\begin{align} 
%   \boldsymbol{\alpha}(t) 
%  = & [ (M(P(t+1)))^{-1} - I_{Np} ]  \Big[ \Theta^\star 
%  + \sum_{u=0}^{t-1} \boldsymbol{\alpha}(u) \Big]  
%   +  [ M(P(t+1)) ]^{-1} ( \lambda  \Theta^\star - S(t+1) ) ,   \notag \\ 
%   \widehat{\boldsymbol{\alpha}}(t) 
%  = & [ (M(\widehat{P}(t+1)))^{-1} - I_{Np} ]  \Big[ \Theta^\star 
%  + \sum_{u=0}^{t-1} \widehat{\boldsymbol{\alpha}}(u) \Big]  
%   +  [ M(\widehat{P}(t+1)) ]^{-1} ( \lambda  \Theta^\star_{(N)} - \widehat{S}(t+1) ) .   \notag 
% \end{align} 
% For $t=0$, we have 
% \begin{align} 
%  |\widehat{\boldsymbol{\alpha}}(0)| \leq  & | (M(\widehat{P}(1)))^{-1} - I_{Np} | \cdot |  \Theta^\star |   
%   + \big| [ M(\widehat{P}(1)) ]^{-1} \big| ( \lambda  |\Theta^\star_{(N)}| + |\widehat{S}(1)| ) ,  \notag 
% \end{align} 
% which implies $|\widehat{\boldsymbol{\alpha}}(0)| \leq C N^{1/2}$. 
% Assume by induction that $|\widehat{\boldsymbol{\alpha}}(u)| \leq C N^{1/2}$ for $u=0$, ..., $t-1$, then 
% \begin{align} 
% \widehat{\boldsymbol{\alpha}}(t) 
%  \leq & \big| (M(\widehat{P}(t+1)))^{-1} - I_{Np} \big|   \Big[ | \Theta^\star | 
%  + \sum_{u=0}^{t-1} | \widehat{\boldsymbol{\alpha}}(u) | \Big] \notag \\  
%  & + \big| [ M(\widehat{P}(t+1)) ]^{-1} \big| ( \lambda | \Theta^\star_{(N)} | + | \widehat{S}(t+1) | ) \notag 
% \end{align} 
% gives that $|\widehat{\boldsymbol{\alpha}}(t)|\leq CN^{1/2}$. By induction we have shown that 
% $|\widehat{\boldsymbol{\alpha}}(t)|\leq CN^{1/2}$ for all $t=0$, $1$, ..., $T-1$. 



% We further write the difference $\boldsymbol{\alpha} - \widehat{\boldsymbol\alpha}$ as    
% \allowdisplaybreaks\begin{align}  
%  & \boldsymbol{\alpha}(t) - \widehat{\boldsymbol\alpha}(t) \notag \\ 
%  = &  \big[(M(P(t+1)))^{-1} - (M(\widehat{P}(t+1)) )^{-1} \big] 
%  \Big[ (\lambda + 1)\Theta^\star + \sum_{u=0}^{t-1}  \boldsymbol{\alpha}(u)    - S(t+1) \Big]  \notag \\ 
%  & + \big[ ( M(\widehat{P}(t+1)) )^{-1} - I_{Np} \big] 
%  \sum_{u=0}^{t-1} (\boldsymbol{\alpha}(u) - \widehat{\boldsymbol{\alpha}}(u)) 
% + [ M(\widehat{P}(t+1)) ]^{-1} (\widehat{S}(t+1) - S(t+1))  \notag \\ 
%  & + \lambda [ M(\widehat{P}(t+1)) ]^{-1} ( \Theta^\star 
%  - \Theta^\star_{(N)} ) . \label{a-hata} 
% \end{align} 


% For $t=0$, the difference 
% \allowdisplaybreaks\begin{align} 
%   \boldsymbol{\alpha}(0) - \widehat{\boldsymbol{\alpha}}(0)  
%  = & \big[ (M(P(1)))^{-1} - (M(\widehat{P}(1)))^{-1}  \big] 
%  \big[ ( \lambda + 1 )   \Theta^\star_{(N)} - \widehat{S}(1)  \big] \notag \\ 
%  & + [ M(P(1)) ]^{-1} [ (\lambda+1) (\Theta^\star - \Theta^\star_{(N)} ) + \widehat{S}(1) - S(1) ]   \notag  
% \end{align} 
% satisfies 
% \allowdisplaybreaks\begin{align} 
%   \big| \boldsymbol{\alpha}(0) 
%    - \widehat{\boldsymbol{\alpha}}(0) \big| 
%   \leq & 
%   C  \cdot \Big\{ \bar{N} N^{3/2} \max_{1\leq i, k, l \leq N} \Big| \frac{1}{N^3} -  w^\star_k w^\star_l w^\star_i \Big| \notag \\ 
%  & \hspace{1cm} + \bar{N} N^{1/2} \max_{1\leq k, l\leq N} \Big| \frac{1}{N^2} - w^\star_k w^\star_l \Big|
%  + |\Theta^\star - \Theta^\star_{(N)}| \Big\} , \notag    
% \end{align} 
% due to \eqref{estMPw-MP1/N}, \eqref{sup|S-hatS|est}, Lemma~\ref{lm:|AB|<=|A||B|}, Corollary~\ref{cor:M(P)invbdd} and Remark~\ref{rmk:M(hatP)bdd}.  
% Assume by induction for all $0 \leq u\leq t-1$, 
% $\boldsymbol{\alpha}(u-1) - \widehat{\boldsymbol{\alpha}}(u-1)$ satisfies
% \allowdisplaybreaks\begin{align} 
%   \big| \boldsymbol{\alpha}(u-1) 
%   - \widehat{\boldsymbol{\alpha}}(u-1) \big| 
%   \leq & C   
%  \cdot \Big\{ \bar{N} N^{3/2} \max_{1\leq i, k, l \leq N} \Big| \frac{1}{N^3} -  w^\star_k w^\star_l w^\star_i \Big| \notag \\ 
% & \hspace{1cm} + \bar{N} N^{1/2} \max_{1\leq k, l\leq N} \Big| \frac{1}{N^2} - w^\star_k w^\star_l \Big| 
%  + |\Theta^\star - \Theta^\star_{(N)}| \Big\}  . \notag   
% \end{align} 
% By \eqref{a-hata} we have  
% \allowdisplaybreaks\begin{align}  
%  & | \boldsymbol{\alpha}(t) - \widehat{\boldsymbol{\alpha}}(t) | \notag \\ 
%  \leq &  \big| (M(P(t+1)))^{-1} - (M(\widehat{P}(t+1)) )^{-1} \big| \cdot 
%  \Big[ \sum_{u=0}^{t-1}  | \boldsymbol{\alpha}(u) |   
%  + | ( \lambda +1 ) \Theta^\star | 
%  +| S(t+1) | \Big]  \notag \\ 
%  & + \big| ( M(\widehat{P}(t+1)) )^{-1} - I_{Np}  \big| 
%  \sum_{u=0}^{t-1} | \boldsymbol{\alpha}(u) - \widehat{\boldsymbol{\alpha}}(u) | 
% + | (M(\widehat{P}(t+1)))^{-1} | \cdot | S(t+1) - \widehat{S}(t+1) | ,  \notag   \\ 
%  & + \big| [ M(\widehat{P}(t+1)) ]^{-1} \big| \cdot |\lambda | \cdot 
%   \big| \Theta^\star - \Theta^\star_{(N)} \big| . \notag  
% \end{align} 
% By the induction hypothesis, \eqref{estMPw-MP1/N}, 
% \eqref{sup|S-hatS|est}, and Remark~\ref{rmk:M(hatP)bdd},  the above inequality implies that  
% \allowdisplaybreaks\begin{align}
%  |\boldsymbol{\alpha}(t) - \widehat{\boldsymbol{\alpha}}(t)| 
%  \leq & C \cdot \Big\{ \bar{N} N^{3/2} \max_{1\leq i, k, l \leq N} \Big| \frac{1}{N^3} -  w^\star_k w^\star_l w^\star_i \Big| 
%   \notag \\
% & \hspace{1cm} + \bar{N} N^{1/2} \max_{1\leq k, l\leq N} \Big| \frac{1}{N^2} - w^\star_k w^\star_l \Big| 
%  + |\Theta^\star - \Theta^\star_{(N)}| \Big\}  . \label{|a(t)-hata(t)|est}  
% \end{align}
% We have shown by induction that \eqref{|a(t)-hata(t)|est} holds for all $t=0$, $1$, ..., $T-1$, 
% and therefore \eqref{eqn:stabilityaw-a1/N} follows.  
% \end{proof} 

% \begin{proposition} 
% \label{prop:stabilityLw-L1/N} 
% Under the hypothesis of Proposition \ref{prop:stabilityaw-a1/N}, the costs \eqref{eq:penalized_regret_functional} under the controls \eqref{optimala} 
% and \eqref{hata}, respectively, satisfy the estimate 
% \allowdisplaybreaks\begin{align} 
%  \big| L^\star (  \boldsymbol{\alpha} ; \mathcal{D} ) 
%  -  L^\star (  \widehat{\boldsymbol{\alpha}} ;  \mathcal{D} )  \big|  
%  \le &  C  \cdot \Big\{ \bar{N} N^3 \max_{1\leq i, k, l \leq N} \Big| \frac{1}{N^3} -  w^\star_k w^\star_l w^\star_i \Big| 
%   + \bar{N} N^{3/2} \max_{1\leq k, l\leq N} \Big| \frac{1}{N^2} - w^\star_k w^\star_l \Big| 
%   \notag \\
% & \hspace{3cm} 
%  + \bar{N} \max_{1\leq i \leq N} \Big|\frac{1}{N} - w_i^\star \Big|
%  + N |\Theta^\star - \Theta^\star_{(N)}| \Big\}  ,  
% \label{stabilityLw-L1/N} 
% \end{align} 
% where $C>0$ is a constant depending on $\lambda$, $\beta$, $\Theta^\star$, $(w_1^\star, ..., w_N^\star)$,  
% $K_x$, $K_y$ and $T$. 
% \end{proposition} 

% \begin{proof}[Proof of Proposition~\ref{prop:stabilityLw-L1/N} ] 
% Let $L^\star(\widehat{\boldsymbol{\alpha}}; \overline{1/N} , \mathcal{D})$, 
% $L^\star( \widehat{\boldsymbol{\alpha}}; w^\star, \mathcal{D})$, and
% $L^\star(\boldsymbol{\alpha}; w^\star , \mathcal{D})$ be as defined in 
% Lemmas~\ref{lm:|L(hata;1/N)-L(hata;w)|est} 
% and~\ref{lm:|L(a;w)-L(hata;1/N)|est}.   
% The difference $L^\star(\boldsymbol{\alpha}; \mathcal{D}) - L^\star( \widehat{\boldsymbol{\alpha}}; \mathcal{D})$ can be decomposed as 
% \begin{align} 
% L^\star(\boldsymbol{\alpha}; \mathcal{D}) - L^\star( \widehat{\boldsymbol{\alpha}}; \mathcal{D}) 
% = L^\star(\boldsymbol{\alpha}; w^\star, \mathcal{D}) - L^\star(\widehat{\boldsymbol{\alpha}}; \overline{1/N}, \mathcal{D}) 
%  + L^\star(\widehat{\boldsymbol{\alpha}}; \overline{1/N} , \mathcal{D}) 
%   - L^\star( \widehat{\boldsymbol{\alpha}}; w^\star, \mathcal{D}) ,\notag 
% \end{align}  
% and satisfies    
% \begin{align} 
%  | L^\star(\boldsymbol{\alpha}; \mathcal{D}) - L^\star( \widehat{\boldsymbol{\alpha}}; \mathcal{D}) | 
% \leq | L^\star(\boldsymbol{\alpha}; w^\star, \mathcal{D}) - L^\star(\widehat{\boldsymbol{\alpha}}; \overline{1/N}, \mathcal{D}) |
%  + | L^\star(\widehat{\boldsymbol{\alpha}}; \overline{1/N} , \mathcal{D}) 
%   - L^\star( \widehat{\boldsymbol{\alpha}}; w^\star, \mathcal{D}) | . \notag 
% \end{align} 
% The desired estimate \eqref{stabilityLw-L1/N} then follows from the above inequality and \eqref{|L(hata,1/N)-L(hata,w)|est} 
% and \eqref{|L(a,w)-L(hata,1/N)|est}. 
% \end{proof} 


% \begin{lemma}
% \label{lm:|L(hata;1/N)-L(hata;w)|est} 
% Let $L^\star(\widehat{\boldsymbol{\alpha}}; w^\star, \mathcal{D})$ be \eqref{eq:penalized_regret_functional} with 
% information sharing weights $w^\star=(w_1^\star, ..., w_N^\star)$ and $\Theta(t+1)-\Theta(t)=\widehat{\boldsymbol{\alpha}}(t)$, 
% and let $L^\star(\widehat{\boldsymbol{\alpha}}; \overline{1/N} , \mathcal{D})$ be \eqref{eq:penalized_regret_functional} with information sharing weights $\overline{1/N}=(1/N, ..., 1/N)$ and $\Theta(t+1)-\Theta(t)=\widehat{\boldsymbol{\alpha}}(t)$. 
% Then it satisfies 
% \begin{align} 
%  | L^\star(\widehat{\boldsymbol{\alpha}}; \overline{1/N} , \mathcal{D}) 
%   - L^\star( \widehat{\boldsymbol{\alpha}}; w^\star, \mathcal{D}) | \leq C  \cdot 
%   \Big\{ \bar{N} \max_{1\leq i \leq N} \Big|\frac{1}{N} - w_i^\star \Big| + N^{1/2} |\Theta^\star-\Theta^\star_{(N)}| \Big\} 
%   \label{|L(hata,1/N)-L(hata,w)|est} , 
% \end{align} 
% where $C>0$ is a constant depending on $\lambda$, $\beta$, $\Theta^\star$, 
% $(w^\star_1, \cdots, w^\star_N)$, $K_x$, $K_y$ and $T$. 
% \end{lemma} 
% \begin{proof} 
% By \eqref{eq:penalized_regret_functional} and \eqref{lwT}, we have 
% \begin{align} 
%    L^\star(\widehat{\boldsymbol{\alpha}}; \overline{1/N} , \mathcal{D}) 
%   - L^\star( \widehat{\boldsymbol{\alpha}}; w^\star, \mathcal{D}) 
%  = & \sum_{t=0}^{T-1} \big( |\Theta(t+1) - \Theta^\ast|^2 - |\Theta(t+1) - \Theta_{(N)}^\ast|^2 \big) \notag \\ 
%  & + l(\Theta(T), \overline{1/N}; \mathcal{D} ) - l(\Theta(T), w^\star ; \mathcal{D} ) .\notag  
% \end{align} 
% We have that
% \begin{equation}
% \label{|L(hata,1/N)-L(hata,w)|rcest} 
% \begin{aligned} 
%  &  \Big| \sum_{t=0}^{T-1} \big( |\Theta(t+1) - \Theta^\ast|^2 - |\Theta(t+1) - \Theta_{(N)}^\ast|^2 \big) \Big|  
%  \\
%  =&   \Big| \sum_{t=0}^{T-1} (\Theta^\star_{(N)} - \Theta^\star)^\top (2 \Theta(t+1) - \Theta^\star - \Theta^\star_{(N)}) \Big| \notag \\ 
%  \le & \sum_{t=0}^{T-1} | \Theta^\star_{(N)} - \Theta^\star | \cdot 
%  | 2 \Theta(t+1) - \Theta^\star - \Theta^\star_{(N)}|  
%  \leq C N^{1/2} \cdot  |\Theta^\star_{(N)} - \Theta^\star| ,  
% \end{aligned} 
% \end{equation}
% %where the last inequality is due to that $|\widehat{\boldsymbol{\alpha}}(t)|\leq C\cdot N$ for all $t=0$, $1$, ..., $T-1$ by %Proposition~\ref{prop:stabilityaw-a1/N}. 
% and 
% \begin{align} 
%  & l(\Theta(T), \overline{1/N}; \mathcal{D} ) - l(\Theta(T), w^\star ; \mathcal{D} )  \notag \\ 
%  = &  \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|}  \Big[ u^{i\top}_j \sum_{k=1}^N w^\star_k \theta_k - y^i_j  \Big]^2 
%  - \sum_{i=1}^N \frac{1}{N} \sum_{j=1}^{|\mathcal{D}_i|}  \Big[ u^{i\top}_j \sum_{k=1}^N \frac{1}{N} \theta_k - y^i_j  \Big]^2 
%   \notag \\ 
%   =& \sum_{i=1}^N (w^\star_i - 1/N) \sum_{j=1}^{|\mathcal{D}_i|}  \Big[ u^{i\top}_j \sum_{k=1}^N w^\star_k \theta_k - y^i_j  \Big]^2 \notag \\ 
%  &  + \sum_{i=1}^N \frac{1}{N} \sum_{j=1}^{|\mathcal{D}_i|}  
%  \Big[ u^{i\top}_j \sum_{k=1}^N (w^\star_k -1/N) \theta_k   \Big] 
%   \Big[ u^{i\top}_j \sum_{k=1}^N ( w^\star_k + 1/N ) \theta_k - 2 y^i_j  \Big]^2 , \notag 
% \end{align} 
% which implies that 
% \begin{align} 
%  | l(\Theta(T), \overline{1/N}; \mathcal{D} ) - l(\Theta(T), w^\star ; \mathcal{D} ) | 
%  \leq C \bar{N} \max_{1\leq i \leq N} |1/N - w_i^\star| . 
%  \label{|L(hata,1/N)-L(hata,w)|Test}
% \end{align} 
% The estimate \eqref{|L(hata,1/N)-L(hata,w)|est} then follows from 
% \eqref{|L(hata,1/N)-L(hata,w)|rcest}
% and \eqref{|L(hata,1/N)-L(hata,w)|Test}. 
% \end{proof} 


% \begin{lemma}
% \label{lm:|L(a;w)-L(hata;1/N)|est} 
% Let $L^\star(\alpha; w^\star, \mathcal{D})$ be \eqref{eq:penalized_regret_functional} with 
% information sharing weights $w^\star=(w_1^\star, ..., w_N^\star)$ and $\Theta(t+1)-\Theta(t)= \boldsymbol{\alpha}(t)$, 
% and let $L^\star(\widehat{\boldsymbol{\alpha}}; \overline{1/N} , \mathcal{D})$ be \eqref{eq:penalized_regret_functional} with information sharing weights $\overline{1/N}=(1/N, ..., 1/N)$ and $\Theta(t+1)-\Theta(t)=\widehat{\boldsymbol{\alpha}}(t)$. 
% Then it satisfies 
% \begin{align} 
%  & | L^\star(\boldsymbol{\alpha}; w^\star , \mathcal{D}) 
%   - L^\star( \widehat{\boldsymbol{\alpha}}; \overline{1/N}, \mathcal{D}) | 
%   \leq   
%    C \cdot  \Big\{ \bar{N} N^3 \cdot \max_{1\leq i, k, l \leq N} \Big| \frac{1}{N^3} -  w^\star_k w^\star_l w^\star_i \Big| 
%   \notag \\
% & \hspace{1.5cm} 
% +\bar{N} N^{3/2} \max_{1\leq k, l\leq N} \Big| \frac{1}{N^2} - w^\star_k w^\star_l \Big|  + \bar{N} \cdot \max_{1\leq i \leq N} \Big| \frac{1}{N} - w_i^\star \Big|
% + N |\Theta^\star - \Theta^\star_{(N)}| \Big\} , 
%   \label{|L(a,w)-L(hata,1/N)|est}
% \end{align} 
% where $C$ is a constant depending on $\lambda$, $\beta$, $\Theta^\star$, 
% $(w^\star_1, \cdots, w^\star_N)$, $K_x$, $K_y$ and $T$. 
% \end{lemma} 

% \begin{proof} 
% By the similar argument for \eqref{ansatzVw}, we have 
% \begin{align} 
%  L^\star( \widehat{\boldsymbol{\alpha}}; \overline{1/N}, \mathcal{D}) 
%   = \Theta^{\star\top}  \widehat{P}(0)  \Theta^\star 
%  + 2\widehat{S}(0)^\top \Theta^\star + \widehat{r}(0) . \label{ansatzV1/N} 
% \end{align} 
% By \eqref{ansatzVw} and \eqref{ansatzV1/N}, the difference $L^\star(\boldsymbol{\alpha}; w^\star, \mathcal{D}) - L^\star( \widehat{\boldsymbol{\alpha}}; \overline{1/N}, \mathcal{D})$ can be written as 
% \allowdisplaybreaks\begin{align} 
%   L^\star(\boldsymbol{\alpha}; w^\star, \mathcal{D}) - L^\star( \widehat{\boldsymbol{\alpha}}; \overline{1/N}, \mathcal{D}) 
% = \Theta^{\star\top} ( P(0) - \widehat{P}(0) ) \Theta^\star 
%  + 2 ( S(0) - \widehat{S}(0) )^\top \Theta^\star + r(0)-\widehat{r}(0) ,  
%  \notag 
% \end{align} 
% and by Lemma~\ref{lm:|AB|<=|A||B|}, the difference satisfies  
% \allowdisplaybreaks\begin{align} 
%   \big| L^\star (  \boldsymbol{\alpha} ; w^\star, \mathcal{D} ) 
%  -  L^\star (  \widehat{\boldsymbol{\alpha}} ; \overline{1/N} , \mathcal{D} ) \big|  
% \le & |\Theta^\star|^2 \cdot |  P(0) - \widehat{P}(0) |  
%  + 2 | S(0) - \widehat{S}(0) | \cdot | \Theta^\star| 
%  \nonumber
%  \\ 
%  & + | r(0)-\widehat{r}(0) | . \label{|L(a,w)-L(hata,1/N)|leqQudratic}
% %\label{estLast-tildeLast} 
% \end{align}
% We claim that $r(0)-\widehat{r}(0)$ has the estimate 
% \allowdisplaybreaks\begin{align} 
%  | r(0)-\widehat{r}(0) | \le &  C  \cdot  \Big\{ \bar{N} N^3 \cdot \max_{1\leq i, k, l \leq N} \Big| \frac{1}{N^3} -  w^\star_k w^\star_l w^\star_i \Big| 
%  +\bar{N} N^{3/2} \max_{1\leq k, l\leq N} \Big| \frac{1}{N^2} - w^\star_k w^\star_l \Big| 
%   \notag \\
% & \hspace{2cm} 
%  + \bar{N} \cdot \max_{1\leq i \leq N} \Big| \frac{1}{N} - w_i^\star \Big|
% + N \cdot |\Theta^\star - \Theta^\star_{(N)}| \Big\}  , 
% \label{eqn:estrw-tilder1/N} 
% \end{align} 
% where $C$ is a constant depending on $\lambda$, $\beta$, $\Theta^\star$, 
% $(w^\star_1, \cdots, w^\star_N)$, $K_x$, $K_y$ and $T$. 
% Then the desired estimate \eqref{|L(a,w)-L(hata,1/N)|est} is established by \eqref{|L(a,w)-L(hata,1/N)|leqQudratic}, \eqref{estPw-P1/N}, \eqref{sup|S-hatS|est} and \eqref{eqn:estrw-tilder1/N}. 



% Now we prove the claim \eqref{eqn:estrw-tilder1/N}. 
% From \eqref{eqn:Vansatz} and \eqref{lwT}, we obtain the equation that $\widehat{r}$ satisfies on $0\leq t \leq T$: 
% \begin{align} 
% &\begin{cases} 
%  \widehat{r}(t) =  - ( \widehat{S}(t+1) - \lambda \Theta_{(N)}^\star )^\top
%  [(\lambda+\beta)I_{Np} + \widehat{P}(t+1)]^{-1} \cdot ( \widehat{S}(t+1) - \lambda \Theta_{(N)}^\star )   \\  
%  \hspace{1.1cm}   + \lambda \| \Theta_{(N)}^\star \|_2^2 + \widehat{r}(t+1), 
%  \label{eqnhatr(t)} \\ \widehat{r}(T) = \sum_{i=1}^N (1/N) \sum_{j=1}^{|\mathcal{D}_i|} |y^i_j|^2 . 
%  \end{cases}  
% \end{align} 
% %\allowdisplaybreaks\begin{align} 
% %\begin{cases}
% %  r(t) =  r(t+1) - S^\top(t+1) (M(P(t+1)))^{-1} S(t+1)  
% % + 2 \lambda S^\top(t+1) (M(P(t+1)))^{-1}  \Theta^\star  \\ 
% %  \hspace{1cm} + \Theta^{\star \top} \big[ \lambda I_{Np} - \lambda^2 (M(P(t+1)))^{-1}  \big] \Theta^\star  ,  \\ 
% %%% 
% %  r(T) = \sum_{i=1}^N w^\star_i \sum_{j=1}^{|\mathcal{D}_i|} |y^i_j|^2 .    
% %\end{cases} 
% %\notag 
% %\label{eqnr(t)}
% %\end{align} 
% Then $r-\widehat{r}$ satisfies the equation on $0\leq t \leq T$
% \allowdisplaybreaks\begin{align} 
%  & r(t) - \widehat{r}(t) \notag \\ 
% = &  r(t+1) - \widehat{r}(t+1) + \lambda (\Theta^\star - \Theta^\star_{(N)}) (\Theta^\star + \Theta^\star_{(N)}) \notag \\  
% & - (S(t+1) - \lambda \Theta^\star)^\top \big[ (M(P(t+1)))^{-1} - (M(\widehat{P}(t+1)))^{-1} \big] (S(t+1)-\lambda \Theta^\star) \notag \\ 
% & - \big[ S(t+1) - \widehat{S}(t+1) - \lambda (\Theta^\star - \Theta_{(N)}^\star ) \big] 
%  (M(\widehat{P}(t+1)))^{-1} 
%  \cdot 
% \\
% \notag
% & \qquad
% \big[ S(t+1) + \widehat{S}(t+1) - \lambda (\Theta^\star + \Theta_{(N)}^\star ) \big] , \notag \\ 
% %%% 
% & r(T) - \widehat{r}(T) = \sum_{i=1}^N (w_i^\star - 1/N) \sum_{j=1}^{|\mathcal{D}_i|} |y^i_j|^2 . \notag  
% \end{align} 
% Inductively, we have  
% \allowdisplaybreaks\begin{align} 
%   r(0) - \widehat{r}(0)  
% = &   r(T) - \widehat{r}(T) + T \lambda (\Theta^\star - \Theta^\star_{(N)}) (\Theta^\star + \Theta^\star_{(N)})   \notag \\  
%  & - \sum_{t=1}^T (S(t) - \lambda \Theta^\star)^\top \big[ (M(P(t)))^{-1} - (M(\widehat{P}(t)))^{-1} \big] (S(t)-\lambda \Theta^\star)   \notag  \\  
% %%% 
% &  - \sum_{t=1}^T \big[ S(t) - \widehat{S}(t) - \lambda (\Theta^\star - \Theta_{(N)}^\star ) \big] 
%  (M(\widehat{P}(t)))^{-1} \big[ S(t) + \widehat{S}(t) - \lambda (\Theta^\star + \Theta_{(N)}^\star ) \big] . \notag 
% \end{align}
% By Lemma~\ref{lm:|AB|<=|A||B|}, we have 
% \allowdisplaybreaks\begin{align} 
%  & | r(0) - \widehat{r}(0) | \leq |r(T) - \widehat{r}(T)| 
%   + T \lambda | \Theta^\star - \Theta^\star_{(N)} | \cdot | \Theta^\star + \Theta^\star_{(N)} |   \notag \\ 
% &  + \sum_{t=1}^T  \big| (M(P(t)))^{-1} - (M(\widehat{P}(t)))^{-1} \big| \cdot 
%  \big| S(t)-\lambda \Theta^\star \big|^2   \notag  \\  
% %%% 
% &  + \sum_{t=1}^T \big[ | S(t) - \widehat{S}(t) | + \lambda | \Theta^\star - \Theta_{(N)}^\star | \big] \cdot 
%  \big| (M(\widehat{P}(t)))^{-1} \big| \cdot \big| S(t) + \widehat{S}(t) - \lambda (\Theta^\star + \Theta_{(N)}^\star ) \big| .  \label{estrw(0)-tilder1/N(0)}  
% \end{align}
% Then the estimate \eqref{eqn:estrw-tilder1/N} follows from 
% \eqref{estrw(0)-tilder1/N(0)}, \eqref{estMPw-MP1/N}, 
% \eqref{sup|S-hatS|est}, and Remark~\ref{rmk:M(hatP)bdd}. 
% \end{proof}

%     \begin{proof}[{Proof of Theorem~\ref{thrm:Epsilon_Efficiency}}]
%         Under Assumptions~\ref{assm:bddxy} and~\ref{assm:PD}, the existence of the regret-optimal algorithm $\theta_{\cdot}$ is implied by Theorem~\ref{thm:RegretOptimal_Dynamics}.  The first claim follows from Proposition~\ref{prop:stabilityaw-a1/N} upon noting that the constant ``$C_w$'' therein is bounded as a function of $w$; whence we take the constant $C$ hidden by $\mathcal{O}$ to be $C\eqdef \sup_{w\in [0,1]^N\,\sum_{i=1}^N\,w_i=1}\, C_w$.  Likewise, the second statement follows directly from Corollary~\ref{cor:stabilityLast} upon defining the constant hidden by $\mathcal{O}$ as before.  
%     \end{proof}



% Further investigation of the ``symmetrized system'' \eqref{eqnhatP1/N(t)} reveals a symmetric form of $\widehat{P}$, which suggests that  $\widehat{P}$ can be decomposed into homogeneous submatrices of lower dimensions. 
% Specifically, if we decompose the high dimensional $Np\times Np$ matrix $\widehat{P}$ into $N\times N$ submatrices of dimensions $p\times p$ each,  and either exchange two submatrices symmetrically positioned with respect to the diagonal of $\widehat{P}$ or exchange two submatrices on the diagonal, the system \eqref{eqnhatP1/N(t)} is invariant. 
% This suggests that all the submatrices on the diagonal are homogeneous and all the off-diagonal submatrices are homogeneous.
% %%%%%%%%%%
% \begin{proposition}[Symmetries in $\widehat{P}$] 
% \label{prop:P1/Nsubmat}
% The solution of \eqref{eqnhatP1/N(t)} has the following submatrix decomposition  
% \begin{align} 
%  \widehat{P} = \begin{bmatrix} \pi_1 & \pi_2 & \cdots & \pi_2 \\ 
%  \pi_2 & \pi_1 & \cdots &\pi_2 \\ 
% \vdots & \vdots & \ddots & \vdots \\ 
%  \pi_2 & \pi_2 & \cdots & \pi_1 
%  \end{bmatrix} \in \mathbb{R}^{Np\times Np}, 
% \quad \pi_1 \in \mathbb{R}^{p\times p}, \quad 
% \pi_2 \in \mathbb{R}^{p\times p} , 
% \label{hatPpi12}
% \end{align} 
% and the submatrices $\pi_1$ and $\pi_2$ are uniquely determined by the system   
% \allowdisplaybreaks\begin{align}  
% \begin{cases}
%   \pi_1(t) =  \beta I_p - \beta^2 \gamma_1(t+1)  ,  
% \label{eqnpi1pi2}  \\ 
%    \pi_2(t) =  - \beta^2 \gamma_2(t+1) ,  \quad 1\leq t \leq T-1 , \\
%  \pi_1(T) = \pi_2(T) = (1/N^3)\sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|} u^i_j u^{i\top}_j ,   
% \end{cases} 
% \end{align}
% where $\gamma_1(\cdot)$ and $\gamma_2(\cdot)$ are defined as 
% \eqref{gamma1} and \eqref{gamma2}. 
% \end{proposition} 


% We argue as in \cite[Lemmata 1]{huang2021linear} in deriving the following submatrix decomposition of $\widehat{P}$. 
% \begin{proof}[{Proof of Proposition~\ref{prop:P1/Nsubmat}}]
% We decompose the $Np\times Np$ identity matrix into $N\times N$ submatrices
% $I=(I_{ij})_{1\leq i, j \leq N}$ with each 
% $I_{ij}\in \mathbb{R}^{p\times p}$.  
% For each $1\leq i, j \leq N$, by $E_{ij} $we denote the $Np\times Np$ elementary matrix by exchanging the $i$th and $j$th rows of submatrices of the $Np\times Np$ identity matrix $I=(I_{ij})_{1\leq i, j \leq N}$. Note that $E_{ij}=E_{ij}^{-1}=E_{ij}^T$. 
% Multiplying both sides of \eqref{eqnP(t)} from the left by $E_{ij}$ and from the right by $E_{ij}$, we obtain  
% \allowdisplaybreaks\begin{align} 
% & \begin{cases}
%    E_{ij} \widehat{P}(t) E_{ij}  
% =  \beta I_{Np} - \beta^2 [(\lambda+\beta ) I_{Np} + E_{ij} \widehat{P}(t+1) E_{ij} ]^{-1} ,  \\ 
%   E_{ij} \widehat{P}(T) E_{ij} =  [ (1/N) I_p ,\cdots, (1/N) I_p ]^\top 
%  \Big( \sum_{i=1}^N \frac{1}{N} \sum_{j=1}^{|\mathcal{D}_i|}  u^i_j u^{i\top}_j  \Big)  
%  [ (1/N) I_p , \cdots, (1/N) I_p ] .   
% \end{cases}   \label{eqnEijtildePEij}
% \end{align} 
% Comparing \eqref{eqnEijtildePEij} and \eqref{eqnhatP1/N(t)} reveals that 
%  $\widehat{P}(t)$ and $E_{ij} \widehat{P}(t) E_{ij}$ satisfy the same ODE for all $1\leq i, j \leq N$. This observation implies that 
% \allowdisplaybreaks\begin{align} 
%  \widehat{P}_{ii} = \widehat{P}_{jj}, \quad \widehat{P}_{ij} = \widehat{P}_{ji} , \quad \widehat{P}_{ik}= \widehat{P}_{jk}, \quad 
% \widehat{P}_{ki} = \widehat{P}_{kj}, \quad \forall 1\leq i, j \leq N, \quad \forall k \neq i, j , \notag 
% \end{align} 
% and the first assertion of the proposition is proved. 


% Since $\widehat{P}$ takes the form \eqref{hatPpi12}, 
% it is straight forward to verify that $[(\lambda+\beta)I_{Np} + \widehat{P}]^{-1}$ takes the form 
% \allowdisplaybreaks\begin{align} 
%  [(\lambda+\beta) I_{Np} + \widehat{P}]^{-1} = \begin{bmatrix} \gamma_1 & \gamma_2 & \cdots & \gamma_2 \\ 
%  \gamma_2 & \gamma_1 & \cdots &\gamma_2 \\ 
% \vdots & \vdots & \ddots & \vdots \\ 
%  \gamma_2 & \gamma_2 & \cdots & \gamma_1 
%  \end{bmatrix} , \label{[(lambda+1)I+P]inv}
% \end{align} 
% with $\gamma_1$ and $\gamma_2$ given by \eqref{gamma1} and \eqref{gamma2}. 

% We substitute \eqref{hatPpi12} and \eqref{[(lambda+1)I+P]inv} into \eqref{eqnhatP1/N(t)} to obtain the equations \eqref{eqnpi1pi2}.  
% \end{proof}

% Upon substituting $\widehat{P}$  into \eqref{eqnhatS1/N(t)}, we find that the $Np\times 1$ matrix $\widehat{S}$ can be decomposed into homogeneous submatrices of dimensions $p\times 1$ each.  
% \begin{proposition} \label{prop:SubmatrixReduction}
% The solution of \eqref{eqnhatS1/N(t)} can be decomposed into submatrices 
% \begin{align} 
% \widehat{S}=(\pi_3^\top, \cdots, \pi_3^\top )^\top \in \mathbb{R}^{Np\times 1}, 
% \quad \pi_3 \in \mathbb{R}^{p\times 1} , 
% \label{hatSpi3}
% \end{align} 
% and $\pi_3$ satisfies
% \allowdisplaybreaks\begin{align} 
% \begin{cases}
%   \pi_3(t) = \beta \big[ \gamma_1(t+1) + (N-1) \gamma_2(t+1)  \big] 
%   ( \pi_3(t+1) - \lambda \theta^\star_{(N)} )   , \\   
%  \pi_3(T) = - (1/N^2) \sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|}  u^i_j y^i_j . 
% \end{cases}   \label{eqnpi3}
% \end{align} 
% \end{proposition}

% \begin{proof}[{Proof of Proposition~\ref{prop:SubmatrixReduction}}]
% We multiply both sides of \eqref{eqnhatS1/N(t)} from the left by $E_{ij}$ defined in the proof of Proposition \ref{prop:P1/Nsubmat}, 
% \allowdisplaybreaks\begin{align} 
%  E_{ij} \widehat{S}(t) = &  E_{ij} \beta [(\lambda + \beta )I_{Np} + \widehat{P}(t+1)]^{-1} (\widehat{S}(t+1) - \lambda \Theta^\star_{(N)})
% \notag \\ 
% = &    E_{ij} \beta [(\lambda + \beta )I_{Np} + \widehat{P}(t+1)]^{-1} E_{ij} E_{ij}(\widehat{S}(t+1) - \lambda \Theta^\star_{(N)}) \notag \\ 
% = &    \beta [(\lambda + \beta )I_{Np} + E_{ij} \widehat{P}(t+1)E_{ij}]^{-1}  ( E_{ij}\widehat{S}(t+1) - \lambda \Theta^\star_{(N)}) 
% \label{EijtildeS1/N(t)}
% \end{align}
% and 
% \allowdisplaybreaks\begin{align} 
%   E_{ij}\widehat{S}(T) = &  - E_{ij}[ (1/N) I_p, \cdots, (1/N) I_p ]^\top \sum_{i=1}^N \frac{1}{N} \sum_{j=1}^{|\mathcal{D}_i|}  u^i_j y^i_j \notag \\ 
% = &  - [ (1/N) I_p, \cdots, (1/N) I_p ]^\top \sum_{i=1}^N \frac{1}{N} \sum_{j=1}^{|\mathcal{D}_i|}  u^i_j y^i_j .   
% \label{EijtildeS1/N(T)} 
% \end{align}
% From \eqref{EijtildeS1/N(t)} and \eqref{EijtildeS1/N(t)}, we have that $E_{ij}\widehat{S}$ also satisfies \eqref{eqnhatS1/N(t)} for all 
% $1\leq i, j \leq N$. This proves that all submatrices of $\widehat{S}=(\widehat{S}_i)_{1\leq i \leq N}$ are equal on $0\leq t \leq T$. 
% We further substitute \eqref{hatPpi12}, \eqref{[(lambda+1)I+P]inv} and 
% $\widehat{S} = [\pi_3^\top, \cdots, \pi_3^\top]^\top$ into \eqref{eqnhatS1/N(t)} to obtain \eqref{eqnpi3}. 
% \end{proof} 



% \begin{corollary} 
% \label{cor:ComplexityAlgorithm__Heuristic}
% Fix a data set $\mathcal{D}$ and assume that \eqref{eq:moredatasets_than_dataperdataset} holds. Then the computational complexity of computing the sequence $\big( \theta(t) \big)_{t=0}^T$ by \eqref{hata} is 
% $\mathcal{O}(Tp^2 \max\{N, p^{0.373}\})$. 
% %$\mathcal{O}(TNp\max\{N,p\}))$. 
% \end{corollary}

% \begin{proof}[{Proof of Corollary~\ref{cor:ComplexityAlgorithm__Heuristic}}]
% \hfill\\ 
% \noindent \textbf{Complexity of computing $\pi_1(T)$, $\pi_2(T)$, and $\pi_3(T)$ is $O(N^2 p^2)$} \\ 
% Computing $u^i_j u^{i\top}_j$ has complexity $O(p^2)$ by Lemma~\ref{lm:matCompComplexity}-(iii) and computing the sum\\
% $\sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|} u^i_j u^{i\top}_j$ has a complexity of $O( N^2 p^2)$ by Lemma~\ref{lm:matCompComplexity}-(i). 
% Moreover, multiplying the $p\times p$ matrix $\sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|} u^i_j u^{i\top}_j$ by the scalar $1/N^3$ has complexity $O(p^2)$. Hence the computing $\pi_1(T)$ and $\pi_2(T)$ has complexity $\mathcal{O}(N^2 p^2)$. 
% Computing the product $u^i_j y^i_j$ has a complexity of $O(p)$ by Lemma~\ref{lm:matCompComplexity}-(iii), and summing $\sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|} u^i_j y^i_j$ has complexity $O(N^2 p)$ by Lemma~\ref{lm:matCompComplexity}-(i). Multiplying the $p\times 1$ vector $\sum_{i=1}^N \sum_{j=1}^{|\mathcal{D}_i|} u^i_j y^i_j$
% by the scalar $1/N^2$ has a complexity of $O(p)$. 
% Therefore computing $\pi_3(T)$ has complexity $O(N^2 p)$, and the complexity of computing $\pi_1(T)$, $\pi_2(T)$, and $\pi_3(T)$ is $\mathcal{O}(N^2 p)$.  

% \noindent\textbf{Complexity of Computing $\gamma_1(T)$ and $\gamma_2(T)$ is $O(p^{2.373})$} 
% \\
% With $\pi_1(T)$ and $\pi_2(T)$ obtained, we can compute $\gamma_1(T)$ and $\gamma_2(T)$ by \eqref{gamma1} and \eqref{gamma2}.  
% From \eqref{gamma1} and \eqref{gamma2}, computing $\gamma_1(\cdot)$ and $\gamma_2(\cdot)$ from $\pi_1(\cdot)$ and $\pi_2(\cdot)$ involves multiplication and addition of $p \times p$ matrices, scalar multiplication of $p\times p$-dimensional matrices, multiplication of a $p\times p$ matrix and a $p\times 1$ vector, and inversion of a $p \times p$ matrix. 
% By Lemma~\ref{lm:matCompComplexity}, multiplication of two $p\times p$ matrices has the dominant complexity of $\mathcal{O}(p^{2.373})$ among the above matrix operations. 
% Moreover, inverting a $p\times p$ matrix has complexity $\mathcal{O}(p^{2,373})$. 
% Hence, computing $\gamma_1(T)$ and $\gamma_2(T)$ has a complexity of $O(p^{2.373})$. 
% %\Anastasis{@Xuwei, multiplication of two \textit{square} $p\times p$ matrices has $\mathcal{O}(p^{2.373})$ complexity}.



% \noindent \textbf{Complexity of computing $\pi_1(t)$, $\pi_2(t)$, $\pi_3(t)$, $\gamma_1(t)$ and $\gamma_2(t)$ for $t=T-1$, $T-2$, ..., $1$ has complexity $\mathcal{O}(T p^{2.373})$.}
% \\ 
% %For each $t=T-1$, $T-2$, ..., $1$ fixed, suppose $\pi_1(t+1)$, $\pi_2(t+1)$, $\pi_3(t+1)$, $\gamma_1(t+1)$ and $\gamma_2(t+1)$ have been obtained. 
% Similar to computing $\gamma_1(T)$ and $\gamma_2(T)$, computing $\gamma_1(t)$ and $\gamma_2(t)$ from $\pi_1(t+1)$ and $\pi_2(t+1)$ has complexity $\mathcal{O}(p^{2.373})$. 
% According to \eqref{eqnpi1pi2}, computing $\pi_1(t)$ and $\pi_2(t)$ from $\gamma_1(t+1)$ and $\gamma_2(t+1)$ involves scalar multiplication and addition along diagonal of $p\times p$ matrices, and therefore has complexity $O(p^2)$ by Lemma~\ref{lm:matCompComplexity}-(i) and (ii), 
% According to \eqref{eqnpi3}, computing $\pi_3(t)$ from $\gamma_1(t+1)$, $\gamma_2(t+1)$, and $\pi_3(t+1)$ involves scalar multiplication and addition of $p\times p$ matrices, scalar multiplication and addition of $p\times 1$ matrices, 
% and multiplication of a $p\times p$ matrix with a $p\times 1$ matrix. By Lemma~\ref{lm:matCompComplexity}, the dominant complexity of these operations is $\mathcal{O}(p^2)$.   
% Summing up the above argument, computing $\pi_1(t)$, $\pi_2(t)$, $\pi_3(t)$, $\gamma_1(t)$ and $\gamma_2(t)$ for each $t$ has a complexity of $\mathcal{O}(p^{2.373})$, and therefore has a complexity of $\mathcal{O}(T p^{2.373})$ for all $t=T-1$, $T-2$,..., $1$. 


% \noindent\textbf{The Cost of Computing Each $\Theta(t)$ is $O(Tp^2 \max\{N, p^{0.373}\})$.}
% \\
% By \eqref{Theta-simple}, the cost of updating from $\Theta(t)$ to $\Theta(t+1)$ is equal to the complexity of computing $\widehat{\boldsymbol{\alpha}}(t)=(\widehat{\alpha}_1^\top(t), \cdots \widehat{\alpha}_N^\top(t))^\top$ for $t=0, 1, ..., T-1$. 

% By \eqref{eq:RegretOptimizationHeuristic_Helper__1}, $\widehat\alpha_i(t)$ for all $i=1$, ..., $N$ share the common term 
% \allowdisplaybreaks 
% \begin{align} 
%  & - \big\{ \gamma_1(t+1) \pi_2(t+1) + \gamma_2(t+1) [ \lambda I_p + \pi_1(t+1) + (N-2)\pi_2(t+1) ] \big\} \sum_{k=1}^N \theta_k(t) 
%  \notag \\ 
%  & - \big[ \gamma_1(t+1) + (N-1) \gamma_2(t+1) \big] (\pi_3(t+1) - \lambda \theta^\star_{(N)}) ,  \notag 
% \end{align} 
% and computing the common term involves matrix multiplication, addition, and scalar multiplication of $p\times p$ matrices, 
% matrix addition and scalar multiplication of $p\times 1$ matrices, 
% and multiplication of a $p\times p$ matrix and a $p\times 1$ matrix.  
% By Lemma~\ref{lm:matCompComplexity}, these operations have complexity $O(Np + p^{2.373})$, where $Np$ is due to adding the $N$ $p$-dimensional vectors $\sum_{k=1}^N \theta_k(t)$, and $p^{2.373}$ is due to multiplication of two $p\times p$ matrices by a CW-like algorithm. 


% Computing the individual terms 
% \allowdisplaybreaks
% \begin{align} 
%  - (\gamma_1(t+1) - \gamma_2(t+1) ) (\lambda I_p + \pi_1(t+1) - \pi_2(t+1) ) \theta_i(t) \notag 
% \end{align} 
% for $\widehat\alpha_i(t)$, $i=1$, ..., $N$ involves addition, scalar multiplication, and matrix multiplication of $p\times p$ matrices, and multiplication of a $p\times p$ matrix and a $p\times 1$ matrix. 
% By Lemma~\ref{lm:matCompComplexity}, these operations have complexity of $\mathcal{O}(p^{2.373} + Np)$, where $p^{2.373}$ is due to multiplication of two $p\times p$ matrices by a CW-like algorithm and $Np$ is due to multiplying a $p\times p$ matrix by the $p$-dimensional vector $\theta_i(t)$ for $i=1$, ..., $N$. 
% Hence the complexity of computing $\widehat{\boldsymbol{\alpha}}(t)$ for $t=0, 1, ..., T-1$ is $\mathcal{O}(T p^2\max\{N, p^{0.373} \} )$. 


% \noindent\textbf{The complexity of computing $(\Theta(t))_{t=0}^T$ is $\mathcal{O}(T p^2 \max\{N,p^{0.373}\})$} \\ 
% Looking over all computations involved, we deduce that the complexity of computing the sequence 
% $(\Theta(t))_{t=1}^T$ starting from $\Theta(0)=\Theta^\star$ has a complexity of $\mathcal{O}(T p^2 \max\{N,p^{0.373}\})$. 
% \end{proof}

% We may now deduce Theorem~\ref{thrm:accelertion_heuristic_regret_optimal_algorithm} and Theorem~\ref{thrm:regretoptimality_SymmetricCase}.  
% \begin{proof}[{Proof of Theorem~\ref{thrm:accelertion_heuristic_regret_optimal_algorithm}}]
%     The result directly follows from Theorem~\ref{thm:ComplexityAlgorithm} and Corollary~\ref{cor:ComplexityAlgorithm__Heuristic}.  
% \end{proof}


% \begin{proof}[{Proof of Theorem~\ref{thrm:regretoptimality_SymmetricCase}}]
% Direct consequence of Propositions~\ref{prop:P1/Nsubmat} and~\ref{prop:SubmatrixReduction}.
% \end{proof}







% \section{Background}
% \label{s:Background}
% In this paper, we consider regret-optimal memoryless training dynamics for \textit{\textbf{f}inite-rank \textbf{k}ernel \textbf{r}idge \textbf{r}egressors} (fKRR) trained from $N$ finite datasets drawn from $N$ (possibly) different data-generating distributions.
% We are considering a scenario in which these datasets can originate from $N$ distinct tasks or be adversarially generated perturbations of the initial dataset, and we aim for our fKRR to exhibit robustness towards them.

% Any continuous \textit{feature map} $\phi:\mathbb{R}^d\rightarrow \mathbb{R}^p$, induces a hypothesis of fKRR $f_{\theta}:\mathbb{R}^d\rightarrow \mathbb{R}$ each of which is uniquely determined by a \textit{trainable parameter} $\theta\in \mathbb{R}^p$ via
% \begin{equation}
% \label{eq:FRKR 1}
% f_{\theta}(x)=\phi(x)^\top\theta;
% \end{equation}
% where all vectors are represented as column-vectors and not row vectors.

% The hypothesis class $\mathcal{H}$ possesses a natural reproducing kernel Hilbert space (RKHS) structure with inner-product given for $f_{\theta},f_{\tilde{\theta}}\in \mathcal{H}$ by $\langle f_{\theta},f_{\tilde{\theta}}\rangle_{\phi}\eqdef \sum_{k=1}^p\, \theta_k\tilde{\theta}_k$.  This RKHS structure suggests an optimal selection criterion to decide which hypothesis in $\mathcal{H}$ best describes a \textit{single} training set $\mathcal{D}_1\eqdef \{(x^1_j,y^1_j)\}_{j=1}^{S^1}$ of $S^1\in \mathbb{N}_+$, by solving the penalized least-squares problem

% \begin{align} 
% \label{eq:FRKR 2}
%  \theta^\star_1 \in \argmin_{\theta \in \mathbb{R}^p } \big\| \Phi(x^1) \theta  - y^1  \big\|_2^2 
%   + \kappa \big\| \theta \big\|_2^2 , 
% \end{align} 
% where 
% \begin{align} 
% \Phi(x^1) \eqdef 
% \big( \phi(x^1_1), \ 
% \phi(x^1_2), \ \cdots , \ 
%  \phi(x^1_{S^1}) \big)^\top \in \mathbb{R}^{S^1 \times p} , \ 
% y^1 \eqdef (y^1_1, y^1_2, \cdots, y^1_{S^1})^\top 
%  \in \mathbb{R}^{S^1} , \notag  
% \end{align} 
% and $\kappa>0$ is a fixed hyperparameter.  In this classical case, the Representer Theorem \cite{KimeldorfWahba__Representer_OriginalI,KimeldorfWahba__Representer_OriginalII} states that the optimal choice of $f_{\theta}$ to the convex optimization problem~\eqref{eq:FRKR 2} is parameterized by
% \begin{equation} 
% \label{eq:loss_one_dataset}
%  \theta^\star_1 = 
%  ( \Phi^\top(x^1) \Phi(x^1)  
%   + \kappa I_p )^{-1} 
%   \Phi^\top(x^1) y^1 ,
% \end{equation} 
% Alternatively, the optimal parameter choice $\theta^\star_1$ can be arrived at via \textit{gradient descent} since~\eqref{eq:FRKR 2} has a strictly convex loss with a Lipschitz gradient.
% The training of fKRR on a single dataset is very-well understood.  Likewise, other aspects of fKRR are well understood; namely, their statistical properties \cite{KRRExactTestError}, their in-sample behaviour in \cite{amini2022target}, and even the approximation power and risk of randomly generated fKRR are respectively known \cite{gonon2022approximation} and \cite{gonon2020risk}.

% Using the fKRR \eqref{eq:FRKR 1}, the joint terminal time objective \eqref{eq:terminal_time_objective} simplifies to
% \allowdisplaybreaks\begin{align} 
% \label{eq:terminal_time_objective__fKRR}
% \begin{aligned}
%         l(\theta_1,\dots,\theta_N, w;\,\mathcal{D} )  
%     \eqdef & 
%         \sum_{i=1}^N 
%         w_i
%         \biggl(
%             \sum_{j=1}^{S_i} 
%                 \big| 
%                 \langle 
%                     u^i_j
%                     ,
%                     \theta^{w}
%                 \rangle - y^i_j  \big|^2 
%         \biggr)
%     \\
%     % \,\,
%     \mbox{ s.t. }
%     \,%\,
%     \theta^w\eqdef & \sum_{i=1}^N \theta_i
%         w_i
%  ,
% \end{aligned}
% \end{align} 
% where $\langle\cdot,\cdot\rangle$ denotes the Euclidean inner-product, $u^i_j\eqdef \phi(x^i_j)$ and, as in~\eqref{eq:terminal_time_objective}, $w = (w_1, \cdots, w_N) \in [0,1]^N$ with $\sum_{i=1}^N\,w_i=1$.










% \end{document}



==> rebuttal <==

%\documentclass{article}
\usepackage[utf8]{inputenc}
\usepackage{enumitem}
\usepackage{geometry}
\usepackage{tcolorbox}

\geometry{margin=1in}

\setlength{\parindent}{0pt} 
\setlength{\parskip}{8pt}

\usepackage{markdown}

\title{Neurips Rebuttal}
\author{}
\date{}

\begin{document}

\maketitle


\section{General Response to AE}

% The following letter to AE: 

% \bigskip 

Dear Associate Editor and Reviewers,
\\ 

We appreciate your efforts in coordinating the rebuttal. 
We have carefully responded to the comments and questions from the reviewers. 


% # 
\textbf{Aggregation Weights for Transfer Learning Not Learning Multi-task Learning}

One major concern of the reviewers is that the regret-based model aggregating $N$ pre-trained models is more like a multi-task model rather than a transfer learning model. 
In multi-task learning, each "task" is to predict well on each dataset $\mathcal{D}_i$; for this to happen, each dataset $\mathcal{D}_i$ must be weighted approximately equally during the aggregation step so as to intentionally not bias the kernel ridge regressor (KRR) towards any one given task.  

In contrast, here, we propose a transfer learning algorithm which intentionally biases the aggregated KRR model towards dataset $1$ by selecting optimal weights $w^{\star}$ (computed in Algorithm 1) to maximize its performance on the focal task ($\mathcal{D}_1$).   

---

% ## 
\textbf{How to modify Algorithm $2$ to perform multi-task learning}

If one desired to perform multi-task learning using Algorithm one, then Algorithm $1$ would be committed, and one should set the aggregation weights to be $w^{\star}\approx (1/N,\dots,1/N)$ (adjusted to account for dataset imbalances such as size and scale).  However, this was not our objective here.

%We emphasize that transfer learning in the paper is realized through the information sharing weights $w^\star_i$, $i\in [N]$ from Algorithm 1, which reflects the relative performance of the individually pre-trained parameters $\theta^\star_i$, $i\in[N]$ on the new dataset $\mathcal{D}_1$. 

%Though the regret-based criteria is based on aggregating models pre-trained on the $N$ datasets $\mathcal{D}_i$, $i\in [N]$, as outlined by Algorithm 2, the role of the new dataset $\mathcal{D}_1$ is different from other datasets  $\mathcal{D}_i$. 


%how the transfer learning is applied to a new dataset $\mathcal{D}_1$ by using pre-trained models on $N$ datasets $\mathcal{D}_1$, $\mathcal{D}_2$ ..., $\mathcal{D}_N$. 




%Algorithm 1, which determines the information sharing level by the performance of the pre-trained models on predicting the new dataset $\mathcal{D}_1$. 

%Then the information sharing levels are passed to Algorithm 2 ... 

\bigskip 
\noindent Best regards, \\
\\
\noindent The Authors 

% \bigskip 
% \textbf{Main questions and responses} (to be summarized in the above letter to AE)
% \\  


% \textbf{Q1.} The paper develops regret-based algorithms to train finite-rank kernel ridge regressors with $N$ data sets $\mathcal{D}_i$, $i\in [N]$. This approach seems more like a multi-task learning rather than transfer learning introduced at the beginning of the introduction section. Please explain how the algorithms in the paper are linked to transfer learning.  
% \\ 

% \textbf{Answer to Q1:} 
% \\ 



% \textbf{Q2.} 
% There are three important parameters: 
% the bias regulation parameter $\lambda$ in transfer learning level and the parameter $\beta$ in the stability. 
% Please explain how these parameters affect the convergence of Algorithm 2, and the optimized fKRR $f_{\theta^\star}$. 




\section{Reviewer Comments and Responses}


\begin{tcolorbox}[colback=white,colframe=black,title={Reviewer Zsc6, Rating 4}]
\footnotesize
\textbf{Summary:} \\
This manuscript designs a regret-optimal optimization algorithm for fine-tuning mixtures of pre-trained kernel regressors. It also provides a theoretical analysis of the proposed algorithm in terms of adversarial robustness and computational complexity.\\

\textbf{Soundness:} 2: fair \\
\textbf{Presentation:} 2: fair \\
\textbf{Contribution:} 2: fair \\

\textbf{Strengths:} \\

1.   The proposed algorithm is accompanied by theoretical guarantees. These theories make it easier for readers to understand the motivation and design of the proposed algorithm.

2. The presentation is overall good and easy to follow. \\ 



\textbf{Weaknesses:} \\

1. Based on the simulation, it looks like, in the regime $\lambda>0$, the loss requires more iteration to converge. This seems to indicate that the regularization term to control the transfer level is not helpful. I think the authors should compare the final loss when $T$ iterations are done to see if having such regularization really helps to achieve lower regrets. \\

2. The regularization term that controls the transfer learning level in the loss is called bias regularization in literature (or hypothesis transfer learning in a larger category). This manuscript focuses on transfer learning, but I didn't see that the technique of bias regularization is discussed in the related work. In case the authors were not aware of it, I listed some below, including topics from parametric models to nonparametric ones; see [1,3] for the parametric model and [2,4] for KRR, and more references therein. I only list some works in the regime of transfer learning, but such techniques have also been widely used in different learning scenarios like multi-task, continual, and meta-learning (and even more). 
While using regularization to count the similarity between models may have been common in recent days, I still encourage the authors to provide related discussions since this regularization technique is the core of knowledge transfer in the proposed loss.
\\

3. The manuscript contains some unclear sentences and notations. I listed some of them (although not exhaustive) in the following question section. A thorough and careful proofreading is needed.
\\ 


4. The total iteration number $T$ seems like a pre-determined parameter. Even though there is a closed-form solution for minimizing the loss, as shown in the simulation, the pre-determined $T$ may not promise a convergence in loss or even a decrease in the loss. There should be more investigation about $T$. Besides, setting $T=1$ in the real data application looks really weird to me.
\\

5. Based on the description of Algorithm 2, it looks like the weight $w_i$
do not change. The derivation in (9) and (10) shows that the "optimal" depend on $i$-th learner’s score. However, in Algorithm 2, the gets updated, making the value of scores change as well. I'm not convinced how the weights can be constants, can the authors elaborate more?
\\

6. Transfer learning usually aims to leverage the pre-trained models/parameters to optimize the performance in the downstream target task. However, while this manuscript aims at transfer learning, it looks like the final learner $\hat{f}_{\theta^{w^\star}}$ is obtained by having it optimize the overall performance of tasks but not specifically focus on the target task (all tasks' data are involved in the loss). I feel like it is more like a multi-task learning or meta-learning setting. Or is it fair to say that the proposed algorithm not only focuses on the downstream target task but also aims to obtain great performance on other tasks? 
\\ 

[1] Kuzborskij, I. and Orabona, F. "Stability and hypothesis transfer learning. International Conference on Machine Learning." 2013.

[2] Xuezhi Wang, Junier B Oliva, Jeff G Schneider, and Barnabás Póczos. "Nonparametric risk and stability analysis for multi-task learning problems." IJCAI. 2016.

[3] Tian, Ye, Yuqi Gu, and Yang Feng. "Learning from similar linear representations: Adaptivity, minimaxity, and robustness." arXiv preprint arXiv:2303.17765 (2023).

[4] Lin, Haotian, and Matthew Reimherr. "Smoothness Adaptive Hypothesis Transfer Learning." International Conference on Machine Learning. 2024. 
\\ 

\textbf{Questions:} \\
1. Lines 146 to 148, there is no subsection for Section 2.

2. Inconsistent notation, line 36 and Equation (1), should use both $\ell$ or $l$
(this also happens in other places that refer to loss). 

3. Line 158, it seems like Equation (18) does not contain the closed-form of $\hat{\Theta}$. 

4.Can authors explain more on why the information sharing probability measure takes the specific form in Line 194 (also Adaptive Prior in Algorithm 1)?
\\ 


\textbf{Limitations:} \\
Yes. The authors mention they would like to extend their pipeline from KRR to deep learning models. 
\end{tcolorbox} 


\newpage

Dear reviewer Zsc6, 

Thank you for your insightful comments. 
We are happy to read the reviewer appreciate the theoretical guarantees and found the paper easy to follow. The reviewer raised many important questions which we believe we can answer with a high degree of certainty. Additional feedback regarding the final evaluation of our paper will be greatly appreciated. 
%We answer each of your questions in two levels, first the main key point, and then additional details.

 
Concerning weaknesses:

\textbf{1. a) The effect of $\lambda>0$ on Convergence Behaviour}


While it is true that large values of $\lambda$ slow down the convergence of the algorithm, they do guide its terminal parameter selection to a different value than would be obtained by small values of $\lambda$.  
The effect of varying $\lambda$ can be understood on a spectrum (ignoring the path regularization $\beta$):

 - $\lambda\approx \infty$ = No Fine-Tuning: the algorithm would output the combination $\sum_i w_i \theta_i^{\star}$ thus no fine-tuning would be performed.  

This is suboptimal if there is one very large and very useful dataset and otherwise small datasets.  For simplicity, consider $N=2$ datasets with the focal dataset $\mathcal{D}_1$ being comparatively small to $\mathcal{D}_2$.  Then, the pre-trained parameter $\theta^\star_1$ would be less informative but would be weighted as equally important to the more informative parameter $\theta^\star_2$.  Thus, when $\lambda=\infty$, the inability to fine-tune will clearly produce a suboptimal aggregation.

 - $\lambda= 0$ = No Transfer: 
then $\theta^w:=\sum_{i}\, w_i \theta_i$ purely minimizes the weighted loss
$$
\sum_i w_i \sum_j (f_{\theta^w}(x_j^i) - y_j^i)^2 , 
$$
completely forgetting about the pre-trained parameters $\theta_1^{\star},\dots,\theta_N^{\star}$.

This is problematic if one dataset is much much larger than the others and only slightly useful for $\mathcal{D}_1$. Indeed this would lead (in the limit where the size of this large dataset goes to $\infty$) to an optimizer of the large dataset simply because it dominates the loss as long as its weight $w_i > 0$. 

In either case, we see that intermediate values of $\lambda$ yield the most desirable outputs of Algorithm $2$.


\textbf{1. b) The $\beta$ parameter actually controls convergence speed.}
The convergence speed is controlled by the $\beta$ parameter.  If $\beta\approx \infty$ means that $\Delta\theta_t:=\theta_{t+1}-\theta_t\approx 0$ for all $t$; in contrast, $\beta=0$ leaves the step size $\Delta\theta_t$ unconstrained allowing the algorithm to directly jump to its optimal value at the first step ($t=1$).  In the latter case, there is no need to consider large values of $T$ as $T=1$ is sufficient.


\textbf{2 and 3.} 
Thank you for providing these additional references, which we were indeed unaware of, and for pointing out sentences that could be further clarified. We have incorporated these changes into our manuscript.


\textbf{4. The number of total iterations $T$}

The total iteration number $T$ indeed represents a trade-off between the computing budget and the convergence of the loss function if $\beta > 0$.  As noted above, if $\beta=0$, then $T=1$ is sufficient.

While investigating the optimal choice of $T$ guaranteeing approximate convergence is indeed interesting, it is beyond the main scope of this paper.  Nevertheless, here is what can be said:  

- \textbf{Convergence in the limit} 
When computational resources permit, choosing $T$ large enough will ensure that the output $\sum_iw_i\theta_t$ of the algorithm will converge to its $T=\infty$ limit; by a similar argument to the proof of Theorem 4 of [1].  However, we did not include this analysis since it is effectively the same [1], again using $\Gamma$-convergence (see [6]) argument, and does not provide enough new insights for added technicality (such as weak converges in certain Banach spaces of algorithms with infinite-run time).  


- \textbf{Cases where $T>1$ is beneficial implicit regularization:} 
The advantage of the value of $T>1$ is that it "spreads out the convergence in time," which allows the option of implicit regularization through an early stopping procedure.  Though the investigation of the statistical properties of early stopping of our algorithm is beyond the scope of this paper, one would expect that using T as a vehicle towards early stopping regularization would likely improve the statistical properties of our aggregated learning; as the benefits to model generalization of early stopping on classical learning algorithms are very well documented [2,3,4,5].

- \textbf{Cases where $T=1$ is optimal:}
If we are not interested in optimization algorithms which exhibit stable iterates; then we may set $\beta=0$.  As discussed above, doing so means that the algorithm can directly jump to its optimal terminal value as there is no constraint on its increments $\delta \Theta_t$.  Thus, $T=1$ is optimal. 
This is precisely what we do in our American option pricing example, as discussed in the first paragraph of our experiment details in Section C.3.  


\textbf{5. Why updating $w$ in Algorithm $2$ is not advantageous}

- \textbf{Why updating $w$ may not be meaningful} 
The weights $w^\star_i$, computed in Algorithm 1, rank the similarity of each dataset $\mathcal{D}_i$ to the focal dataset $\mathcal{D}_1$, which we would like to transfer their information towards by encoding the scores $s_1,\dots,s_N$.  These are computed once in Algorithm $1$ and then kept constant while Algorithm $2$ is run.   

It is, therefore, not meaningful to update the weights $w$ throughout Algorithm 2 since these weights already quantify how similar each dataset $\mathcal{D}_i$ is to the focal dataset $\mathcal{D}_1$, and this does not change as these datasets do not change.

\textbf{Why updating $w$ creates a feedback loop}
Dynamically updating the weights $w$ is undesirable as it creates a dynamic Stackelberg game where the leader player sets $w$, and the follower plays $\theta$.  The optimal algorithm would be an equilibrium of this game, which is computable via a bi-level optimization or an auxiliary reinforcement learning algorithm, eg [7].  However, doing so would lead to significant computational overhead without significant improvement to the aggregated model.  


\textbf{6. The optimization criterion is not unbiased as in multi-task learning but is biased towards $\mathcal{D}_1$ as in transfer learning}

We evaluate the predictive performance of each $\theta^\star_i$, $i\in[N]$ on the primal dataset $\mathcal{D}_1$ to determine the weights $w^\star_i$, $i \in [N]$, which quantify how much knowledge $\mathcal{D}_i$ provides for the task on $\mathcal{D}_1$. 
Based on those weights the ensemble parameters are biased towards maximizing performance on the primary dataset $\mathcal{D}_1$.  In contrast in multi-task learning, the weights $w^{\star}$ should rather be selected to be all equal (adjusting for dataset imbalances) so as to ensure that the aggregated learner is not biased towards any individual dataset.



For example, consider the extreme case where all datasets are completely orthogonal to each other, then the full weight is on $\mathcal{D}_1$ and no "orthogonal" knowledge is transferred (as it should be).  Indeed, in this case, the kernel regressors pre-trained on datasets $\mathcal{D}_i$ for $i>1$ will not exhibit any predictive power on the focal dataset $\mathcal{D}_1$, and visa-versa, and so Algorithm $1$ will set $w^{\star}=(1,0,0,\dots,0)$.  Therefore, Algorithm $2$ returns
 $$
 \sum_i w_i \theta_i^\star = 1\theta_1^{\star} + 0\sum_{i>1}\theta_i^{\star} = \theta_1^{\star}
 .
 $$
The aggregated model will have no predictive performance on datasets $\mathcal{D}_i$ for $i\neq 1$ (since the datasets were assumed to be orthogonal to one another).  Thus, Algorithm $2$ does not perform multi-task learning.


Our algorithm can, however, be modified to perform multi-task learning.  Though we are not interested in this for this research paper, we do describe how it can be done in our main rebuttal, above.  
 \\


\textbf{Concerning questions:} \\ 

1. In line 146, the word "subsection" has been changed to "section".  

2. Thank you for pointing out the inconsistent notation. We have now unified the notation for loss throughout the paper to consistently use $l$.  


3. The optimal $\hat{\Theta}$ is determined inductively by equation (18) with the initial condition $\hat{\Theta}(0) = \Theta^\star$ and with increments $\Delta \hat{\Theta}(t)$ provided by equation (6) in Theorem 1 (line 157). While equation (18) does not provide a closed-form expression for $\hat{\Theta}$, it outlines the iterative process used to compute it. 


4. The information sharing probability measure takes the specific form in line 194 and the Adaptive Prior in Algorithm 1 because this probability measure maximizes the average performance of the random learner on the dataset $\mathcal{D}_1$, as regularized by the information sharing level $\eta > 0$. This result is formally summarized in Theorem 4 (line 202).

[1] Casgrain, P. and Kratsios, A. (2021, July). Optimizing Optimizers: Regret-optimal gradient descent algorithms. In Conference on Learning Theory (pp. 883-926). PMLR.

[2] Zhang, Tong, and Bin Yu. "Boosting with early stopping: Convergence and consistency." (2005): 1538-1579.

[3] Yao, Yuan, Lorenzo Rosasco, and Andrea Caponnetto. "On early stopping in gradient descent learning." Constructive Approximation 26.2 (2007): 289-315.

[4] Wei, Y., Yang, F., \& Wainwright, M. J. (2017). Early stopping for kernel boosting algorithms: A general analysis with localized complexities. Advances in Neural Information Processing Systems, 30.

[5] Heiss, J., Teichmann, J., \& Wutte, H. (2019). How Implicit Regularization of ReLU Neural Networks Characterizes the Learned Function--Part I: the 1-D Case of Two Layers with Random First Layer. arXiv preprint arXiv:1911.02903.

[6] Dal Maso, G. (2012). An introduction to $\Gamma$-convergence (Vol. 8). Springer Science \& Business Media.

[7] Li, M., Qin, J., Freris, N. M., \& Ho, D. W. (2020). Multiplayer Stackelberg–Nash game for nonlinear system via value iteration-based integral reinforcement learning. IEEE Transactions on Neural Networks and Learning Systems, 33(4), 1429-1440.



\begin{comment} 
\newpage 
\textbf{\color{red} Short answer for Zsc6}

Dear reviewer Zsc6, 


Thank you for your insightful comments. 
We answer each of your questions in two levels, first the main key point, and then additional details.

 
Concerning weaknesses:

\textbf{1. a) The effect of $\lambda>0$ on Convergence Behaviour}


While it is true that large values of $\lambda$ slow down the convergence of the algorithm, they do guide its terminal parameter selection to a different than would be obtained by small values of $\lambda$.  
The effect of varying $\lambda$ can be understood on a spectrum (ignoring the path regularization $\beta$):

 - $\lambda\approx \infty$ = No Fine-Tuning: the algorithm would output the combination $\sum_i w_i \theta_i^{\star}$ thus no fine-tuning would be performed.  

  - This is suboptimal if there is one very large and very useful dataset and otherwise small datasets.  For simplicity, consider $N=2$ datasets with the focal dataset $\mathcal{D}_1$ being comparatively small to $\mathcal{D}_2$.  Then, the pre-trained parameter $\theta^\star_1$ would be less informative but would be weighted as equally important to the more informative parameter $\theta^\star_2$.  Thus, when $\lambda=\infty$, the inability to fine-tune will clearly produce a suboptimal aggregation.

 - $\lambda= 0$ = No Transfer: 
then $\theta^w:=\sum_{i}\, w_i \theta_i$ purely minimize the weighted loss
$$
\sum_i w_i \sum_j (f_{\theta^w}(x_j^i) - y_j^i)^2
$$
completely forgetting about the pre-trained parameters $\theta_1^{\star},\dots,\theta_N^{\star}$.

  - This is problematic if one dataset is much much larger than the others and only slightly useful for $\mathcal{D}_1$. Indeed this would lead (in the limit where the size of this large dataset goes to $\infty$) to an optimizer of the large dataset simply because it dominates the loss as long as its weight $w_i > 0$. 

In either case, we see that intermediate values of $\lambda$ yield the most desirable outputs of Algorithm $2$.


\textbf{1. b) The $\beta$ parameter actually controls convergence speed.}
The convergence speed is controlled by the $\beta$ parameter.  If $\beta\approx \infty$ means that $\Delta\theta_t:=\theta_{t+1}-\theta_t\approx 0$ for all $t$; in contrast, $\beta=0$ leaves the step size $\Delta\theta_t$ unconstrained allowing the algorithm to directly jump to its optimal value at the first step ($t=1$).  In the latter case, there is no need to consider large values of $T$ as $T=1$ is sufficient.


\textbf{2 and 3.} 
Thank you for providing these additional references, which we were indeed unaware of, and for pointing out sentences that could be further clarified. We have incorporated these changes into our manuscript.


\textbf{4. The number of total iterations $T$}

The total iteration number $T$ indeed represents a trade-off between the computing budget and the convergence of the loss function if $\beta > 0$.  As noted above, if $\beta=0$, then $T=1$ is sufficient.

While investigating the optimal choice of $T$ guaranteeing approximate convergence is indeed interesting, it is beyond the main scope of this paper.  Nevertheless, here is what can be said:  

- \textbf{Convergence in the limit} 
When computational resources permit, choosing $T$ large enough will ensure that the output $\sum_iw_i\theta_t$ of the algorithm will converge to its $T=\infty$ limit; by a similar argument to the proof of Theorem 4 of [1].  However, we did not include this analysis since it is effectively the same [1], again using $\Gamma$-convergence (see [6]) argument, and does not provide enough new insights for added technicality (such as weak converges in certain Banach spaces of algorithms with infinite-run time).  


- \textbf{Cases where $T>1$ is beneficial implicit regularization:} 
The advantage of the value of $T>1$ is that it "spreads out the convergence in time," which allows the option of implicit regularization through an early stopping procedure.  Though the investigation of the statistical properties of early stopping of our algorithm is beyond the scope of this paper, one would expect that using T as a vehicle towards early stopping regularization would likely improve the statistical properties of our aggregated learning; as the benefits to model generalization of early stopping on classical learning algorithms are very documented [2,3,4,5].

- \textbf{Cases where $T=1$ is optimal:}
If we are not interested in optimization algorithms which exhibit stable iterates; then we may set $\beta=0$.  As discussed above, doing so means that the algorithm can directly jump to its optimal terminal value as there is no constraint on its increments $\delta \Theta_t$.  Thus, $T=1$ is optimal. 
This is precisely what we do in our American option pricing example, as discussed in the first paragraph of our experiment details in Section C.3.  




\textbf{5. Why Updating $w$ in Algorithm $2$ is not advantageous}

- \textbf{Why Updating $w$ may not be meaningful} 
The weights $w^\star_i$, computed in Algorithm 1, rank the similarity of each dataset $\mathcal{D}_i$ to the focal dataset $\mathcal{D}_1$, which we would like to transfer their information towards by encoding the scores $s_1,\dots,s_N$.  These are computed once in Algorithm $1$ and then kept constant while Algorithm $2$ is run.   

It is, therefore, not meaningful to update the weights $w$ throughout Algorithm 2 since these weights already quantify how similar each dataset $\mathcal{D}_i$ is to the focal dataset $\mathcal{D}_1$, and this does not change as these datasets do not change.

- \textbf{Why Updating $w$ creates a feedback loop via by embedding the optimization problem into a Stackelberg game} 
A more technical reason why dynamically updating the weights $w$ is undesirable is that it would effectively create a dynamic Stackelberg game where the major player/leader sets the $w$ and the minor player updates the $\theta$ parameters.  The optimal algorithm would then be an equilibrium of this game, which could be computed using standard iterative methods or by a bi-level optimization using an auxiliary reinforcement learning algorithm, such as [7], to play the game. However, this would break the closed-form expressions, making the algorithm extremely computationally intensive, requiring several forward-backwards iterations to converge, which it currently is not.  Moreover, it is not at all clear that this large computational overhead would bring any meaningful improvement to the aggregated model.  


\textbf{6. The optimization criterion is not unbiased as in multi-task learning but is biased towards $\mathcal{D}_1$ as in transfer learning}

We evaluate the predictive performance of each $\theta^\star_i$, $i\in[N]$ on the primal dataset $\mathcal{D}_1$ to determine the weights $w^\star_i$, $i \in [N]$, which quantify how much knowledge $\mathcal{D}_i$ provides for the task on $\mathcal{D}_1$. 
Based on those weights the ensemble parameters are biased towards maximizing performance on the primary dataset $\mathcal{D}_1$.  In contrast in multi-task learning, the weights $w^{\star}$ should rather be selected to be all equal (adjusting for dataset imbalances) so as to ensure that the aggregated learner is not biased towards any individual dataset.



For example, consider the extreme case where all datasets are completely orthogonal to each other, then the full weight is on $\mathcal{D}_1$ and no "orthogonal" knowledge is transferred (as it should be).  Indeed, in this case, the kernel regressors pre-trained on datasets $\mathcal{D}_i$ for $i>1$ will not exhibit any predictive power on the focal dataset $\mathcal{D}_1$, and visa-versa, and so Algorithm $1$ will set $w^{\star}=(1,0,0,\dots,0)$.  Therefore, Algorithm $2$ returns
 $$
 \sum_i w_i \theta_i^\star = 1\theta_1^{\star} + 0\sum_{i>1}\theta_i^{\star} = \theta_1^{\star}
 .
 $$
The aggregated model will have no predictive performance on datasets $\mathcal{D}_i$ for $i\neq 1$ (since the datasets were assumed to be orthogonal to one another).  Thus, Algorithm $2$ does not perform multi-task learning.


Our algorithm can, however, be modified to perform multi-task learning.  Though we are not interested in this for this research paper, we do describe how it can be done in our main rebuttal, above.  
 \\


\textbf{Concerning questions:} \\ 

1. In line 146, the word "subsection" has been changed to "section".  

2. Thank you for pointing out the inconsistent notation. We have now unified the notation for loss throughout the paper to consistently use $l$.  


3. The optimal $\hat{\Theta}$ is determined inductively by equation (18) with the initial condition $\hat{\Theta}(0) = \Theta^\star$ and with increments $\Delta \hat{\Theta}(t)$ provided by equation (6) in Theorem 1 (line 157). While equation (18) does not provide a closed-form expression for $\hat{\Theta}$, it outlines the iterative process used to compute it. 


4. The information sharing probability measure takes the specific form in line 194 and the Adaptive Prior in Algorithm 1 because this probability measure maximizes the average performance of the random learner on the dataset $\mathcal{D}_1$, as regularized by the information sharing level $\eta > 0$. This result is formally summarized in Theorem 4 (line 202).

[1] Casgrain, P. and Kratsios, A. (2021, July). Optimizing Optimizers: Regret-optimal gradient descent algorithms. In Conference on Learning Theory (pp. 883-926). PMLR.

[2] Zhang, Tong, and Bin Yu. "Boosting with early stopping: Convergence and consistency." (2005): 1538-1579.

[3] Yao, Yuan, Lorenzo Rosasco, and Andrea Caponnetto. "On early stopping in gradient descent learning." Constructive Approximation 26.2 (2007): 289-315.

[4] Wei, Y., Yang, F., \& Wainwright, M. J. (2017). Early stopping for kernel boosting algorithms: A general analysis with localized complexities. Advances in Neural Information Processing Systems, 30.

[5] Heiss, J., Teichmann, J., \& Wutte, H. (2019). How Implicit Regularization of ReLU Neural Networks Characterizes the Learned Function--Part I: the 1-D Case of Two Layers with Random First Layer. arXiv preprint arXiv:1911.02903.

[6] Dal Maso, G. (2012). An introduction to $\Gamma$-convergence (Vol. 8). Springer Science \& Business Media.

[7] Li, M., Qin, J., Freris, N. M., \& Ho, D. W. (2020). Multiplayer Stackelberg–Nash game for nonlinear system via value iteration-based integral reinforcement learning. IEEE Transactions on Neural Networks and Learning Systems, 33(4), 1429-1440.

\end{comment}



% \end{markdown}
%\end{tcolorbox}



\bigskip 
\textbf{Comments from reviewer Zsc6, 12 Aug, 23:46} 

I appreciate the detailed responses to these questions.

Regarding the comments on updating $\omega$, while I agree that updating $\omega$ can result in computational difficulty, I disagree with the authors' responses on "since these weights already quantify how similar each dataset $\mathcal{D}_i$ is to the focal dataset $\mathcal{D}_1$". The similarity is not only measured by the datasets but also by the models one uses to obtain the scores. In Algorithm 2, the $\theta_i$ changes, making the model changes as well, this change also propagates to the scores.

After going through the author's responses and the comments from other reviewers, I will currently maintain my rating and modulo potential insights in the discussion phase with the other reviewers.


\bigskip 

\textbf{\color{blue} Response to reviewer Zsc6, 12, Aug, 23:46}

Dear reviewer Zsc6, 

We greatly appreciate your feedback. 

- Of course you are right that the models one uses to obtain the scores are an important part when computing the similarity. We are interested in the similarity between the datasets (i.e., the knowledge that other datasets can contribute to the focal task), which should be quantified by the $w_i$. Hence, only information of the dataset $D_i$ should be used in the model that is used to compute this similarity.
The initial $\theta_i^*$ are from an OLS perspective the best possible models for each dataset $D_i$ and only use information of this dataset. As soon as the $\theta_i$ are updated, they are also based on information of other datasets, hence, they cannot be used to quantify the similarity between the datasets $D_i$ and $D_1$ anymore (in the sense that their score is now (potentially) improved through knowledge available only in other datasets). In this sense, only for the initial $\theta_i^*$, the score can be interpreted as the similarity between the dataset $D_i$ and $D_1$.
For example, in the (extreme) case of $\beta = \lambda = 0$, all $\theta_i(1)$ are identical, hence they are useless for quantifying how much information $D_i$ has for the focal task of $D_1$.

- Introducing an algorithm that loops between Algorithms 1 and 2 would indeed require additional conditions that guarantee convergence to an equilibrium pair of $w^*$ and $\theta^*$. Such a study is beyond the scope of the current paper. However, we recognize the potential interest of this convergence analysis and will explore it in our future research.

Best regards, 

The Authors







\newpage

\begin{tcolorbox}[colback=white,colframe=black,title={Reviewer NMBE, Rating 3}]
\footnotesize
\textbf{Summary:} \\
The paper studies how to aggregate kernel ridge regressors, pre-trained on some tasks in order to perform well on a new task. The main result of the paper is an algorithm that aggregates the models in order to minimize some notion of regret aiming to capture the (i) performance of the final model and (ii) the transfer cost.\\

\textbf{Soundness:} 4: excellent \\
\textbf{Presentation:} 2: fair \\
\textbf{Contribution:} 3: good \\

\textbf{Strengths:} \\
The main goal of the paper is to compute parameters $\theta_i$ and mixing weights $w_i$ so that the aggregated model with parameters $\sum_i w_i \theta_i$ minimizes the regret bound, which counts for the (i) accuracy of the final model across all tasks and (ii) the cost of going from the initial parameters $\theta_i^\star$ 
to $\theta_i$. The main result of the paper is a regret-minimizing algorithm (Algorithm 2).

Algorithm 1 essentially solves a collection of kernel ridge regression task and serves as the initialization of Algorithm 2. Then the authors use some known results from control theory to get some "closed-form" updates for the parameter vectors $\theta_i$
and this iterative procedure provides the unique regret minimizing weights and parameters, under some assumptions.

Next the authors analyze the adversarial robustness of their algorithm to some adversarial attacks.\\

\textbf{Weaknesses:} \\
The paper actually deals with the problem of aggregating models pre-trained on datasets $D_1$, ..., $D_N$ into a single model that we would like to perform well across all the $N$ tasks. The first paragraph and even the title/abstract focus on transfer learning, which I cannot see how it is related to the content of the paper. One way to view the connection is by considering the "out-of-distribution" dataset as the union of all the pre-training tasks but this feels confusing to me based on the existing literature on transfer learning. Maybe using the notion of multi-task learning is better.


I think that the aggregation problem is relevant and interesting but several parts of the presentation need to fixed. E.g., in lines 55-60, the authors talk about the connection of control theory to the regret minimization task but terms like "terminal, running cost" are unclear to a non-expert in control theory. More to that, showing that the provided algorithm is robust to adversarial attacks feels highly disconnected from the prior content of the paper. In particular, I do not see how the paper gains from such a result.


Another aspect that is missing from the paper to make it more readable is intuition. The regret minimization problem ends up having a closed form solution based on solving a system of Riccati equations. I think that the paper would highly benefit if the authors provided some intuition about the results in the area of control theory, hence making the main result (Theorem 2) and algorithm (Algorithm 2) more readable and parsable.


Given all the above comments, I think that the paper is not yet ready for publication and requires several re-writting.\\


\textbf{Questions:} \\
1. In the first paragraph of the paper, the parameters are defined as a mixture of $\theta_i$ for $i\in[N]$, where $\theta_i$ is a fine-tuning of the pre-trained model $\theta^\star_i$. For $i>2$, I assume that the authors mean that one fine-tunes the parameter of $\theta_i^\star$
using the dataset $D_1$ (the new task). But what is $\theta^\star_1$? Do we assume that the size of $D_1$ is much smaller than 
$D_{i>1}$, so that we cannot simply train the model? More to that, since essentially the message of the paper is to answer how to aggregate a bunch of models into a single one and evaluate the performance of the aggregated model to all tasks simultaneously, it feels to me that the first paragraph is a little bit confusing. \\ 


2. The paper considers the minimization of a regret criterion that captures the whole trajectory of going from $\theta_i^\star$
to $\theta_i$ for $i\in [N]$. It is not completely clear to me why such a measure is relevant to the transfer learning task, since eventually our goal is to perform well on the new task $D_1$. I would be happy if the authors could motivate more this metric for transfer learning; I understand why it is relevant to model aggregation. \\ 


3. In Assumption 1, does $K_x$ depend on the dimension of $x$ (or $\phi(x)$) or is it considered an absolute constant? How does it appear in the bounds? Could you elaborate on Assumption 2? When does Assumption 2 fail to hold true?

\textbf{Limitations:} \\
No limitations
\end{tcolorbox}

%\textbf{Rating:} 3: Reject: For instance, a paper with technical flaws, weak evaluation, inadequate reproducibility and/or incompletely addressed ethical considerations. 


\newpage

%\begin{tcolorbox}[colback=white,colframe=blue,title={Response to Reviewer NMBE}]
\noindent Dear reviewer NMBE, \\ 

\noindent Thank you for your insightful comments. The following are our responses to your questions and comments about the manuscript. \\


\textbf{Multi-Task Learning vs. Transfer Learning in Algorithm 2}\
In multi-task learning, each "task" or dataset $\mathcal{D}_i$ is weighted approximately equally in the aggregation step so that the (foundation) model is not biased towards anyone.  In contrast, here, we intentionally use the optimal weights (computed in Algorithm 1) to bias the aggregation of the pre-trained models towards the focal dataset $\mathcal{D}_1$.  

In this way, our algorithm can be modified to be used in multi-task learning simply by replacing the weights generated by Algorithm $1$ to roughly uniform weights (possibly adjusting for imbalances in dataset sizes and magnitudes).  However, with Algorithm $1$ there is a focal bias towards transforming the performance of the pre-trained models on the $N$ datasets to their performance on task/dataset $\mathcal{D}_1$.

 
This is confirmed by our ablation experiments in Section 4.2, where the regret-optimal algorithm (RO) consistently outperformed its accelerated counterpart (ARO), the latter of which relies on uniform weights (as in the multi-task learning setting).  In this way, we also numerically see that the bias encoded by our RO algorithm into the aggregated learner does increase performance, thus "transferring knowledge" to the intended dataset $\mathcal{D}_1$, while the multi-task version of the algorithm (ARO) fails to do so with similar accuracy. We will add a brief discussion on why ARO is a multi-task learning variant of RO and why RO is not in our discussion section.


\textbf{Concerning Control-Theoretic Terminology}
\\
Though our paper is aimed at the optimization community, which often do have some prior knowledge of optimal control, we acknowledge that this may not be the case for the reader base interested in transfer learning.  A few words of clarification will be added to ensure everyone is on the same page. 


\textbf{Adversarial Robustness}
Our objective is to pose and understand the problem of optimal optimization algorithms for our aggregation problem (1).  In optimal control a full solution of such a problem entails, elicitation of the optimizer (here the optimal algorithm), uniqueness, and well-posedness (i.e. stability with respect to the initial data).  
In practice, this latter property translate to a robustness guarantee showing that our algorithm is still approximately regret-optimal (i.e. minimizing (1)) even if there is noise or errors present in most real-world datasets.


\textbf{Control Theoretic Background}\\
Our paper is aimed at the optimization sub-community in machine learning many of which have a strong background in control, e.g. most optimizers and any reader familiar with reinforcement learning.  We understand that not every remember of the broader ML community has the background to fully appreciate papers from other sub-communities, such as the optimization community, but that is not our target audience.  As such, we do no feel there is a need to explain concepts like solving systems of Ricatti Equations or basic control-theoretic terminology.  


\textbf{Q1.}
The parameter $\vartheta_1^{\star}$ is obtained, just like the others, from training the kernel ridge regressor (KRR) on the corresponding dataset; in this case the focal dataset $\mathcal{D}_1$. The importance of computing $\vartheta_t^{\star}$ is that is create a reference point the KRR parameter space, by which we can rank the suitability of models in prediction on dataset $\mathcal{D}_1$.  

\textit{Concerning training on the union of the datasets: }
As shown in our experiments, simply training a single KRR on the union the datasets does not perform nearly as well as our aggregation algorithm.  

We note that aspects of dataset imbalance, either in scale or size, can easily be dealt with by our algorithm and refer to the answer to reviewer Zsc6 for more details.



\textbf{The Message of our Paper}
We want to emphasize again at this point that the paper's message is not how to aggregate models so that they perform well on all tasks but how to transfer knowledge from other datasets to use it on the primal task $\mathcal{D}_1$. However, we understand that the first paragraph might have been a bit confusing and have clarified it now.


\bigskip  
\textbf{Q2} We consider path dependence since our objective is to identify the optimization algorithm which arrives at the best parameter aggregation for transfer learning as \textit{efficiently as possibly}.  The objective of this paper is not questions about generalization, but rather question of efficient optimization.  If the path is not considered then one can easily construct slower "pathological" algorithms which arrive at the same parameter aggregation values but arbitrarily slower.  

For instance, let $\theta:=(\theta_t)_{t=0}^{T}$ be the (path of) the regret optimal algorithm.  Then, for any positive integer $k$, the algorithm $\theta^k$ whose iterates are: $\theta_0$ if $t<k$ and $\theta_{t-k}$ if $t\ge k$, arrives at the same terminal value as $\theta$ but requires $k$ more iterations.  Thus, both algorithms offer produce regressors offering the exact same performance but $\theta^k$ is strictly slower.  Therefore, considering path dependence is key when designing efficient optimization algorithms for transfer learning.

We also highlight that simply performing gradient descent on the inner objective in (1) yields a strictly slower convergence; as we saw in the experiments of section $4.1$.

If one is not interested in stable convergence, one can simply set $\beta = 0$ and then use $T=1$ (which is most efficient), then no path needs to be considered. Nevertheless, the regime $\beta > 0, T>1$ can be advantageous since it allows for implicit regularization through early stopping (also see the answer to reviewer Zsc6 for more details).




\textbf{Q3}
In Assumption 1, $K_x$ is considered an absolute constant that does not depend on the dimension of $x$ (or $\phi(x)$). Nevertheless, since all these dimensions are fixed, also a constant which depends on the dimension would boil down to an absolute constant.  
The bounds $K_x$ and $K_y$ in Assumption 1 are utilized in Theorem 3, Lemma 4, and Proposition 1. 
Assumption $2$ is a positive-definiteness condition required to ensure that the Riccatti system is well-posed; it is difficult to imagine a scenario where this fails. 
% Regarding Assumption 2, we have confirmed that it always holds true. We have moved Assumption 2 to Appendix B and restated it as Lemma 1.

# Question

We really appreciate that it seemed that your enjoyed our paper, giving it a 3/4 rating total across the soundness, presentation, and contribution categories.  
We would also like to ask one question then, why did you assign us a final score of 3/10 on our final score (we would have expected 7.5/10 based on the above ratings)?

Best regards, 

The Authors

%\end{tcolorbox}



\newpage 


\textbf{\large Comments from Reviewer NMBE, 08 Aug, 04:44}

I would like to thank the authors for the detailed and helpful response in my concerns. 

Transfer Learning

My main concern about the transfer learning vs. multi-task learning issue was that usually (at least from my experience) transfer learning is about the following problem: one has a source distribution $S$
over labeled examples and a target distribution $T$. The model is trained on examples from $S$ and may or may not have access to unlabeled examples from $T$. A standard setting is that of covariate shift, where the $x$-marginals remain the same. Crucially, the challenge in this setting is that the learner does not have access to labels from $T$ and hence it is not generally possible to transfer from $S$ to $T$. 

In the present work, the learner, if I understand correctly, has access to the target distribution $\mathcal{D}_1$ but also there is sample access to different distributions $\mathcal{D}_2$, ..., $\mathcal{D}_N$. Hence, one could obtain a weak yet non-trivial learner by only training a model on $\mathcal{D}_1$ ignoring the other distributions (something that is not generally possible in the standard transfer learning setting). To the best of my understanding, the authors' goal is to see how the other distributions could help by obtaining an ensemble model (biased towards $\mathcal{D}_1$). For instance, if $\mathcal{D}_2$ is very similar to $\mathcal{D}_1$, then this is expected to be helpful.

Hence, given the above, my understanding is that one could compare the performance of the weak learner trained only on $\mathcal{D}_1$ vs. the aggregated model, to see how the samples from $\mathcal{D}_2$, ..., $\mathcal{D}_N$ can actually help learning. To be more clear, if we fix $n_t$ samples from
$\mathcal{D}_t$
, one could come up with two potential learning algorithms:

1. The weak learner trained only with the $n_1$ labeled examples from $\mathcal{D}_1$.

2. The aggregated model of the proposed algorithm trained with all the available samples
$n=\sum_{t} n_t$.


A clear question is when and by how much model (2) beats model (1), i.e., when the out-of-distribution samples actually help learning. Is this implied by the regret minimization task? Can a result comparing the performance of (1) vs (2) be obtained? Are there any theoretical statistical guarantees about the model obtained from the regret minimization task against some benchmark such as (1)?

\bigskip 
Assumption 1

Regarding the parameter $K_x$, the reason for my question is that if $\|x\|_2$ is identity, then there are many natural settings where scales with the square-root of the dimension of $x$. Are these settings captured by Assumption 1? I am mentioning this because in learning theory, we do not treat the dimension of $x$ as an absolute constant but our goal is to be e.g., polynomial in it in terms of samples/runtime.

Score

As a last comment, regarding my score, I evaluated the paper's soundness with 4 since I did not find any technical issues (I am not an expert in control theory), the presentation by 2 because I found the transfer learning discussion confusing and the contribution by 3, since the paper provides a non-trivial result about regret minimization but it was not clear to me to what extent it relates to transfer learning. I was not aware that my total evaluation score should be that strongly aligned with these metrics, as the authors mention, and I apologize for that. The reason I evaluated the paper as a 'reject' is that (i) it was not clear to me how the provided result about regret minimization is related to the performance of the obtained model on the transfer learning task and (ii) I found that the paper requires several re-writing to be suitable for acceptance; I believe that the paper needs careful re-writing regarding the learning setting considered and the problem formulation. As a non-expert in control theory, I think that the paper would benefit from discussing the control theoretic ideas further but if the other reviewers believe that the level of presentation is sufficient, I am fine with that.

Summary

I would be happy to know if the above discussion regarding the transfer learning setting makes sense or if the authors have a different point of view. The authors' rebuttal was helpful in understanding that the main goal of the paper is to provide an optimization algorithm for minimizing the regret functional with the goal to improve the performance on $\mathcal{D}_1$ using the other models. My main issue is about the presentation of the paper. That said, I am happy to increase my score to 6, if the authors aim to improve the presentation especially regarding

(i) the transfer learning setting (what is the source \& target distributions, what type of sample access do we have, what is the learning goal);

(ii) motivate further the regret functional and why it is a helpful objective to minimize statistically;

(iii) compare with multi-task learning;

(iv) emphasize that the goal of the paper is about optimization and not generalization (this is related to my questions in the "Transfer Learning" section of this comment).


\bigskip 
\textbf{\large\color{blue}Response to Comments from Reviewer NMBE, 08 Aug, 04:44}

Dear reviewer NMBE, 

Thank you for appreciating our rebuttal and for clarifying your learning theoretic perspective on our problem; we found the discussion very beneficial.  

\textbf{How we will Implement the Requested Explanations: }

Your summary of our setting and algorithm is correct.  Though the goal of our paper is indeed to study the optimization algorithm design for transfer learning, we do agree that the statistical motivations of the regret objective can be further used as motivation.  

Following your insights, we would be happy to make the following modifications to our story in the final version of our paper, when motivating our regret objective for our optimization problem:

 - \textbf{Tasks in Transfer Learning:} Let $\mathbb{P}_1,\dots,\mathbb{P}_N$ be probability measures on $\mathbb{R}^d\times \mathbb{R}$, generating data for $N$ (possibly distinct) tasks, and consider a threshold $\eta\ge 0$ determining when any one task is relevant to the focal task $\mathbb{P}_1$.  Here, \textit{relative} relevance of the $i^{th}$ task is quantified by the $KL$-divergence 
 \[
    \bar{w_i} := 
        \frac{[\eta-D_{KL}(\mathbb{P}_1|\mathbb{P}_i)]_+   }{
        \sum_{k=1}^N\,[\eta-D_{KL}(\mathbb{P}_1|\mathbb{P}_i)]_+   
        }
 \]
 however, we may use any other measure of dissimilarity between probability measures (e.g. as a metric on the space of probability measures over $\mathbb{R}^{d\times 1}$ or a divergence on those which have a density with respect to $\mathbb{P}_1$); where $[t]_+:=\max\{0,t\}$ (the ReLU function).

    - If $\mathbb{P}_1=\mathbb{P}_i$ for each $i$ then $\bar{w}_i=1/N$.
    - If all tasks are very dissimilar to the focal task, i.e. $D_{KL}(\mathbb{P}_1|\mathbb{P}_i)\gg \eta$ then $\bar{w}_1=1$ and all other weights are $0$.

- \textbf{An Idealized Statistical Objective}:  We are interested in optimizing the following objective
 \[
    \sum_{i=1}^N\, \bar{w}_i \sum_{j=1}^{\mathcal{D}_i}\, (f_{\theta^{\bar{w}}}(x_j^i)-y_j^i)^2
    \qquad \mathbf{(1)}
    .
 \]

- \textbf{Practical Statistical Objective:} In practice, we do not have access to this objective function since we do not have access to the true "relative task relevances" $\bar{w}$ to the focal task $\mathbb{P}_1$.  Instead, our goal will be to *infer* the similarity of each pre-trained learner $f_{\theta^{\star}_i}$, trained on sample data $\{x^i_j\}$ on the $i^{th}$ task, by evaluating its predictive power on the focal task using the weights $w^{\star}$ computed in Algorithm $1$; which is a modification of the optimization procedure of [1,2] and others.  The min-max optimality of the weights $w^{\star}$ generated by Algorithm $1$ are proven in Theorem $1$.  

Once these weights are inferred, our objective is to identify an aggregated learner which can pool information from each relevant task, according to their inferred relative importance, towards task $1$ by optimizing the following proxy to the objective function $\mathbf{(1)}$ 
 \[
    \sum_{i=1}^N\, w_i^{\star} \sum_{j=1}^{\mathcal{D}_i}\, (f_{\theta^{\bar{w}}}(x_j^i)-y_j^i)^2
    \mathbf{(2)}
    .
 \]
 Following standard practice, we would note that the parameter $\eta$ is inferred by cross-validation in practice.

 - \textbf{Segway to Optimization Goal:} Unlike most work in transfer learning, the goal of our work differs from the bulk of the available literature in that we are not focused on the statistical aspects of the transfer learning problem, but rather on the design of an optimization algorithm which identifies a learner approximately optimizing $\mathbf{(2)}$; subject to regularization.   

Since there is no currently available literature on this problem, in this paper, we will not be focusing on the case of general learners but rather kernel regressors since these are linear in their parameters but non-linear in their inputs.  Thus, this can be the first concrete step towards a general solution of an optimal optimization-algorithm design problem for transfer learning where one can hope to gain insights through closed-form solutions of our optimal optimization algorithm (Theorem 1), and we can analyze its computational complexity (Theorem 2).

 
 We would then briefly comment that, though we provide some statistical guarantees in Theorem $4$ and some adversarial robustness guarantees in Theorem $3$, a serious statistical investigation of the (regularized) optimizers to $\mathbf{(2)}$ would be a very interesting avenue of future research; which some of the authors are keen on investigating.

 - \textbf{Differences with Multi-Task Learning and How our Framework can be Modified for Multi-Task Learning}: 
 We then would add a few words building on the very fruitful rebuttal discussion, explaining the similarities and differences between our setup and a multi-task version of that.  We could then briefly comment on how one could modify our algorithm to perform transfer learning.  


 [1] Alquier, P., Ridgway, J., Chopin, N., and Teh, Y. W. On the properties of variational approximations of Gibbs posteriors. Journal of Machine Learning Research, 2016
 
 [2] Rothfuss, J., Fortuin, V., Josifoski, M., and Krause, A. PACOH: Bayes-optimal meta-learning with pac-440
guarantees. In Meila, M. and Zhang, T. (eds.), Proceedings of the 38th International Conference441
on Machine Learning, volume 139 of Proceedings of Machine Learning Research, pp. 9116–9126.442
PMLR, 18–24 Jul 2021


\textbf{Details about our experiments} 

 One possible real world scenario could be the fine-tuning of large language models to user-specific data, which is available as a training set but often scarce compared to typical training datasets for such models. More precisely, if one wants to fine-tune to a chat with a specific person then this has only little data, but all chats with other persons are possible additional datasets which are more or less similar to the target one.

In our experiments we focused on the American option pricing problem with very limited data of the target distribution but additional data of more or less similar distributions. In Table 1, we compare exactly the models that you described. LO-1 is the local optimizer on $D_1$, or as you called it, the weak learner trained only with the samples of $D_1$. RO is our regret-optimal algorithm, i.e., our proposed aggregated model trained with all available samples. Additionally, we compare to the baselines MLO, JO and JSO, which are also aggregated models using all available data, however, not in an optimal way. Our results show how much our model can outperform the others in two settings, where simple aggregation, as MLO and JO do, does lead to a performance decrease, because not all of the available data is beneficial for the downstream task.

Generally answering your question is hard. The intuition is the following. Whenever the additional datasets are similar enough to $D_1$ our aggregated model will outperform the weak learner because it has additional information that it can use.   

For example, when all other datasets are actually independently sampled from the same distribution as $D_1$, then our algorithm will approximately put the weight $w_i^* = 1/N$ on each dataset and (for $\lambda = \beta = 0$) our model will simply be optimized on the joint dataset with all available samples. The outperformance of our model compared to the weak learner is then quantifiable through the performance gain by the dataset increase. In particular, the theoretical statistical guarantees of ordinary least squares apply, which can be used to quantify the improvement through the increase of the dataset size.
 (For more details on the influence of $\lambda, \beta$ please see the answers to reviewer Zsc6.)   

On the other hand, if all other datasets are orthogonal to $D_1$ such that they do not provide any information about the target task on $D_1$, then our algorithm (approximately) puts full weight $w_1^*=1$ on $D_1$ and 0 weight on the other datasets. Hence, it performs as good as the weak learner, while the other baseline aggregation models (MLO, JO, JSO) would perform (much) worse than the weak learner.    

In both of these examples, our model (approximately) coincides with the optimally possible algorithm. For intermediate cases, we also expect to see an intermediate performance increase of our model compared to the weak learner, however, the analysis of such cases is non-trivial.


\textbf{Assumption 1}
We allow $K_x$ to depend on the dimension $p$ of $\phi(x)$. Indeed, the complexity of Algorithm 2 is influenced by the dimension $p$, as outlined in Theorem 2. The purpose of Assumption 1 is to support the proof of Theorem 3, which establishes the adversarial robustness of Algorithm 2. In Theorem 3, we are particularly interested in understanding how the regret changes in response to attack persistence and severity. Therefore, we treat the dimension $p$ as a constant and incorporate it into the big $\mathcal{O}$ notation for robustness in Theorem 3. 


\textbf{Score}
Thank you very much for your clarifications, this helps us a lot.


\textbf{Regarding the summary:} 

Thank you very much for this in-depth discussion, from which our paper benefits significantly. We are happy to improve the presentation of our paper as you outlined, by including the insights from the reviewing process.

Best regards, 

The Authors 


\bigskip 
\textbf{Comments from Reviewers NMBE 12 Aug 2024, 04:50} 

I thank the authors for the response. I clarify some of my points.

Algorithm 1 optimizes a minimax statistical objective

I agree that Algo 1 may have some statistical implications; I would like to see a formal statement (maybe extracted from prior work?) that makes it clear. For instance, this min-max optimality is not clear from the current manuscript. To make my point more clear, I believe that achieving robustness is a desirable property. Nevertheless, I think that using classical learning theory to obtain (non-robust) rigorous statistical guarantees is still important.

NeurIPS Papers studying optimization itself

Probably my point was misunderstood. Definitely I agree that (pure) optimization papers are a fundamental area for the NeurIPS community. For instance, the first paper [1] that you mention falls in this category: it proposes a new optimization algorithm which works for general constrained nonconvex-nonconcave minimax problems (i.e., arbitrary objective functions that satisfy some very general properties). The importance of this paper for the ML community is that if the (specific) loss function that I would like to optimize for some specific learning task satisfies the properties, then I can use the off-the-shelf given algorithm.

My point is that the present paper does not fall in this category (at least in the way it is presented): it aims to solve a learning theoretic task using samples, namely find a good parameter vector (and some mixing weights
) so that the induced model performs good predictions in using data from

. Hence, after introducing a natural learning theoretic setup, I guess the reasonable thing to do is to follow the pipeline of Steps (A)-(C) of my previous comment:

(A) Design the loss function (e.g., the population and empirical versions);

(B) Show that if you could minimize the empirical loss function, then the achieved set of parameters is statistically good;

(C) Finally show how to actually optimize the sample-based objective.

For instance, the difference between optimization in the current paper and [1] that you mention, is that, in the current work, the method is explicitly tailored for the proposed objective function, while in [1], it is for a general collection of functions. Hence for your problem, Step (B) is actually very important and this is why I think that adding all the discussions in the previous comments about the ideal objective of Eq.(1) and the empirical one of Eq.(2), etc., would be a good starting point.

As for paper [2] that you mention, I think that it does not fill in the same category as paper [1]. Paper [2] fixes a specific family of loss functions and fixes the optimization method to be (S)GD. The statistical properties of the loss essentially follow by definition of the learning problem and as an objective, it has been extensively studied by the applied community (e.g., by Bello et al. (2016) as I see in the paper). Hence, we know that the global minima of the loss function are desirable. The non-trivial question is how can SGD find them. The main inquiry of [2], as the paper mentions, is how to design a model that has a small number of parameters and the induced optimization landscape allows gradient-based methods to converge to the optimal solution without getting trapped at local minima.

In short, I believe that there are some differences between the current work and the works that you mention. In the revised version of the paper, it may be useful to add a discussion on how the optimization perspective of the present paper differs from other optimization papers (e.g, the ones that you mentioned and maybe others?).

Summary

I hope that my points are more clear now. I repeat that I think that the paper requires heavy re-writing making the learning-theoretic setup very clear: source-target distributions, ideal loss function, empirical loss function, motivation for these two losses, statistical guarantees for the two losses, optimization guarantees, etc.

References

[1] Liu, Y., Shang, F., An, W., Liu, J., Liu, H., \& Lin, Z. (2024). A single-loop accelerated extra-gradient difference algorithm with improved complexity bounds for constrained minimax optimization. Advances in Neural Information Processing Systems, 36.

[2] Caramanis, C., Fotakis, D., Kalavasis, A., Kontonis, V., \& Tzamos, C. (2023). Optimizing solution-samplers for combinatorial problems: The landscape of policy-gradient method. Advances in Neural Information Processing Systems, 36, 14035-14069. and several other non-oral presentation papers focused solely on optimization theory motivated by machine learning problems.





\bigskip 

\textbf{\color{blue} Response to reviewer NMBE 12 Aug 2024, 04:50}


Dear reviewer NMBE,

Thank you for your further detailed explanation. We truly appreciate the time and effort you've invested in providing this additional clarification.

-  In machine learning, the true test of viability of a model/algorithm is not a statistical guarantee but that it works numerically (e.g. dropout, attention, etc.). In Section 4.1 of the initial submission, we had already implemented natural benchmarks you asked for in the numerical experiments, and showed that our regret optimal algorithm outperforms the standard gradient descent algorithm. 

- Theorems 1, 3, and 4 support the optimality of our optimization algorithms, i.e., Algorithms 1 and 2; which is the main focus of our paper.

- We are happy to incorporate your proposed statistically inspired motivation to the end of our paper, to broaden our paper's reader base.

We greatly appreciate your time and consideration in reviewing our rebuttal.

Best regards,

The Authors









\newpage
\section{uJWn}
\begin{tcolorbox}[colback=white,colframe=black,title={Reviewer ujWn, rating 6}]
\footnotesize
\textbf{Summary:} \\
This paper studies the meta-optimization problem of designing good transfer learning algorithms. The target is a weighted average of fine-tuned model parameters. In particular, this paper considers a deterministic objective that captures data performance, transfer learning, and stability and proposes algorithms to obtain weights and .\\



\textbf{Soundness:} 3: good \\
\textbf{Presentation:} 3: good \\
\textbf{Contribution:} 3: good \\

\textbf{Strengths:} \\

1.     The topic of improving transfer learning is interesting and important

2.    This paper is well-written with rich content on both theoretical analysis and numerical illustration



\textbf{Weaknesses:} \\
1. The numerical plot texts are rather small and unreadable, which is understandable due to limited space, but maybe can have a larger one in the appendix at least. \\

\textbf{Questions:} \\

1.    Can authors explain what it means by regret-optimal since the regret is not even defined?

2.    Other than wide adoption in finance, can authors further explain why using the finite-rank kernels? Are there any other benefits?

3.    The analysis primarily focuses on deterministic optimization whereas more probabilistic analysis on data distribution or generalization errors are neglected. Can authors enrich the discussion of the algorithm performances from this perspective?



\textbf{Limitations:} \\
N/A
\end{tcolorbox}


\begin{tcolorbox}[colback=white,colframe=blue,title={Response to Reviewer ujWn}]
Dear reviewer ujWn,\\ 

Thank you for your insightful comments. The following are our responses to your questions and comments about the manuscript. \\ 

\textbf{Concerning weaknesses:}\\ 

1. Thank you for pointing this out. We have enlarged the plots of numerical examples in the manuscript to enhance readability. 
\\ 

\textbf{Concerning questions:} \\ 

1. As defined in equation (1), the regret-based criterion which we optimize is $\mathcal{R}(\Theta^{0...T})$, which we call regret, given by
$$
\mathcal{R}(\Theta^{0...T})
:=
\underbrace{
    \sum_{i=1}^N w_i
    \sum_{j=1}^{|\mathcal{D}_i|} 
    (f_{\theta^w}(x_j^i) - y^i_j)^2 - l^\star
}_{\text{performance criterion}}
    +
    \underbrace{
        \sum_{t=0}^{T-1}  
        \,
             \big(
                        \lambda \left\| \Theta(t+1) - \Theta^\star \right\|_2^2    
                + 
                        \beta  \left\| \Delta \Theta(t) \right\|_2^2 
                \big) 
    }_{\text{penalty terms}}
$$
i.e., the penalized difference between the error of the trained model $f_{\theta^w}$ and the achievable error 
$ l^{\star} = \min_{\Theta \in R^{Np}}\, \sum_{i=1}^N 
w_i
    \sum_{j=1}^{|\mathcal{D}_i|} 
        (
        f_{\theta^w}(x_j^i)
        - y^i_j  
        )^2$ 
across all tasks. Similarly to [1], we call an optimization algorithm regret-optimal $\Theta^{0...T}$ if it is a minimizer of the regret criterion $\mathcal{R}$.
\\ 

2. Since our paper is the first one to consider the problem of optimizing optimization algorithms for transfer learning, we decided to begin by investigating kernel ridge regressors simply due to their linear structure, in their parameters, not in their inputs, as compared to the non-linear structure of deep learning models.  

The applicability of kernel regressors has seen a recent resurgence in the fine-tuning for deep learning models literature; a pre-trained foundation model has only its final linear layer trainable.  As discussed on page 3 of [2], this defines a finite-rank kernel regressor.  In this way, many of our tools are applicable to any such scenario where a deep neural network's final layer is being fine-tuned. \\


As explained in the paragraph around equation (2), our method is applicable to any transfer learning task where the models for the single tasks are randomized or standard neural networks. In such a setting, optimizing the final layers is an efficient way for transfer learning. The benefit is that we can combine the feature expressiveness of neural networks with the efficiency of parameter optimization via OLS, which leads to a very fast and tractable transfer learning procedure. 
\\ 


3. We expect that the analysis for the stochastic algorithms can be largely ported from that of our deterministic regret-optimal algorithm, where,  at each iteration, we perform our deterministic algorithm on random mini-batches.  This is an interesting link which we will elaborate on in the discussion section.


[1] Casgrain, P. and Kratsios, A. (2021, July). Optimizing Optimizers: Regret-optimal gradient descent algorithms. In Conference on Learning Theory (pp. 883-926). PMLR.

[2] Cheng, T. S., Lucchi, A., Kratsios, A., Dokmanić, I., and Belius, D. (2023). A theoretical analysis of the test error of finite-rank kernel ridge regression. Advances in Neural Information Processing Systems, 36, 4767-4798.




\end{tcolorbox} 







\end{document}

